Integrability and RG flow in 2d sigma models

Motivated by the search for solvable string theories, we consider the problem of classifying the integrable bosonic 2d $\sigma$-models. We include non-conformal $\sigma$-models, which have historically been a good arena for discovering integrable models that were later generalized to Weyl-invariant ones. General $\sigma$-models feature a quantum RG flow, given by a 'generalized Ricci flow' of the target-space geometry. This thesis is based on the conjecture that integrable $\sigma$-models are renormalizable, or stable under the RG flow. It is widely understood that classically integrable theories are stable at the leading 1-loop order with only a few parameters running. Here we address what happens at higher-loop orders. We find that integrable $\sigma$-models generally remain RG-stable at higher-loops provided they receive a particular choice of finite counterterms, or quantum ($\alpha'$) corrections to the target-space geometry. We explicitly construct these quantum corrections for examples of integrable $\eta$- and $\lambda$-deformed $\sigma$-models. We then reformulate the $\lambda$-models as $\sigma$-models on a "tripled" $G \times G \times G$ configuration space, where they become automatically renormalizable due to manifest symmetries and a decoupling of some fields. We also consider the integrable $G \times G$ and $G \times G/H$ models and construct a new class of integrable $G \times G/H$ models with abelian $H$. We then present a new and different link between integrability and the RG flow in the context of $\sigma$-models with 'local couplings' depending explicitly on 2d time. Such models are naturally obtained in the light-cone gauge in string theory, pointing to the possibility of a large, new class of solvable string models.

==> v arxiv v2/1910v2.tex <==
\def\id{\protect{{1 \kern-.28em{\rm l}}}}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\bi{\bibitem}
\def\tr{{\rm tr}}
\def\ha{\tfrac{1}{2}}
\def\td{\tilde}
\def\ci{\cite}
\def\N{{\mathcal N}}
\def\ww{\Omega}
\def\S{{\mathcal S} }
\def\nn{\nu}
\def\z{\zeta}
\def\dg{\dagger}
\def\a{\alpha}
\def\b{\beta}
\def\ap{\alpha^\prime}
\def\aa{{\a'}}
\def\g{\gamma}
\def\ok{\frac{1}{k}}
\def\jL{{J}}
\def\cL{{\mathcal L}}
\def\cH{{\mathcal H}}
\def\E{{\mathcal E}}
\def\w{\omega}
\def\vep{\varepsilon}
\def\De{{\mathcal D}}
\def\k{\kappa}
\def\four{\tfrac14}
\def\third{\tfrac{1}{3}}
\def\det{\hbox{det}}
\def\tid{\tilde}
\def\vv{{\rm v}}
\def\XX{{\rm X}}
\def\ta{{\tilde \a}}
\def\fo{\frac{1}{4}}
\def\K{{\rm S}}
\def\el{\ell}
\def\Tr{{\rm Tr}}
\def\P{\Phi}
\def\l {\lambda}
\def\bl{{\tilde \l}}
\def\const{{\rm const}}
\def\vn{\vec n}
\def\Prod{\Pi}
\def\O{{\mathcal O}}
\def\m{\mu}
\def\vs{\vec \s}
\def\ie{i.e.}
\def\rS{{\rm S}}
\def\as{{\a}}
\def\e{\epsilon}
\def\foot{\footnote}
\def\ra{\rightarrow}
\def\F{{\cal F}}
\def\cc{\circ}
\def\eqv{\equiv}
\def\ni{\noindent}
\def\bw{{\rm w}}
\def\cT{{\cal T}}
\def\no{\nonumber}
\def\J{{\cal J}}
\def\om{\omega}
\def\l{\lambda}
\def\tk{{\tilde k}}
\def\tl{{\tilde \l}}
\def\sqtl{{\sqrt{\tilde \l}}}
\def\adss{$AdS_5 \times S^5$\ }
\def\D{\Delta}
\def\p{\phi}
\def\r{\rho}
\def\rN{{\rm N}}
\def\tw{{\tilde w}}
\def\vl{ \vec \ell}
\def\varpi{{\rm w}}
\def\bG{\bar \G}
\def\ve{\varepsilon}
\def\I{{\cal I}}
\def\La{{\Lambda}}
\def\R{{\rm R}}
\def\bt{\bar\theta}
\def\Z{{\cal Z}}
\def\pa{\partial}
\def\bea{\be}
\def\eea{\ee}
\def\DD{{\rm D}}
\def\chii{\varepsilon}
\def\th{\theta}
\def\t{\tau}
\def\beq{\be}
\def\eeq{\ee}
\def\beqa{\bea}
\def\eeqa{\eea}
\def\bs{\bigskip}
\def\c{{\rm a}}
\def\del{\partial}
\def\s{\sigma}
\def\eps{{\epsilon}}
\def\n{\nu}
\def\dag{\dagger}
\def\bd{\bar \del}
\def\ed{\end{document}}
\def\iffa{\iffalse}
\def\xp{x_+}
\def\xm{x_-}
\def\te{\textstyle}
\def\rx{{\rm x}}
\def\C {{\rm C}}
\def\hC {{\rm \hat C}}
\def\dd {{\rm d}}
\def\bb{{\rm b}}
\def\sql{{\sqrt{\l}}}
\def\ep{\epsilon}
\def\G{\Gamma}
\def\dx{\dot x}
\def\vp{\varphi}
\def\tx{{\tilde x}}
\def\ad{{\rm ad}}
\def\d{\delta}
\def\de {\del}
\def\L{\mathcal{L} }
\def\pcm {{\rm PCM}}
\def\wz{{\rm WZ}}
\def\pcmq {{\rm PCM}$_q$\ }
\def\ZMq {{\rm ZM}$_q$\ }
\def\ZM {{\rm ZM} }
\def\pp{{\rm p}}
\def\qq{{\rm q}}
\def\rk {{\rm u}}
\def\rrk{{\rm e}}
\def\ss{{\rm s}}
\def\tt{{\rm t}}
\def\uu{{\rm u}}
\def\sm{$\sigma$-model }
\def\sms{$\sigma$-models }
\def \ov {\over}
\def\Ad{\text{Ad}}
\def\lmp{\Lambda}
\def\bl{\bar \lambda}
\def \hb {\hbar}
\def \k {\varkappa} \def \h {{\rm h}}
\def \dt {\dt}
\def\ddt{\frac{d}{dt}}
\def \bb {{\rm b}}
\def \vv {{ v}}
\def \kk {{\rm k}}
\def \ka {{\kappa}}
\def \np { }
\def \cM {\mathcal{M}}
\def\H{{\rm H}}
\def \BB {{\rm B}}
\def \HH {{\rm H}}
\def \GG {{\rm G}}
\def \PCM {{\rm PCM}}
\def \WZ {{\rm WZ}}
\def \Lie {{\rm Lie}}
\def\lam{$\lambda$-model}
\def\etm{$\eta$-model}
\def\bh{\bar h}
\def\hh{{\rm h}}
\def \OO {{\cal O}}
\def \etm {$\eta$-model\ }
\def \lam {$\l$-model\ }
\def \dt {\frac{d}{dt}}
\def \rrr {x} \def \qp {{\rm q}}
\def \qp {{\mathrm h} }
\def \bq {{q'}} \def \barp {x} \def \barq {y}
\def \rk {{\rm k}}
\def\F{H}
\def\cg{c_{_G}}
\def\cf{c_{_\F}}
\def\cff{c_{_\F}}
\def\HH{\F}
\def\XX{{X}}
\def\hhh{\widetilde {\hh}}
\def\q{{\rm q}}
\def\RR{{J}}
\def\LL{{K}}
\def\M{{\cal M}}
\def\e{\varepsilon}
\def\tih{{\hat h}}
%\def\gg{\gamma}
\def\bl{\bar\lambda}


\chapter{``Tripled'' formulation of the \texorpdfstring{$\l$}{lambda}-model \label{CT}}

We have been studying a close link between 
renormalizablility, 
or stability under the RG flow,
and
 integrability in 2d $\s$-models.
 Having previously been observed
\cite{Fateev:1992tk,fateev96,lukyanov,Fateev:2019xuq,Fateev:2018yos,Litvinov:2018bou} only at the 1-loop (Ricci flow) level, it
is important to study this relation also at higher loop orders.


This question of higher loops was addressed above in Chapters \ref{QCS} and \ref{GGS},
 where we found that, starting from 2 loops,
renormalizability typically requires a specific deformation of the classical target space
geometry, which may be interpreted as the result of adding
finite
local counterterms. In Chapter \ref{QCS},  we considered the simplest examples of 
integrable $\eta$- and $\l$-deformed bosonic \sms with 2- and 3-dimensional target spaces.
In Chapter \ref{GGS}, we looked at another class of  integrable \sms with target spaces $G\times G$ and $G\times G/H$.
 
 
 Here we shall concentrate on the $\l$-deformation \cite{Sfetsos:2013wia,Hollowood:2014rla} and address the \textit{general case} where the model is based on an arbitrary 
group
$G$ or  symmetric space $G/\HH$. Its Lagrangian is (repeating eq.\ \eqref{lam} for clarity)
\begin{align} 
&\L  = k \, \Big( \L_G(g) \la{1}  + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_- - A_+ A_- - ( \lambda^{-1}-1) A_+ P A_-\big] \Big) , \\
& %{\PCM} = - \ha \Tr[J_+ J_-] \ , \quad dB_{\rm WZ}=\tfrac{1}{6} \Tr [J\wedge J \wedge J] \ , \quad
J=g^{-1} dg \ , \quad K = dg \, g^{-1} \ ,\no\\
& P = \begin{cases}
1 \ , \quad \ \ \ \ \ \text{group space }G\\
P_{G/\HH} \ , \quad \text{symmetric space }G/\HH \ ,
\end{cases} \la{1111}
\end{align}
where $\L_G=\L_\PCM+ \L_\WZ$ is the WZW Lagrangian, $g \in G$, $A_\pm \in \Lie(G)$ and $P_{G/\HH}$ is the projector onto the orthogonal complement of $\Lie(\HH)$ in $\Lie(G)$.
Instead of $\l$ it is often convenient to use
a redefined parameter,
\begin{equation}\la{133}
%\g = \lambda^{-1}-1
%\ , \qquad \qquad 
\ka = \frac{1-\lambda}{1+\lambda} \ .
\end{equation}
The limit $\lambda \to 0$ (or $\ka \to 1$)
yields the conformal  WZW model  on $G$ (or  gauged WZW model on $G/\HH$)
 with level $k$,
which should thus be a fixed point of the RG flow.
The $\l$-model's $\mathbb{Z}_2$ transformation \eqref{z2sym} then implies that the opposite limit $\l \to\infty$ (or $\ka \to -1$)  should also be a fixed point.
Indeed, in the group case the $\l \to \infty$ limit of \rf{1} is conformal:
it is the $G/G$ chiral gauged WZW model \cite{Chung:1992mj}, which, on
integrating out $A_\pm$, gives the $G$ WZW model at level $-k$.
Similarly, in the coset case we find in this limit the $G/H$ gauged WZW model at level $-k$.

Integrating out the 2d gauge field $A_\pm$ in \rf{1}, i.e. reducing the model to the standard (or ``physical'') configuration space,
one finds a \sm with parameters $k$ and $\l$ (see eq. \eqref{lamc}).  
As we found in Chapter \ref{QCS}, to preserve renormalizability of the $\l$-model 
at the 2-loop level,
 one must make a non-trivial modification of
the classical target space geometry.

In this chapter our central observation will be that, \textit{before} integrating out $ A_\pm$,
the \lam \rf{1} is renormalizable without any deformation.
As was done in the context of gWZW models \cite{Karabali,Tseytlin:1992ri,Sfetsos:1993bh,Sfetsos:19932}, we shall change variables from $A_\pm$ to scalar fields $h, \bar h \in G$ as
\be A_+ = h \,  \del_+ h^{-1}, \ A_- = \bar{h} \, \del_+ \bar h^{-1}  \ , \la{cov} \ee
resulting in  a \sm
on the extended or ``tripled'' ($G \times G \times G$) configuration space $(g, h, \bh)$.
It may be interpreted as the sum of two decoupled parts: (i) a  WZW model on $G$ and (ii) a deformation of a 
WZW model on $G \times G$ by a particular left-right current interaction.
This special decoupling is expected to be a manifestation of integrability and, as a result, 
the \textit{manifest} global symmetries become sufficient to protect  
 the model
 under the RG flow
without the need for any additional finite counterterms. 



\

The rest of the chapter is organized as follows. In Section \ref{revg} we shall review the previous application of the change of variables \rf{cov} to gauged  and chiral gauged WZW models.

In Sections \ref{1910extended} and \ref{trips}, we consider the $\lambda$-models, respectively based on groups and symmetric spaces, on the configuration space $(g,A_+,A_-)$, i.e.\ with the gauge field unintegrated.
By using the change of variables \rf{cov} to write the $\l$-models as  certain ``tripled'' $\s$-models
with extra manifest symmetries, we shall argue that they are automatically renormalizable to all orders and explicitly compute their 2-loop $\b$-functions.
In the
 non-abelian dual (NAD)
  limit \eqref{limr}, these  will correctly reproduce the (scheme-invariant) 2-loop $\b$-functions of the PCM and symmetric space $\s$-model, suggesting that the interpolating models for NAD are also automatically renormalizable without needing corrections.


\sloppy
In Section \ref{lowd} we consider some simple examples of the models obtained in the ``tripled'' formulation of the $\l$-models based on $SU(2) \ov U(1)$ and $SU(2)$. In Section \ref{1910TO} we construct  analogous ``tripled'' or ``extended'' space formulations of some other integrable $\s$-models (a variant of the $\l$-model built on $G^N$ \cite{Bassi:2019aaf} and the \mbox{$G\times G/H$} models of \cite{ABL}).
Some concluding remarks are made in Section \ref{1910conclusions}.

\

\noindent This chapter is based on the paper \cite{HLT2} and we closely follow the presentation there.


\section{Review of gWZW model \label{revg}}
First let us review the  original use of the change of variables \rf{cov} in the context of the gauged WZW models \cite{Karabali,Tseytlin:1992ri,Sfetsos:1993bh,Sfetsos:19932}. The gauged WZW model is closely related to the $\l$-model \rf{1} but with the gauge field being valued in some subalgebra $\Lie(F)\subset \Lie(G)$ (see Section \ref{gWZW}),
\be \begin{aligned}
&\L  = k \, \Big( \L_G(g) + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_- - A_+ A_- ] \Big) \ , \\
&g\in G \ , \ \ A_\pm \in \Lie(F) \ . \la{gg}
\end{aligned} \ee
Changing variables $(A_+, A_-) \to (h,\bar h)$ as in \rf{cov}, now with with $h,\bar h \in F$, and using the Polyakov-Wiegmann identity\foot{The Polyakov-Wiegmann identity is a multiplicative  identity for the WZW Lagrangian \cite{Polyakov:1983tt},

$\qquad \L_G(u v) = \L_G(u) + \L_G(v) - \Tr[ u^{-1} \del_+ u \, \del_- v v^{-1} ]  \ . $  \la{PW}} 
 \cite{Polyakov:1983tt},
 the Lagrangian  \rf{gg} can be written as a combination of WZW models, 
\begin{equation}\begin{split}\la{22g}
\L &= k \Big( \L_G (h^{-1} g \bar{h}) - \L_F ( h^{-1} \bar{h} )\Big) \ .
\end{split}\end{equation}
The change of variables
in \rf{cov} results in a Jacobian contributing to the action as
\cite{Polyakov:1983tt,Polyakov:1988qz}
\begin{align}
\Delta \L & = - 2 c_{_F} \Big( \L_F(h^{-1} \bar{h} ) + \q \Tr [A_+ A_-]\Big)\la{jac1} \\
&= - 2 c_{_F} \Big( \L_F(h^{-1} \bar{h} )+  \q \Tr [ \del_+ h \, h^{-1} \, \del_- \bar{h} \, \bar{h}^{-1} ]\Big) \ , \la{jacg}
\end{align}
where $c_{_F}$ is the dual Coxeter number\foot{More precisely, $c_{_F}$ denotes here a rescaled version of the dual Coxeter number of $F$ by an index factor relating to the embedding of $F$ into $G$ (see discussion in the final paragraph of App.\ \ref{conv} for  subgroups $H \subset G$). If $G$ and $F$ are both classical groups with the same index for their fundamental representation (e.g. both $A$-type) then this index factor is trivial and $c_{_F}$ is the dual Coxeter number of $F$.} of $F$ and
an arbitrary coefficient $\q$ parametrizes the ambiguity of adding a finite local  counterterm $\Tr [A_+ A_-]$.
Combining \rf{jacg} and the classical Lagrangian \rf{22g} gives
\be
\L = k \L_G (h^{-1} g \bar{h}) - (k+2 c_{_F}) \L_F ( h^{-1} \bar{h} ) -  2 \q c_{_F} \big[ \L_F (h^{-1} \bar{h}) - \L_F ( h^{-1} )- \L_F (\bar{h} ) \big] \ . \ \la{5termg}
\ee
Now one can choose the coefficient $q=0$ to obtain the sum of two decoupled WZW models (e.g. after defining $\tilde{g}=h^{-1} g h$, $\tilde h=h^{-1} \bar h$)
\be
L = k \L_G (h^{-1} g \bar{h}) - (k+2 c_{_F}) \L_F ( h^{-1} \bar{h} ) \la{ggr}
\ee
Expressing the gWZW model as this sum of decoupled WZW models makes manifest its properties of (i) exact conformal invariance and (ii) gauge invariance under $g\to u g u^{-1} $, $h\to u h$, $\bar h \to u \bar h$.

The exact form of the  gWZW metric and $\BB$-field can be derived \cite{Tseytlin:1992ri} from \rf{ggr} (agreeing with \cite{Dijkgraaf:1991ba,Bars:1992sr}) by considering the quantum effective action. The WZW model's effective action is just the classical one with a shifted level (respectively $k \to k+ c_{_G}$  or $k\to k+c_{_F}$), leading to
\be \begin{aligned}
\L_{\rm eff} {}&{}= (k+c_{_G}) \L_G (h^{-1} g \bar{h}) + [ - (k+2 c_{_F}) + c_{_F} ]\L_F ( h^{-1} \bar{h} ) \\
 &{}=  (k+c_{_G}) \L_G (h^{-1} g \bar{h}) - (k+ c_{_F}) \L_F ( h^{-1} \bar{h} ) \ .
\end{aligned} \ee
Transforming back to $A_\pm$, the resulting theory is not local but the ``local part'' gives a prescription for a corrected version of \rf{gg} in which $A_\pm$ can be integrated out \textit{classically} to get an exactly conformal $\s$-model (of which the $SL(2,R)/U(1)$ example is given in \eqref{6}).


\bigskip

Now let us briefly consider the related  $G/F$ \textit{chiral gauged WZW model}  (cWZW) \cite{Chung:1992mj}, for which a similar argument was carried out in \cite{Sfetsos:1993bh},
\be \begin{aligned}
&\L  = k \, \Big( \L_G(g) + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_-  ] \Big) \ , \\
&g\in G \ , \ \ A_\pm \in \Lie(F) \ . \la{cg}
\end{aligned} \ee
 This theory differs from the gWZW model \rf{gg} by the addition of $k \, \Tr[A_+A_-]$. Again changing variables as in \rf{cov}, the extra classical term in \rf{cg} is proportional to the ambiguous local term with coefficient $\q$ in \rf{jac1}. Thus the result for the cWZW model is obtained by replacing  $-2\q c_{_F} \to k-2\q c_{_F}$ in \rf{5termg},
\be
\L = k \L_G (h^{-1} g \bar{h}) - (k+2 c_{_F}) \L_F ( h^{-1} \bar{h} ) +  (k-2 \q c_{_F}) \big[ \L_F (h^{-1} \bar{h}) - \L_F ( h^{-1} )- \L_F (\bar{h} ) \big] \ . \ \la{5termc}
\ee
Again in this case, there is a choice $\q=-1$ that leads to cancellations and gives a sum of decoupled WZW models \cite{Sfetsos:1993bh},
\be
\L = k \L_G (h^{-1} g \bar{h}) +  (k+ 2 c_{_F}) \big[ \L_F ( h^{-1} )+ \L_F (\bar{h} ) \big] \ , \la{cgg}
\ee
illustrating that the cWZW model is also exactly conformal.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{``Tripled'' \texorpdfstring{$\l$}{lambda}-model based on a group}\la{extended}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Now let us turn to the $\l$-model based on a group $G$ (putting $P=1$ in eq.\ \rf{1}),
\begin{align} 
&\L = k \, \Big( \L_G(g) + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_- - \lambda^{-1} A_+  A_-\big] \Big) , \la{1G}  \\
&g\in G \ , \quad A_\pm \in \Lie(G) \ . \no
\end{align}
This model interpolates between the gWZW model \rf{gg} ($\l=1$) and the cWZW model \rf{cg} ($\l=\infty$) in the particular case $F=G$. Hence, upon making the same change of variables $(A_+, A_-)\to (h,\bar h)$ as in \rf{cov}, the resulting theory is just the weighted average of the gWZW and cWZW results \rf{5termg},\rf{5termc} above,
\be \begin{aligned}
\L = &k \, \L_G (h^{-1} g \bar{h}) - (k+2 c_{_G}) \L_G ( h^{-1} \bar{h} )\\
 &\qquad \qquad -  (k(\l^{-1}-1)+2 \q c_{_G}) \big[ \L_G (h^{-1} \bar{h}) - \L_G ( h^{-1} )- \L_G (\bar{h} ) \big] \ , \ \la{5term}
\end{aligned} \ee
with the new scalar fields $h,\bh$ now valued in the full group $G$. This expression includes the Jacobian contribution \rf{jacg}, with the coefficient $\q$ parametrizing the local term ambiguity. In this case $\q$ just specifies a particular redefinition of the coupling $\l$, so the choice of $\q$ is not important and we shall pick $\q=-1$ (as in the cWZW case above).


Again using the Polyakov-Wiegmann identity (see footnote \ref{1910PW}), we may rewrite \rf{5term} as
\begin{align}
&\L= k \L_G (\tilde{g}) + \L'(\tih, \bh) \ ,\qquad \qquad \qquad \qquad \tilde{g} \equiv h^{-1} g \bar{h}\in G \ ,  \qquad \tih\equiv h^{-1} \in G \ , \la{277} \\
&\L'= - (k+2 \cg) \big[ \L_G ( \tih) + \L_G (\bar{h} ) \big] + k\l^{-1} \Tr [ \tih^{-1} \del_+ \tih \, \del_- \bh \bh^{-1}] \ .
\la{27}
\end{align}
This is a \sm with fields valued in  the extended configuration space $(\tilde{g},\tih,\bar{h}) \in G \times G\times G $. 
As for the gauged WZW models considered  above,
the first WZW term  $k \L_G (\tilde{g})$ still decouples from the other fields in \rf{277}. This decoupling is a special property expected to be associated with integrability: indeed if one deformed the $\l$-model \rf{1G} in an arbitrary way preserving its global symmetry but breaking integrability, the decoupling would be lost.\foot{I thank N. Gromov for a discussion of this point.}  Since the decoupled WZW term is conformal on its own, then its coefficient $k$ will not run, and the RG flow of $\l$ is determined by the other ``truncated'' part $\L'$.

Redefining the couplings as
\be
\la{redef}
\tk \equiv k + 2 \cg \ ,\qquad \qquad \tl \equiv
 \frac{k}{\tk}\l^{-1}  \ ,
\ee
then the truncated part,
\begin{align} \la{6dmodel}
& \L'(\tih, \bar h)
= - \tk \Big( \L_G ( \tih ) + \L_G (\bar{h} ) - \tl \Tr [ \tih^{-1}\del_+ \tih \, \del_- \bh \bh^{-1} ] \Big) \ , \qquad \quad \tih \equiv h^{-1}, \ \bh \in G\ , 
\end{align}
 may be interpreted as the sum of
  two WZW models for the group $G $
with the same level $-\tk$
perturbed by a current-current interaction.
Classical integrability of the model \rf{6dmodel} (implying integrability of the group space $\l$-model) 
was first shown in \cite{Bardakci:1996gs} (see also \cite{Hull:1995gj}).
In fact \rf{6dmodel} is a particular instance of the integrable $G\times G$ models \cite{DLMV} in \eqref{2103par},\eqref{2103cond} above, with the couplings and fields  related by 
\be
(k_1,k_2,s,u,t,b) =(-\tk, +\tk, -\tk, -\tk, \tk \tl^{-1},\tk \tl^{-1}) \ , \qquad (g^{(1)},g^{(2)})=(\tih, \bh^{-1}) \ . \la{crel}
\ee
At the value $\wt \l=1$ of the coupling, the model \rf{6dmodel} becomes a special case ($G\times G/G$ with equal levels) of the conformal GMM model \cite{Guadagnini:1987ty}.
A generalization of the model \rf{6dmodel} was also considered in
\cite{sfetsos,s19},
where it was interpreted as a special case of a ``doubly $\l$-deformed'' $\s$-model.
Our path-integral relation
between the $\l$-model \rf{1} and the truncated model \rf{6dmodel}
should be equivalent (at least at the classical and 1-loop level)
to the canonical equivalence between the doubly $\l$-deformed model
and two copies of the $\l$-model found in \cite{Georgiou:2017oly}
(upon setting one of the two $\l$-parameters to zero).
The leading order in $1/k$ (1-loop) renormalization of similar models
was also studied earlier in \cite{Gerganov:2000mt,LeClair:2001yp}.

Our central observation is that the ``truncated'' model \rf{6dmodel}
is automatically renormalizable to all orders with only $\tl$ (or equivalently $\l$) running. 
This is because, thanks to the decoupling of the first WZW term in \rf{277}, the truncated model is fully protected under the RG flow by its manifest symmetries:
the global $G$ symmetry (present in the usual formulation \rf{1G} of the $\l$-model),
\be \tih \to \tih \,  g_0 \ , \qquad \bh \to g_0^{-1} \, \bh \ , \qquad\qquad g_0 \in G \ , \ee
and chiral gauge symmetries (cf. the symmetry \eqref{cgs} of the WZW model),
\be \la{210}
\tih \to u(\s^-)\, \tih \ , \qquad \bh \to \bh\, w(\s^+) \ , \qquad \qquad u, w \in G\ , \ee
arising ubiquitously from the change of variables \rf{cov}. These symmetries uniquely  protect the structure of  \rf{6dmodel}, with $\tl$ and $\tk$ being the only free parameters.
 In particular, the chiral symmetries \rf{210} prohibit the appearance of other current-current interaction terms under the RG flow.  



We shall now directly compute the 2-loop $\b$-function for the coupling $\tl$ of the truncated \sm \rf{6dmodel} in large $\tk$ perturbation theory, demonstrating its renormalizability with only  $\tl$ (or $\l$) running. Let us emphasize that  --- modulo a finite renormalization, or redefinition, of $\l$ encoded in the choice of the coefficient $\q$ in \rf{jac1} --- the RG evolution of  the tripled \sm \rf{277} 
 is exactly equivalent to that of the $\l$-model \rf{1G},  since they were related at the level of the path integral including the necessary Jacobian \rf{jac1}.\foot{The
  $\b$-function of the truncated $G\times G$ model \rf{6dmodel} can actually be extracted from that of the more general $G\times G$ model studied in Chapter \ref{GGS} (given explicitly in App.\ \ref{2103GGapp}). For completeness, we explicitly run through the computation again here. The results are in agreement those in App.\ \ref{2103GGapp} for the special values of the parameters in \rf{crel}.}


Let us introduce the basis $\{T_A\}$ for $\Lie(G)$ (see Appendix \ref{conv} for conventions).
We shall use the indices $A$ and $\bar{A}$ respectively for the two
$G$-valued fields $\tih$ and $\bar{h}$ in \rf{6dmodel} (with the tangent space index for $G \times G$ denoted as
$M = \{A,\bar A\}$). As in
\cite{Georgiou:2017jfi} we introduce the vielbein
\begin{align}
&E^M = (e^A, e^{\bar{A}}) = (\sqrt{1-\tl^2}\, \RR^A,\, \LL^{\bar{A}} + \tl \RR^A) \ , \la{vielbein}\\
&\RR  \equiv T_A \RR^A  = \tih^{-1} d \tih\ , \qquad  \LL^{\bar{a}}  \equiv  T_A \LL^A =  d \bar{h} \bar{h}^{-1} \ ,
\end{align}
where $\RR$ and $\LL$ are the
currents that appear in the deformation term in \rf{6dmodel}.
Up to permutations, the non-zero components of the metric and $\H$-tensor of the $G\times G$ model \rf{6dmodel} are (cf. \eqref{13})
\begin{gather} \GG_{AB} = \GG_{\bar{A}\bar{B}} = \tfrac{\tk}{2} \, \Tr[T_A T_B]\ , \la{vielmet}
\\
\H_{ABC} = -i \tfrac{\tk}{2} \tfrac{\sqrt{1-\tl^2}(1+2\tl)}{(1+\tl)^2} f_{ABC} \ , \qquad
\H_{\bar{A}\bar{B}\bar{C}} = -i \tfrac{\tk}{2} f_{ABC} \ , \qquad
\H_{\bar{A}BC} = -i \tfrac{\tk}{2} \tfrac{\tl}{1+\tl} f_{ABC} \ . \la{Hflux}
\end{gather}
Our aim is to compute the corresponding 2-loop $\b$-function in \eqref{BMT}.
Let us formally define the torsion as
$T^M = \ha {\H^M}_{NP} E^N \wedge E^P $ where the tangent space index is raised with the inverse of the metric \rf{vielmet}.
Then, from the Cartan structure equation
$d E^M + {\widehat{\w}^M}{}_{N} \wedge E^N = T^M$, we obtain the torsionful spin connection
${{\widehat \w}^M}{}_{N} = {\widehat{\w}^M}{}_{NP} E^P$ with non-zero components
\be
(\tl^{-1}+1){{\widehat \w}^A}_{ \ B} =
\widehat \w^{\bar{A}}{}_{\bar{B}} = i f^{A}{}_{BC} \big(- \tfrac{\tl}{\sqrt{1-\tl^2}} e^C + e^{\bar{C}} \big) \ .
\ee
The non-zero components of the curvature,
${\widehat{R}^M}{}_{N} = d{\widehat{\w}^M}{}_{N} + {\widehat{\w}^M}{}_{P} \wedge {\widehat{\w}^P}{}_{N}=\ha {\widehat{R}^M}{}_{NPQ} E^P \wedge E^Q$, are then found to be
\begin{equation}\begin{split}\la{torsionriem}
(\tl^{-2}-1){\widehat{R}^A}{}_{BDE} =
-\sqrt{\tl^{-2}-1}{\widehat{R}^A}{}_{BD \bar{E} }
= {\widehat{R}^A}{}_{B \bar{D} \bar{E} } = - \frac{\tl}{(1+\tl)^2} f^A{}_{BC} f^C{}_{DE} \ .
\end{split}\end{equation}
Substituting \rf{torsionriem} into the 2-loop RG equation \eqref{BMT} in the \GB scheme, one obtains
\begin{equation}\la{220}
%(\beta^{(1)}_{\m\n} + \beta^{(2)}_{\m\n} )\,
\big[ \ddt(G_{mn} + B_{mn})\big]  dx^m \otimes
dx^n = \sum^{{\rm dim}\, G}_{A=\bar A=1}\Big[ \frac{2 \cg \tl^2}{(1+\tl)^2}
+ \frac{4 \cg^2}{\tk} \frac{\tl^4(1-2\tl)}{(1+\tl)^5(1-\tl)} \Big] \, \Tr[ \RR \,  \otimes \, \LL ] \ .
\end{equation}
Here $\otimes$ indicates that the product is not symmetrized.
We conclude that only the $\tl$-dependent term in \rf{6dmodel} gets renormalized, i.e.
the 2-loop RG equation \eqref{BMT} is solved with $\xi_m=\l_m=0$ and
\be\la{01}
\ddt \tk =0 \ ,\qquad \qquad \ddt \tl = \frac{2 \cg}{\tk} \Big[ \frac{\tl^2}{(1+\tl)^2} + \frac{2 \cg}{\tk} \frac{\tl^4(1-2\tl)}{(1+\tl)^5(1-\tl)} \Big] \ .
\ee
The 1-loop term here agrees with previous results, both for the standard $\l$-model (eq.\ \eqref{la1} with $\ka = \frac{\tl-1}{\tl+1}$)  \cite{Sfetsos:2014jfa,Appadu:2015nfa} and  the ``truncated'' $G\times G$ model \rf{6dmodel}
\cite{Georgiou:2017aei,Georgiou:2017jfi}).

The level $k=\tk-2\cg$ is thus RG-invariant as it should be. 
The fixed points of the RG flow are as expected:
 $\tl=\infty$ (i.e. $\l=0$), corresponding to the $G$ WZW model with level $k$, and 
$\tl=0$ (i.e. $\l=\infty$) corresponding to the $G/G$ cWZW model, or the $G$ WZW model with level $-k$ after integrating out the gauge field.
\unskip\foot{Taking
$\tl=1$ (i.e. $\l=1$) with finite $k$ (in contrast to the NAD limit
\eqref{limr}) gives the trivial $G/G$ gWZW model
in which one can fix a gauge so that the remaining degrees of
freedom correspond to the Cartan torus.}

Expressing $\tk$ and $\tl$ in \rf{redef} in terms of $k$ and the coupling
$\ka$ using \rf{133}, we find
\be\ddt k =0 \ ,\qquad \qquad
\ddt \ka = \frac{\cg}{4k}(1-\ka^2)^2 \Big[ 1 + \frac{\cg(1-\ka)^2 (1 -10\ka - 3 \ka^2)}{8k \ka} \Big] \ . \la{24}
\ee
Note that the 2-loop term in \rf{24} is scheme-dependent: it can be changed by
redefining $\ka$ by a $1/k$ term (or shifting $k$ by a finite term): for example, it will depend on the choice of the  parameter $\q$ in
\rf{jac1}.
Even though $k$ is not running, we effectively have a 2-coupling theory
(with $1/k$ playing the role of a loop-counting parameter)
so only the 1-loop term in the $\b$-function \rf{24} is scheme-independent.

In a general scheme, the symmetry $k \to - k, \ \l \to \l^{-1}$ \eqref{z2sym}
of the 1-loop RG equation in \rf{01},\rf{24} is not manifest 
at the 2-loop level.
To preserve it requires a particular formulation of the quantum theory, i.e.\
a specific definition of the couplings, or choice of scheme.
For example, if we redefine the parameters as
\begin{align} \la{2777}
(\tk, \tl) \to (\kk, \bl) \ , \qquad \qquad \tk =\kk + \cg\ , \qquad \quad \tl=\bl\Big[ 1 + \cg \kk^{-1} \frac{1-\bl}{1 +\bl} \Big]
\ , \end{align}
then the RG equation for $\bl$ resulting from \rf{01} is
\be \la{2789}
\frac{d}{dt}\bl = \frac{2 \cg}{\kk}\frac{\bl^2}{(1+\bl)^2}\Big[1 - \frac{2\cg}{\kk} \frac{\bl^2}{(1+\bl)^2} \frac{\bl+\bl^{-1}-1 }{1-\bl^2}
\Big] \ ,
\ee
which is invariant under
the following quantum version of \eqref{z2sym}
\be\la{227}
\kk \to -\kk \ , \qquad \qquad \bl \to \bl^{-1} \ .\ee
Note that here $\kk=k+ \cg$ is the same as the shifted level of the WZW theory.
It is also worth observing that \rf{2777} is not the only redefinition that
restores the symmetry \eqref{z2sym}. 
Indeed, even restricting to those that preserve the
existence of the fixed points and the NAD limit discussed below, there are many.

In the non-abelian dual (NAD) limit \eqref{limr} (i.e. $\ka= \tfrac14 \hh k^{-1}, \ k\to \infty$) when the $\l$-model \rf{1G} with unintegrated gauge field becomes the interpolating model \eqref{NADi} for non-abelian duality of the PCM,
the $\b$-function \rf{24} becomes
\be
\ddt \hh = {\cg} + \ha {\cg^2}\hh^{-1} \ . \la{25}
\ee
This result matches the standard expression  \eqref{Prg} for the 2-loop $\b$-function of the PCM on a simple group $G$ (see, e.g., \cite{McKane:1979cm,Hikami:1980hi,friedan}).  The 2-loop term in \rf{25} is scheme-independent as the NAD limit produces a single-coupling theory. Hence the scheme-dependent 2-loop term in the $\l$-model $\b$-function \rf{24} does still contain some invariant information, which passes a non-trivial test in this limit.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{``Tripled'' \texorpdfstring{$\l$}{lambda}-model based on a symmetric space \label{trips}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next let us consider the $\lambda$-model based on a symmetric space
 $G/\F$ (setting $P=P_{G/\F}$ in \rf{1}),
\be \begin{aligned}
%&\L  = k \, \Big( \L_G(g)   + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_- - A_+\big( 1 - (\l^{-1}-1)P_{G/H}\big) A_- ] \Big) \ , \\  %v2
&\L  = k \, \Big( \L_G(g)   + \Tr\big[ J_+ A_- - A_+ K_- + g^{-1} A_+ g A_- - A_+\big( 1 + (\l^{-1}-1)P_{G/H}\big) A_- ] \Big) \ , \\
&g\in G \ , \ \ A_\pm \in \Lie(G) \ . \la{ggu}
\end{aligned} \ee
This model has a special subgroup $H\subset G$ corresponding to its gauge symmetry, however we note that the 2d gauge field $A_\pm$ is still  valued in the algebra of the full group $G$. 

We shall repeat the same steps as in the group case above,   obtaining a  similar tripled formulation:
redefining $(A_+, A_-) \to (h,\bh)$ according to  \rf{cov}, using the Polyakov-Wiegmann identity (see footnote \ref{1910PW}), 
including the contribution from the Jacobian \rf{jac1}, and
setting $\tilde{g} = h^{-1} g \bar h$ and $ \tih=h^{-1}$, we now get
\be\la{effectivecoset1} \begin{aligned}
\L = {}&{}k \L_G (\tilde{g}) - (k+2\cg) \L_G ( \tih\bar{h} )+ k (\l^{-1}-1) \Tr [ \tih^{-1}\del_+ \tih \, P_{G/H} \, \del_- \bh \bh^{-1} ] \\
{}&{}
+ 2 \q \cg \Tr [ \tih^{-1}\del_+ \tih \, \del_- \bh \bh^{-1} ]\ . 
\end{aligned} \ee
Classically (i.e. for large $k$)
this model has the
expected $\F$ gauge symmetry
\begin{equation}\la{gsym}
\tih \to \tih \,  f \ , \qquad \bar h \to f^{-1}  \, \bar h \ , \qquad\qquad f=f(\s^+,\s^-) \in \F \ .
\end{equation}
Since the term proportional to $q$ in \rf{effectivecoset1}
 does not respect this gauge symmetry, then we
 should make the
 choice  $\q=0$ in the ambiguous Jacobian term in \rf{jac1}, 
corresponding to a natural scheme
preserving the gauge symmetry (this is the same choice as in the gWZW case \rf{ggr} above). Again applying the Polyakov-Wiegmann identity, we then obtain
\begin{equation}\begin{split}\la{effectivecoset2}
\L 
%& = {}&{} k \L_G (\tilde{g}) - (k+2\cg) \L_G ( \tih\bar{h} ) + k (\l^{-1}-1) \Tr [ \tih^{-1}\del_+ \tih \, P_{G/H}\, \del_- \bh \bh^{-1} ] \ ,
%\\
 &= k \L_G (\tilde{g}) - (k+2\cg) \big[\L_G ( \tih)
+ \L_G(\bar{h} )\big]\\
{}&{} \qquad \qquad \qquad  + \Tr [ \tih^{-1}\del_+ \tih\, \big(k+2\cg + k (\l^{-1}-1)  P_{G/H}\big)\, \del_- \bh \bh^{-1}] \ .
\end{split}\end{equation}
As in the group case, the first WZW term $k \L_G(\tilde{g})$ decouples,
leaving the RG flow  to be determined by the ``truncated'' $\s$-model,
\begin{align}
&\L'(\tih, \bh)
=- \tk \Big(\L_G ( \tih) + \L_G(\bar{h} ) - \Tr \Big[\tih^{-1}\del_+\tih\, (P_H + \tl \, P_{G/H})\, \del_-\bh\bh^{-1} \Big] \Big) \la{214} \ ,
% -\tl \Tr [ \tih^{-1}\del_+ \tih \, P_{G/H} \,\del_- \bh \bh^{-1}] \Big), 
\\
& \la{215}
\qquad \tk \equiv k + 2 \cg \ , \qquad \tl \equiv %1+ \frac{k {\g}}{k+2\cg}
\frac{k}{\tk}\l^{-1} +\frac{2 \cg}{\tk} \ .
%= \l^{-1} + \O (k^{-1} ) \ .
\end{align}
This  is a WZW model on  $G \times G$, deformed a left-right current interaction term, now containing projectors $P_\F$,$P_{G/\F}$ onto the subalgebra $\Lie(H)$ its orthogonal complement.
The classical integrability of the model \rf{214} (implying also the integrability of the $G/H$ $\l$-model)
was argued in \cite{Bardakci:1996gs} (example 4 there). It is also a special case of the integrable $G\times G/H$ models \cite{ABL} considered above in eqs.\ \eqref{2103couH},\eqref{2103bb1},\eqref{2103condH}, with the couplings and fields related according to
\be
\la{grel}
(k,r,s,u,t,b)=(-\tk, -\tk,-\tk,-\tk, \tk\tl,\tk\tl) \ , \qquad (g^{(1)},g^{(2)})=(\tih, \bh^{-1}) \ .
\ee

The  truncated model \rf{214}  is again automatically renormalizable due to manifest symmetries.
As well as the gauge symmetry \rf{gsym} and discrete symmetries,
it is also invariant under the same chiral gauge transformations \rf{210} as the group case. These symmetries protect the structure of \rf{214}, with $\tl$ and $\tk$ being the only free parameters.




We shall explicitly demonstrate the renormalizability of the symmetric space \lam \rf{ggu} by computing the 2-loop $\beta$-function for the truncated model \rf{214}.\foot{Like the group case above, the RG flow for the truncated model \rf{215} is a special case of the that of the $G\times G/H$ models in Chapter \ref{GGS} (given explicitly in App.\ \ref{2103GGHapp}). The results here are in agreement with those in App.\ \ref{2103GGHapp} for the special values of the parameters in \rf{grel}.}
The computation runs analogously to the group case above, with the only difference being that one must correctly handle the gauge invariance.
We decompose the generators $\{T_A\}$ of $G$
into the generators $\{T_\a\}$ of $H$ and the remaining generators $\{T_a\}$ chosen to be orthogonal to $\Lie{}(H)$ under the trace, i.e.\ splitting the algebra index of $G$ as $A=\{\a,a\}$ (see Appendix \ref{conv} for conventions). Since $G/H$ is a symmetric space then the $\mathbb{Z}_2$ grading of $\Lie(G)$ implies $f_{\a \b c} = f_{abc} =0$ (i.e. the only non-zero structure constants are $f_{
\a\b\g}$ and $f_{\a b c}$).
The tangent space index for $G \times G$ now splits as $M = \{ A; \bar{A} \} =\{\a, a; \bar{\a}, \bar{a} \}$, with the unbarred and barred indices corresponding respectively to the two $G$-valued fields $\hat h$ and $\bar{h}$.

Here we use the vielbein,
\be
E^M = (e^a, e^{\bar{a}}, e^\a, e^{\bar\a}) = (\sqrt{1-\tl^2} \RR^a, \, \LL^{\bar{a}} + \tl \RR^a, \,
\RR^\a + \LL^{\bar\a}, \, \RR^\a - \LL^{\bar \a}) \ . \la{vielbein2}
\ee
Up to permutations, the non-zero components of the metric and $\H$-tensor are
\begin{gather}
\GG_{ab} = \GG_{\bar{a}\bar{b}} = \tfrac{\tilde k}{2} \, \Tr[T_a T_b] \ , \qquad \GG_{\a\b} = \tfrac{\tilde k}{2}  \, \Tr[T_\a T_\b] \ ,
\\
\H_{\a\b\g} = -i \tfrac{\tilde k}{2} f_{\a\b\g} \ , \qquad \H_{\a bc} = - i \tfrac{\tilde k}{2} f_{\a bc} \ , \qquad \H_{\a \bar{b} \bar{c}} = - i \tfrac{\tilde k}{2} f_{\a bc} \ . \la{Hcoset}
\end{gather}
The $\F$ gauge symmetry of the model \rf{214} leads to the 
vanishing of all $\bar{\a}$-components of the metric and the $\H$-tensor.

As discussed in App.\ \ref{2103GGHapp},
there are various possible approaches  to treat the $H$ gauge symmetry.
Here we shall use the trick of lifting the degeneracy of the metric with a small parameter $\e$ acting as a ``regulator'',
\be \GG_{\bar \a \bar \b} = \e \, \tfrac{\tilde k}{2} \, \Tr[ T_\a T_\b] \ , \ee
computing the (torsionful) Riemann tensor, projecting out the $\bar{\a}$ directions and setting the regulator $\e$ to zero. This is a short-cut for a proper gauge-fixing procedure explained in footnote \ref{2103fgs}.


The resulting torsionful curvature has
the non-zero components 
\begin{equation}\begin{split}\la{torsionriem2}
(\tl^{-2}-1){\widehat{R}^a}{}_{bde} =
-\sqrt{\tl^{-2}-1}{\widehat{R}^a}{}_{b d \bar{e} }
= {\widehat R}^a{}_{b \bar{d} \bar{e} } = - f^a{}_{b\g} f^{\g}{}_{de} \ .
\end{split}\end{equation}
Substituting this
into the RG equation \eqref{BMT}, one obtains
\begin{equation}\la{2202}
{\big[ \ddt(\GG_{mn} + \BB_{mn})\big]} \, dx^m \otimes dx^n = \sum^{{\rm dim}\, G - {\rm dim}\, \F}_{i=\bar \imath=1}\Big[ \cg \tl + \frac{\cg}{\tk} \frac{ \tl(\cf - (2\cg - \cf)\tl^2)}{1-\tl^2} \Big] \, \Tr[\RR \,  \otimes \, P_{G/H}  \LL ] \ .
\end{equation}

We conclude that only the $\tl$-dependent term in \rf{214} gets renormalized, i.e.\
the 2-loop RG equation \eqref{BMT} is solved with $\xi_m=\l_m=0$ and
\be \la{02}
\ddt \tk =0 \ , \qquad \qquad \ddt \tl = \frac{\cg \tl}{\tk} \Big[ 1 + \frac{1}{\tk} \frac{ \cf - (2\cg - \cf)\tl^2}{1-\tl^2}\Big] \ .
\ee
The 1-loop term here agrees with the standard results for the symmetric space $\l$-model (eq.\ \eqref{la2} with $\ka = \frac{\tl-1}{\tl+1}$) \cite{Sfetsos:2014jfa,Appadu:2015nfa}.
The level $k$ is RG-invariant, and, as expected, $\tl =\infty$ and $\tl=0$ are fixed points.
At the fixed point $\tl = \infty$ ($\l=0$) the \lam reduces to the $G/\F$ gWZW model.
The other fixed point $\tl=0$ ($\l=-\tfrac{k}{2\cg}$) is a quantum-corrected version of the 1-loop fixed point $\l=\infty$; this model is like a version of the $G/G$ cWZW model with an additional $H$ gauge symmetry, and after integrating out $A_\pm$
it corresponds to   the $G/ H$ gWZW model with level $-k$.

Expressing $\tk$ and $\tl$ in \rf{215} in terms of $k$ and the coupling
$\ka$ using \rf{133}, we find
\begin{align}
&\ddt k =0 \ , \la{6d2loopbetacoset}
\qquad\qquad
\ddt \ka = \frac{\cg}{2k} \Big[ (1-\ka^2) + \frac{\cg(1-\ka)^2(1+4\ka-\ka^2) - \cf(1-\ka^4)}{2k\ka} \Big] \ .
\end{align}

As in the group space case \rf{24}, the 2-loop term in the
$\b$-function \rf{02} is, in general, scheme-dependent.
Again, we find that the symmetry under $k \to - k$, $\l \to \l^{-1}$ in \eqref{z2sym},
present at the 1-loop order is absent in the 2-loop term of \rf{02}.
However, after introducing the shifted level $\kk = \tk- \cg = k + \cg$ as in \rf{2777}, the 2-loop RG equation for $\tl$ \rf{02} becomes
\be
\ddt \tl = \frac{\cg \tl}{\kk} \Big[ 1 - \frac{1}{\kk} (\cg-\cf)
\frac{1+\tl^2}{1-\tl^2} \Big] \ ,
\ee
which is manifestly invariant under $\kk \to -\kk$, $\tl \to \tl^{-1}$, i.e.
a quantum version of the symmetry \eqref{z2sym} of the original couplings (cf. \rf{227}).

In the NAD limit \eqref{limr}, when the extended-space $\l$-model becomes the interpolating model \eqref{NADi} for NAD of the symmetric space, we get from \rf{6d2loopbetacoset}
\be
\la{555}
\ddt \hh = 2 {\cg} + 4{\cg (\cg - \cf)}{\hh}^{-1} \ .
\ee
As verified in Appendix B of \cite{HLT2}, equation \rf{555} is the correct 2-loop $\beta$-function for the $G/\F$ symmetric space $\s$-model (matching eq.\ \eqref{sb} above and, in particular cases, the results in \cite{Brezin:1975sq,Hikami:1980hi}). Like the group case above, the 2-loop coefficient here is also scheme-independent in this single-coupling limit, providing a non-trivial, scheme-invariant test of the $\l$-model's 2-loop $\b$-function.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Low-dimensional examples: \texorpdfstring{$\l$}{lambda}-models for \texorpdfstring{$SU(2)$}{SU(2)} and
\texorpdfstring{$SU(2)/U(1)$}{SU(2)/U(1)}\label{lowd}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let us study the simplest case of the truncated model \rf{6dmodel} in the group case with $G = SU(2)$.
Parametrizing
\begin{equation}\la{hhbpar}
\tih = \exp(i\phi \sigma_3) \exp(i \theta \sigma_1) \exp(i \psi \sigma_3) \ , \qquad\quad
\bh = \exp(i\bar \phi \sigma_3) \exp(i \bar \theta \sigma_1) \exp(i \bar \psi \sigma_3) \ ,
\end{equation}
where $\sigma_A$ are the standard Pauli matrices, we find the following 6-dimensional metric and $\BB$-field (with $\BB = \ha \BB_{mn} dx^m \wedge dx^n$)
\begin{align}
&\qquad \qquad ds^2  = (ds^2)_{G\times G} + (ds^2)_{\rm int} \ , \qquad \quad  \BB = \BB_{G\times G} +  \BB_{\rm int} \ , \la{su2geom}
\\ \no
&(ds^2)_{G\times G}   = - \tk (d\theta^2 + d\phi^2 + d\psi^2 + 2\cos 2\theta d\phi d\psi +
d\bar\theta^2 + d\bar\phi^2 + d\bar\psi^2 + 2\cos 2\bar\theta d\bar\phi d\bar\psi) \ ,
\\ \no
&\BB_{G\times G}   = - \tk(\cos2\theta d\phi\wedge d\psi + \cos 2\bar \theta d\bar \phi \wedge d\bar \psi) \ ,
\\ \no
&(ds^2)_{\rm int}  = - 2\tk\tl \big[\cos 2(\psi+\bar\phi) (d\theta d\bar \theta - \sin 2\theta \sin 2\bar \theta d \phi d\bar \psi) + ( d\psi +\cos2\theta d\phi)(d\bar \phi + \cos 2\bar \theta d \bar \psi)
\\ \no & \qquad  \qquad \qquad \qquad + \sin 2(\psi+\bar \phi)(\sin 2 \theta d\phi d \bar \theta + \sin 2 \bar \theta d \theta d \bar \psi)\big] \ ,
\\ \no
&\BB_{\rm int}  = -\tk\tl \big[\cos 2(\psi+\bar\phi) (d\theta \wedge d\bar \theta - \sin 2\theta \sin 2\bar \theta d \phi \wedge d\bar \psi) + ( d\psi +\cos2\theta d\phi)\wedge(d\bar \phi + \cos 2\bar \theta d \bar \psi)
\\ & \qquad \qquad \qquad \qquad + \sin 2(\psi+\bar \phi)(\sin 2 \theta d\phi \wedge d \bar \theta + \sin 2 \bar \theta d \theta \wedge d \bar \psi)\big] \ . \no
\end{align}
Here the ``$G\times G$'' terms come from the WZW models and the ``int'' terms come from the current-current interactions between them.
One can check explicitly that this metric and $\BB$-field solve the 2-loop RG equation \eqref{BMT} with vanishing $\xi^m$ and $\l_m$, and the couplings running as in \rf{01} (with the dual Coxeter number $c_{_{SU(2)}} = 2$).

Next, let us consider the truncated model \rf{214} obtained from the $\l$-model  based on the symmetric space $G/\F = SU(2)/ U(1)$.
Using the parametrization for $\tih$ and $\bar{h}$ given in eq.\ \rf{hhbpar},
we find that the corresponding
target space background depends on $\psi$ and $\bar\phi$ only
through the combination $\chi = \psi + \bar \phi$, which is a manifestation of the $U(1)$ gauge symmetry.
The resulting 5-dimensional metric and $\BB$-field are
\begin{align}
&\qquad \qquad ds^2  = (ds^2)_{G\times G/H} +(ds^2)_{\rm int} \ , \qquad \qquad \BB = \BB_{G\times G/H} + \BB_{\rm int} \ ,
\\ \no
&(ds^2)_{G\times G/H}  = - \tk (d\theta^2 + d\phi^2 + d\bar\theta^2 + d\bar\psi^2 ) \ , \qquad \BB_{G\times G/H} = 0 \ ,
\\ \no
&(ds^2)_{\rm int}  = - 2\tk\tl \big[\cos 2\chi (d\theta d\bar \theta - \sin 2\theta \sin 2\bar \theta d \phi d\bar \psi)
+ \sin 2\chi(\sin 2 \theta d\phi d \bar \theta + \sin 2 \bar \theta d \theta d \bar \psi)\big]
\\ \no & \qquad  \qquad \qquad \qquad + \tk d\chi^2 -2\tk( d\chi +\cos2\theta d\phi)(d \chi + \cos 2\bar \theta d \bar \psi)
\ ,
\\ \no
&\BB_{\rm int} = -\tk\tl \big[\cos 2\chi (d\theta \wedge d\bar \theta - \sin 2\theta \sin 2\bar \theta d \phi \wedge d\bar \psi)
+ \sin 2\chi(\sin 2 \theta d\phi \wedge d \bar \theta + \sin 2 \bar \theta d \theta \wedge d \bar \psi)\big]
\\ & \qquad  \qquad \qquad \qquad -\tk( d\chi +\cos2\theta d\phi)\wedge(d\chi + \cos 2\bar \theta d \bar \psi)\ .\no
\end{align}
Again one can check explicitly that this metric and $\BB$-field solve the 2-loop RG equation
\eqref{BMT} with vanishing $\xi^m$ and $\l_m$, and the couplings running as in \rf{02}
(with the dual Coxeter numbers  $c_{_{SU(2)}}=2$ and $c_{_{U(1)}}=0$).

\section{``Tripled'' formulations of other models \la{TO}}
In principle the trick of rewriting 2d gauge fields in terms of group-valued scalars can be applied to any theory with 2d gauge fields. In this section, containing unpublished work, we shall construct analogous ``tripled'' or ``extended'' formulations of two other classes of $\s$-models.


\subsection{\texorpdfstring{$G^N$}{G^N} \texorpdfstring{$\l$}{lambda}-models}
First let us consider a  generalization of the $\l$-model to $N$ copies of the group $G$, which was recently obtained from affine Gaudin models \cite{Bassi:2019aaf},
\be
\L = k_i  \, \L_{G/G}(g^{(i)}, A^{(i)}) - \ha \,  \g_{ij} \, \Tr[ A^{(i)}_+ A^{(j)}_- ] \ ,  \qquad \qquad i=1,\ldots n \ .\la{ln}
\ee
Here $k_i$ are the WZ levels and  $\g_{ij}$ is $2\times 2$ matrix of coupling constants. Integrating out the quadratic gauge fields $A_\pm^{(i)}$ yields a $\s$-model with scalar fields $g^{(i)} \in G$.

This may be viewed as an example of  Tseytlin's ``universal class'' model \eqref{uc} adapted to $G^N$, with the constant operator $Q$ chosen to preserve the  global  $G$  symmetry $(g^{(i)}, A^{(i)}) \to (u g^{(i)} u^{-1},u A^{(i)} u^{-1})$, $u\in G$. Like the $G^N$ models discussed in Chapter \ref{GGS}, the theory \rf{ln} is classically integrable only for special values of the coupling constants $(k_i,\g_{ij})$, parametrized algebraically in terms of the twist function in \cite{Bassi:2019aaf}. Although we shall not work out the details here, this parametrization may be recast as a set of polynomial equations in $(k_i,\g_{ij})$ (cf. the equation \eqref{2103cond} for undeformed $G\times G$ models).

Like standard $\l$-models, the $G^N$ $\l$-model \rf{ln} is a deformation of a WZW model (when $\g_{ij}$ is taken to infinity while being non-degenerate)
and becomes in a particular limit, $k_i \to \infty$, $g^{(i)} = e^{-\tfrac{v^{(i)}}{2k_i}}$, the non-abelian dual of a particular $G^N$ model \eqref{2103cou} in its $(G_L)^N$ symmetry,
\be
\L = - \ha  \, \Tr[ \g_{ij}  A^{(i)}_+ A^{(j)}_-   -  v^{(i)} F_{+-}(A^{(i)})] \ , \qquad F_{+-}(A) \equiv  \del_+ A_- - \del_- A_+ + [A_+, A_-] \ .
\ee

Our observation is that the tripled formulation of the $\l$-model generalizes very easily to this $G^N$  case. Let us perform the same change of variables $(A^{(i)}_+,A^{(i)}_-) \to (h^{(i)}, \bh^{(i)})$ on each copy of the group, where  $A^{(i)}_+= h^{(i)} \del_+ \big(h^{(i)}\big)^{-1} $, $A^{(i)}_- = \bh^{(i)} \del_- \big(\bh^{(i)}\big)^{-1}$ (cf.\ eq.\ \rf{cov}). Including the Jacobian \rf{jac1} for this transformation (and picking again $\q=-1$), the resulting theory is a ``tripled'' $\s$-model with fields $(g^{(i)},h^{(i)},\bh^{(i)}) \in G^{3N}$,
\be \begin{aligned} \la{ne}
&\L = k_i  \,\L_G(\tilde{g}^{(i)}) + \L'(\hat{h}^{(i)}, \bh^{(i)}) \ , \qquad \qquad \tilde{g}^{(i)} \equiv\big( h^{(i)}\big)^{-1} g^{(i)} \bh^{(i)} \ , \quad \hat{h}^{(i)}\equiv \big(h^{(i)}\big) \ , \\
&\L' = -(k_i+2\cg)\big[ \L_G(\hat{h}^{(i)}) + \L_G(\bh^{(i)}) \big] + \Tr\big[ (k_i  \d_{ij} -\ha \g_{ij}) \, J_+^{(i)} \, \bar{K}_-^{(j)} \big] \ , \\
&\qquad J_+^{(i)} \equiv \big(\hat{h}^{(i)} \big)^{-1} \del_+ \hat{h}^{(i)} \ , \qquad \bar{K}_-^{(i)} \equiv \del_+ \bh^{(i)} \big( \bh^{(i)} \big)^{-1} \ . \la{trin}
\end{aligned} \ee
This is a particular case of the undeformed $G^M$ model  \eqref{2103cou} with $M=3N$ (after a redefinition $\bh^{(i)} \to \big( \bh^{(i)}\big)^{-1} $).

As in the $\l$-model considered above, the first WZW terms $k_i \, \L_G(\tilde{g}^{(i)})$ in \rf{ne} decouple, leaving the RG flow to be determined by the ``truncated'' Lagrangian $\L'$, which is a $\s$-model with fields $(h^{(i)},\bh^{(i)}) \in G^{2N}$. This truncated theory is also a particular case of  the undeformed  $G^M$ model  \eqref{2103cou} with $M=2N$.

Hence we have produced a quantum equivalence between (i) the $\l$-deformation \rf{ln} based on $G^N$ models  and (ii) certain $G^M$ models with $M=2N$ (plus $N$ decoupled WZW models). In effect, moving from the $G^N$ model to the related $\l$-deformation is equivalent to replacing $N\to 2N$, restricting to particular class of the $G^{2N}$ model's couplings, and adding $N$ decoupled WZW models.

\bigskip 
Let us make some observations. As mentioned above, the $G^N$ $\l$-model is only integrable for special values of the couplings solving polynomial equations. This is indeed consistent with the equivalence found here, since the same is true for the undeformed $G^M$ models of which the tripled formulation \rf{trin} is a special case. Hence one should be able to understand the integrability conditions for $G^N$ $\l$-models in terms of those of undeformed $G^M$ models; in this respect the $\l$-deformation does not introduce any new elements. It would be interesting to understand the relation between these models at the level of affine Gaudin models and the twist functions.

Renormalizability of the $G^N$ $\l$-model  \rf{ln} does not seem obvious based alone on its manifest $G$ symmetry, which  is not  sufficient to protect the form of the action. However, in the tripled formulation \rf{trin}, there is again a decoupling of some fields $\tilde{g}^i$ and the remaining  truncated theory $\L'$ is protected by $G(\xi^-)^N \times G(\xi^+)^N \times G$ chiral gauge symmetry,
\be
\begin{aligned}
&(\hat{h}^{(i)}, \ \bh^{(i)}) \to (u^{(i)}(\xi^-) \,  \hat{h}^{(i)}  \, w,  \   w^{-1} \, \bh^{(i)}  \, v^{(i)}(\xi^+))  \ ,\\
&u^{(i)}(\xi^-) \in G(\xi^-) \ , \quad v^{(i)}(\xi^+) \in G(\xi^+) \ , \quad w\in G \ ,
\end{aligned}
\ee
which uniquely fixes the theory up to the parameters $(k_i, \g_{ij})$.  Hence it will be renormalizable to all orders with just $\g_{ij}$ running (while the WZ levels do not run for general reasons).  Since the original and tripled formulations are equivalent at the quantum level then we have proved  the renormalizability of the $G^N$ $\l$-model \rf{ln} with  unintegrated gauge field  to all orders.

So far we have established the renormalizability of the  $G^N$ $\l$-model \rf{ln} before imposing the integrability condition. We expect the ``integrable surface'' in the space of couplings $(k_i,\g_{ij})$ to be a stable  subspace under the RG flow (cf. the $G\times G$ and $G\times G/H$ models studied in Chapter \ref{GGS}). It would be interesting to check this fact and to see whether the integrability conditions require quantum corrections to remain stable beyond 1-loop. The tripled formulation \rf{trin} is the natural arena to study these questions since it is already RG-stable with a finite set of couplings  before imposing the integrability condition.



\subsection{\texorpdfstring{$G\times G/H$}{GxG/H}  models}
Now let us consider the $H$-gauge-invariant  $G\times G/H$ models considered in Section \ref{2103gu}, with Lagrangian,
\be \begin{aligned}
&\L = -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] -\ha \, r_{ij} \, \Tr[ \B^{(i)}_+ \B^{(j)}_- ] + k_i  \, \L_{_{\rm WZ}}(g^{(i)}) \ ,  \\
&
 k_1 = - k_2\equiv k  \ , \qquad  r_{ij} = \begin{pmatrix} r  & - r - k \\ -r +k & r  \end{pmatrix} \ , \\
& P^{(i)} = P_{{G/H}}  J^{(i)} \ , \qquad   \B^{(i)} = P_H J^{(i)}\ ,  \ \ \qquad 
 J^{(i)} =  {g^{(i)}}^{-1} d g^{(i)}  \ . % \quad  (g^{(i)}) \in G^N  \ ,
  %\ \  i=1,2 \ , 
  \la{ghr}
\end{aligned} \ee
First let us re-write the theory in terms of a 2d gauge field by starting with an ungauged ($G\times G$)-type model (here $R_{ij}$ are arbitrary constants and $k_1=-k_2=-k$),
\be
\L = -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] -\ha \, R_{ij} \, \Tr[ \B^{(i)}_+ \B^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \ ,
\ee
and gauging the $H$  global symmetry $(g^{(1)}, g^{(2)}) \to (g^{(1)} h, g^{(2)} h)$, $h\in H$ by the same gauging procedure discussed for coset spaces in Section \ref{sssm}. Promoting $h \to h(\xi)$ to a local parameter, the  Lagrangian transforms as
\be\begin{aligned}
&\L \to -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \\
&\qquad   -\ha \, \Tr[ R_{ij} \, \B^{(i)}_+ \B^{(j)}_-  + \del_+ h h^{-1} (\a \,  B_-^{(1)} +\b \, B_-^{(2)}) 
\\
&\qquad  \qquad\qquad  \qquad\qquad  \qquad \quad 
+ \del_- h h^{-1} (\g  \, B_+^{(1)} +\d  \, B_+^{(2)} ) + \e \, \del_+ h h^{-1} \, \del_- h h^{-1} ] , \\
&\a = R_{11} + R_{21} - k \ , \quad \b = R_{12}+R_{22}+k \ , \\
&\g = R_{11} + R_{12} + k \ , \quad \d = R_{21}+R_{22}-k \ , \quad \e = R_{11}+R_{12}+R_{21}+R_{22} \ . \la{prev}
\end{aligned}\ee
Now promoting $\del_+ h h^{-1} \to - A_\pm$ in the transformed Lagrangian \rf{prev}, the resulting theory is gauge invariant (under $g \to h^{-1} g h$, $A_\pm \to h^{-1} A_\pm h + h^{-1} \del_\pm h$,\ \, $h(\xi)\in H$),
\begin{align}
\L(g,A) = {}&{}-\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big)   \la{Am} \\
&   -\ha \, \Tr[ R_{ij} \, \B^{(i)}_+ \B^{(j)}_-  - A_+ (\a \,  B_-^{(1)} +\b \, B_-^{(2)}) 
%\\
%&  \qquad\quad  
-  A_- (\g  \, B_+^{(1)} +\d  \, B_+^{(2)} ) + \e \, A_+ A_- ] \ . \no
\end{align}
Upon integrating out the 2d gauge field $A_\pm$, one indeed obtains the desired  $G\times G/H$ model  \rf{ghr} with the following identification of parameters
\be
r = \frac{k^2 + k (R_{12}-R_{21}) + R_{11} R_{22} - R_{12} R_{21}}{R_{11}+R_{12}+R_{21}+R_{22}} \ , \qquad k=k \ . \la{ip}
\ee

Hence  the model \rf{Am} with the gauge field is equivalent to the $G\times G/H$ model \rf{ghr} and, moreover, only one combination of the couplings $R_{ij}$ appears after integrating out $A_\pm$. This means one is free to fix any 3 components (or combinations of components) of $R_{ij}$ to arbitrary values, as long as  $R_{11}+R_{12}+R_{21}+R_{22} \neq 0$ so that \rf{ip} does not diverge. 

For general $R_{ij}$ we may again change variables $(A_+, A_-) \to (h,\bh)$ according to \rf{cov} (this is like replacing $\del_- h h^{-1} \to \del_- \bh \bh^{-1}$ in \rf{prev}). The resulting theory is a $\s$-model with an enlarged configuration space $(g^{(1)}, g^{(2)}, h, \bh) \in G\times G \times H \times H$,
\be \begin{aligned}
\L(g^{(1)},g^{(2)},h,\bh) = {}&{}-\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \\
&   -\ha \, \Tr[ R_{ij} \, \B^{(i)}_+ \B^{(j)}_-  + \del_+ h h^{-1} (\a \,  B_-^{(1)} +\b \, B_-^{(2)}) \\
&  \qquad\qquad\qquad\quad  + \del_- \bh \bh^{-1}  (\g  \, B_+^{(1)} +\d  \, B_+^{(2)} ) + \e \, \del_+ h h^{-1}  \del_- \bh \bh^{-1} ] \ .  \la{AM}
\end{aligned}\ee
One may fix the gauge symmetry as, e.g., $\bh=1$ (or $A_-=0$) to obtain
\be \begin{aligned}
&\L(g^{(1)},g^{(2)},h) = -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \\
& \qquad \qquad \qquad \qquad \qquad \quad   -\ha \, \Tr[ R_{ij} \, \B^{(i)}_+ \B^{(j)}_-  + \del_+ h h^{-1} (\a \,  B_-^{(1)} +\b \, B_-^{(2)}) ] \ , \la{gff} \\
&\a = R_{11} + R_{21} - k \ , \qquad \b = R_{12}+R_{22}+k \ . 
\end{aligned}\ee
The resulting gauge-fixed model \rf{gff} is a $\s$-model with configuration space $(g^{(1)}, g^{(2)}, h) \in G \times G \times H$.  It may be described as a particular ``squashed'' $G\times G\times H$ model, since the $G\times G$ sector includes dependence on the projectors $P_H$ and $P_{G/H}$. 


One simple example of \rf{gff} obtained from the choice
\be
R_{ij} = \begin{pmatrix}
r & 0 \\
-r+k & 0 
\end{pmatrix} \ , \la{Rc}
\ee
is given by
\be\begin{aligned}
\L(g^{(1)},g^{(2)},h) ={}&{}-\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \\
&   -\ha \, \Tr[ (r \B^{(1)}_+ + (k-r) \B^{(2)}_+ )\B^{(1)}_-  + k \, \del_+ h h^{-1} B_-^{(2)}  ] \ . \la{gfm}
\end{aligned}\ee

Another natural choice consistent with \rf{ip} is 
\be
R_{ij} = \eps \,  \rho_{ij} \  , \qquad r = \frac{k^2 \e^{-1} + k  (R_{12}-R_{21}) + \e (R_{11} R_{22} - R_{12} R_{21})}{R_{11}+R_{12}+R_{21}+R_{22}}  \ .
\ee
Then \rf{gff} becomes 
\be\begin{aligned}
&\L(g^{(1)},g^{(2)},h) = -\ha \, \rho_{ij} \, \Tr[ \e B^{(i)}_+ B^{(j)} + P^{(i)}_+ P^{(j)}_- ] + k  \, \big( \L_{_{\rm WZ}}(g^{(1)})- \L_{_{\rm WZ}}(g^{(2)}) \big) \\
& \qquad \qquad \qquad \quad   -\ha  \, \Tr[  \del_+ h h^{-1}  \, \big(\a \,  B_-^{(1)} +\b \, B_-^{(2)}\big) ] \ ,  \la{gfm2} \\
&\a = \e( \r_{11} + \r_{21}) - k \ , \qquad \b = \e(\r_{12}+\r_{22}) +k \ . 
\end{aligned}\ee




These extended-space reformulations of the $G\times G/H$ models will inherit the same classical integrability and RG flow properties as the original theory (modulo the inclusion of a Jacobian of the same form as \rf{jac1}). Hence we learn that the extended $G\times G \times H$ models \rf{gff} (and the particular cases \rf{gfm} and \rf{gfm2}) should also be integrable when the couplings $r,k,\rho_{ij}$ satisfy the integrability conditions \eqref{2103condH} of the $G\times G/H$ model.
Speculatively, one might hope that, after imposing the integrability conditions, there could be a decoupling of some fields (as for the $\l$-models studied above), which may leave the remaining theory  manifestly renormalizable due to its global symmetries. Such a phenomenon would be interesting as (i) it could provide  another origin for the integrability conditions \eqref{2103condH} of the $G\times G /H$ model and (ii) in such a reformulation, the $G\times G/H$ model's integrability condition would become automatically stable at higher-loop orders (cf. eq. \eqref{2103318} in the standard formulation).




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}\la{conclusions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Formulating the \lam on an extended
($G\times G\times G$)
configuration space
``linearizes'' the RG flow, i.e.\ makes its renormalizability manifest without the need
for extra local counterterms apart from the running of the coupling $\l$. 
This implies that the $\l$-model with {unintegrated} gauge field is renormalizable to all orders.


 As well as eliminating  the need for quantum corrections to remain renormalizable at higher-loop orders,  the tripled formulation also explains  the $\l$-model's renormalizability already at the 1-loop order. Whereas the standard formulation \rf{1} is apparently protected under the RG flow by \textit{hidden} symmetries,  the tripled formulation is protected by \textit{manifest} symmetries.
 
The decoupling of one of the WZW models $k \L_G(\tilde g)$ in \rf{277} and \rf{effectivecoset2} appears to be the special property that renders the manifest global symmetries sufficient for renormalizability of the remaining ``truncated'' models. This property should be associated with integrability, since it would be lost under generic deformations of the $\l$-model \rf{1} preserving its manifest symmetries but breaking integrability. It would be interesting in future to understand  the precise relationship between integrability and this special decoupling in the tripled formulation.
 


\

In the non-abelian dual limit \eqref{limr}, the resulting scheme-invariant 2-loop $\b$-functions  matched the known $\b$-functions for the PCM and symmetric space. One may regard this tripled computation as a particular scheme for  the renormalization of  the interpolating models \eqref{NADi} for non-abelian duality (obtained from the tripled $\l$-model in this limit). One might worry that the NAD limit could be too singular to commute with the RG flow (e.g., the decoupling of the $\L_G(\tilde g)$ term in \rf{277} breaks down in that limit),
but  this is not likely since one can independently argue the renormalizability of the interpolating models  \eqref{NADi}
 through their relation to the original PCM/symmetric space models
by 
 an integral over the linear Lagrange multiplier $v$.
 This integral is not summing any loops as $v$ only appears linearly, so the classical result $\delta(F_{+-}(A))$ is expected to be consistent with the RG flow, without needing any extra counterterms.\foot{I thank A.A. Tseytlin for a discussion of this point.} It would be interesting in future to check this fact directly, e.g.\  computing the RG flow for a ``tripled'' formulation of the interpolating models for NAD.
 
 If one regards the  interpolating models, or the corresponding tripled $\s$-models, as  particular formulations of the corresponding NAD theories at the quantum level,
 then 
it is natural to conclude that non-abelian duality  commutes
with the RG flow beyond the 1-loop order on arbitrary  groups $G$  and symmetric spaces $G/H$,
with the original and NAD models having the same 2-loop $\beta$-function. This is in line with  previous 1-loop conclusions \cite{Fridling:1983ha,Fradkin:1984ai}  and resolves related confusions at the 2-loop level \cite{n1,n2,n3,Bonneau:2001za}.

 
\


Hence, for  (i) the $\l$-models with unintegrated gauge field and (ii) the  interpolating models for NAD,
  the non-trivial corrections that were required in the standard configuration space in Chapter \ref{QCS} should be
understood as finite counterterms resulting from the integral over the 2d gauge field appearing quadratically in the action.
It remains to understand the general structure of those counterterms, or equivalently the 
correct prescription for the 2d gauge field integral consistent with integrability
(generalizing \eqref{7}, which was sufficient only in the simple $SU(2) \ov U(1)$ example).

 The 2-loop $\b$-functions \rf{24} and \rf{6d2loopbetacoset} obtained through the tripled formulation are consistent with those found for
particular examples of the $\l$-model in the standard formulation in eqs.\ \eqref{49} and \eqref{19100}, modulo a redefinition of the couplings $k,\l$, i.e.\ scheme change (see \cite{HLT2} for the precise redefinitions that relate them). In particular this means that the
scheme-invariant 1-loop terms match exactly; moreover the 2-loop terms also match in the single-coupling  NAD limit when they become scheme-invariant.



\ 



\sloppy
A similar ``tripled'' approach may also be useful
for clarifying the higher-loop deformation in abelian T-duality.
For example, consider the metric \mbox{$ds^2 = dy^2 + a(y) dx^2$} and its classical dual
\mbox{$\wt{ds^2} = dy^2 + a(y)^{-1} d\td x^2$,}
with the interpolating model given by
\be
-\L= (\del_\m y)^2 + a(y) (p_\m)^2 + \td x \, \e^{\m\n}  \del_\m p_\n \ ,
\ee
such that $y$ is a spectator coordinate (cf.\ eq.\ \eqref{int}).
If we integrate out $\td x$ to give $p_\m = \del_\m x$, we recover the
original model for $x$.
If we integrate out $p_\m$, we find the T-dual model for $\td x$.
If instead we set $p_1=\del_1 x $ and integrate out $p_0$ we get the
``doubled'' model of \cite{Tseytlin:1990va} for $x$ and $\td x$ (equivalent
to the ``axial'' gauge choice in the Appendix of \cite{Rocek:1997hi}).
The  ``tripled'' model for ($x, \td x, \bar x$), analogous to the ones discussed above, is obtained by setting \mbox{$p_\m= \del_\m x + \e_{\m\n}\del^\n \bar x$:}
\be
-\L =  (\del_\m y)^2 + a(y) [ (\del_\m x)^2 - (\del_\m \bar x)^2 + 2 \e^{\m\n} \del_\m x \del_\n \bar x ] + \del_\m \td x \del^\m \bar x  \ .
\ee
This may be interpreted as a \sm on 4-dimensional target space with pp-wave metric and $\BB$-field.


\ 





We also considered similar ``tripled'' or ``extended'' formulations for other models.  
We found that the tripled formulation of the $\l$-model generalizes easily to $\l$-models based on $G^N$. In this tripled formulation, it is clear that the $G^N$ $\l$-models are renormalizable to all orders due to manifest symmetries (before imposing the integrability condition). 
The resulting tripled $\s$-models are particular class of $G^{3N}$ models, or  $G^{2N}$ models after removing decoupled WZW models. 
 Hence in this case we find a correspondence between the integrability and RG flow properties of $G^N$ $\l$-models and certain undeformed $G^{2N}$ models.
 
 
 We reformulated the $G\times G/H$ models studied in Chapter \ref{GGS} in terms of a gauge field and  found a 3-parameter family of extended formulations (3 of the components of $R_{ij}$, with the 4th being fixed by the relation \rf{ip}). The resulting $\s$-model has configuration space $G\times G\times H \times H$, or $G\times G\times H$ after fixing the $H$ gauge symmetry. Hence we find a correspondence between the integrability and RG properties of $G\times G/H$ models and certain  ``squashed'' $G\times G \times H$ models.  It would be interesting to study the RG flow for both   $G^N$ $\l$-models and $G\times G/H$ models in these new, extended formulations.


A useful extension of the tripled formulation  would be to the $\eta$-model. 
Up to analytic continuation, the $\eta$-model and \lam are related by limits and T-duality \cite{Hoare:2015gda,Hoare:2017ukq}
or by Poisson-Lie duality \cite{Hoare:2015gda,Klimcik:2015gba,Vicedo:2015pna,Hoare:2017ukq},
so it seems plausible that the tripled formulation of the $\l$-model could lead to a similar approach for the $\eta$-model.
This could allow a generalizaton of our results for the $SU(2) \ov U(1)$ $\eta$-model in Section \ref{Seta} to general groups and symmetric spaces.



Another obvious generalization would be  to $\s$-models on supergroups and
supercosets (see, e.g.,
\cite{Kagan:2005wt,Babichenko:2006uc,Zarembo:2010sg,Appadu:2015nfa}), and to integrable-deformed superstring $\s$-models.
See Section \ref{stric} for further discussion of this possibility.

  


==> v arxiv v2/2008.tex <==
%\documentclass[12pt,a4paper]{article}
%\pdfoutput=1
%\usepackage[english]{babel}
%\usepackage[latin1]{inputenc}
%\usepackage[T1]{fontenc}
%\usepackage{amsfonts,amsbsy,bm,euscript,mathrsfs}
%\usepackage{amssymb,faktor,slashed}
%\usepackage{color}
%\usepackage[tbtags]{amsmath}
%\usepackage[bookmarks=true,colorlinks=true,linkcolor=black,citecolor=black,urlcolor=black,bookmarksnumbered,linktocpage=true]{hyperref}
%\usepackage{graphicx}
%\usepackage{chngcntr}
%\usepackage{makecell}
%\usepackage{mathtools}

%\usepackage[left]{showlabels}
%\usepackage{showkeys}

%\usepackage[a4paper,text={170mm,257mm},centering]{geometry}
%
%\numberwithin{equation}{section}
%
%\renewcommand{\arraystretch}{1.3}

%\makeatletter
%\renewcommand\section{\@startsection {section}{1}{\z@}%
%{-3.5ex \@plus -1ex \@minus -.2ex}%
%{2.3ex \@plus.2ex}%
%{\normalfont\large\bfseries}}
%\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
%{-3.25ex\@plus -1ex \@minus -.2ex}%
%{1.5ex \@plus .2ex}%
%{\normalfont\normalsize\bfseries}}
%\makeatother

%\expandafter\def\expandafter\bfseries\expandafter{\bfseries\ifmmode\else\boldmath\fi}
%\expandafter\def\expandafter\mdseries\expandafter{\mdseries\ifmmode\else\unboldmath\fi}
%\expandafter\def\expandafter\normalfont\expandafter{\normalfont\ifmmode\else\unboldmath\fi}

%\providecommand{\href}[2]{#2}


%\newcommand{\arxivlink}[1]{\href{http://arxiv.org/abs/#1}{[arXiv:#1]}}
%\newcommand{\doilink}[2]{\href{http://doi.org/#2}{#1}}
%
%\newcommand{\mathsym}[1]{{}}
\def\id{\protect{{1 \kern-.28em{\rm l}}}}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\bi{\bibitem}
\def\tr{{\rm tr}}
\def\ha{\tfrac{1}{2}}
\def\td{\tilde}
\def\ci{\cite}
\def\N{{\mathcal N}}
\def\ww{\Omega}
\def\S{{\mathcal S} }
\def\nn{\nu}
\def\z{\zeta}
\def\dg{\dagger}
\def\a{\alpha}
\def\b{\beta}
\def\ap{\alpha^\prime}
\def\aa{{\a'}}
\def\g{\gamma}
\def\ok{\frac{1}{k}}
\def\jL{{J}}
\def\cL{{\mathcal L}}
\def\cH{{\mathcal H}}
\def\E{{\mathcal E}}
\def\w{\omega}
\def\vep{\varepsilon}
\def\De{{\mathcal D}}
\def\k{\kappa}
\def\four{\tfrac14}
\def\third{\tfrac{1}{3}}
\def\det{\hbox{det}}
\def\tid{\tilde}
\def\vv{{\rm v}}
\def\ta{{\tilde \a}}
\def\fo{\frac{1}{4}}
\def\K{{\rm S}}
\def\el{\ell}
\def\Tr{{\rm Tr}}
\def\P{\Phi}
\def\l {\lambda}
\def\bl{{\tilde \l}}
\def\const{{\rm const}}
\def\vn{\vec n}
\def\Prod{\Pi}
\def\O{{\mathcal O}}
\def\m{\mu}
\def\vs{\vec \s}
\def\ie{i.e.}
\def\rS{{\rm S}}
\def\as{{\a}}
%\newcommand{\bra}[1]{\mbox{$\langle #1 |$}}
%\newcommand{\ket}[1]{\mbox{$| #1 \rangle$}}
%\newcommand{\auth}{AUTHORS}
\def\foot{\footnote}
%\newcommand{\rf}[1]{(\ref{#1})}
\def\ra{\rightarrow}
\def\F{{\cal F}}
\def\cc{\circ}
\def\eqv{\equiv}
\def\ni{\noindent}
\def\bw{{\rm w}}
\def\cT{{\cal T}}
\def\no{\nonumber}
\def\J{{\cal J}}
\def\om{\omega}
\def\l{\lambda}
\def\tl{{\tilde \l}}
\def\tk{{\tilde k}}
\def\sqtl{{\sqrt{\tilde \l}}}
\def\adss{$AdS_5 \times S^5$\ }
\def\D{\Delta}
\def\p{\phi}
\def\r{\rho}
\def\rN{{\rm N}}
\def\tw{{\tilde w}}
%\newcommand{\sfrac}[2]{{\textstyle\frac{#1}{#2}}}
\def\vl{ \vec \ell}
\def\varpi{{\rm w}}
\def\bG{\bar \G}
\def\ve{\varepsilon}
\def\I{{\cal I}}
\def\La{{\Lambda}}
\def\R{{\rm R}}
\def\bt{\bar\theta}
\def\Z{{\cal Z}}
\def\pa{\partial}
\def\bea{\be}
\def\eea{\ee}
\def\DD{{\rm D}}
\def\chii{\varepsilon}
\def\th{\theta}
\def\t{\tau}
\def\beq{\be}
\def\eeq{\ee}
\def\beqa{\bea}
\def\eeqa{\eea}
\def\bs{\bigskip}
\def\c{{\rm a}}
\def\del{\partial}
\def\s{\sigma}
\def\eps{{\epsilon}}
\def\n{\nu}
\def\dag{\dagger}
\def\bd{\bar \del}
\def\ed{\end{document}}
%\newcommand{\mc}{\mathcal }
\def\iffa{\iffalse}
\def\xp{x_+}
\def\xm{x_-}
\def\te{\textstyle}
\def\rx{{\rm x}}
\def\C {{\rm C}}
\def\hC {{\rm \hat C}}
\def\dd {{\rm d}}
\def\bb{{\rm b}}
\def\sql{{\sqrt{\l}}}
\def\ep{\epsilon}
\def\G{\Gamma}
\def\dx{\dot x}
\def\vp{\varphi}
\def\tx{{\tilde x}}
\def\ad{{\rm ad}}
\def\d{\delta}
\def\de {\del}
\def\L{\mathcal{L} }
\def\pcm {{\rm PCM}}
\def\wz{{\rm WZ}}
\def\pcmq {{\rm PCM}$_q$\ }
\def\ZMq {{\rm ZM}$_q$\ }
\def\ZM {{\rm ZM} }
\def\pp{{\rm p}}
\def\qq{{\rm q}}
\def\rk {{\rm u}}
\def\rrk{{\rm e}}
\def\ss{{\rm s}}
\def\tt{{\rm t}}
\def\uu{{\rm u}}
\def\sm{$\sigma$-model}
\def\sms{$\sigma$-models}
\def\ov{\over}
\def\Ad{\text{Ad}}
\def\lmp{\Lambda}
\def\bl{\bar \lambda}
\def\Lie{\operatorname{Lie}}
\def\hb{\hbar}
\def\k{\varkappa} \def \h {{\rm h}}
\def\dt{\tfrac{d}{dt}}
\def\ddt{\frac{d}{dt}}
\def\bb{{\rm b}}
\def\vv{{ v}}
\def\kk{{\rm k}}
\def\ka{{\kappa}}
\def\np{ }
\def\cM{\mathcal{M}}
\def\bh{\bar{h}}
\def\lam{$\lambda$-model}
\def\etm{$\eta$-model}
\def\bh{\bar h}
\def\hh{{\rm h}}
\def\PCM{\L_{\rm PCM}}
\def\WZ{\L_{\rm WZ}}
\def\M{{\cal M}}
\def\q{{\rm q}}
\def\RR{{J}}
\def\LL{{K}}
\def\kold{k_{\text{old}}}
\def\kaold{\ka_{\text{old}}}
\def\ed{\end{document}}
\def\F{H}
\def\cgg{c_{_G}}
\def\cg{c\,}
\def\cf{c_{_\F}}
\def\cff{c_{_\F}}
\def\HH{\F}
\def\XX{{X}}
\def\hhh{\widetilde {\hh}}
\def\e{\varepsilon}
\def\tih{{\hat h}}
\def\H{{\rm H}}
\def\GG{{\rm G}}
\def\BB{{\rm B}}
\def\g{\gamma}
\def\bl{\bar\lambda}
\def\ol{\underline}
\def\ul{\overline}
\def\MM{\mathcal M}
\def\hz{z}
\def\hhz{z} %\def\hhz{\widehat{z}} %v3
\def\wcL{\widehat{\L}}
\def\wL{\widehat{L}}
\def\XX{X}
\def\bw{\a}
\def\xx{{\rm x}}
\def\cR{{\mathcal R}}
\def\sms{$\s$-models\ }
\def\sm{$\s$-model\ }
\def\wLL{\widehat{\L}}
\def\br{\big[}
\def\bl{\big]}
\newcommand\ei[1]{\mathbf{\underline{#1}}}
\def \FF {h}
\def\GG{{\rm G}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\chapter{Sigma models with local couplings \label{loc}}


There is a remarkable link between the 
integrability of 2d $\s$-models and their stability under RG flow, i.e.\ their
renormalizability with finitely many running couplings. 
 However, it
remains rather mysterious how the integrability translates into simple
 RG behaviour.

In this chapter we shall present a new and different link between
classical integrability and the RG flow (based on the paper \cite{HLT2008} and closely following the presentation there).
Consider a familiar example of an integrable 2d $\s$-model, the 
principal chiral model (PCM). Suppose we
formally replace its overall coupling $h$
by a function of 2d time $\t$,
obtaining
the
Lagrangian
\be\la{1}
\wcL = -\ha h(\t)  \, \Tr[J_+ J_-] \ .
\ee
The resulting time-dependent theory is not Lorentz-invariant but one may wonder if
some notion of classical integrability still applies even for a non-constant $h(\t)$.
As we shall see below,
this is indeed the case {\it provided} the function $h(\t)$ is special:
the same as the solution of the 1-loop RG equation of the standard PCM,
i.e.\ $h(\t) \sim \t$.

More generally, starting with a Lorentz-invariant
2d theory
that is classically integrable (i.e.\ admitting a Lax connection),
one may formally promote
its coupling constants $h_\a$ to functions $h_\a (\t)$ depending on 2d time.
We address the question of which functions $h_\a (\t)$
allow the integrability to survive in the resulting time-dependent theory, in the sense that the resulting equations of motion still
admit a Lax representation.
We shall suggest a certain natural ansatz for the corresponding Lax connection
generalizing that of the time-independent theory and
will find that the unique functions $h_\a (\t)$ preserving the integrability under this ansatz are the ones solving the 1-loop RG equations of the original theory,
\be
\del_\t h_\a = \b_\a(h) \ , \la{1lr}
\ee
with
2d time $\t$ playing the role of
RG time $t=\log \mu$.
We observe this new `integrability--RG flow' connection
in a number of non-trivial examples but will not give a general proof of it.

One may wonder how such
time-dependent models (where, e.g.,
energy is no longer conserved)
can be integrable. In fact, integrable examples of time-dependent 1d
mechanical models
are known (see, e.g., \cite{t-dep-1d} and refs. there).
Our present interest in such 2d models is motivated by the desire to find new solvable examples
of
conformal $\s$-models representing consistent string backgrounds with Minkowski signature.
One class of examples would be conformal \sms with $(D+2)$-dimensional
target space metric
$ds^2 =\GG_{mn} (x) dx^m dx^n = -2 dudv + K(u,x) du^2 + dx^i dx^i$ \ ($x^m=(u,v,x^i)$, \ $i=1, ..., D$),
admitting a covariantly constant null Killing vector.
In the light-cone (l.c.)\ gauge $u=\tau$, one then gets
a  
 model with a time-dependent potential $K(\t,x)$, which is formally solvable in some cases if
$K$ is quadratic in $x^i$ (see, e.g., \cite{Papadopoulos:2002bg} and refs. there).\foot{Another solvable example obtained as a certain Yang-Baxter deformation of flat 4d Minkowski space was found in \cite{yoshida}.
Examples with $K$ not depending on $\t$ corresponding to
integrable l.c.-gauge theories (sine-Gordon, Liouville,
etc.) were discussed, e.g., in
\cite{Maldacena:2002fy,Russo:2002qj,Bakas:2002kt}. }

The most general metric with a covariantly constant
null Killing vector has the Brinkmann-Walker form,
$ds^2 = -2 dudv + K(u,x) du^2 + A_i(u,x) du dx^i + \GG_{ij} (u,x) dx^i dx^j$.  Once one relaxes the assumption that $\GG_{ij}$ is flat, the $K$ and $A_i$
terms can be absorbed into  $\GG_{ij}(u,x)$ by a coordinate transformation
to give 
$ds^2 = - 2 dud v + \GG_{ij}(u,x) d x^i d x^j$.
We shall focus on the remarkable class of string \sms on such backgrounds \cite{Tseytlin:1992pq,Tseytlin:1992ee},
\begin{align}
\L =- 2 \del_+ u \del_- v + \GG_{ij}(u,x) \del_+ x^i \del_- x^j \ . \la{csm}
\end{align}
Moving to a curved 2d background $h_{\m\n}$ and incuding also a dilaton term $\L_\p= - \a' \sqrt{-h} \,  R^{(2)} \phi(v,u,x)$,
this $\s$-model is Weyl-invariant, i.e.\ $\bar \b_{mn} = R_{mn} + 2 D_m D_n\p + ...=0$,
provided $\phi$ is linear in the null coordinate $v$
and $\GG_{ij}(u,x)$ depends on $u$ according to the RG equation of the  `transverse' $\s$-model
$\L=\GG_{ij}(x) \del_+ x^i \del_- x^j $ \cite{Tseytlin:1992pq,Tseytlin:1992ee},
\begin{align}
& \del_u \GG_{ij} = \bar{\beta}_{ij} (\GG)= \beta_{ij} + 2 D_i D_j \bar{\phi}
\ , \qquad \quad \beta_{ij} = R_{ij} + \ldots
\ , \la{bd} \\
&\phi = v + \bar{\phi}(u,x) \ . \la{dilv}
\end{align}
The `first-order' equation \rf{bd} comes from the contribution of the connection in the $D_m D_n\p$ term
in the Weyl-invariance condition due to the null Killing form of the metric and the $v$-term in the dilaton.\foot{The exact
RG evolution equation \rf{bd} in the l.c.\ direction $u$
may be compared to an approximate RG equation
(see, e.g., \cite{Schmidhuber:1994bv}) appearing in the
case of a `cosmological' metric
and a time-dependent dilaton which provides a `friction' term in the string
generalization of the Einstein equations.
}
We have ignored an additional
diffeomorphism term $D_{(i}W_{j)}$  in \rf{bd} that appears only at higher loop orders.
The model \rf{csm}  also admits a natural generalization to the case of non-zero `transverse'
$\BB$-field coupling $\BB_{ij}(u,x)$: the resulting $(D+2)$-dimensional $\s$-model is Weyl invariant
provided $\del_u(\GG_{ij} + \BB_{ij}) = \bar{\beta}_{ij}(\GG,\BB)$
where $ \bar{\beta}_{ij}$ is the corresponding Weyl anomaly coefficient 
\cite{Tseytlin:1992pq,Tseytlin:1992ee}. 

One example of such a conformal background with a sphere $S^D$ as the transverse space is (to 1-loop order)\,
$ds^2 = - 2 du dv + u \, d\Omega^2_D, \ \ \p= v  + \tfrac{D-24}{6} u+ \frac{1}{8} D \log u $ .


This construction is also naturally generalized to supersymmetric $\s$-models \cite{Tseytlin:1992ee}. On certain \textit{special} K\"{a}hler symmetric spaces, the supersymmetric $\s$-models (which then have $\mathcal{N}=(2,2)$ supersymmetry \cite{Zumino:1979et}) 
 are known to have a 1-loop exact $\b$-function \cite{Novikov}.\foot{In general, $\mathcal{N}=(2,2)$ supersymmetric $\s$-models on K\"{a}hler manifolds have a non-trivial 4-loop $\b$-function coefficient \cite{Grisaru:1986px,Grisaru2} (which may be absorbed into a non-local redefinition of the metric in the case of Ricci-flat K\"{a}hler (Calabi-Yau) manifolds \cite{Nemeschansky:1986yx}).}
 Hence, taking one of those as the transverse theory, the  background in \rf{csm},\rf{bd},\rf{dilv} resulting from the 1-loop RG flow will be \textit{exact} string backgrounds \cite{Tseytlin:1992ee}.



Starting with the classical string $\s$-model \rf{csm} in conformal gauge and fixing the residual conformal symmetry by the l.c.\ gauge condition $u=\t$, we get a time-dependent
theory for the transverse coordinates\foot{Here
we ignore
the `diffeomorphism vector'
term that will also contribute to the time dependence of the metric; however,
this term can be eliminated or modified as desired by an appropriate field redefinition
in \rf{lct}
depending on time, $x^i \to y^i(x,\t)$ (see discussion in Section \ref{2008sec2} below).}
\be
\L_{l.c.} = \GG_{ij}(\t ,x) \del_+ x^i \del_- x^j \ , \qquad\qquad
\del_\t \GG_{ij} = \beta_{ij}(\GG) \ . \la{lct}
\ee
If we now assume that the transverse $\s$-model
$\L=
\GG_{ij}(x) \del_+ x^i \del_- x^j$ is classically
integrable, then the fact that $\GG_{ij}(\t ,x)$ is subject to the RG equation in \rf{lct}
suggests, in view of the above `integrability--RG flow' connection,
that the l.c.\ gauge theory \rf{lct} is classically integrable
(admits a flat Lax connection)
and thus may potentially be solvable.

\


Let us note that a special class of the $\s$-models \rf{csm} with $\GG_{ij}(u,x) = u\, g_{ij}(x) $ 
are obtained upon fixing the conformal gauge $h_{\m\n} d\xi^\m d \xi^\n = e^{-2v } \eta_{\m\n}$ (so that $\sqrt {-h} \, R^{(2)} = - 2 \del_+ \del_- v$) in 
a theory of 
 2d dilaton gravity (with dilaton $u$) coupled to a $\s$-model \ci{Tseytlin:1992pq} with $g_{ij}(x)$ as the target space metric,
\be \la{dig}
\L = - \sqrt {-h} \, u \big[R^{(2)} + g_{ij}(x) \, h^{\m\n} \, \del_\m x^i \del_\n x^j \big] \ .
\ee
Particular 2d models of the type \rf{dig}, with $g_{ij}(x)$
corresponding to specific symmetric spaces,
appear upon dimensional reduction (in 2 Killing vector directions) of 4d Einstein gravity
\ci{Belinsky:1971nt,Breitenlohner:1986um,Nicolai:1991tt}.
After solving $\del_+ \del_- u=0$ (the equation from varying $v$) to obtain $u(\t,\s) = f^+ (\xi^+) + f^- (\xi^-)$,
the resulting `local coupling' $\s$-model,
\be \la{ff}
\L = u(\t, \s)\, g_{ij}(x) \del_+ x^i \del_- x^j \ , \qquad \quad u(\t,\s) = f^+ (\xi^+) + f^- (\xi^-) \ , \ee
was shown, in some special cases
\ci{Belinsky:1971nt} and for general symmetric spaces
\ci{Breitenlohner:1986um} (see also \ci{Nicolai:1991tt}), to be integrable in the sense of admitting a Lax
pair.
The spectral parameter is now replaced by a function of $\t,\s$ expressed in terms of $f^+ (\xi^+) $, $
f^- (\xi^-)$ and an integration constant $w$ (which may be viewed as a new spectral parameter ---
see below).

Here will go beyond this related earlier work in two important ways:
(i) showing that there are other integrable  $\s$-models with `local couplings' (e.g., related to integrable-deformed models)
for which the dependence of $\GG_{ij} (u,x)$ on $ u(\t,\s)$ is not simply through an overall factor as in \rf{ff};
(ii) establishing the link between the dependence on $u$ required for
integrability and the RG evolution of couplings in the original $\s$-model defined by the transverse metric $\GG_{ij} (u,x)\big|_{u=\const}$.

\ 

The rest of this chapter is organized as follows.
In Section \ref{2008sec2} we will show that, starting from a certain class of classically integrable $\s$-models 
admitting a flat Lax connection, it is possible to find a Lax connection for the corresponding
time-dependent theory obtained from the original one by replacing the couplings
by functions of $\t$ satisfying the 1-loop RG equations. We will explicitly discuss the case of the PCM, and a similar statement is
also true for several classes of integrable $\s$-models (PCM with WZ term, symmetric spaces,
$\eta$-model, $\l$-models) presented in Table \ref{2008tab1}.

In Section \ref{2008s3} we will demonstrate that the converse is also true: demanding the existence of a Lax pair for the time-dependent model implies that the couplings must solve the 1-loop RG equations
of the original theory. Details of the derivation of the RG flow will be presented in Appendix \ref{2008A}.

In Section \ref{2008s4} we will discuss how the monodromy matrix associated with
the Lax connection can be used to construct, at least in principle, non-local
conserved charges for time-dependent models.\foot{See also Section 5 of \cite{HLT2008} for an attempt to construct higher-spin, local charges for  the PCM with a local ($\s$-dependent) coupling.} 
We will concentrate on the PCM example
with comments on other models relegated to Appendix \ref{2008om}.
To shed light on the notion of integrability in the time-dependent case we
will also consider consistent 1d
reductions of some simple 2d $\s$-models, investigating their solvability.
In Appendix \ref{2008C} we will further discuss a particular linear 1d model which is a special case
of a time-dependent harmonic oscillator.


Section \ref{2008s6} contains a discussion of the results and possible extensions.
In particular, we will mention that the relation between integrability of the time-dependent
theory and the RG flow should extend to models with potentials, illustrating this
on the example of the sine-Gordon model (see also Appendix \ref{2008sing}).

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Lax connection for time-dependent 
sigma models}\la{sec2}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Below we shall discuss how,
starting from a classically integrable model (with Lagrangian $\L$) admitting a Lax pair $L_\pm$,
it is possible to find also a Lax pair $ \widehat{L}_\pm $ for the corresponding
time-dependent theory $\widehat{\L}$ obtained from the original one
by replacing the couplings $h_\a$ by functions $ h_\a (\t)$ depending on $\t$
according to the 1-loop RG equation \rf{1lr},\foot{Here and below for simplicity
we are only indicating the dependence of the Lagrangian on the couplings, suppressing dependence on fields.}
\begin{align}
&h_\a \to h_\a (\t) \ , \qquad \qquad \tfrac{d}{d\t} h_\a (\t) = \b_\a(h(\t)) \la{tins} \ ,\\
&\L(h_\a)\ \to\ \widehat{\L} = \L(h_\a (\t)) \ . \la{lcg}
\end{align}
The Lax connection must be modified to account for `extra' terms in the equations of motion following from \rf{lcg} that are proportional to the derivatives $\del_\t h_\a$ of the couplings.
We propose a very simple ansatz for this modification: the extra terms can be effectively `absorbed'
into the spectral parameter $z$
with the structure
of the Lax connection remaining the same, i.e.
\begin{align}
&L_\pm(h_\a, z) \to \widehat{L}_{\pm} = L_\pm (h_\a(\t), \hhz(w; \t,\s) )\ , \la{lac2}\\
&z \to \hhz = \hhz(w;\t,\s) \ , \ \ \ \qquad h_\a \to h_\a (\t) \ .
\la{lac1}
\end{align}
While $z$ was regarded as constant
in the original Lax connection,
it is now promoted to a particular function $\hhz(w;\t,\s)$ of the 2d coordinates.
Here $w$ is an arbitrary (complex) constant playing the role of a new spectral parameter.
As we shall see below, the explicit form of the function $\hhz(w;\t,\s)$ will be model-dependent.

Let us note that if the original theory is a \sm on flat 2d Minkowski space,
which
is classically invariant under the 2d conformal transformations $\xi^\pm \to f^{\pm}(\xi^\pm)$,  
then the Lagrangian of the corresponding time-dependent theory \rf{lcg} changes
under such transformations as
\be
\widehat{\L}= \L(h_\a (\t))\ \to\ \L( h_\a(\t')) \ , \qquad \ \ \ \ \ \t = \xi^+ + \xi^-\ \to\ \t'=
f^+ (\xi^+)+ f^- (\xi^-) \ . \la{nlc}
\ee
In the case of the
string
\sm \rf{csm},\rf{lct},
this is equivalent to replacing the l.c.\ gauge $u=\t$ with a
more general one given by the solution $u = f^+ (\xi^+)+ f^- (\xi^-)$ of the
equation of motion $\del_+ \del_- u = 0$.
One special choice is $u=\xi^-$ for which
we get
$
\wcL_{\rm ch} = \L(h_\a (\xi^-))
$.
One may formally consider that theory,
which only fixes one `half' of the conformal reparametrizations, as an extreme limit $(f^+(\xi^+),f^-(\xi^-)) =(0, \xi^-)$ of \rf{nlc}.

To provide evidence for the above proposal, we have considered
six examples of integrable $\s$-models (each introduced in Section \ref{rev}) with the results summarized in Table \ref{2008tab1} below.
There, for each model, we give the original Lagrangian, original Lax pair, 1-loop RG equation and its solution, and the expression for the function $\hhz(w;\t,\s)$ that generalizes the original spectral parameter in such a way
that \rf{lac2} gives a Lax pair for the time-dependent theory \rf{lcg}.

The classically integrable $\s$-models in Table \ref{2008tab1} are each 1-loop renormalizable
 assuming a particular choice of
`renormalizable'
diffeomorphism vector. This means that the insertion of time dependence according to the RG flow in \rf{tins},\rf{lcg}
will only apply to a finite set of couplings. 
As discussed
at the beginning of this chapter,
a time-dependent $\s$-model
arises in the light-cone gauge from a conformal string $\s$-model.
There, the time dependence is governed by the RG flow with
a specific diffeomorphism vector (generally different from the renormalizable one)
following from the $(D+2)$-dimensional dilaton solving the Weyl-invariance condition. 
However,
these two patterns of time dependence
(according to the RG flow with different diffeomorphism vectors)
are simply related by a time-dependent field redefinition in
the corresponding time-dependent models, and  such a redefinition preserves the existence of a Lax representation.

All of our examples are built on either a group $G$ or a symmetric space $G/H$. Our notation is the same as that of Section \ref{rev}, except that here $h$ denotes a coupling constant, or $h_\a$ to denote many of them (whereas before they were called  $\h$ to distinguish from group elements).
 We again denote $J_\pm = g^{-1} \del_\pm g$, where $g\in G$ is scalar field.
PCM$_k$ stands for the principal chiral model plus a Wess-Zumino ($\BB$-field)
term with coefficient $k$
(and the special case $h=\pm k$ is the conformal WZW model).
The group space $\eta$-model is an integrable deformation of the PCM
while the group space and symmetric space $\l$-models are integrable
deformations of the WZW and gauged WZW models.

\begin{table}
{
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{l || l | l | l }
& PCM& PCM$_k$ \\ \hline\hline
Lagrangian& $\L =-\ha h \Tr[J_+ J_-]$ & $\L =-\ha h \Tr[J_+ J_-]+ k\, \L_{\rm WZ}$\\ \hline

Lax connection & $L_\pm =\ha (1+z^{\pm 1})J_\pm$ & $L_\pm =\ha (1 + z^{\pm 1}) (1\pm \frac{k}{h})J_\pm$ \\ \hline

\makecell[l]{1-loop RG equation \\
and its solution}& $\begin{matrix*}[l]\ddt h = \cg \\ h(t) =\cg t \end{matrix*}$ & $\begin{matrix*}[l]\ddt h = \cg(1-\frac{k^2}{h^2}), \ \ \ \ddt k = 0 \\ h(t) -k \tanh^{-1}{\big(\frac{h(t)}{k}\big)} = \cg t \end{matrix*}$\\ \hline

\makecell[l]{Spectral parameter\\function }& $\hz=
\sqrt{\frac{w+\s-\t}{w+\s+\t}}$ & $\begin{matrix*}[l] \cg (w+\s-\t) + 2zh(\t)\, \frac{k+\hz(k+h(\t))}{k(1+\hz)^2+h(\t)(\hz^2-1)} \\ \quad \quad \qquad + k \log{\big(\frac{(1+\hz)(k-h(\t))}{(k-h(\t))+\hz(k+h(\t))}\big)} = 0 \end{matrix*}$
\vspace{0.5cm}
\end{tabular}

\begin{tabular}{l || l | l | l}
& Group space $\eta$-model & Group space $\l$-model \\ \hline\hline
Lagrangian& $\L =-\ha h \Tr [ J_+ \frac{1}{1-\k \cR} J_- ] $ & $\begin{matrix*}[l]\L =k\big[ \L_{G/G}(g,A)\\
\qquad \qquad - (\l^{-1}-1) \Tr( A_+ A_-)\big] \end{matrix*}$\\ \hline

Lax connection & $\begin{matrix*}[l] L_\pm = \ha (1+z^{\pm 1}) C_\pm \\ C_\pm = - (1+\k^2)\Ad_g\frac{1}{1\pm \k \cR} J_\pm \end{matrix*}$ & $ \begin{matrix*}[l] L_\pm = \ha (1+z^{\pm 1}) \frac{2}{1+\l} A_\pm \\
A_\pm \text{ takes on-shell value}\end{matrix*}$ \\ \hline

\makecell[l]{1-loop RG equation \\
and its solution}
& $\begin{matrix*}[l] \ddt h = \cg (1+\k^2)^2 ,\ \ \ddt (h \k^{-1}) = 0\\
\nu \equiv  \tfrac{h(t)}{4\k(t)} = \text{const} \\
{\tan}^{-1}\, {\k(t)} + \frac{\k(t)}{1+\k(t)^2} = \frac{\cg}{2\nu} t
\end{matrix*}$
& $\begin{matrix*}[l]
\ddt \l = - \frac{2\cg}{k}\frac{\l^2}{(1+\l)^2}, \ \ddt k =0, \\
- 2\log{\l(t)} - \l(t) + \l(t)^{-1} = \frac{2\cg}{k} t
\end{matrix*}$
\\ \hline

\makecell[l]{Spectral parameter \\
function}
& $\begin{matrix*}[l]
\frac{\cg}{2 \nu} (w+\s) - \frac{1-\hz}{1+\hz} \frac{\k(\t)}{1+\k(\t)^2} \\
\qquad \qquad + \tan^{-1}{ \big(\frac{1}{\k(\t)} \frac{1-\hz}{1+\hz} \big)} = 0
\end{matrix*}$ &
$\begin{matrix*}[l]
\frac{2\cg}{k} (w+\s) + \frac{1-\hz}{1+\hz} [\l(\t)-\l(\t)^{-1}] \\
\qquad \qquad - 2\log{\big( \frac{\hz\l(\t)-1}{\hz-\l(\t)} \big)} = 0\end{matrix*}$
\vspace{0.5cm}
\end{tabular}

\begin{tabular}{l || l | l | l}
& Symmetric space $\s$-model & Symmetric space $\l$-model \\ \hline\hline

Lagrangian& $\L = -\ha h \Tr [ J_+P_{G/H} J_- ] $ & $\begin{matrix*}[l]\L =k\big[ \L_{G/G}(g,A)\\
\qquad \qquad - \Tr \big[ A_+ (\l^{-1} P_{G/H} -1) A_-\big] \end{matrix*}$\\ \hline

Lax connection &
$\begin{matrix*}[l] L_\pm = J^{H}_\pm + z^{\pm 1} J^{G/H}_\pm \\ J^{H}_\pm = P_H J_\pm , \ J^{G/H}_\pm = P_{G/H} J_\pm \end{matrix*}$
& $\begin{matrix*}[l] L_\pm = A^{H}_\pm + z^{\pm 1} \frac{1}{\sqrt{\l}} A^{G/H}_\pm \\ A^{H}_\pm = P_H A_\pm , \ A^{G/H}_\pm = P_{G/H} A_\pm \\
A_\pm \text{ takes on-shell value} \end{matrix*}$ \\ \hline

\makecell[l]{1-loop RG equation \\
and its solution} & $\begin{matrix*}[l] \ddt h = 2\cg \\
h(t) = 2\cg t
\end{matrix*}$
& $\begin{matrix*}[l]
\ddt\l = -\frac{\cg}{k} \l \\
\l(t) = \exp{(- \frac{\cg}{k} t )}
\end{matrix*}$
\\ \hline

\makecell[l]{Spectral parameter \\
function}
& $\hz=
\sqrt{\frac{w+\s-\t}{w+\s+\t}}$ &
$ \hz =
\exp{( - \frac{\cg}{2k} \t)} \sqrt{\frac{1+\exp{(\frac{\cg}{k} [w+\s-\t] )}}{1+\exp{( \frac{\cg}{k} [w+\s+\t] )}}}
$
\vspace{0.5cm}
\end{tabular}

\caption{\small Examples of integrable \sms and their time-dependent generalizations.
$t$ is the RG time which is replaced by the 2d time $\t$ in the couplings entering the
Lagrangian $\wcL$ in \rf{lcg}.
\la{tab1}}
}
\end{table}

In this section we shall explicitly consider only the basic PCM example,
postponing a more general discussion to Section \ref{2008s3},
where we shall also explain that the existence of the spectral function $\hhz(w;\t,\s)$ is a highly non-trivial feature, depending on
specifically choosing the coupling functions $h_\a(\t)$ to solve the 1-loop RG equation.

For the PCM corresponding to a simple Lie group $G$
\be
\L =-\ha h \Tr[J_+ J_-] \ , \qquad J=g^{-1} dg \ , \ \ g\in G \ , \la{pl}
\ee
the global $G\times G$ symmetry implies
that only the overall coupling $h$ runs under the 1-loop
RG,\foot{The constant $c\equiv c_{_G}$ is the dual Coxeter number of the group $G$ (see Appendix \ref{conv} for the group theory conventions).
\la{fo8}
}
\be
\ddt h = \cg \ ,\qquad \qquad h(t) =\cg t \ , \qquad \qquad \cg \equiv \cgg.
\ee
The corresponding time-dependent theory
\rf{lcg} is then
given
by
\be
\widehat{\L} = - \tfrac{1}{2} \cg \t \, \Tr[J_+ J_-] \ . \la{lcPCM}
\ee
As explained above, this theory arises naturally in the l.c.\ gauge $u=\t$ from the conformal string $\s$-model (cf.\ \rf{csm},\rf{lct})
\be
\L =-2 \del_+ u \del_- v - \tfrac{1}{2} \cg u \Tr[J_+ J_-] \ , \la{nPCM}
\ee
where the constant $\cg$ can be eliminated by a rescaling $(u,v) \to ( \cg^{-1} u,\, \cg v)$.

The equations of motion for the model \rf{lcPCM} written in first-order form are
\begin{align}
&\del_+ (\t J_- ) + \del_- (\t J_+) = 0 \ , \la{pe1} \\
&F_{+-}(J) \equiv \del_+ J_- - \del_- J_+ + [J_+, J_-] = 0 \ . \la{pe2}
\end{align}
Starting from the Lax connection of the original PCM \rf{pl}
\be
L_\pm = \ha(1+z^{\pm 1}) J_\pm \ , \la{pla}
\ee
and making the replacement
$z \to \sqrt{\frac{{w+\s-\t}}{{w+\s+\t}}} $ where $w$ is a constant spectral parameter
(see Table \ref{2008tab1}), we obtain the following expression for the
Lax connection \rf{lac2} of the time-dependent theory
\be
\widehat{L}_\pm = \ha \big( 1+ {{z}\, }^{\pm 1}
\big) J_\pm \ , \qquad \qquad {z}=\sqrt{\frac{{w+\s-\t}}{{w+\s+\t}}} \ . \la{lpl}
\ee
Indeed,
its curvature is
\begin{align}
&F_{+-}(\widehat{L}) \equiv \del_+ \wL_- - \del_- \wL_+ + [\wL_+, \wL_-] \la{curv} \\
&\qquad \ \ \ \, \, = \frac{{z}}{2(w+\s-\t)} \Big[ \del_+ (\t J_- ) + \del_- (\t J_+) \Big]
+ \tfrac{1}{4} (1+{z})(1+{{z}\, }^{-1} ) \ F_{+-}(J)
\ , \no
\end{align}
so that, at
any $(\t, \s)$, its vanishing for all $w$ implies
the equations of motion \rf{pe1},\rf{pe2} of the time-dependent theory.

A surprising feature
(shared also by the other examples in Table \ref{2008tab1})
is that, despite the Lagrangian \rf{lcPCM} explicitly involving only $\t$,
the Lax connection \rf{lpl}
also depends on the 2d spatial coordinate $\s$.
The spatial coordinate $\s$ and the spectral parameter $w$ appear only through
the combination $w+\s$. Since $w$ is a complex constant, it cannot be
eliminated by a shift of real $\s$. Moreover, what is important is the
existence of a Lax connection depending on $w$, which can in principle be used
to construct conserved charges, etc. Indeed, we can instead interpret the
formal possibility to shift $\s$ as the freedom to introduce a spectral
parameter in the first place.

Another unusual property (shared by all the examples) is that the Lax connection has branch cuts in the spectral $w$-plane
(e.g., for the PCM the branch cuts end at $w=-\s\pm \t$).
Normally, one could simply remove square roots by redefining the spectral parameter (or more formally moving to an appropriate Riemann surface on which the Lax connection is meromorphic).
However, this is not possible since the positions of the branch cuts depend on $(\t,\s)$ and one cannot redefine the spectral parameter in a way depending on $(\t,\s)$ without changing the equations of motion encoded in the zero curvature condition.

In each case in Table \ref{2008tab1}, one can freely choose any branch of the function $z(w;\t,\s)$ (in the $w$-plane) while still encoding the correct equations of motion in the zero-curvature equation. For example, in the PCM case, one may choose either sign of the square root ${z} =\pm \sqrt{\tfrac{{w+\s-\t}}{{w+\s+\t}}}$ in the Lax connection \rf{lpl}.
All similar square roots in the spectral functions below
have the same branch ambiguity, corresponding to the option to reverse their sign.


\medskip


Applying a general conformal transformation to the action corresponding to \rf{lcPCM},\rf{lpl} we get (cf.\ \rf{nlc})
\begin{align}
& \widehat{\L} =- \tfrac{1}{2}\cg \, \big(f^+( \xi^+) + f^-(\xi^-)\big) \, \Tr[J_+ J_-] \ , \qquad \la{lac} \\
&\widehat{L}_\pm= \ha \big( \, 1+ z^{\pm 1} \big) J_\pm \ , \qquad \quad
z= \sqrt{ \frac{{w- 2f^-(\xi^-)}}{{w+ 2 f^+ (\xi^+)}}} \ . \la{laca}
\end{align}
This theory may equivalently be obtained from the string $\s$-model \rf{nPCM}
by picking up a generalized l.c.\ gauge $u =\t'= f^+(\xi^+) + f^-(\xi^-)$.
A (degenerate) limit $u=a+b \t$, \ $a\to 1$, $b\to 0 $ eliminates the explicit $\tau$-dependence and gives back the original PCM \rf{pl}, with \rf{lac} becoming
the original Lax connection in \rf{pla} with a redefined spectral parameter $z\to \sqrt{\frac{{w-2 a_-}}{{w+2 a_+}}}$, where $a_\pm$ are constants satisfying $a_+ + a_- = 1$.
We note that the theory \rf{lac} is a special case of \rf{ff} where $\GG_{ij}$ is the group-space metric. Indeed, an equivalent expression for the Lax connection
of this `local' PCM (or symmetric space $\s$-model, see Table \ref{2008tab1})
was originally found in \cite{Breitenlohner:1986um}
where the dependence of the analog of the
spectral parameter on the functions $f^+(\xi^+) $ and $f^-(\xi^-)$ was
discovered. The spectral function $z$ in \rf{laca} depends separately on $u$ and its dual field $\td u =f^+( \xi^+) - f^-(\xi^-) $, \
$d u= *d\td u $,
and thus separately on $f^+$ and $f^-$ \cite{Breitenlohner:1986um,Nicolai:1991tt}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{RG flow from condition of integrability of time-dependent theory}\la{s3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As we have found above on several examples,
if the couplings of an integrable $\s$-model are promoted to functions of time that
solve the 1-loop RG equations, $h_\a \to h_\a(\t),\ \del_\t h_\a = \b_\a(h)$,
then the Lax connection of the original model $\L(h_\a)$ admits a natural generalization
to a classical Lax connection for the time-dependent model $\L(h_\a(\t))$.
Here we shall argue that the converse is also true:
demanding the existence of a Lax pair for the time-dependent theory implies that $h_\a (\t)$ must solve
the 1-loop RG equations.

It is useful to start with a more general theory with local couplings\foot{We generally expect integrable models to have a finite number of couplings $h_\a$.
A natural way to identify these couplings is
as the parameters that run under the RG flow.}
$h_\a(\t,\s)$ depending on both $\t$ and $\s$, i.e.
\begin{align}
&\widehat{\L} = \L(h_\a(\t,\s)) \ , \la{sth}
\end{align}
and demand the existence of a Lax representation for this
theory.
For the examples in Table \ref{2008tab1}, the original Lax connection
takes a particular form
(which is generic to many integrable $\s$-models built on groups $G$ or symmetric spaces $G/H$):
\begin{alignat}{2}
&\hspace{-2.5cm}G \ : \qquad\qquad & &L_\pm = \ha (1+z^{\pm 1}) \mc{A}_\pm \la{gl} \ ,\\
&\hspace{-2.5cm} G/H \ :
\qquad\qquad & &L_\pm = \mc{B}_\pm + z^{\pm 1} \mc{P}_\pm \la{sl} \ .
\end{alignat}
Here the connection components $\mc{A}_\pm \in \Lie(G)$,
$\mc{B}_\pm \in \Lie(H)$, $\mc{P}_\pm \in \Lie(G)/\Lie(H)$ depend implicitly on the fields and their derivatives
and the couplings $h_\a$ (e.g.\ for PCM, $\mc{A}_\pm = J_\pm $, cf.\ \rf{pla}), while the dependence on the
spectral parameter $z$ is indicated explicitly.
Let us now take the following natural ansatz for the Lax connection $\widehat{L}_\pm$
corresponding to the $(\t,\s)$-dependent theory \rf{sth}
\begin{alignat}{2}
&G \ : \qquad \qquad & &\widehat{L}_\pm = p_\pm(w;\t,\s)\, \mc{A}_\pm\ , \la{glt}\\
& G/H \ : \qquad \qquad & &\widehat{L}_\pm = q_\pm(w;\t,\s)\, \mc{B}_\pm + r_\pm(w;\t,\s)\, \mc{P}_\pm \la{slt} \ ,
\end{alignat}
where $p_\pm, q_\pm, r_\pm$ are some functions, and $\mc{A}_\pm$, $\mc{B}_\pm$, $\mc{P}_\pm$ are assumed to take the same form as in \rf{gl},\rf{sl}, but now depending on the coupling \textit{functions} $h_\a(\t,\s)$ in place of the couplings, i.e.
$\mc{A}_\pm = \mc{A}_\pm (x,\del x; h_\a(\t,\s))$, etc.

Demanding that the flatness of the connection \rf{glt},\rf{slt}
is equivalent to the equations of motion of the `local coupling' theory \rf{sth},
we shall first prove that it is sufficient to use just
a single function
$\hz(w;\t,\s)$, so that the Lax connections \rf{glt},\rf{slt} become the same as the original ones \rf{gl},\rf{sl}
with the replacement $z\to \hz(w;\t,\s)$
as in \rf{lac2},
\be
\widehat{L}_\pm = L_\pm\big( h_\a(\t,\s), \hz(w;\t,\s)\big) \ . \la{laxs}
\ee
Indeed, the equations of motion for the theory \rf{sth} contain 
two types of terms:
the ``original'' terms (not depending on $\del_\pm h_\a$), and ``new'' terms (depending on $\del_\pm h_\a$).
To match the ``original'' terms with the corresponding terms in the zero-curvature condition for $\widehat{L}_\pm$, one needs
to impose the following conditions on $p_\pm$, $q_\pm$, $r_\pm$
(see Appendix \ref{2008det} for details)
\begin{alignat}{2}
& G \ : \qquad \qquad & &p_+^{-1} + p_-^{-1} = 2 \ , \la{alg}\\
& G/H \ : \qquad \qquad & &q_\pm = 1 \ , \qquad r_+ r_- = 1 \ . \la{als}
\end{alignat}
Substituting \rf{alg},\rf{als} into the Lax ansatz \rf{glt},\rf{slt} then gives \rf{gl},\rf{sl} but with $z\to \hz(w;\t,\s)$, where we set
 $\hz(w;\t,\s) = 2 p_+ - 1$ (for models on $G$) and
$\hz(w;\t,\s) = 2 r_+ $ (for models on $G/H$).

All of our examples are single-coupling theories\foot{We do not promote the WZ level $k$ in PCM$_k$ or $\l$-models to
a function of $(\t,\s)$ since the resulting model
would not be well-defined: starting with the
3d representation of the WZ term and replacing $k \H \to k(\t,\s) \H$
would no longer give a local 2d action
while $k \BB \to k(\t,\s) \BB $ in the 2d action would not be  globally well-defined, or locally consistent with global symmetry
(invariance of the 2d action under global symmetry transformations requires dropping total derivatives).}
except for the group $\eta$-model. Here we shall
specialize to the simplest case with one coupling $h(\tau,\sigma)$
but the same result will also be true for the group $\eta$-model (see Appendix \ref{2008mr}).
To reproduce the ``new''  terms (proportional to  $\del_\pm h$) in the
equations of motion for \rf{sth} from the flatness condition for the generalized Lax connection \rf{laxs}, one needs to additionally impose certain constraints on both $h(\t,\s)$ and $\hz(w;\t,\s)$.
For the models in Table \ref{2008tab1}
this leads to the following two first-order differential equations for the function $\hz(w;\t,\s)$
(here $h=h(\t,\s)$)
\begin{align}
\del_\t z = V_\t (z,h) \ , \qquad\qquad \del_\s z = V_\s (z,h) \ , \la{pd1}
\end{align}
where $V_{\t,\s} (z,h)$ are model-dependent functions. For all five single-coupling examples in Table \ref{2008tab1}, the consistency condition ($\del_\t V_\s - \del_\s V_\t =0$) for the system \rf{pd1} takes the
remarkable form,
\be
\del_+ \del_- h - \frac{\b'(h)}{\b(h)}\, \del_+ h \del_- h = 0 \la{2w} \ ,
\ee
where $\b(h)$ is precisely the 1-loop $\b$-function for the coupling $h$ in the original model.
In addition
to the appearance (in this purely classical context)
of the 1-loop $\beta$-functions, a remarkable feature of \rf{2w}
that it does not depend on $z$ (which completely factors out of the consistency condition).

The condition \rf{2w} may be written simply as $ \del_- ( \frac{\del_+ h}{\b(h)}) =0$ or
$ \del_+ ( \frac{\del_- h}{\b(h)}) =0$ and thus leads to two first-order equations,
\be
\frac{\del_+ h}{\b(h)} = s_+(\xi^+) \ , \qquad \qquad \frac{\del_- h}{\b(h)} = s_-(\xi^-) 	\ , \la{cfs}
\ee
where $s_\pm (\xi^\pm)$ are arbitrary functions of the 2d light-cone coordinates $\xi^\pm =\ha ( \t \pm \s)$.
By applying a conformal transformation (i.e.\ redefining $\t$ and $\s$), one can absorb $s_\pm$ into $\del_\pm$, i.e.\ replace
$s_\pm \to 1$,
so that in terms of the redefined coordinates the first-order equations \rf{cfs}
take the form of the 1-loop RG equation in $\tau$
\be
\del_\t h = \b(h) \ , \qquad \qquad \del_\s h = 0 \ . \la{RGs2}
\ee
Thus, modulo a conformal transformation,
the 1-loop RG solution is the only choice
of local coupling
$h(\t,\s)$
for which the Lax connection can be uplifted to the $(\t,\s)$-dependent theory according to \rf{laxs}.
This argument (in eqs.\ \rf{pd1}-\rf{RGs2}) is demonstrated explicitly for the example of the PCM in Appendix \ref{2008fdr}.

The same conclusion is reached of course if one starts directly with the theory where
the couplings $h_\a$ depend only on time (giving 
 $\del_\pm \to \del_\t$
and $s_+=s_-=\const$ in eqs.\ \rf{2w},\rf{cfs}):
using the same ansatz for the Lax connection
one finds that the only functions $h_\a(\t)$ consistent with preserving integrability
are the solutions of the 1-loop RG flow ---  modulo
a rescaling of time, i.e.\ the part of the conformal group that does not introduce spatial dependence.
By performing a classical conformal transformation, one could instead assign a preferred role to space $\s$ rather than time $\t$, and in that case the RG equation \rf{RGs2} will hold with $\t \to \s$.

To finish the construction of the generalized Lax pair let us now explain how to obtain the explicit form of the spectral parameter function
$z(w;\t,\s)$ in \rf{laxs}.
Starting with $h=h (\t)$ that satisfies the 1-loop RG equation in \rf{RGs2}
(so that the consistency conditions \rf{cfs} of \rf{pd1}
are satisfied) one can solve the second equation in \rf{pd1} as
\be
\del_\s z = V_\s (z, h(\t)) \qquad \rightarrow \qquad \int \frac{dz}{V_\s(z,h_\a(\t))} =\s + \ell (\t) \ . \la{sold}
\ee
The function $\ell(\t)$ is then fixed by substituting this solution into the first equation in \rf{pd1}.
The solution for $\ell(\t)$ leaves one free integration constant, which we call
$w$. Finally, eq.~\rf{sold} becomes an algebraic equation for $z(w;\t,\s)$
that can be explicitly solved in some simple cases (see Table \ref{2008tab1}).
Note that since the parameter $w$ appears as an integration constant in the function $\ell(\t)$,
it always appears in the combination $w+\s$ with the spatial coordinate,
implying that constant shifts of $\s$ can be compensated by shifts of $w$.

Although we do not have a proof that the 1-loop RG flow always follows from requiring
integrability of the time-dependent generalizations of integrable models, the examples
in Table \ref{2008tab1} reveal a highly non-trivial pattern.
In particular, 
some of the 1-loop RG equations obtained in this way are quite non-trivial, not admitting simple closed form solutions.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Non-local conserved charges in time-dependent integrable models}\la{s4}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have shown in the previous sections that some well-known examples of classically integrable $\s$-models admit generalizations of their Lax connections to models with time-dependent couplings under the condition that the latter solve
the 1-loop RG equation in $\tau$.
However, one may question the usefulness of the resulting Lax connections since they have several unusual properties: they depend on $\t$ and $\s$ explicitly; the spectral parameter only enters as a `constant piece' of the spatial coordinate $\s$;  and they
have branch cuts in the spectral plane (whose positions depend on $\t$ and $\s$).

In this section we shall argue that, nevertheless, the Lax connections can still be used to construct the `non-local' charges typical of integrable models. However, the space-time dependence of the Lax connection renders these charges difficult to compute explicitly. We shall focus here on the case of the PCM, while the other examples from Table \ref{2008tab1} are discussed in Appendix \ref{2008om}.

\subsection{Non-local charges}\la{s41}

The derivation of non-local conserved charges from the  monodromy matrix $\M = \mathcal P \,  \exp \, \int^b_a d\s \, L_\s$  discussed in Section \ref{ci} still applies for Lax connections with explicit space-time dependence. Indeed, the zero-curvature condition $\del_\s L_\t - \del_\t L_\s + [L_\s,L_\t]=0$ implies that
\be
\del_\t \M = \M \, L_\t(b) - L_\t(a) \, \M \ . \la{ce}
\ee
Hence, if we assume a periodicity condition on the spatial domain $a<\s<b$,
\be
L_\t(a) = L_\t(b)\ , \la{pe}
\ee
then we obtain
\begin{align}
\del_\t \M = [\M, L_\t(a)] \ , \la{lp}
\end{align}
and so the eigenvalues of $\M$ are conserved ($\del_\t \Tr[\M^n]=0$). If also the value at the endpoints vanishes, $L_\t(b) = L_\t(a)=0$, then all of the components of $\M$ are conserved ($\del_\t \M=0$).


We shall focus on the time-dependent PCM on an infinite spatial interval $(a,b)=( -\infty,\infty)$.\foot{It seems much harder to satisfy the periodicity condition \rf{pe} on a spatial circle due to the explicit non-periodic $\s$ dependence in the Lax connections for the time-dependent models.}
Picking the `negative' branch\foot{We note that it is consistent to `pick a branch' here: e.g., by assuming
that $w$ has an imaginary part, it then follows that the sign of the square root does not change from $\s=-\infty$ to $\s=\infty$. The choice of a branch is arbitrary but this negative choice is more useful for satisfying the periodicity condition and constructing conserved charges. Also, for the group $\eta$-model and PCM$_k$, which are deformations of PCM, the function
${z}$ is single-valued at $\s=\pm \infty$, with $z_{\infty}\equiv z\big|_{\s=\infty}=-1$. It is then natural to obtain $z_{\infty}=-1$
for the PCM as a limit of these models.} of the square root,
then the spectral function ${z}(w;\t,\s)$ in \rf{lpl} has the finite limit ${z} =\sqrt{\frac{w+\s+\t}{w+\s-\t}} \to z_{\infty} = -1$ at $\s \to \pm \infty$.
Hence, assuming $J_\pm$ is bounded for large $|\s|$, the Lax connection $\widehat{L}_\pm = \ha (1+{z}^{\pm 1} ) J_\pm$
vanishes at spatial infinity. The periodicity condition \rf{pe} is satisfied with $\widehat{L}_\t$  vanishing at spatial infinity,
so it follows  that all the components of $\M$ are conserved.

The boundary condition (that $J_\pm$ is bounded), needed above for the conservation of $\M$, is quite weak. A further, more stringent boundary condition comes from the requirement that $\M$ converges
as $(a,b)\to (-\infty, +\infty)$
to produce well-defined charges.

Although the monodromy is conserved, it is only defined implicitly by the first-order ordinary differential equation \eqref{px}, i.e.
\begin{align}
&\M^{-1} \del_\s \M = \widehat{L}_\s = \tfrac{1}{4}\big(1+\big[ \tfrac{w+\s-\t}{w+\s+\t} \big]^{1/2} \big)J_+ - \tfrac{1}{4}\big(1+\big[ \tfrac{w+\s-\t}{w+\s+\t} \big]^{-1/2}\big)J_- \ , \qquad \M\big|_{\s=-\infty} = I \ . \la{mpe}
\end{align}
Such an equation generally admits a solution but it is hard to find its explicit form. One possible approach
is to develop an expansion in the spectral parameter around a point where $\wL_\s$ vanishes (and thus the monodromy is trivial, $\M=I$).

In the usual time-independent PCM case (obtained by replacing $\sqrt{\tfrac{w+\s-\t}{w+\s+\t}} $ by a constant $z$ in \rf{mpe}), such an expansion around $z=-1$ yields the conserved `multi-local' Yangian charges in eq.\ \eqref{me}.
Each term in the expansion  around $z=-1$ is individually conserved because each term in the corresponding expansion of $L_\t$ (and hence the right hand side of \rf{ce}) vanishes at spatial infinity.

For the time-dependent theory, the only zero around which to expand $\widehat{L}_\s$ in \rf{mpe} is $w=\infty$ (again taking the negative branch of the square root). But, due to its explicit spatial dependence, the corresponding expansion of the Lax connection
is a sum of terms $w^{-n} P_{n-1}$, where $P_{n-1}$ is a polynomial of degree $n-1$ in $\s$. Then for any polynomial decaying boundary conditions on the fields at spatial infinity, the periodicity condition \rf{pe} on $\widehat{L}_\t$ will be broken at sufficiently high orders in this expansion.

Hence, while we have shown the formal existence of conserved non-local charges defined implicitly by \rf{mpe}, it appears to be hard to compute the monodromy matrix $\M$ explicitly: due to the explicit $\s$ dependence in the Lax connection, the usual expansion trick \eqref{me} does not easily work.
It is not clear at the moment how
to verify
if the resulting conserved charges are infinite in number (and independent)
as they should be for an integrable 2d theory.

\subsection{1d reductions}\la{s43}

One useful test of 2d integrability is to check the integrability of various 1d mechanical theories obtained as
consistent reductions of the 2d equations of motion.

Assuming an ansatz for a classical solution of an integrable 2d model
yielding a 1d system of equations (say with $\t$ as the remaining independent variable), one may expect
the resulting 1d system also to be integrable in the sense of admitting a Lax pair, $\tfrac{d}{d\t} A = [B, A]$. One should further demand that the conserved charges are in involution.

In general, if the solution satisfies the periodicity condition \rf{pe}, then  the flatness of the 2d Lax connection leads to a 1d Lax pair
given by $(A,B)=(\M, -L_\t(\infty))$ in \rf{lp}, evaluated on the reduction ansatz. For example, in \cite{Arutyunov:2003za}, such a reduction was performed for a certain `spinning string' ansatz in $AdS_5 \times S^5$, resulting in an integrable 1d Neumann-Rosochatius model. There (reversing the roles of $\t$ and $\s$ from that paper to match the above discussion) the $\s$-dependence of the ansatz was simple and it was possible to completely remove the $\s$-dependence from the Lax connection using a gauge transformation --- which is essentially the same problem as computing the monodromy matrix. In our case, with explicit $\s$-dependence already in the Lax connection, the problem of directly removing the $\s$-dependence by gauge transformations would appear to be much more difficult.

\paragraph{Trivial reduction.}
In the simplest `trivial' 1d reduction one assumes that the
fields do not depend on $\s$. This is indeed a consistent truncation of the above time-dependent models, obtained by replacing $\del_\pm \to \t$ in their Lagrangians.
For example, in the PCM case, setting $g=g(\tau)$ in \rf{lcPCM} gives the 1d action for
geodesic motion on a group space with a time-dependent radius.
The solvability of geodesics in this model is
obvious since the explicit time dependence may be eliminated by a redefinition of $\t$
\be
\la{48} S_1 \sim \int d\t \ \t \ \Tr\big[ (g^{-1} \del_\t g )^2 \big] = \int d\t' \ \Tr\big[ (g^{-1} \del_{\t'} g )^2 \big] \ , \qquad \ \ \t'=\log \t \ .
\ee
The resulting equation of motion $\del_{\t'} (g^{-1} \del_{\t'} g) = 0$ is solved by
\be
g = g_0\, e^{\t' u_0} = g_0\, \t^{u_0 } \ , \qquad \quad g_0 = \const \in G \ , \quad \ u_0=\const \in \Lie(G) \ .
\ee
The same argument equally applies for any case where the time dependence only appears as an overall factor rescaling the Lagrangian -- which will follow if there are enough global symmetries that only the overall `radius' can run under the RG flow (e.g.\ also in the symmetric space $\s$-model case).

In general, the global symmetry charges may be found from the monodromy $\M$. Formally, the monodromy on an infinite line does not converge upon the trivial reduction since $J_\t = g^{-1} \del_\t g$ does not decay at spatial infinity (as it is now independent of $\s$).
On a finite space interval, the periodicity condition \rf{pe} is not satisfied so charges will not be conserved. However, making an expansion around the zero of the Lax connection at $w=\infty$ (cf.\ \eqref{me}), the global symmetry is reflected in the $\s$ independence of the leading $\O(w^{-1})$ term in $\wL_\t$,
\begin{align}
\wL_\t &= \tfrac{1}{4}(1+\big[ \tfrac{w+\s-\t}{w+\s+\t} \big]^{1/2})J_+ + \tfrac{1}{4}(1+\big[ \tfrac{w+\s-\t}{w+\s+\t} \big]^{-1/2})J_-
= \tfrac{1}{2} \t J_\s \, w^{-1} + \O(w^{-2})\ .
\end{align}
This puts the leading term on the right hand side of \rf{ce} in the commutator form \rf{lp}. Since the monodromy matrix is the identity at the leading order,
the right hand side of \rf{ce} is of $\O(w^{-2})$. It then follows that the $\O(w^{-1})$ term in the monodromy matrix, which is the global $G_R$ Noether charge, is
still conserved\foot{The Noether charge for $G_L$ symmetry is obtained similarly after a gauge transformation of the Lax connection and choosing instead the positive branch of the square root.}
\begin{align}
&\M = 1 + \ha w^{-1} Q_R + \O(w^{-2}) \ , \qquad \del_\t Q_R = 0 \ , \qquad Q_R = \int d\s \ \t J_\t \ . \la{noet}
\end{align}

\paragraph{Non-trivial reduction.}
Now let us consider a non-trivial 1d reduction when the 2d fields \textit{do} depend on $\s$ in a particular prescribed way. Such a reduction will lead to a
non-trivial 1d model, giving a more stringent test of the integrability of the time-dependent 2d model.

Starting from the time-dependent $SU(2)$ PCM \rf{lcPCM} parametrized as
\begin{align}
&\wLL = -\tfrac{c}{2} \, \t \, \Tr [ J_+ J_- ] = c\, \t \, \big[ \del_+ \theta \del_- \theta + \sin^2{\theta} (\del_+ \phi \del_- \phi + \sin^2{\phi}\, \del_+ \psi \del_- \psi)\big] \ , \la{412} \\
&\qquad g = n^a \s_a \ , \qquad \s_a = (I, \s_i ) \ , \ \ i=1,2,3 \ , \no \\
&\qquad n^0 n^0 - n^i n^i = 1 \ , \qquad n^a = ( \cos{\theta} , \ i \sin{\theta} \cos{\phi} , \ i \sin{\theta} \sin{\phi} \cos{\psi} , \ i \sin{\theta} \sin{\phi} \sin{\psi} ) \ , \no
\end{align}
let us consider, e.g., the following ansatz for a classical solution
\be
\theta = \theta(\t) \ , \qquad \phi = m \s \ , \qquad \psi = 0 \ . \la{wan}
\ee
This leads to a consistent reduction of the 2d theory: the $\phi$ and $\psi$ equations are both satisfied,
while the equation for $\theta(\t) $ follows from the 1d Lagrangian ($\dot{\theta} \equiv \del_\t \theta$)
\be
\L_1 = {c} \, \t\, \big( \dot{\theta}^2 - m^2 \sin^2 {\theta}\big) \ . \la{s1}
\ee
Thus the effective 1d model is a time-dependent analog of the `sine-Gordon' mechanics.

Let us assume the $\s$-direction is an infinite line, still using the ansatz \rf{wan} (e.g.\ by taking $m$ to be a continuous parameter and formally decompactifying $\phi$).
Then
one can check that $J_\pm$ is oscillating but bounded at spatial infinity. Hence, as discussed above, the right hand side of \rf{ce} vanishes and the entries of the monodromy matrix are conserved.
While again it is not easy to compute the monodromy explicitly in terms of $\theta$ and $\dot{\theta}$,
it can be done in the small field expansion $(\theta,\dot{\theta}) \to \e (\theta,\dot{\theta})$, $\e \ll 1$ since the Lax component $\wL_\s$ vanishes as $(\theta, \dot{\theta}) \to 0$. In this expansion the Lagrangian \rf{s1} becomes (after rescaling it by a factor of $c^{-1} \e^{-2}$)
\begin{align}
&\L_1' = \t\big[ \dot{\theta}^2 - m^2 \e^{-2} \sin^2 {(\e \theta)}\big] = \L^{lin} + \tfrac{1}{3} \e^2\, m^2\, \theta^4 + \O(\e^4) \ , \la{ne}\\
&\L^{lin} = \t \, \big[ \dot{\theta}^2 - m^2 \theta^2 \big] \ . \la{lt}
\end{align}
The leading (`linearized') Lagrangian \rf{lt} describes (after the same redefinition $\tau = e^{\tau'}$ as in \rf{48})
a harmonic oscillator with time-dependent frequency $m^2 e^{2 \tau'}$.
The corresponding $\O(\e)$ terms in the monodromy matrix lead to the conserved charge
\begin{align}
&\dot{Q}^{lin} = 0 \ , \qquad Q^{lin} = \t \big[ \bw(\t; w) \, \dot{\theta} - \dot \bw(\t; w) \, \theta \big] \ , \la{ql} \\
& \bw(\t;w) = \int_{-\infty}^{+\infty} d\s\, e^{-im \s} \tfrac{ i}{2 s_+ s_- }
\ , \qquad \qquad s_\pm \equiv \sqrt{w+\s \pm \t}\ . \la{ql2}
\end{align}
In Appendix \ref{2008C} we use this conserved charge to construct the general solution of the linearized equation of motion
(with $\theta=\bw$ being a particular solution).

Computing the perturbative corrections to the monodromy, one then finds for the
conserved charge of the non-linear theory \rf{ne}
\begin{align}
&\dot{Q} = 0 \ , \ \ \ Q = Q^{lin} + \e^2 \Big[\int d\s \, q^{(1)} + \int_{\s_1<\s_2} d\s_1 d\s_2 \, q^{(2)} + \int_{\s_1<\s_2<\s_3} d\s_1 d\s_2 d\s_3 \, q^{(3)} \Big] + \O(\e^4) \ , \no \\
&\ \ \ q^{(1)} = - \tfrac{m \, e^{-im\s} }{3s_+ s_-} (s_+ s_- -w-\s) \, \theta^3 \ , \la{cq}\\
&\ \ \ q^{(2)} = \tfrac{i m }{4s^1_+ s^1_-s^2_+ s^2_-} \Big[ e^{-im \s_2} ( s_+^1 s_-^1 - w - \s_1)\big[m(s_+^2 s_-^2 -w- \s_2)\theta +i \t \dot{\theta}\big] - (\s_1 \leftrightarrow \s_2) \Big] \, \theta^2\ , \no \\
&\ \ \ q^{(3)} = \tfrac{e^{-im(\s_1 - \s_2 + \s_3)}}{8 s^1_+ s^1_-s^2_+ s^2_-s^3_+ s^3_-} \big[m(s_+^1 s_-^1 -w- \s_1)+i \t \dot{\theta}\big] \no \\
&\qquad \qquad \times \big[ - m(s_+^2 s_-^2 -w- \s_2)+i \t \dot{\theta}\big]\big[m(s_+^3 s_-^3 -w- \s_3)+i \t \dot{\theta}\big] \ , \ \ \quad s_\pm^n \equiv \sqrt{w+\s_n \pm \t} \ . \no
\end{align}
This perturbative procedure of constructing the conserved charge can be extended to higher orders,
computing more and more $\s$ integrals at each step.

Let us also mention that the time-dependent $SL(2,\mathbb{R})$ PCM (cf.\ \rf{412}),
\be\la{420}
\wLL = - c \, \t \Big[ \del_+ \r \del_- \r + \ha e^{-2\r} \, (\del_+ x^+\del_- x^- + \del_- x^+\del_+ x^-) \Big] \ ,
\ee
admits a `non-trivial' reduction that is manifestly integrable.
Indeed, if we set $x^+ = a \s, \ x^- = b\s, \ \r=\r(\t)$ then the $x^\pm$ equations are solved
and the equation for $\r(\t)$ follows from the 1d action (cf.\ \rf{s1})
\be\la{421}
S_1 = - c \,\int d \t \, \t \big[ (\del_\t{\r})^2 - ab \, e^{-2\r} \big] \ .
\ee
Here the explicit time dependence can be eliminated by redefining $\t=e^{\t'}$ and $\r = \r' + \t'$
so that we end up with the standard 1d Liouville mechanics with the energy being a conserved charge.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}\la{s6}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We have
observed
a surprising new connection between
classical integrability and the RG flow in 2d theories:
starting with an integrable theory and promoting its couplings to time-dependent functions, its
Lax connection generalizes naturally to the resulting
time-dependent theory only if the coupling functions
solve the 1-loop RG equations
of the original theory.
We demonstrated this on six classes of integrable $\s$-models.


One interesting implication is
that the 1-loop $\beta$-functions, which are normally associated with 1-loop divergences in quantum theory,
can thus be obtained in these models through the classical procedure of requiring the existence of a flat Lax connection in
the corresponding time-dependent theory.

As we discussed at the start of the chapter,
such time-dependent models can be naturally embedded into string theory by
starting with a Weyl-invariant $\s$-model \rf{csm} with two extra null directions $(u,v)$
and fixing a l.c.\ gauge $u=\t$.
If the l.c.\ theory \rf{lct} is classically solvable, it is natural to expect that the corresponding
 string $\s$-model \rf{csm}  should be solvable,
since one may move
from $u=\t$ to
any other
solution of the $u$-equation $\del_+\del_- u = 0 $
by a conformal transformation. The $v$-equations
$ \del_\pm v =\ha \GG_{ij}(\t,x) \, \del_\pm x^i \del_\pm x^j$
(following from the conformal constraints)
are
linear and so are also readily solvable. It is not immediately clear, however,
if integrability in the sense of admitting a Lax representation should similarly lift up to the $(D+2)$-dimensional string $\s$-model directly.

The Lax connections for the time-dependent theories have an
unusual form (depending explicitly on $\t$ and $\s$, as in the special
examples discussed in \cite{Belinsky:1971nt,Breitenlohner:1986um}). However, given certain boundary conditions, the entries or
the eigenvalues
of the monodromy matrix on an infinite spatial line are conserved.
Due to the explicit $\s$ dependence in the Lax connection, it is hard to
evaluate the monodromy and find the conserved charges explicitly.
We considered some consistent reductions of the 2d equations of motion to time-dependent 1d systems.
The `trivial' ($\s$-independent)
reduction of the PCM is clearly integrable due to the remaining global symmetry.

For the `non-trivial' 1d reduction in Section \ref{2008s43} we evaluated the monodromy, and hence constructed a conserved charge \rf{cq} in perturbation theory in a small field expansion. The perturbative existence of this conserved charge (following from the existence of a Lax connection)
is a non-trivial property, suggesting
that the 1d theory \rf{s1} may be interpreted as integrable.  In contrast, with generic (time-dependent) potentials added to the linearized theory \rf{lt}, we would not expect the linearized conserved charge \rf{ql} to admit even a perturbative extension to the non-linear theory.
The time-dependent 1d theory \rf{s1} is certainly not integrable in the Liouville sense as it would fail the Kovacic algorithm test used in \cite{Basu:2011fw,Stepanchuk:2012xi}.
Here we are suggesting a broader notion of integrability relating  to the explicit solvability of the equations of motion (allowing non-Liouvillian solutions like Bessel functions, etc.).


One way to fully establish the classical integrability of the $\s$-models with local couplings
would be to construct an infinite tower of local conserved charges in involution, in the spirit of \cite{Goldschmidt:1980wq,Evans:1999mj,Evans:2000qx,LMV}.
In Section 5 of \cite{HLT2008} we  attempted this
for the PCM with `local couplings'
in the Hamiltonian formulation.
A naive application of the method used for constant couplings does not yield such charges, except in the case of the `chiral' theories only depending on $\xi^+$ or on $\xi^-$,
where it works with a slight modification (see Appendix D of \cite{HLT2008}).
Nevertheless, the form of the Lax matrix and $R$-matrix is suggestive of an underlying algebraic structure.
Understanding it may provide additional insights into the question of integrability.

While we considered time-dependent models at the classical level only, one may wonder if they themselves
are renormalizable, i.e.\ stable under RG flow. Renormalization of generalized
$\s$-models with target-space metric depending on the 2d coordinates was considered in \cite{Osborn:1987au}. In the case
we discussed (cf.\ \rf{lct}) when $\GG_{ij}$ depends only on $\t$, i.e. $\L=\GG_{ij}(\t, x) \del_+ x^i \del_- x^j$, the 1-loop logarithmic counterterm
is proportional to $ K_1= \GG_{ml} \GG^{jk} \del_\t x^m\, \del_\t \Gamma^l_{jk} + \frac{1}{4} \del_\t \GG^{ij} \del_\t \GG_{ij} $, where
$\Gamma^l_{jk}$ is the Christoffel connection of $\GG_{ij}$. Thus in general one needs to add also counterterms with one and no derivatives, i.e. $V_m(x) \del_\t x^m + T(x)$. However, in the `factorized' case when $\GG_{ij} (\t, x) = f(\t) \GG_{ij}(x),$
like in the time-dependent PCM \rf{lcPCM}, the above counterterm becomes an $x$-independent function,
$K_1\sim ( \del_\t f)^2 $. Furthermore, if $f$ is linear in $\tau$ as in \rf{lcPCM} then this $K_1$ is just a constant
and thus such a model is renormalizable.
This suggests that at least some time-dependent integrable models
discussed in this chapter may have
well-defined quantum generalizations.

\

Among other possible directions, it would be important to generalize the present investigation to
other integrable $\sigma$-models, e.g.\ the class of models based on complex homogeneous spaces
whose  Ricci flow was studied in \ci{byk,byk2} and  the $\mathbb{Z}_T$ coset models of \cite{Young:2005jv,yo}.
Another interesting class of examples would be the integrable $G\times G$ and $G\times G/H$ models studied in Chapter \ref{GGS} above.
Furthermore, while in this chapter we have only studied 2-derivative $\s$-models,
we expect the connection between
the requirement of integrability of the time-dependent theory and the RG flow to be more general and to apply also to
models with potentials.
Indeed,
one also finds this remarkable connection in the case of the sine-Gordon model,
\be
S= \tfrac{1}{4\pi} \int d\t d\s \, \tfrac{1}{g^2}\big[ \ha \del_+ x \del_- x + m^2 \cos{x}\big]\ . \la{sgm}
\ee
Replacing the couplings $(g,m)$ by functions\foot{For a discussion of the sine-Gordon model with a particular `non-integrable'
local coupling $m=m(\s)$ see \cite{Levkov:2020lfa} and references there.}
of $\t$
one can show
that, for the resulting theory to be integrable
(assuming a natural ansatz for a generalization of the Lax connection to the time-dependent theory
---
see Appendix \ref{2008sing}),
the functions $(g(\t),m(\t))$ should be solutions of the 1-loop RG flow equation for \rf{sgm}, i.e.
should be given by
\be m^2(\t) = e^{ \b(g)\, \t} \, m_0^2 \ , \ \ \ \qquad g(\t) = g \ , \ \ \ \ \qquad \b(g) = - 2 + g^2 \ . \la{52}\ee
The time-dependent theory,
\be
\widehat{S}= \tfrac{1}{4\pi} \int d\t d\s \, \tfrac{1}{g^2} \big[ \ha \del_+ x \del_- x + e^{\b(g)\, \t}\, m^2_0\, \cos{x}\big]\ ,\la{53}
\ee
is indeed classically integrable since the explicit $\t$-dependence in \rf{53} can
be removed by a 2d conformal transformation getting back to \rf{sgm}:
under $\xi^\pm \to f^\pm (\xi^\pm)$ the action
\rf{sgm} retains its form with
$m^2 \to {f^+}'(\xi^+)\, {f^-}'(\xi^-)\, m^2 $.
Note that
the non-trivial 1d reduction of the $SU(2)$ PCM in eq.\ \rf{s1} is also obtained as the `trivial' reduction $x=x(\t)$
of \rf{53}
after a redefinition $\t \to \log \t $, supporting the expectation that \rf{s1} is an integrable 1d theory.
It would be interesting to explore
whether
this time-dependent integrability--RG flow connection applies also to
other examples of integrable massive theories, such as complex sine-Gordon and Toda models.

\

One of the features of our construction of the Lax connection for time-dependent theories is that
the constant spectral parameter of the original theory
is replaced by
a function
$z\to z(w;\t,\s)$ of a new spectral parameter $w$ and the 2d coordinates (cf.
\rf{pla},\rf{lpl}).
This puts the spectral parameter and 2d space-time coordinates on a more equal footing,
suggesting a possible interpretation from the point of view of the
construction \cite{Costello:2019tri}
of many
integrable 2d theories from a 4d Chern-Simons theory,
with the two extra directions related to the complex spectral parameter (see also \cite{Delduc:2019whp} and refs.\ there).
In that context the redefinition of $z$ is like changing
the differential structure of the 4d space, i.e.\ replacing $\del_{\t,\s} z = 0$
with $\del_{\t,\s} z = V_{\t,\s}(z;\t,\s)$ (cf.\ \rf{pd1}).
It would be interesting to see if the time-dependent models considered above
can  be reproduced from the 4d Chern-Simons construction. 
Indeed, the $\s$-dependent version of the PCM discussed above
has already been obtained \cite{Penna:2020uky} from a closely related Chern-Simons theory on twistor space.






==> v arxiv v2/2103.tex <==
\numberwithin{equation}{chapter}

\renewcommand{\arraystretch}{1.3}

\makeatletter
\renewcommand\section{\@startsection {section}{1}{\z@}%
{-3.5ex \@plus -1ex \@minus -.2ex}%
{2.3ex \@plus.2ex}%
{\normalfont\large\bfseries}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
{-3.25ex\@plus -1ex \@minus -.2ex}%
{1.5ex \@plus .2ex}%
{\normalfont\normalsize\bfseries}}
\makeatother

\expandafter\def\expandafter\bfseries\expandafter{\bfseries\ifmmode\else\boldmath\fi}
\expandafter\def\expandafter\mdseries\expandafter{\mdseries\ifmmode\else\unboldmath\fi}
\expandafter\def\expandafter\normalfont\expandafter{\normalfont\ifmmode\else\unboldmath\fi}

\providecommand{\href}[2]{#2}

\def\id{\protect{{1 \kern-.28em{\rm l}}}}
\def\be{\begin{eqnarray}}
\def\ee{\end{eqnarray}}
\def\bi{\bibitem}
\def\tr{{\rm tr}}
\def\ha{\tfrac{1}{2}}
\def\td{\tilde}
\def\ci{\cite}
\def\N{{\mathcal N}}
\def\ww{\Omega}
\def\S{{\mathcal S} }
\def\nn{\nu}
\def\z{\zeta}
\def\dg{\dagger}
\def\a{\alpha}
\def\b{\beta}
\def\ap{\alpha^\prime}
\def\aa{{\a'}}
\def\g{\gamma}
\def\ok{\frac{1}{k}}
\def\jL{{J}}
\def\cL{{\mathcal L}}
\def\cH{{\mathcal H}}
\def\E{{\mathcal E}}
\def\w{\omega}
\def\vep{\varepsilon}
\def\De{{\mathcal D}}
\def\k{\kappa}
\def\four{\tfrac14}
\def\third{\tfrac{1}{3}}
\def\det{\hbox{det}}
\def\tid{\tilde}
\def\vv{{\rm v}}
\def\ta{{\tilde \a}}
\def\fo{\frac{1}{4}}
\def\K{{\rm S}}
\def\el{\ell}
\def\Tr{{\rm Tr}}
\def\P{\Phi}
\def\l {\lambda}
\def\bl{{\tilde \l}}
\def\const{{\rm const}}
\def\vn{\vec n}
\def\Prod{\Pi}
\def\O{{\mathcal O}}
\def\m{\mu}
\def\vs{\vec \s}
\def\ie{i.e.}
\def\rS{{\rm S}}
\def\as{{\a}}

\def\foot{\footnote}
\def\ra{\rightarrow}
\def\F{{\cal F}}
\def\cc{\circ}
\def\eqv{\equiv}
\def\ni{\noindent}
\def\bw{{\rm w}}
\def\cT{{\cal T}}
\def\no{\nonumber}
\def\J{{\cal J}}
\def\om{\omega}
\def\l{\lambda}
\def\tl{{\tilde \l}}
\def\tk{{\tilde k}}
\def\sqtl{{\sqrt{\tilde \l}}}
\def\adss{$AdS_5 \times S^5$\ }
\def\D{\Delta}
\def\p{\phi}
\def\r{\rho}
\def\rN{{\rm N}}
\def\tw{{\tilde w}}
\def\vl{ \vec \ell}
\def\varpi{{\rm w}}
\def\bG{\bar \G}
\def\ve{\varepsilon}
\def\I{{\cal I}}
\def\La{{\Lambda}}
\def\R{{\rm R}}
\def\bt{\bar\theta}
\def\Z{{\cal Z}}
\def\pa{\partial}
\def\bea{\be}
\def\eea{\ee}
\def\DD{{\rm D}}
\def\chii{\varepsilon}
\def\th{\theta}
\def\t{\tau}
\def\beq{\be}
\def\eeq{\ee}
\def\beqa{\bea}
\def\eeqa{\eea}
\def\bs{\bigskip}
\def\c{{\rm a}}
\def\del{\partial}
\def\s{\sigma}
\def\eps{{\epsilon}}
\def\n{\nu}
\def\dag{\dagger}
\def\bd{\bar \del}
\def\ed{\end{document}}
\def\iffa{\iffalse}
\def\xp{x_+}
\def\xm{x_-}
\def\te{\textstyle}
\def\rx{{\rm x}}
\def\C {{\rm C}}
\def\hC {{\rm \hat C}}
\def\dd {{\rm d}}
\def\bb{{\rm b}}
\def\sql{{\sqrt{\l}}}
\def\ep{\epsilon}
\def\G{\Gamma}
\def\dx{\dot x}
\def\vp{\varphi}
\def\tx{{\tilde x}}
\def\ad{{\rm ad}}
\def\d{\delta}
\def\de {\del}
\def\L{\mathcal{L} }
\def\pcm {{\rm PCM}}
\def\wz{{\rm WZ}}
\def\pcmq {{\rm PCM}$_q$\ }
\def\ZMq {{\rm ZM}$_q$\ }
\def\ZM {{\rm ZM} }
\def\pp{{\rm p}}
\def\qq{{\rm q}}
\def\rk {{\rm u}}
\def\rrk{{\rm e}}
\def\ss{{\rm s}}
\def\tt{{\rm t}}
\def\uu{{\rm u}}
\def\sm{$\sigma$-model}
\def\sms{$\sigma$-models}
\def\ov{\over}

\def\Ad{\text{Ad}}
\def\lmp{\Lambda}
\def\bl{\bar \lambda}
\def\Lie{\operatorname{Lie}}
\def\hb{\hbar}
\def\k{\varkappa} \def \h {{\rm h}}
\def\dt{\tfrac{d}{d\t}}
\def\ddt{\frac{d}{d\t}}
\def\bb{{\rm b}}
\def\vv{{ v}}
\def\kk{{\rm k}}
\def\ka{{\kappa}}
\def\np{ }
\def\cM{\mathcal{M}}
\def\bh{\bar{h}}
\def\lam{$\lambda$-model}
\def\etm{$\eta$-model}
\def\bh{\bar h}
\def\hh{{\rm h}}
\def\PCM{\L_{_{\rm PCM}}}
\def\WZ{\L_{_{\rm WZ}}}
\def\M{{\cal M}}
\def\q{{\rm q}}
\def\RR{{J}}
\def\LL{{K}}
\def\kold{k_{\text{old}}}
\def\kaold{\ka_{\text{old}}}
\def\ed{\end{document}}
\def\F{H}
%\def\cgg{c_{_G}}
\def \cgg {\ccg}
\def\cg{c\,}
\def\cf{c_{_\F}}
\def\cff{c_{_\F}}
\def\HH{\F}
\def\XX{{X}}
\def\hhh{\widetilde {\hh}}
\def\e{\varepsilon}
\def\tih{{\hat h}}
\def\H{{\rm H}}
\def\GG{{\rm G}}
\def\BB{{\rm B}}
\def\g{\gamma}
\def\bl{\bar\lambda}
\def\ol{\underline}
\def\ul{\overline}
\def\MM{\mathcal M}
\def\hz{z}
\def\hhz{z} %\def\hhz{\widehat{z}} %v3
\def\wcL{\widehat{\L}}
\def\wL{\widehat{L}}
\def\XX{X}
\def\bw{\a}
\def\xx{{\rm x}}
\def\cR{{\mathcal R}}
\def\sms{$\s$-models\ }
\def\sm{$\s$-model\ }
\def\wLL{\widehat{\L}}
\def\br{\big[}
\def\bl{\big]}
\def \FF {h}
\def\GG{{\rm G}}
\def\wt{\widetilde}
\def \wh  {\wt \rh}

\def \foot{\footnote}\def \ci{cite}\def \l {\lambda}\def \iffa {\iffalse}
\def \RR {{R}} \def \ov {\over }\def \a  {\alpha} \def \ha {{1\ov 2}}
\def \ed {\end{document}}
\def \bi {\bibitem}
\def \adss {${\rm AdS}_5 \times S^5~$ }

\def \ov {\over}
\def \tr {{\rm tr}}
\def \ha {{1 \over 2}}
\def \td {\tilde}
\def \ci {\cite}
\def \bi {\bibitem}
\def \N  {{\cal N}}
\def \aa  {{\rm a}}
\def \te {\textstyle} 
\def \Z {{\cal Z}}
\def \RR {{L}}
\def \aa {{\rm a}} \def \eps {\epsilon}\def \rr {{\rm r}}

\def \rh {{\rm h}}
%\def \GB {{$\GG \BB$}\ }
\def \cg {{\rm c}}

\def \ccg {{\cg_{_G}}} \def \ch {{\cg_{_H}}}
\def \cggg  {{\cg^2_{_G}}} 
 \def \ep {\epsilon}

\def \ww {{\rm w}}

  \def \bpsi {\bar \psi}
\def\cG{\ccg}

\def\ol{\overline}
\def \ha {\tfrac{1}{2}}

\def \B {{ B}}

\def \lh {{\rm h}}
    \def \ta  {U}   \def \tb {V} 

\def \hij  {p_{ij} }  \def\Hij  {\chi_{ij}}



\chapter{\texorpdfstring{$G\times G$}{GxG}  and \texorpdfstring{$G\times G/H$}{GxG/H}   sigma  models \label{GGS}}


It is  
 expected  that classically  integrable 2d \sms   should be   stable  under the  renormalization group  flow, 
 the intuition  being that hidden symmetries 
will constrain
 the  RG evolution. 
Constraints on coupling constants   required for integrability should thus be RG-invariant. 


The aim of this chapter is to explore the  connection between integrability and the RG flow  on 
another class of examples ---   integrable $G\times G$ and $G\times G/H$ models that were derived from  the affine Gaudin construction \cite{DLMV, ABL}.  These models may be viewed as    generalizations  of the PCM$_k$,
\be
\L_{_{{\rm PCM}_k}} = {\rh} \, \L_{_{{\rm PCM}}}  + k \, \L_{_{\rm WZ}}(g)\ , \qquad  
\L_{_{{\rm PCM}}}  = -\ha \,  \Tr[ J_+ J_- ]\ ,   \qquad J \equiv g^{-1} dg \ , \ \ g\in G \ , \la{Pk}
\ee
i.e.\   the principal chiral model    (with inverse coupling $\rh$)   with  the WZ term  (with level $k$).
The conformal WZW model is obtained at the special points $\rh=\pm k$ (see Secrtions \ref{PkS}-\ref{WS}).

The PCM$_k$   admits  various  integrable deformations (see, e.g., \cite{Klimcik:2002zj,Klimcik:2008eq,Ki,Balog:1993es,Delduc:2013fga,DMV} and Section \ref{etas} above), which have been  interpreted 
  \cite{DLMV} as  particular  cases  of   integrable affine Gaudin models. 
The  affine Gaudin construction also produces    natural generalizations  of the  PCM$_k$  to integrable models on products of group  spaces $G^N = G\times \ldots \times G$ \cite{DLMV}. 

Here  we shall  consider  a  subclass of  such  models  defined  by 
\begin{align}
&\L = -\ha \, \rho_{ij} \, \Tr[ J^{(i)}_+ J^{(j)}_- ] + k_i  \, \L_{_{\rm WZ}}(g^{(i)}) \ ,  \qquad \qquad \la{cou}\\
&J^{(i)}\equiv {g^{(i)}}^{-1} d g^{(i)} \ , \qquad \qquad  g^{(i)} \in G^N  \ , \qquad i=1,\ldots,N \ . \no
\end{align}
We denote by  $J^{(i)}$   the Maurer-Cartan 1-form  corresponding to $i$-th copy of  $G$  and 
 $\rho_{ij}$ is a \textit{constant}  coupling   matrix (summation over repeated  $i,j$ is assumed). 

The PCM$_k$ \rf{Pk} corresponds to the special case $N=1$ (with $\rho_{11}=\rh$ and $k_1=k$), and is integrable for any values of its couplings. However, for $N>1$,   the model \rf{cou} is  classically integrable only for \textit{special}  couplings $(\rho_{ij}, k_i)$
 that correspond to  
 the  affine Gaudin models \cite{DLMV}. 
These are
selected  as the solutions 
 of certain polynomial equations.
We will focus  on the first  non-trivial case of $N=2$, i.e.\  on  $G\times G$  models.

 As we shall find in  Section \ref{21032},
  the 
classical integrability condition for 
 $G\times G$ theories \rf{cou} 
is 
 automatically stable 
 under the  \textit{2-loop} RG flow 
 in
 a particular  subtraction scheme (extending the 1-loop results of \cite{today}). 
 Here the  2-loop stability is  obtained without the need for any  finite counterterms.

\

The model  \rf{cou}  
is a special case   of the 2d 
 $\s$-model
 \eqref{13},
 whose 2-loop $\b$-functions are given in the ``\GB scheme'' in eq. \eqref{BMT} (see also Section \ref{SD} on subtraction schemes).
This special 2-loop   scheme  
 effectively  treats 
$\GG_{mn}$ and $\BB_{mn}$  as symmetrically as possible, with the respective 
$\beta$-functions   being the symmetric and antisymmetric parts of a single tensor expression \cite{Bos:1987mw,mt}  (see also \cite{Hull:1987pc,Ketov}). We note that in the context of this chapter, the diffeomorphism ($L_{\xi}(\GG+\BB)_{mn}$) and B-gauge transformation ($\del_{[m}\l_{n]}$) terms in \eqref{BMT} may be ignored
 since they  
automatically 
   vanish in the examples  considered below 
 due  to  manifest global $G_L \times G_L$  symmetry. 


Applied  to the   case of the PCM$_k$  in  \rf{Pk},  the 2-loop $\b$-function in \GB scheme  \eqref{BMT}  gives (here we set $\a'=1$)\foot{In this chapter we denote $\t=\log\m$ (instead of $t$) since we will use a coupling constant called $t$.}
\be \ddt{\rm h} = \ccg\, (1-\tfrac{k^2}{\rh^2})\, \Big[ 1 +  \tfrac{\ccg}{2\rh} (1-  \tfrac{3\, k^2}{\rh^2}) \Big] \ ,  \qquad \qquad   \ddt{k}=0  
 \ , \la{Pkb}\ee
so that  the  position  of the WZW  fixed point $\h= \pm k$ remains unchanged at the 2-loop order. 
The  2-loop PCM$_k$ $\beta$-function \rf{Pkb} was 
found in  \cite{Bos:1987mw}  
using a scheme equivalent this one  at the 2-loop level. 
To recall, part of the scheme freedom
comes from the  prescription of how one treats  the  antisymmetric  2d tensor  $\e^{\m\n}$  appearing  in the $\BB$-term in \eqref{13} 
 in dimensional regularization. Ref.  \cite{Bos:1987mw}  used a  't Hooft-Veltman  prescription of treating $\e^{\m\n}$ as effectively 2-dimensional. 
 In  \cite{mt} it was  assumed  that, in $d=2+\ep$ dimensions,  $\e^{\m\n}\e_{\r\s} = 
  f(\ep) ( \delta^\m_\r \delta^\n_\s - \delta^\m_\s \delta^\n_\r ) $  where   $f= 1 + f_1 \ep +...$,    and then the  \GB scheme  \eqref{BMT}  corresponds to 
the choice  $f_1= -1$.  As noted in \cite{Bap}, the scheme used in \cite{Bos:1987mw}   
is equivalent (at least at the 2-loop level)  to  
$f(d) = \frac{1}{ d-1}= 1 - \ep + ...$, i.e.\  to the choice $f_1= -1$
 \ci{mt}
of the \GB scheme.


The  \GB   scheme    is naturally  ``adapted'' to the  vicinity of the WZW  conformal point: 
the derivative $\del_\rh \b_\rh\big|_{\rh=k}$ of the $\beta$-function for $\rh$ at the fixed point
correctly  reproduces \cite{Bos:1987mw}  the  anomalous  dimension of  the $\Tr (J_+J_-)$ operator (PCM  Lagrangian)
as computed \cite{KZ} using the  underlying  infinite dimensional 
Kac-Moody  symmetry  of the WZW   model.   Thus   this scheme is 
apparently 
 consistent  with the preservation of the KM symmetry  in 
  the vicinity of  
the conformal point. 

  It is then natural to expect that this scheme   should also  play  a special role   in  a more general  class  of 
 integrable  models \rf{cou}   containing   WZW  models as  special    limits,\foot{Similar logic was recently used 
    in \cite{shifman} in the  discussion of the 2-loop RG   evolution  of a   ``squashed''  $SU(2)$  variant  of  
   PCM$_k$.} 
   and should  facilitate  preservation   of the  hidden integrable structure of these models at the quantum level.  
We will indeed  see    evidence for this below:  the 
classical integrability  conditions for the $G\times G$ model  \rf{cou} 
will be automatically  preserved by the 2-loop   RG evolution 
 provided  one uses the $\beta$-functions in the \GB scheme  \eqref{BMT}. 

\

We shall also  study, 
in Section \ref{2103gu}, 
 a  gauged  analog  of the  models \rf{cou}  defined  on a coset space $G\times G/H$.
 This theory,  
  which
 was  recently derived from  affine Gaudin models  in  \cite{ABL},
may be   viewed as a
    generalization  of the standard  $G/H$ symmetric space $\s$-model,   
    also including 
 WZ terms.
    For these $G\times G/H$ theories to be gauge invariant, the  corresponding 
    couplings must satisfy certain linear relations. In addition, for a gauge invariant   model to be  classically integrable,
    the couplings  should  further satisfy certain polynomial relations \cite{ABL}. 
        
    We will 
    compute  the RG flow for these 
     integrable $G\times G/H$ theories, finding that  they  are stable under the 
      1-loop RG flow.  
      However, at the 2-loop level, 
RG stability 
does  not
 automatically   
 arise  and,  in general,   
          requires   certain 
      finite redefinitions of the couplings. These  are  
       equivalent to adding specific  finite counterterms,         
which  may  be  interpreted  as  required for preservation of integrability  
at the quantum level
 (analogous to what was observed  on other   examples in Chapter \ref{QCS}). 
       There are still a few special  cases, in particular the integrable $T^{1,1}$ model of  \cite{ABL},   that are  automatically stable 
       under the 2-loop RG flow (see Section \ref{2103T11}). 

\

\sloppy
In Section \ref{2103sq} we shall present a new  integrable \sm with 
target space  metric  
${T^{1,q} = SU(2) \times SU(2)/U(1)}$ \ci{romans} 
   and a particular $B$-field. The model admits as a special limit 
 the  conformal GMM model  with unequal levels \ci{GMM,PZT}.
Our central observation is that, in the case of the  subgroup $H$ in $G\times G/H$  being 
 abelian, the gauge invariance conditions of  \cite{ABL}  are too restrictive and  there is also a second 
 ``branch'' 
  of gauge invariant theories. This allows a natural generalization of the integrable $T^{1,1}$ model of \cite{ABL}  to $T^{1,q}$ 
  with a general  parameter 
$q$. We demonstrate that the resulting $T^{1,q}$ model is classically integrable, admitting a Lax representation. We  observe 
 that the $T^{1,q}$ model is self-dual  under T-duality in one  isometry direction, and argue that this  property 
forces it to be stable under the RG flow. 
We verify this fact  explicitly  by computing  the corresponding  2-loop RG flow of the two  coupling constants.

 \

A few concluding remarks  will be made in  Section \ref{2103CS}. 
Appendix \ref{2103A}  contains discussion of the integrability conditions for the $G^N$ model \rf{cou} relevant to this chapter. 
 The explicit formulae for the 2-loop $\beta$-functions of the $G\times G$ and $G\times G/H$ models used in this chapter, and their derivations, are presented in  Appendix \ref{2103B}.
  
 \
 
\noindent This chapter is based on the paper \cite{LT2103} and we closely follow the presentation there.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\texorpdfstring{$G\times G$}{GxG} models \la{2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As 
 mentioned  above, the  $G^N$ model \rf{cou} is  classically integrable for \textit{special} values of its couplings $(\rho_{ij}, k_i)$ satisfying certain polynomial relations, which originate from the  affine Gaudin  construction
 \cite{DLMV}. For such values of the couplings the model  admits a  Lax connection of the form
\be
L_+ = \a_i \,  J^{(i)}_+ \ , \qquad\qquad  L_- = \b_i  \, J^{(i)}_- \ , \la{Lan}
\ee
whose flatness condition, $F_{+-}(L) \equiv \del_+ L_- - \del_- L_+ + [L_+, L_-] =0$, is equivalent to the equations of motion
following from \rf{cou}.  Moreover, the affine Gaudin construction 
guarantees 
the existence of  an infinite tower of conserved,  commuting higher-spin charges 
\cite{LMV}, as reviewed above in Section \ref{agm}.

Below  we shall consider  the simplest $N=2$ case of  the $G^N$ model  \rf{cou} for a simple Lie group $G$.  
We shall parametrize the $2\times 2$ matrix $\rho_{ij}$ in \rf{cou} in terms of the 4 components $s,t,u,b$ as follows 
\begin{align} 
\L = -\ha \,\begin{pmatrix}
s & t+b \\ t-b& u
\end{pmatrix}_{ij} \, \Tr[ J^{(i)}_+ J^{(j)}_- ] + k_i  \, \L_{_{\rm WZ}}(g^{(i)}) \ . \la{par}
%\qquad  
%\rho_{ij} \equiv  \rh_{(ij)} + b_{[ij]}
%= \begin{pmatrix}
%s & t \\ t& u
%\end{pmatrix}
%% \ , \quad b_{mn} = 
%+ \begin{pmatrix}
%0& b\\ -b& 0
%\end{pmatrix} \ .
\end{align}
Then the  affine Gaudin condition for   integrability is the vanishing of  a  cubic polynomial \cite{DLMV,today},
\be
f(s,t,u,b ,k_1,k_2) \equiv -t \, (s+t)\, (t+u)+b^2\, (s+t+u)+t \, k_1\,  k_2 + b \, (u\,  k_1 - s\,  k_2) = 0  \la{cond} \ .
\ee

Let us  note that the 
affine Gaudin conditions for integrability 
(e.g.\ \rf{cond} in the $N=2$ case) are certainly sufficient for integrability. However, it is not  a priori  clear  if they are  necessary,  
  since there could also be integrable theories of the form \rf{cou} that are unrelated to the affine Gaudin  construction 
of   \cite{DLMV}.
In Appendix \ref{2103A} we   presented a  check that the condition \rf{cond} is also \textit{necessary} for the integrability
of the $G\times G$ model \rf{par},  assuming the natural ansatz \rf{Lan} for the corresponding  Lax connection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{RG flow in   \texorpdfstring{$G\times G$}{GxG} models}

The general $G^N$ model \rf{cou} has  global $(G_L)^N \times G_R$ symmetry acting as
\be
g^{(i)} \to u_L^{(i)} g^{(i)} u_R\ , \qquad\qquad   (u_L^{(i)}, u_R) \in (G_L)^N \times G_R \ . \la{GGs}
\ee
In fact,  \rf{cou} is  the most general 2-derivative  local Lagrangian  having  this symmetry. 
 This implies  that only $\rho_{ij}$ can  run  under the RG flow
(with the WZ parameters $k_i$  not renormalized as usual, since WZ terms do not have a local 2d representation that could be produced by the beta functions \eqref{BMT}).

Starting with the \sm couplings $(\GG_{mn},\BB_{mn})$   corresponding to the   $G \times G$ model 
\rf{par}   and  computing the 
corresponding 2-loop $\beta$-functions   in the \GB  scheme  \eqref{BMT}, 
we find  
\be\la{2c} \begin{aligned}
 & \qquad\qquad \ddt \rho_{ij}  = \a' \, \b_{ij}^{(1)} + \a'^2\,  \b_{ij}^{(2)} + \ldots \ , \\
 \b_{ij}^{(1)} = {}&{} \cgg \, F^{(4)}_{ij}(s,t,u,b ,k_1,k_2) \ ,  \qquad  
  \b_{ij}^{(2)} = {\rm c}_{_G}^2 \, (su-t^2)^{-5} \, F^{(9)}_{ij}(s,t,u,b ,k_1,k_2) \ , 
\end{aligned} \ee
where the matrices $F^{(4)}, F^{(9)}$ are  homogeneous polynomials of degrees 4 and 9 in their arguments 
and $\ccg$  is the dual Coxeter number of  the group $G$, as in  the PCM$_k$ case in \rf{Pkb}.
The   explicit  expressions 
for $F^{(4)}, F^{(9)}$
 are given in  Appendix \ref{2103GGapp}    and also in an example below.

Remarkably, despite the complicated   expressions  for the   $\beta$-functions,  one is able to verify   that 
  the integrability condition \rf{cond} is, in fact, preserved by the 2-loop RG flow:
\be { d f\ov d \tau} \Big|_{f=0} = \big( \a' \, \b_{ij}^{(1)} + \a'^2 \, \b_{ij}^{(2)} + ... \big) \, { \del f \ov \del {\rho_{ij}}  }\Big|_{f=0} = \a'\times 0+ \a'^2\times 0 + ... \ .  \la{GGstab}
\ee
The vanishing of the 1-loop $\O(\a')$ term in \rf{GGstab} was already established in \cite{today}, and the vanishing of the 2-loop 
 term is a  new  non-trivial  result. Let us stress   that 
 this property of 
 the integrability condition \rf{cond}
not being deformed  at the 2-loop level is specific to the 
  \GB   scheme \eqref{BMT}. 




\iffa

\subsubsection{\texorpdfstring{$\rho_{21}=0$}{rho_21=0} and the \texorpdfstring{$G\times G$}{GxG} model related to \texorpdfstring{$\l$}{lambda}-model}
The most general integrable model with $\rho_{21}=0$  corresponds to the  following choice  of the parameters in \rf{par}
(this case was also considered in Appendix C of \cite{today})
\be
b=t \ , \qquad u = -k_2 \ .
\ee 
After the redefinition $  (g^{(1)},g^{(2)})\equiv(g,\wt{g}^{-1})$, the corresponding Lagrangian \rf{par}  
depending on $s,t, k_1, k_2$ 
may be written as 
  (cf. \rf{Pk}) 
\begin{align}
\L ={} &\big[ s \L_{_{\rm PCM}}(g) +k_1  \L_{_{\rm WZ}}(g)\big]  -  k_2 \big[  \L_{_{\rm PCM}}(\wt g) + \L_{_{\rm WZ}}(\wt g)
\big]+ t \, \Tr
\big[ J_+(g) K_-(\wt g)\big]  \ , \la{1}
\end{align}
where 
$J= g^{-1} d g,   \  K(\wt g) = d \wt{g}\,  \wt{g}^{-1}$. 
This is   just a  PCM$_{k_1}$    and  WZW model (with level $-k_2$) 
 coupled  via   the $J_+(g) K_-(\wt g)$ term. 
In this case the global $G_R$ symmetry in \rf{GGs} is enlarged to a chiral symmetry  $G_R(\xi^+)$,\foot{We denote by $G(\xi^+)$  right $G$  multiplications 
 depending on  light-cone coordinate $\xi^+= \ha (\xi^0 + \xi^1)$.\la{chir}}
\be\la{29}
(g,\, \wt{g}) \to (u\, g\, v, \ v^{-1} \wt{g}\,  w(\xi^+)) \ , \qquad \qquad (u,v,w(\xi^+))\in G_L \times G_L \times G_R(\xi^+)   \ .
\ee
These   symmetries protect the structure of \rf{1}  under
 renormalization so  that only the parameters $s$ and $t$ are expected to run  with the RG scale.  Indeed,  in this case the RG equations  \rf{2c}  take the following explicit  form\foot{As in \rf{Pkb},   here we set 
the loop counting parameter $\a'$ to  be 1. 
The 1-loop terms in \rf{sr},\rf{tr} match those in \cite{today} (after  reversing the sign  of the WZ terms $k_i \to - k_i$  to match the conventions).}
\begin{align}
\ddt s {}&{}= \frac{\cgg\, (s-k_1)  }{\left(k_2 s+t^2\right)^2} \Big[k_2^2 (k_1+s)+4 k_2 t^2-2 t^3\Big] \no \\
&\quad + \frac{\cggg\, (s-k_1) }{2 \left(k_2 s+t^2\right)^5} \Big[ 2 k_2 t^5 \left(38 t^2-11 k_1t +2 s^2+41 s t\right) \la{sr} \\
&\quad %quad \qquad \qquad
 +2 k_2^3 t^3 \left(-8 k_1 s-42 k_1 t+9 k_1^2-5 s^2+18 s t\right) % \no\\
%&\qquad\qquad \qquad
  -2 k_2^2 t^4 \left(-7 k_1 s-46 k_1 t+s^2+48 s t+28 t^2\right)\no\\
&\quad %\qquad \qquad \qquad 
+k_2^5 (k_1+s) \left(s^2-3 k_1^2\right)+2 k_2^4 t^2 (3 k_1+2 s) (3 s-5 k_1)-4 t^7 (5 s+6 t)\Big]\no  \ , \\
\ddt t{}&{} =\frac{ \cgg\, t (t-k_2)  }{\left(k_2 s+t^2\right)^2} \Big[ k_2 (k_1-s)+2 t (s+t)\Big] \no \\
&\quad + \frac{\cggg\, t (t-k_2)}{2 \left(k_2 s+t^2\right)^5}  \Big[4 t^5 \left(t (4 t-k_1)+5 s^2+10 s t\right)-k_2^4 (s-k_1) \left(s^2-3 k_1^2\right)\la{tr} \\
&\quad %\qquad \qquad \qquad
+2 k_2^2 t^2 \left(s^2 (28 t-3 k_1)+2 s t (13 t-16 k_1)+6 k_1 t (k_1-4 t)+3 s^3\right)\no\\
&\quad %\qquad \qquad \qquad
-2 k_2 t^3 \left(-k_1 t (13 s+19 t)+2 s^3+31 s^2 t+45 s t^2+10 t^3\right) %\no\\
%&\quad %\qquad \qquad \qquad
-2 k_2^3 t (s-k_1) (5 s t-3 k_1 (s+4 t))\Big] \ . \no % \la{tr}
\end{align}
At the obvious  fixed point   $s=k_1, \ t= k_2$, the model  \rf{1}   becomes  \cite{today}  
the sum of two decoupled WZW models,
$\L = (k_1+k_2) \L_{_{\rm WZW}} (g) - k_2 \L_{_{\rm WZW}}(g \wt g)$.
 As discussed in \cite{today}, the fixed points are all decoupled WZW models of this type.
  The RG trajectories either interpolate between such WZW-type fixed points or 
flow to them in the IR from the  asymptotically free  UV fixed  point $s, t \to \infty$.

An  interesting  special case of \rf{1}  is $s=k_1=- k_2\equiv - k' $, when it becomes 
\be
\L =- k'  \Big(  \L_{_{\rm WZW}}(g)  + \L_{_{\rm WZW}}(\wt {g})  - \l' \, \Tr\big[ J_+(g)  K_-(\wt g)\big]  \Big)  \ , \qquad \quad  \l' \equiv k'^{-1}t \ .\la{212}
\ee 
This particular $G\times G$ model  appears from the ``tripled''  version \cite{HLT2} 
of the $\l$-model \ci{Sfetsos:2013wia,Hollowood:2014rla}
after removing the  decoupled WZW part.  It is also 
 a special case of the ``doubly $\l$-deformed'' model of \cite{sfetsos,Georgiou:2017aei,Georgiou:2017oly,Georgiou:2017jfi}. 
 Here  the  $\beta$-functions   \rf{sr},\rf{tr} reduce to just $\l'$ running as 
\be\la{213}
\ddt \l' = \frac{2\cgg\, \l'^2}{k' (1+\l')^2} + \frac{4{\rm c}^2_{_{G}}\,  \l'^4(1-2\l')}{k'^2 (1-\l')(1+\l')^5} \ .
\ee
This is the 2-loop $\beta$-function \cite{HLT2}
for the $\l$-model 
based on  
the group $G$ 
with  parameters $(k, \lambda)$  related to $(k',\l')$ as 
$k' =k+2 \cgg$, $\l' = \tfrac{k}{k+2\cgg}\l^{-1}$.\foot{See also \cite{s19}. For the 1-loop $\b$-functions of the $\l$-models based on $G$ and $G/H$, see \cite{Sfetsos:2014jfa} and \cite{Appadu:2015nfa} respectively.} 

\fi
\subsection{Example with \texorpdfstring{$k_1=k_2=0$}{k_1=k_2=0}  \la{sc}}
Let us consider the special case of the  integrable $G\times G$ models \rf{par},\rf{cond}
 with vanishing WZ levels, $k_1=k_2=0$.
  In that case 
 the integrability condition \rf{cond}  implies that 
\be \la{214}
b = b(s,t,u) \equiv \Big[{ t(t+s)(t+u)\ov t + s+u}\Big]^{1/2} \ . \ee
 We thus obtain 
 from  \rf{par} 
 an integrable  $G \times G$ model  with  3  independent couplings $s,t,u$,
\be
\L = -\tfrac{1}{2} \begin{pmatrix}
s & t+ b(s,t,u) \\
t- b(s,t,u) & u
\end{pmatrix}_{ij} \Tr[ J^{(i)}_+ J^{(j)}_- ]   \ .
\ \la{matb}
\ee
Since $k_i$  do not run, this special case of the model \rf{par},\rf{cond}  should also  be stable under the RG flow, i.e.\ 
\rf{matb}   should be renormalizable  with only $s,t,u$  running. 
 Indeed, 
using for convenience the redefined 
couplings  $(s,t,u)\to (x,y,z)$ with
 \be\la{216}
x = s+t+u \ , \qquad y = \frac{s}{t} \ , \qquad z = \frac{u}{t} \ ,\la{rc}
\ee
 the 2-loop $\beta$-functions \rf{2c}  become 
 \begin{align}
&\ddt x = 2 \cgg - \frac{ \cggg }{2 x (y z-1)^3} \  \Big[ 16 +32 (y + z) + 16 ( y^2 + z^2) + 88 y z + 68 y z (y+z)    \la{br1} \\
 & \qquad \qquad  \qquad \qquad \qquad\qquad + 12 y z (y^2+z^2 + 5 y z )   + 8 y^2 z^2 (y+z)    - y^2 z^2 (y +  z)^2  \Big]\ ,  \no\\
%\no \\
%& \qquad \qquad \qquad\qquad \ \ \  + y^2 (z^4-8 z^3-60z^2-68z -16)-4 y (z+1) (z+4) (3 z+2)\Big]\ ,  \la{br1}\\
&\ddt y =F(x;y,z)\ , \qquad \qquad \ddt z = F(x;z,y) \ , \la{218} \\
&F(x;y,z)\equiv  \frac{  \, y  (y+1) (y+2) }{ \,  (zy-1)^2} \ \bigg(  \frac{ \cgg}{x} \big[ 1-zy- 3(z+1)^2 \big]   \la{br3} \\
& \qquad \ \   %\qquad\qquad \quad \qquad
 -\frac{ \cggg}{2x^2} \frac{1}{ (z y-1)^3 }\Big[  -z^6 y^2- y^6 (3z  y-38z-44) %\no\\
%& \qquad\qquad \qquad \quad \qquad \qquad 
 +2 z (y+1) (26 zy+101y+58) \no \\
&\qquad\qquad \qquad  \qquad  \qquad \ \ \ +20 (y+1)^2 -z^4 (y (3 y ((y-14) y-100)-296)-38) \no\\ 
&\qquad\qquad \qquad  \qquad  \qquad \ \ \ -z^3 (y (y (y ((y-4) y-178)-728)-708)-152) \no\\
& \qquad\qquad \qquad \qquad   \qquad \ \ \  +2 z^2 (y+1) (y (y (5 y+89)+262)+105)  \Big] \bigg)\ .\no 
\end{align}
The obvious symmetry  between $s$ and $u$ in \rf{matb}  is  translated into  the symmetry of the RG equations under 
$y\leftrightarrow z$. 


The fact  that 
these 2-loop $\beta$-functions are much simpler than  
 the general (not necessarily integrable) case  of \rf{2c} 
 (see also  
 Appendix  \ref{2103GGapp}) 
 suggests that a   substantial simplification  happens 
 upon specifying the 
 couplings to be  at  the integrable locus $f=0$
 in 
  \rf{cond}
  (this   was already observed at the 1-loop order in \cite{today}).
  

\section{\texorpdfstring{$G\times G/H$}{GxG/H} models \la{gu}}

Let $H$ be a subgroup  of $G$ such  that $G/H$ is a symmetric space (we assume that both $G$ and $H$ are simple real Lie groups).  Then the 
 Lagrangian for the gauged $G\times G/H$ model  of \cite{ABL} takes the form\foot{Our conventions in 
\rf{couH} are related to the ones of  \cite{ABL}  by  $r_{ij} \to 2 \rho^{(0)}_{ij}$, $\rho_{ij} \to 2 \rho_{ij}^{(1)}$ and
 the  opposite sign  for 
the WZ terms, i.e. $k_i \to - k_i %^{\rm (ABL)}
$.}
\begin{align}
&\L = -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] -\ha \, r_{ij} \, \Tr[ \B^{(i)}_+ \B^{(j)}_- ] + k_i  \, \L_{_{\rm WZ}}(g^{(i)}) \ , \la{couH} \\
& P^{(i)} = P_{{G/H}}  J^{(i)} \ , \qquad   \B^{(i)} = P_H J^{(i)}\ ,  \ \ \qquad 
 J^{(i)} =  {g^{(i)}}^{-1} d g^{(i)}  \ . % \quad  (g^{(i)}) \in G^N  \ ,
  %\ \  i=1,2 \ ,
  \la{31}
\end{align}
Here  $P_{{G/H}}  $ and $P_H$ are projectors to the corresponding  parts of
 the algebra of $G$,   and 
$\r_{ij}$, $r_{ij}$ are  
 constant $2\times 2$ matrices.  
The global symmetry 
consists of 
 left multiplication $G_L\times G_L$, as well as the discrete  $\mathbb{Z}_2$  corresponding to
 the symmetric space structure of $G/H$.
The  action  for \rf{couH}
 is required  to be gauge invariant under the local  right action  by an element of $H$ (acting 
 the 
 same 
 on  both $g^{(i)}$) 
\be
g^{(i)} \to g^{(i)} \ww\ , \qquad \qquad  \ww(\xi^+, \xi^-)\in H \ .  \la{gI}
\ee
 For general choices of $G$ and $H$,  
   gauge invariance  imposes the 
   linear  
   constraints  \cite{ABL}\foot{The   special case of  abelian $H$   will be   
 discussed below in Section \ref{2103sq}.}
\be
 k_1 = - k_2\equiv k  \ , \qquad \qquad r_{ij} = \begin{pmatrix} r  & - r - k \\ -r +k & r  \end{pmatrix} \ . \la{bb1}
\ee
The remaining free parameters  of the gauge invariant model 
are then $r$, $k$ and  the $2\times 2$ matrix $\rho_{ij}$.

Requiring integrability imposes  further constraints  which,
as for the
$G^N$ models \rf{cou}, 
can be  obtained from the affine Gaudin  construction. 
The following parametrization of  the 6 constants $r,k, \rho_{ij}$ 
 in terms of   4 parameters $K,x,\z_+,\z_-$ was shown  in \cite{ABL} to be   sufficient for   integrability
\begin{align}
&r=r_{11} = r_{22} = K \frac{\z_-^2-\z_+^2}{(1-x^2)^2} \ , \ \ \qquad \qquad  r_{12} = 2K \frac{(1-\z_+^2)(x^2-\z_-^2)}{(1-x^2)^3}\ ,  \la{iH1}  \\
&r_{21} = -2K \frac{(1-\z_-^2)(x^2-\z_+^2)}{(1-x^2)^3} \ , \\
&\r_{11} = K\frac{1-2\z_+^2 +\z_-^2 \z_+^2}{(1-x^2)^2} \ , \ \ \qquad \qquad  \r_{12} = x \, r_{12}= 2 K \frac{x (1-\z_+^2)(x^2-\z_-^2)}{(1-x^2)^3} \ , \\
& \r_{21} = x^{-1} \, r_{21} = -2K \frac{(1-\z_-^2)(x^2-\z_+^2)}{x (1-x^2)^3}  \ , \qquad \qquad \r_{22} = K\frac{x^4-2\z_+^2 x^2 +\z_-^2 \z_+^2}{x^2(1-x^2)^2} \ , \\
&k=k_1 = -k_2 = - K \frac{2x^2 +2\z_-^2\z_+^2-(1+x^2)(\z_-^2+\z_+^2)}{(1-x^2)^3} \ . \la{iH4}
\end{align}
This parametrization  is simply equivalent to the gauge invariance conditions \rf{bb1} 
combined with the   two extra polynomial integrability conditions
\be \begin{aligned} 
f_1 \equiv {} &{} r^2 - k^2 - \r_{12} \r_{21}=0  \ , \\
 f_2 \equiv {}&{}  (r - k)^4  \r_{12} + (r - k)^2 (r -k -  2 \r_{11}) (r -k + 2 \r_{22})  \r_{21}    \\
&{} \qquad \qquad \ \ \ 
 - 2(r-k)   (\r_{11} + \r_{22})  \r_{12} \r_{21}^2 +  (\r_{12} +  \r_{21})\r_{12}  \r_{21}^3  =0   \ . 
\end{aligned}  \la{condH} \ee
Two  simple solutions of  these   conditions are found by setting 
 $r=k$ (i.e. $r_{21}=0$  in \rf{bb1})     and   
either 
    $\r_{21}=0$  or   $\r_{12}=0$.
    
We note that the integrable $G\times G/H$ models satisfying \rf{couH}\rf{bb1},\rf{couH}  were recently found  to be obtainable \cite{Fukushima:2021eni} from 4d Chern-Simons theory \cite{Costello:2019tri}.

\subsection{RG flow in  \texorpdfstring{$G\times G/H$}{GxG/H}  models}


The structure of the gauge invariant $G\times G/H$   action  \rf{couH},\rf{bb1} is protected 
by the  right $H$ gauge symmetry \rf{gI}  and the global $G_L\times G_L $ and  $\mathbb{Z}_2$ symmetry.
This rules out 
all
counterterms    
except those
  corresponding  to   renormalizations 
  of the 6 couplings $r,k,\rho_{ij}$ (of which $k$ is not renormalized as usual). 
Let us  parametrize $\rho_{ij}$ as in \rf{par},
\be\la{rrr}
\rho_{ij} = \begin{pmatrix}
s & t+b \\
t-b & u 
\end{pmatrix} \ .
\ee 
Computing the  $\beta$-functions \eqref{BMT} corresponding to the  \sm couplings $(\GG_{mn},\BB_{mn})$   for the model \rf{couH},\rf{bb1},\rf{rrr}, 
we find for  the 1-loop $\beta$-functions of the 5 running  couplings
\begin{align}
& \ddt \lh_p  = \a' \b_{\lh_p}^{(1)} \ , \qquad \qquad \lh_p\equiv (r,s,t,b,u) \ , \la{1H}  \\
&\b_r^{(1)} = \frac{\ccg- \ch}{(t^2 - s u)^2} \Big( r^2 s^2 - 2 b^2 t^2 - 2 r^2 t^2 + 2 t^4 -  2 b^2 s u - 2 s t^2 u + r^2 u^2 \\
   &\qquad \qquad \qquad \qquad + 4 b s t k + 4 b t u k - s^2 k^2 - 2 t^2 k^2 -  u^2 k^2 \Big) 
    + \ch \big(1-\tfrac{k^2}{r^2}\big) \ , \no \\
&\b_s^{(1)} = \frac{\ccg}{r (t^2 - s u)} \big[ b^2 s - s t^2 + r^2 u + 2 r (t^2 - s u) -  2 b t k + u k^2 \big]  \ , \\
  &\b_t^{(1)}= \frac{\ccg}{r (t^2 - s u)} \big[-b^2 t + b (s + u) k + t (r^2 - s u - k^2) \big] \ , \\
  & \b_b^{(1)} = \frac{\ccg}{r (t^2 - s u)} \big[-b (t^2 + s u) + t (s + u) k \big] \ , \\
  &\b_u^{(1)} =  \frac{\ccg}{r (t^2 - s u)} \big[ r^2 s + b^2 u - t^2 u + 2 r (t^2 - s u) - 2 b t k + s k^2 \big] \ . \la{fH}
\end{align}
 We observe   that the integrability conditions \rf{condH} are 
 stable under the 1-loop RG flow \rf{1H}--\rf{fH},
\be\la{317}
{d  f_a\ov d \tau} \Big|_{f_1=f_2=0} = \a'  \beta_{\lh_p} ^{(1)} {\del f_a\ov\del \lh_p} \Big|_{f_1=f_2=0} + \O(\a'^2)  = 0 + \O(\a'^2) \ , \qquad\qquad  a=1,2 \ .
\ee
However,  it turns out   that (as for   the  examples discussed in Chapter \ref{QCS})
 this property of RG stability does not automatically  extend to the 2-loop order. 
Computing the 2-loop $\beta$-functions  for the model \rf{couH},\rf{bb1} in the \GB scheme \eqref{BMT} (given explicitly in Appendix \ \ref{2103GGHapp}), 
we find that  
 the subleading correction to \rf{317} is non-zero at general values of the couplings, 
\be\la{318}
 \beta_{\lh_p} ^{(2)} {\del f_a\ov\del \lh_p} \Big|_{f_1=f_2=0} \not= 0\ ,  
 \qquad\qquad  a=1,2 \ .
\ee 
Moreover, we checked that 
 \rf{318} is also non-vanishing  in  
arbitrary  covariant  2-loop subtraction schemes.\foot{More precisely, we considered arbitrary subtraction schemes related to the \GB scheme \eqref{BMT} by covariant redefinitions of $\GG_{mn}$ and $\BB_{mn}$ (see Section \ref{SD}).} 


As in other examples \cite{HLT1,HLT2}, one may expect to restore the property of  RG stability at the 2-loop order by adding certain finite quantum $\a'$-corrections to the target space geometry.
Because of the global and local symmetries, the only possible corrections would 
correspond to   redefinitions  $\lh_p \to \bar \lh_p$  of the couplings  $\lh_p= (r,s,t,b,u)$,
\be 
 \lh_p=\bar  \lh_p + \a' Q_p(\bar \lh) + \ldots \   \ . \la{319}
 \ee
 Such redefinitions may be interpreted as quantum corrections to the integrability conditions \rf{condH}:
if  the original couplings  $\lh_p$ satisfied
 $f_a(\lh)=0$, then the corrected ones $\bar \lh_p$ would satisfy a \textit{corrected} version of the integrability conditions,
\be
\bar{f}_a(\bar \lh)   = 0\ , \qquad \bar{f_a} \equiv  f_a + \a'  \, Q_p \,  \del_{\lh_p} f_a   + \ldots \ \ .
\ee
 



\subsection{Example: integrable deformation of GMM model on \texorpdfstring{$G\times G/H$}{GxG/H}   and  \texorpdfstring{$T^{1,1}$}{T11} model \la{T11}}
There are still special exceptional cases of the integrable $G \times G/H$ model \rf{couH},\rf{bb1},\rf{condH}  that are automatically stable under  the  2-loop  RG flow 
in the \GB  scheme. As we shall demonstrate below, one of them is the
 particular solution  of the integrability conditions \rf{condH} that was studied in \cite{ABL}, 
\be \la{3244}
r=k\ , \qquad \qquad \r_{12}=\r_{21}=0  \ , \ \ \ {\rm i.e.} \ \  t=b=0 \ . \ee 
The Lagrangian of the corresponding theory \rf{couH},\rf{bb1} is given by 
\be \begin{aligned}
\L ={}&-\ha \, \Tr \big[ \rh \, P_+ P_-  + \wt{\rh} \,  \widetilde P_+ \widetilde P_- \big] -\ha k \, \Tr \big[ \B_+ \B_-  + \widetilde{\B}_+ \widetilde{\B}_-  -2 \B_+ \widetilde \B_- \big]  \\
&{}\quad + k \, \big[ \L_{_{\rm WZ}} (g)  - \L_{_{\rm WZ}} (\widetilde g) \big]  \la{3c}   \ , 
\end{aligned} \ee
where  we  have  set\foot{Ref. \cite{ABL}  used the notation $(k, \, \rh, \, \wt \rh) \equiv (\l^2, \, \l_2^2,  \, \l_1^2 )$.}
\be\la{3255} \begin{aligned}
  & (g^{(1)}, g^{(2)})\equiv (g,\wt g)\ , \quad  \wt P_\pm =  P_\pm (\wt g)\ , \quad  \wt \B_\pm =  \B_\pm (\wt g)\ , \\
 &  \rh\equiv \rho_{11}=s\ , \quad  \wt \rh\equiv\r_{22}=u \ . \end{aligned} \ee 
This is an integrable deformation of the special point $\rh=\wt \rh = k$ that corresponds to the conformal GMM model \ci{GMM} on the homogeneous space $G\times G/H$ with equal levels.

 Specializing the 1-loop   and 2-loop $\beta$-functions in \rf{1H}--\rf{fH} and   Appendix \ref{2103GGHapp} to this case, 
 we find that the model \rf{3c} is automatically stable  under 2-loop renormalization 
  with only $\rh$ and $\wt \rh$ running,
\be \la{bg} \begin{aligned}
& \ddt \rh = 2 \cgg \big(1- \tfrac{k}{ \rh}\big) \Big( 1 + \tfrac{ 1}{ \rh} \Big[ 2(\cgg-\ch) -  (3\cgg-2\ch) \tfrac{k}{\rh}\Big] \Big)  \ , \qquad \\
&\ddt \wt \rh = 2 \cgg (1- \tfrac{k}{ \wt \rh}\big)  \Big( 1 + \tfrac{ 1}{ \wt \rh} \Big[ 2(\cgg-\ch) -  (3\cgg-2\ch) \tfrac{k}{\wt \rh}\Big]\Big)  \ , \quad \qquad
\ddt k =0 \ .
\end{aligned} \ee
Remarkably, the RG evolution of $\rh$ and $\wh$  is  decoupled.  Note that the  structure of their   $\beta$-functions  is  similar to the  one in the PCM$_k$ case   \rf{Pkb}. 
As expected, the GMM model $\rh=\wh=k$ is a fixed point. 

 Let us consider  the  simplest  example of this theory  \rf{3c}   with  $G= SU(2) $ and $H=U(1)$  and   
choose the parametrization 
\be g=e^{\p_1 T_1} e^{\theta_1 T_2} e^{\psi T_3} \ , \qquad \qquad   \wt g=e^{-\p_2 T_1} e^{-\theta_2 T_2} e^{-\wt \psi T_3} 
 \ , \la{coo} \ee
 where the $SU(2)$ generators are 
$T_A = \tfrac{i}{2} \s_A$   
 and  the generator of  $H=U(1)$ 
  is  $T_3$. We shall fix the $H$ gauge freedom   by setting $\wt \psi=0$. As a result,   we get an integrable 
   5-dimensional \sm  (cf. \eqref{13})
  \begin{align}
\L ={} & (G_{mn} + B_{mn})  \del_+ x^m \del_- x^n 
=\tfrac{1}{4} k \, \Big[ \del_+ \psi \del_- \psi + \cos^2{\th_1} \, \del_+\p_1 \del_- \p_1 + \cos^2{\th_2} \, \del_+\p_2 \del_- \p_2 \no \\
&\qquad +  2  \cos{\th_1}\,  \del_+ \p_1 \del_- \psi + 2   \cos{\th_2}\,  \del_+\psi \del_- \p_2 + 2 \cos{\th_1}\cos{\th_2} \,  \del_+ \p_1 \del_- \p_2 \Big]   \la{mod}  \\
&\qquad  + \tfrac{1}{4} \rh\,  \big[ \del_+ \th_1 \del_- \th_1 + \sin^2{\th_1}\,  \del_+ \p_1 \del_- \p_1 \big]+ \tfrac{1}{4} \wh \, \big[ \del_+ \th_2 \del_- \th_2 + \sin^2{\th_2} \, \del_+ \p_2 \del_- \p_2  \big] \ . \no
  \end{align}
  The resulting  target space  geometry 
corresponds to 
 the  $T^{1,1}$  metric  
     and a  particular $B$-field \cite{ABL}\foot{Due to 
   differing conventions, the $B$-field here  is opposite in sign to that  in  \cite{ABL}.
   This difference is not significant, and can  be removed by a parity transformation.}
 \begin{align}
ds^2_{T^{1,1}} ={} & G_{mn} dx^m dx^n  = \tfrac{1}{4} k \,  (d\psi + \cos{\th_1} \, d\phi_1 + \cos{\th_2} \, d\phi_2)^2  \la{t11}  \\
 &\qquad \qquad \qquad\ \ + \tfrac{1}{4} \rh \, (d \th_1^2 + \sin^2{\th_1} \, d \p_1^2)+ \tfrac{1}{4} \wh \,  ( d  \th_2^2 + \sin^2{\th_2} \, d \p_2^2 )  \ ,  \no\\
 B ={}& \ha B_{mn} dx^m  \wedge dx^n 
  = \tfrac{1}{4} k \, (d\psi + \cos{\th_1} \, d\phi_1) \wedge (d\psi + \cos{\th_2} \, d\phi_2) \ . \la{b11}
\end{align}
The 3 parameters $\rh,\wt \rh, k$ of \rf{3c} are thus mapped to the 3 parameters of the $T^{1,1}$ metric  in    \cite{romans}. To recall, the $T^{1,1}$   metric 
\rf{t11} 
is
 an Einstein space 
 if $\rh=\wt \rh= {3\ov 2} k $. 
 It then serves  as a  base of a  Ricci flat 6d conifold  with metric $dr^2 + r^2 ds^2_{T^{1,1}}$ if we formally 
set 
$k=\tfrac{1}{9}$
 so that  $R_{ij} = 4 g_{ij}$. 
 In general, the non-zero components  of the  Ricci tensor of  the
 cone geometry 
 $ds^2= G_{mn}(X) dX^m dX^n= dr^2 + r^2  g_{ij}(x) dx^i dx^j$ (with $i=1, ..., d$) 
 are  ${R_{ij} (G)  = R_{ij} (g) -  (d-1) g_{ij}}$. Thus  it vanishes if $g_{ij}$ is an Einstein metric with a particular value of the scalar curvature 
 $R(g) = d (d-1)$ (this condition  is satisfied, e.g., for a unit-radius  sphere $S^d$  when  $G_{mn}$ is flat). 
 
 
For the integrable $T^{1,1}$ model \rf{mod}, the 2-loop  RG equations  \rf{bg} become (putting $ \cgg=2, \ \ch=0$)
\be \la{bet} \begin{aligned}
 \ddt \rh = 4 \big(1- \tfrac{k}{ \rh}\big) \big[ 1 + \tfrac{ 4}{ \rh} \big( 1 -  \tfrac{3\, k}{2\,  \rh}\big) \big]  \ , \qquad \qquad   \ 
&\ddt \wt h = 4 \big(1- \tfrac{k}{ \wt \rh}\big) \big[ 1 +  \tfrac{4 }{ \wt \rh} \big( 1 -  \tfrac{3\, k}{ 2\, \wt \rh}\big) \big]  \ .
\end{aligned} \ee
As we shall discuss in Section \ref{2103T}, the 2-loop RG stability of this  $T^{1,1}$ model  may be  understood 
 as  consequence 
of  the fact 
 that  the \sm \rf{mod} is self-dual  under T-duality  in the $\psi$-direction.

%%%%%%%%%%%%%%%%%%%

\section{Integrable \texorpdfstring{$T^{1,q}$}{T1q}  model \la{sq}}

Let us  now  introduce a new  integrable \sm  with  
target space metric 
 $T^{1,q}$
  and a particular $B$-field,  which is a
  one-parameter generalization of  the $T^{1,1}$ model \rf{mod} of \cite{ABL}. 
  Its   special  conformal  case will be the $SU(2) \times SU(2)/U(1)$  GMM  model, 
  now 
  with \textit{unequal}  
   WZ levels \ci{GMM,PZT} (with their ratio related to
  the parameter  $q$). 

Our central observation is that,  starting with the $G \times G/H$ model \rf{couH}  and considering 
the case   when  the subgroup $H$ is {\it abelian},  the gauge invariance condition \rf{bb1} of \cite{ABL}    is too restrictive.
 At the particular point $\rho_{12}=\rho_{21}=0$, there is also a second 
 ``branch'' 
 of gauge invariant  models,
\be
\begin{aligned}
&\L = -\ha \, \rho_{ij} \, \Tr[ P^{(i)}_+ P^{(j)}_- ] -\ha \, r_{ij} \, \Tr[ \B^{(i)}_+ \B^{(j)}_- ] + k_i  \, \L_{_{\rm WZ}}(g^{(i)}) \ ,
 \\
 &\rho_{12}=\rho_{21}=0 \ , \qquad r_{ij} = \begin{pmatrix} r  & q( - r - k_1) \\ q(-r +k_1) & q^2 r  \end{pmatrix} \  , \qquad q^2\equiv -k_2/k_1  \ , 
\end{aligned}
\la{bb2}
\ee
where $k_1$, $k_2$   are assumed to  be  of opposite sign. 
 The theory \rf{bb2} 
 is  invariant under a modified  gauge transformation
\be\la{42} 
(g^{(1)}, \, g^{(2)}) \to (g^{(1)} \ww^q , \,  g^{(2)} \ww) \ , \qquad \qquad  \ww=\ww(\xi^+, \xi^-)\in H \ .
\ee
Here $\ww^q$ is the  $q$-th power of the abelian  group element $\ww$.  
 In the case  when   the  abelian $H$  is compact
 then, 
to make   $\ww^q$   single-valued,  one  should  
 assume   that 
$q= \sqrt{ |{k_2\ov k_1}|}$ is an {integer}.\foot{More generally,  one could consider   a ``twisted'' action of the abelian subgroup, $(g^{(1)}, \, g^{(2)}) \to (g^{(1)} \ww^q , \,  g^{(2)} \ww^p)$  
characterized by integers $p,q$ satisfying $q^2/p^2=-k_2/k_1$.
In the $SU(2) \times SU(2)/U(1)$   example discussed below,   that would  lead to the  $T^{p,q}$  model.}
The reason for the 
  restriction of  $H$ to be abelian if $q\neq 1$ is that the  variation of the Lagrangian \rf{couH}  under \rf{42}  with 
 $\ww\in H$ will  be proportional to $(q-1)\L_{_{\rm WZ}}(\ww)$, which vanishes for abelian $H$   for any $q$. We also need to assume $\rho_{12} = \rho_{21}$ to prevent mixing between $P^{(1)}$ and $P^{(2)}$ terms, which are rotated differently  by $\ww^q$ and $\ww$ respectively.
At the value $q=1$  (i.e. $k_1=-k_2$),  this model 
 intersects with 
 the first ``branch'' of gauge-invariant $G\times G/H$ theories \rf{couH},\rf{bb1} considered above.
 
 Note that, in generic cases, WZ terms present a topological obstruction to gauging \cite{HS}. There are, however, special ``anomaly-free'' subgroups of the  WZ term's global symmetry $G_L\times G_R$ that can be gauged \cite{witten}, satisfying $\Tr_L[T_A T_B] - \Tr_R[T_A T_B] = 0$. This condition is satisfied here by the gauge transformations \rf{gI} and  \rf{42} on both ``branches'' of theories, due to cancellation between the two copies of $G$ in $G\times G/H$.
 
We 
claim 
that  model \rf{bb2} is integrable (admitting a Lax representation) 
 if\,\foot{The case $r=-k$ is also integrable since it is related to \rf{rk} by parity.}
 \be r=k  \ . \la{rk}
   \ee
 In this case it becomes a 
generalization of \rf{3c} to  
 the case of  
 unequal  levels $k,\wt k$,
\begin{align}
\hspace{-0.2cm}\L ={}&{}-\ha \, \Tr \big[ \rh \, P_+ P_-  + \wh \,  \widetilde P_+ \widetilde P_- \big]
-\ha  \, \Tr \big[ k\,  \B_+ \B_-  +  \wt k \, \widetilde{\B}_+ \widetilde{\B}_-  -2  \sqrt{k \wt k} \, \B_+ \widetilde \B_- \big]  \la{4c}  \\
&\quad  + k \L_{_{\rm WZ}} (g)   - \wt k  \L_{_{\rm WZ}} (\widetilde g)  \  ,\no \end{align}
where we have set (cf.  \rf{3255})
  \be \la{455}
    \begin{aligned}  &
    (g^{(1)}, g^{(2)})\equiv (g,\wt g)\ , \qquad  \wt P_\pm =  P_\pm (\wt g), \qquad   \wt \B_\pm =  \B_\pm 
  (\wt g),\ \\
& \rh\equiv \r_{11}, \qquad \wh\equiv \r_{22} \ , \qquad  k\equiv k_1, \quad \wt k \equiv - k_2 \ , \qquad 
q= \sqrt{ \tfrac{\wt k}{k}} \ .
 \end{aligned}\ee
 
 The fact that the $\wt k =k$ limit  \rf{3c}  is an integrable theory provides a first check of the integrability of \rf{4c}:
its Lax connection was obtained \cite{ABL} by taking the limit $r=k$, $\r_{12}=\r_{21}=0$ of the affine Gaudin Lax connection for the general  integrable $G\times G/H$ model \rf{couH},\rf{bb1},\rf{condH}.
 It was found   that certain components of the $\Lie(G)$-valued Lax connection degenerate to zero and thus the flatness condition  of the resulting 
 connection $L_\pm$ does not imply  all of the equations of motion.  
 However, one can  consider a generalized limiting procedure 
   by  infinitely rescaling  the spectral parameter while taking this limit, thus 
   obtaining a second  connection $\wt L_\pm$ that ``misses''  a different  subset of equations of motion. 
   The  flatness conditions of the two Lax connections   together  encode the full set of the equations
  of motion \cite{ABL},
  \begin{align}
&L_+(z) = \B_+ + z^{-1} P_+ \ ,\qquad  \ \ \  \ L_- (z) = \frac{1}{k z^2 - \rh} \Big[ (k-\rh)(\B_- + z P_-) + k (z^2-1) \wt \B_- \Big] \ ,\la{44}\\
&\wt L_-(z) = \wt \B_- + z \wt P_- \ , \quad  \ \ \ \,
\wt L_+(z) = \frac{1}{k z^{-2} - \wh} \Big[ (k-\wh)(\wt \B_+ + z^{-1} \wt P_+) + k (z^{-2}-1) \B_+ \Big]  \ .\la{45}
\end{align}
  The fact of having two separate Lax connections  may  seem   unusual but should be sufficient for the 
   integrability applications: for example, each Lax connection  will lead to its own family of conserved charges.
  They may also be regarded as a single   block-diagonal connection valued in $\Lie(G) \oplus \Lie(G)$. Indeed for $k=0$  the  two Lax connections \rf{44},\rf{45}  become the  familiar ones \eqref{sll}
    of the two decoupled  $G/H$ 
$\sigma$-models.\foot{I thank B. Hoare for this comment.}


We observe that the Lax connections \rf{44},\rf{45} naturally  generalize to the new model  \rf{4c} with unequal levels by replacing certain  factors of $k 
\to \wt k$,
\begin{align}
&L_+(z) = \B_+ + z^{-1} P_+ \ , \la{Lf}
\qquad   L_- (z) = \frac{1}{k z^2 - \rh} \Big[ (k-\rh)(\B_- + z P_-) +  \sqrt{k\wt k}(z^2-1) \wt \B_- \Big] \ ,\\
&\wt L_-(z) = \wt \B_- + z \wt P_- \ , \la{Ll} \ \ \,   
\wt L_+(z) = \frac{1}{\wt k z^{-2} - \wh} \Big[ (\wt k-\wh)(\wt \B_+ + z^{-1} \wt P_+) + \sqrt{k\wt k} (z^{-2}-1) \B_+ \Big]  \ .
\end{align}

 Assuming the  simplest case  $G=SU(2)$, $H=U(1)$, 
 using the same  coordinate parametrization of this $SU(2) \times SU(2)/U(1)$ model as in \rf{coo}, 
and  fixing again the  $H=U(1)$  gauge  as  $\wt \psi=0$,  we find the following generalization of \rf{mod}
 \begin{align}
\L ={} & (G_{mn} + B_{mn})  \del_+ x^m \del_- x^n 
=\tfrac{1}{4} k \, \Big[ \del_+ \psi \del_- \psi + \cos^2{\th_1} \, \del_+\p_1 \del_- \p_1 + q^2 \cos^2{\th_2} \, \del_+\p_2 \del_- \p_2 \no \\
&\qquad +  2  \cos{\th_1}\,  \del_+ \p_1 \del_- \psi + 2q   \cos{\th_2}\,  \del_+\psi \del_- \p_2 + 2q \cos{\th_1}\cos{\th_2} \,  \del_+ \p_1 \del_- \p_2 \Big]  \la{modq} \\
&+ \tfrac{1}{4} \rh\,  \big[ \del_+ \th_1 \del_- \th_1 + \sin^2{\th_1}\,  \del_+ \p_1 \del_- \p_1 \big]+ \tfrac{1}{4} \wh \, \big[ \del_+ \th_2 \del_- \th_2 + \sin^2{\th_2} \, \del_+ \p_2 \del_- \p_2  \big] \ , \qquad  q=\sqrt{\tfrac{\wt k}{k}} \  . \no 
  \end{align}
The resulting  target space metric is that of the $T^{1,q}$  space \cite{romans}
 and the $B$-field is a natural generalization of the one in \rf{b11},
\begin{align}
ds^2_{T^{1,q}} ={} & G_{mn} dx^m dx^n  = \tfrac{1}{4} k \,  (d\psi + \cos{\th_1} \, d\phi_1 +q \cos{\th_2} \, d\phi_2)^2  \la{gq}
\\
 &\qquad \qquad \qquad
 + \tfrac{1}{4} \rh \, (d \th_1^2 + \sin^2{\th_1} \, d \p_1^2)+ \tfrac{1}{4} \wh \,  ( d \th_2^2 + \sin^2{\th_2} \, d \p_2^2 )  \ , \no \\
 B ={}& \ha B_{mn} dx^m  \wedge dx^n 
  = \tfrac{1}{4} k \, (d\psi + \cos{\th_1} \, d\phi_1) \wedge (d\psi + q\cos{\th_2} \, d\phi_2) \ . \la{bq}
\end{align}
 Like the $q=1$   case \cite{ABL}  in \rf{mod}, 
       the   presence of  the $B$-field  is  crucial here for   integrability
(the $T^{1,q}$ \sm  without $B$-field  is not  integrable \cite{bpz,Basu:2011fw}).
The   coordinate form of the Lax connections \rf{Lf},\rf{Ll} is  ($T_A$ 
 are the $SU(2)$ generators  in \rf{coo}) 
\begin{align}
&{L'}_+(z) = \cos{\theta_1} \, \del_+ \phi_1 \, T_3 + z^{-1} \big( \del_+ \th_1  \, T_2 + \sin \th_1 \, \del_+ \p_1  \, T_1 \big) \ , \\
&{L'}_- (z) = \tfrac{1}{k z^2 - \rh} \Big[ (k-\rh)\big( \cos \th_1  \, \del_- \p_1  \, T_3 + z  ( \del_- \th_1  \, T_2 + \sin \th_1 \, \del_- \p_1  \, T_1 )   \big) \no  \\
&\qquad \qquad \qquad \qquad \qquad 
 - (z^2-1) \big( \sqrt{k \wt k}   \, \cos \th_2 \, \del_- \p_2 + k \,  \del_- \psi \big)  \Big]    \ ,  \no\\
 \ \no \\ 
&\wt L_+(z) = \tfrac{1}{\wt k z^{-2} - \wt h} \Big[ (\wt k-\wh)\big( - \cos \th_2  \, \del_- \p_2  \, T_3 + z^{-1}  ( - \del_+ \th_2  \, T_2 + \sin \th_3 \, \del_+ \p_3  \, T_1 )   \big)  \\
&\qquad \qquad \qquad \qquad \qquad \  + \sqrt{k\wt k} (z^{-2}-1)\big( \cos \th_1 \, \del_+ \p_1 + \del_+ \psi   \big)\Big]  \ , \no\\
&\wt L_-(z) =  - \cos{\theta_2} \, \del_- \phi_2 \, T_3 + z \big( - \del_- \th_2  \, T_2 + \sin \th_2 \, \del_- \p_2  \, T_1 \big)  \ .\no
\end{align}
To simplify the expressions   we followed   \cite{ABL}  here in   replacing $L_\pm $ by its gauge transformed   version 
 ${L'}_\pm = \ww^{-1} L_\pm \ww + \ww^{-1} \del_\pm \ww$,   with $\ww=\exp (- \psi T_3)$. 

At the special point 
 $\rh=k, \ \wh=\wt k= q^2 k $,  the model  \rf{modq} 
 becomes the $SU(2)\times SU(2)/U(1)$  case of the  conformal GMM   model  with   levels $k_1=k, \ k_2 =-\wt k$. 
 It was  pointed out in \cite{PZT} that the $SU(2)\times SU(2)/U(1)$  GMM model corresponds to the 
 $T^{1,q}$ 
  metric  and 
  a particular $B$-field,   and its 2-loop conformality was explicitly  checked (see also \ci{belo}). 
  The  general GMM model has a  current algebra  symmetry \cite{GMM} and is  also  integrable in the    Lax connection   sense  \cite{Bardakci:1996gs}.
 What we have shown above  is that 
  it   admits an  integrable extension \rf{modq} 
    away from the conformal point $\rh=k, \ \wh=\wt k$.
  

\subsection{Stability under the 2-loop RG flow}

Let us   now show   that the integrable  
$T^{1,q}$ model \rf{modq}   is  stable under the 2-loop RG flow. 

The general gauge invariant model \rf{bb2} (with the  $r=k$ 
condition   \rf{rk} relaxed) must be 
stable  under the RG   with  only $(r,\rh,\wt\rh)$   running,  due to  its $H$ gauge invariance and  global $G_L \times G_L$ symmetry. Even at the point $q=1$ or $\wt k = k$ where the two 
 ``branches'' 
 of gauge invariant theories \rf{bb2},\rf{bb1} intersect, the RG flow cannot `turn on' the extra couplings  
 $\r_{12}$, $\r_{21}$ since this is forbidden by an extra global ``center'' symmetry  \cite{romans, ABL},
$ (g,\, \widetilde g) \to (g\, z ,\, \widetilde g) , \   z\in 
{\rm Z}(H) 
 \subset H$  when $H$ is abelian.\foot{Note, however, that  the center symmetry alone is not sufficient to explain the stability of the $T^{1,q}$ model since it does not prevent $r$ from running.}


 We shall see that the integrable $T^{1,q}$ model, obtained by fixing $r=k$, is a ``fixed line'' of the RG flow.
Relaxing  $r=k$  has the effect of replacing $k\to r$ in the metric,\foot{It was recently argued by observing chaotic behaviour \cite{Ishii:2021asw} that relaxing the $r= k$ condition indeed destroys classical integrability, as  least in the equal level case $q=1$ (i.e.\ $\wt k =k$). This implies that, with $q=1$, the fixed line $r=k$ and its parity conjugate $r=-k$ are the only integrable models among the  $\s$-models on the class of backgrounds \rf{bQ2}.}
 with $k$ still appearing in the $B$-field (cf. \rf{gq},\rf{bq}),\foot{Rescaling $r\to  r' k  $  and $\psi\to { 1\ov \sqrt k   } \psi'$   the  background \rf{bQ2}  can be put into the  form 
    symmetric under 
   $k\leftrightarrow \wt k, \ \rh \leftrightarrow  \wt \rh$:
   
   $\qquad  \ ds^2  = \tfrac{1}{4} r' \,  (d\psi' + \sqrt k \cos{\th_1} \, d\phi_1 + \sqrt {\wt k}  \cos{\th_2} \, d\phi_2)^2 + %\la{gQ2}  % \\
%&\quad +
 \tfrac{1}{4} \rh \, (d \th_1^2 + \sin^2{\th_1} \, d \p_1^2)+ \tfrac{1}{4} \wh\,  (  d\th_2^2 + \sin^2{\th_2} \, d \p_2^2 )  \ , $
 \ \ 
 
 $
\qquad \ \ \    B = \tfrac{1}{4}  \, (d\psi' + \sqrt k \cos{\th_1} \, d\phi_1) \wedge (d\psi' + \sqrt {\wt k}  \cos{\th_2} \, d\phi_2) \ . $
   }
\begin{align}
ds^2  ={}& \tfrac{1}{4} r \,  (d\psi + \cos{\th_1} \, d\phi_1 + q \cos{\th_2} \, d\phi_2)^2 + %\la{gQ2}  % \\
%&\quad +
 \tfrac{1}{4} \rh \, (d \th_1^2 + \sin^2{\th_1} \, d \p_1^2)+ \tfrac{1}{4} \wh\,  (  d\th_2^2 + \sin^2{\th_2} \, d \p_2^2 )  \ \no ,\\
  \la{bQ2} B ={}& \tfrac{1}{4} k \, (d\psi + \cos{\th_1} \, d\phi_1) \wedge (d\psi + q \cos{\th_2} \, d\phi_2)  \ , \qquad \ \  q= \sqrt {\tfrac{\wt k}{ k} }\ .  
\end{align}
   The corresponding 
      2-loop  $\beta$-functions in the \GB scheme   following from \eqref{BMT}  are 
     ($k, \wt k$ do not run)
  \begin{align}
%&\ddt k =0 \ , \\
&\ddt r = 2(r^2-k^2) \Big[  \tfrac{1}{\rh^2 }  + 
\tfrac{\wt k}{k} \tfrac{1}{{\wt \rh}^2 }  + %\frac{1}{  \rh^2 {\wt \rh}^2 k r} 
  \tfrac{r^2-3 k^2}{ r } \big(\,  \tfrac{1}{\rh^4}  +   \tfrac{{\wt k}^2}{k^2} \tfrac{ 1}{\wt \rh^4}
  \big)\Big] \ ,\la{b3}\\
&\ddt \rh = 4\big[ 1 - \tfrac{r}{2\rh}(1+\tfrac{k^2}{r^2}) \big] %\no \\
%&\qquad \qquad 
+ \tfrac{2}{ \rh^3   r^2} \Big[   8 \rh^2 r^2     - 8 \rh k^2r  
  - 12  \rh r^3  + 4 r^2  k^2 +    3 k^4  + 5 r^4  \no  \\
 &\qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad  \qquad +   \tfrac{\wt k}{k}
  \tfrac{{\rh}^2}{\wt \rh^2} (r^2-k^2) (3r^2- k^2)   \Big] \ ,  \la{b4}  \\
&\ddt {\wt\rh} =  4\big[ 1- \tfrac{ \wt k}{k} \tfrac{ r }{{2\wt \rh  }}(1+\tfrac{k^2}{r^2})\big]  %\no  \\
%&\qquad \qquad
 +\tfrac{2 }{  {\wt \rh}^3  r^2}\Big[8  {\wt \rh}^2 r^2 -8 {\wt \rh}  {\wt k}k r -12 \tfrac{\wt k}{k}  {\wt \rh} r^3 
  + 4 r^2 {\wt k}^2  
 +3 {\wt k}^2 k^2+5 \tfrac{{\wt k}^2}{k^2} r^4   \no\\
&\qquad \qquad\qquad \qquad \qquad \qquad \qquad \qquad  \qquad +
  \tfrac{\wt k}{k} \tfrac{{\wt \rh}^2}{\rh^2}  (r^2-k^2) (3r^2- k^2) \Big] \ . \la{b5}
\end{align}
Thus   
$r=\pm k$  are fixed lines 
 of 
 \rf{b3}, 
both at 1-loop and 2-loop order. 
 The  couplings $(r,\rh,{\wt \rh})$ grow   linearly with $\tau\to \infty $ in the UV (reflecting asymptotic  freedom), 
 while they decrease to the GMM fixed point $(r,\rh,{\wt \rh}) = (k,k,\wt k)$ in the IR. In fact, as  argued in \cite{GMM}, the GMM model on $G\times G'/H$ is an exact CFT, 
assuming at least one of  the  cosets  $G/H$ or $G'/H$ is a symmetric space (as is indeed the case for 
 $SU(2) \times SU(2)/U(1)$).


Specialising to the fixed line $r=k$  of \rf{b3},  
 the expressions \rf{b4},\rf{b5}  simplify, giving  the 
 2-loop  $\beta$-functions  of  the  integrable $T^{1,q}$ model \rf{4c},\rf{modq},
\begin{align}
& 
\ddt \rh = 4 \big(1- \tfrac{k}{ \rh}\big) \Big[ 1 + \tfrac{ 4}{ \rh} \big( 1 -  \tfrac{3\,k}{ 2\,\rh}\big) \Big]  \ ,  %\no \\
 \qquad \qquad 
 \ddt \wt h = 4 \big(1- \tfrac{\wt k}{ \wt \rh}\big) \Big[ 1 +  \tfrac{4 }{ \wt \rh} \big( 1 - \tfrac{3\, \wt k}{ 2\, \wt \rh}\big) \Big]  
%\ddt k = \ddt \wt k  =0
\ .  \la{betq} 
\end{align}
These   are   a  natural generalization of the  $\beta$-functions  for the $T^{1,1}$ model     in \rf{bet} to the case of $\wt k \not= k$.
 Like  in \rf{bet}, the  RG evolution of $\rh$ and $\wh$  happens to be  decoupled (while
 this is  not the case for $r\not=k$
 in \rf{b4},\rf{b5}).


We note that,  in addition to  the $r=k$  case of the $T^{1,q}$ model, 
  the $\s$-model   corresponding to    \rf{bQ2} admits  \textit{another} integrable limit,
 $\wt k = 0$. 
 In this case it  factorizes  into 
 a squashed $S^3$   with  WZ  term    and a round $S^2$.
   The $\b$-functions
   \rf{b3} and \rf{b4} 
   become those of this
   squashed $S^3$  WZ-model  
 in
 \ci{shifman} (for 1-loop $\beta$-functions see   \ci{yosh,Demulder:2017zhz})\foot{The relation to the 
   notation used in  \ci{shifman} is 
   $\eta= k \rh^{-1}, \ \lambda^2= {2\pi}  \rh ^{-1} $, \ $ \kappa= 1 - r \rh^{-1} $. } and the 
    $\beta$-function \rf{b5} for  the  coefficient $\wt \rh$ becomes that of  the $S^2={SU(2) \ov U(1)}$
 $\s$-model (eq.\ \eqref{sb} with $\cgg=2, \ \ch=0$).
 Taking  further limits, the $\beta$-functions   \rf{b3},\rf{b4},\rf{b5} agree with  
 other  previously known expressions:
\begin{enumerate}[(i)]
\item   Setting  $\wt k=0$   
     and $r=\rh$, we get from \rf{bQ2}    
       the direct  sum of the  PCM$_k$  (round $S^3$ with a WZ term) 
 and the $S^2$  $\s$-model.  In this  case \rf{b3},\rf{b4} are  indeed equivalent to the $\b$-function 
 of PCM$_k$, i.e.  \rf{Pkb}  with $\cgg=2$. 
 
\item Setting  $\wt k = 0$ (i.e.\  $q=0$) 
   and  then   $k=0$, we 
   instead 
   get the  direct sum of a squashed $S^3$ (with no WZ term) and a round $S^2$.
    The  $\beta$-functions  for $r$ and $\rh$ agree with those of the   ``squashed'' PCM in  \cite{HLT2}  
  (with $G=SU(2)$ 
   and the  ``squashing'' parameter $\varepsilon= {r\ov \rh}$):
    
 \noindent
 $
 \qquad \ddt r = {2r^2 }{\rh^{-2} }    +  {r^3}{\rh^{-4}}  \ , \qquad
 \ddt \rh = 4\big( 1 - \tfrac{1}{2} r \rh^{-1} \big) + {2}{ \rh^{-3 } } \big(   8 \rh^2      
  - 12  \rh r   + 5 r^2 \big)  \ .
%\ddt {\wt\rh} =  4 + 16 \wt h^{-1}
$ 

\end{enumerate}
        
\subsection{Covariance under T-duality \la{T}}
One can argue that  the RG stability of the  integrable  $T^{1,q}$ model \rf{modq}, i.e.\ the presence of the fixed line $r=k$ of \rf{b3},   is related  to
its property of being  self-dual under T-duality in the isometric $\psi$-direction.
To see this, let us write the  Lagrangian \rf{modq}  
in the following form\foot{Note that  $ \widehat{\L}$
   becomes   simply quadratic in the fields 
 at the  GMM point $\rh=k,\  \wh= \wt k= q^2  k$. }
\begin{align}
&\L = \tfrac{1}{4} k \, \Big[ (\del_+ \psi +\ta_+) ( \del_- \psi + \tb_- ) - \ha \ta_+ \tb_-\Big]  + \widehat{\L}  \ , \la{413} \\
&\qquad \qquad  \ta_\pm \equiv   2\cos{\th_1}\, \del_\pm \phi_1\ , \qquad  \qquad   \tb_\pm\equiv   2 q \cos{\th_2}\, \del_\pm \phi_2\ ,   \la{notU}\\
&\widehat{\L} 
\equiv   
 \tfrac{1}{4}\rh  \Big[   \del_+ \th_1 \del_- \th_1 + (  \sin^2{\th_1}  + \tfrac{k }{\rh}  \cos^2{\th_1} )   \del_+ \p_1 \del_- \p_1 \Big]  
% +    \tfrac{1}{4}k \, \cos^2{\th_1} \, \del_+\p_1 \del_- \p_1 
 \la{mmm} \\ 
 &\qquad 
+  \tfrac{1}{4}  \wh  \Big[  \del_+ \th_2 \del_- \th_2 +  (  \sin^2{\th_2}   
+ \tfrac{k q^2}{\wh}  \cos^2{\th_2} )\, \del_+\p_2 \del_- \p_2 \Big]  \no\ . 
% \la{mmm}
  \end{align}
\sloppy
Starting from the interpolating Lagrangian (obtained by $\del_\pm \psi \to A_\pm$   and adding the condition ${\del_+ A_-  - \del_- A_+=0}$  with a  Lagrange multiplier $\bpsi$), 
\be
\L_{\rm int} =  \tfrac{1}{4} k \Big[ (A_+ + \ta_+) (A_- + \tb_- ) - \ha \ta_+ \tb_- - {\bpsi}(\del_+ A_-  - \del_- A_+) \Big] +  \widehat{\L}   \ , \la{int}
\ee
 and integrating out $A_\pm$, we obtain the  following  T-dual  Lagrangian 
\be\la{417}
\bar{\L} = \tfrac{1}{4}  k\Big[ (\del_+ \bpsi + \ta_+) ( \del_- \bpsi - \tb_- ) + \ha \ta_+ \tb_-\Big] + \widehat{\L} \ .
\ee
This  is the same  as
the original theory 
 \rf{413}, 
with $\psi \to \bpsi$ and a coordinate redefinition $\phi_2 \to -\phi_2$ (under which $\tb_- \to -\tb_-$). 


To appreciate  the special  structure of 
\rf{413},
   let us  relax the condition $r=k$ and go back to  the 
 general non-integrable  model \rf{bb2} 
  corresponding to the background \rf{bQ2}.
 Using again the notation \rf{notU}, 
  we find the following generalization of \rf{413}
 \begin{align} \la{m1}
\L = &\tfrac{r+k}{8} \Big[ (\del_+ \psi +\ta_+) ( \del_- \psi + \tb_- ) - \ha \ta_+ \tb_-\Big]   \\
&\qquad \qquad + \tfrac{r-k}{8} \Big[ (\del_- \psi +\ta_-) ( \del_+ \psi + \tb_+ ) - \ha \ta_- \tb_+\Big]   + \widehat \L \ . \no
\end{align}
Applying   the T-duality  $\psi\to \bpsi$  to \rf{m1} we get, instead of \rf{417},
\begin{align} \la{m2}
\bar \L ={} & \tfrac{1}{4} r \Big[ \Big (\del_+ \bpsi +\tfrac{r+k}{2r}\ta_+ + \tfrac{r-k}{2r}\tb_+ \Big) \Big(\del_- \bpsi - \tfrac{r-k}{2r}\ta_-  - \tfrac{r+k}{2r}\tb_- \Big) \\
 &\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad + \tfrac{r+k}{4r}\ta_+ \tb_- + \tfrac{r-k}{4r} \ta_- \tb_+ \Big] +  \widehat \L    \ .  \no
%\bar \L ={} & \tfrac{1}{4} r \Big[ \Big (\del_+ \bpsi + \ha (1+\tfrac{k}{r})a_+  + \ha (1-\tfrac{k}{r})b_+ \Big) \Big(\del_- \bpsi - \ha (1 -\tfrac{k}{r})a_-  - \ha (1+\tfrac{k}{r})b_- \Big)  \\
%& \qquad + \tfrac{1}{4}(1+\tfrac{k}{r})a_+ b_- + \tfrac{1}{4}(1-\tfrac{k}{r}) a_- b_+ \Big] +  \widehat \L  \no 
%
%\tfrac{r}{4}  \del_+ \bpsi \del_- \bpsi  + \tfrac{r+k}{8} \big( a_+  \del_- \bpsi  - b_-  \del_+ \bpsi )  -
%\tfrac{r-k}{8} \big( a_-  \del_+ \bpsi  
% + b_+  \del_- \bpsi )  \no \\
%& - \tfrac{r^2-k^2}{16r}\big( a_+ a_- -  b_+ b_-) - \tfrac{r+k}{16}\tfrac{k}{r}a_+ b_- -  \tfrac{r-k}{16}(2+\tfrac{k}{r})a_- b_+ + \widehat \L \  .
\end{align}
For  general values of $r$  and  $k$,  
\rf{m2} is different from  \rf{m1}; the only self-dual theory where  \rf{m1} and \rf{m2} coincide is the $T^{1,q}$ model  \rf{413} corresponding to $r=k$ (or its parity-conjugate $r=-k$). 

\sloppy
By the standard  path integral argument,  the  T-dual models \rf{m1},\rf{m2}   should be  quantum-equivalent. In general,  the 
  T-duality  transformation rules  are
   subject to quantum  $\a'$ corrections  \ci{Tseytlin:1991wr,Haagensen:1997er,Kaloper:1997ux}
    that may be attributed to extra  finite counterterms  resulting  from 
     integration over  the auxiliary gauge field $A_\pm$ (see eq.\ \eqref{7} above).  If
      the kinetic term of the  isometric coordinate  is non-trivial, i.e.\ 
      the
      term 
      quadratic in $A_\pm $ 
      is  $A_+ M(x) A_-$, then the leading  quantum correction to the effective Lagrangian 
      is represented by   the   term  $\Delta \L \sim \a' \, \del_+ \log M \, \del_- \log M$ (as well as a shift of the dilaton \ci{Buscher:1987qj,Schwarz:1992te}). 
     In the case of \rf{m1} we have $M=1$ and thus  this  correction  is absent.
     
Since the model  \rf{m1}  is stable
under the RG 
 due to its symmetries,  
 with  the 3  running couplings $r,\rh,\wt\rh$,  
its T-dual \rf{m2} must also be stable.
 Given that   the self-dual  points ${r=\pm k}$ are part of both RG-stable families 
 \rf{m1} and \rf{m2}  then they must also 
 remain in both families after the renormalization. Since they are the \textit{only} such self-dual  models, then $r=\pm k$ must be   fixed lines  of the RG flow.
     This   was  indeed  confirmed above 
     by the explicit computation of the $\beta$-functions  leading to 
    \rf{b3}.  
 
 
\section{Discussion \la{CS}}
%%%%%%%%%%%%%%%%%%%%%%

In this   chapter we discussed  further
 instances 
 of  a close connection    between 
the conditions of  integrability and  a  consistent restriction of the RG flow to a subspace of couplings. 

We have found the  2-loop  $\b$-functions of  the 6-parameter  $G \times G$ model \rf{par} 
and  have shown that  its integrability condition \rf{cond} is automatically preserved by the RG flow. 
 In \cite{today}, the 1-loop $\beta$-functions for this integrable 
   model were written in a universal form in terms of the twist function, revealing a hidden simplicity. 
   It would be  interesting to see if the complicated  expressions we have found 
   for the 2-loop $\b$-functions (see  Appendix \ref{2103GGapp}) 
simplify on the 
``integrable surface''
 once expressed in terms of the 
    twist function. Indeed, one may try to extend  the method of \cite{today} from 1-loop to 2-loop order, i.e.\  computing the Riemann tensor and thus the 2-loop  $\beta$-function in terms of the twist function. 
    It   would  also be interesting   to investigate  the connection  
    to  the ``doubled''  approach of   \cite{hassler}  which   studied the model \rf{par},\rf{cond}  with 
 additional  integrable $\eta$- or $\l$-deformation parameters   turned on.
  
 We   also studied  the  6-parameter gauged $G\times G/H$  model \rf{couH},\rf{bb1},
 which is integrable   under the conditions \rf{condH}. 
 The latter  were  found
  to be stable under the 1-loop  RG flow,  but generally require   a certain  deformation 
 (i.e.\ the addition of  finite counterterms)  at the 2-loop level
to preserve  renormalizability. 

 There are  still  some special cases   in which integrable $G\times G/H$  models
are automatically stable under the 2-loop RG flow. One simple example is  the $T^{1,1}$ model of \ci{ABL}. 
We also   constructed   a    new   class of integrable $G\times G/H$ models  \rf{4c} in the case  when the subgroup  $H$ 
is abelian (see \rf{bb2},\rf{rk},\rf{4c}). 
For $G=SU(2)$ and $ H=U(1)$,  this  led to 
 an integrable $T^{1,q}$ 
 model  generalizing  the  $T^{1,1}$ model, 
which   
we also found to be stable under the 2-loop  RG flow  
for general values of the parameter $q$. 
 This  model 
 may be interpreted as
an integrable  deformation of the 
conformal 
GMM model 
 with unequal levels  \ci{GMM}. 
An open question is whether the integrable $T^{1,q}$ model  admits a description in terms of affine Gaudin models (like the $T^{1,1}$ case) or if it is outside of that formalism. 
 
Since the GMM model  admits a  $G\times G'/H$   generalization (with $G\neq G'$),
this raises   the question of whether  there is a larger class of integrable  $G\times G'/H$ 
models that flow to 
such 
conformal 
theories. One obvious possibility is to   consider   some analytic continuations, e.g., 
 take  $G'$  to be a different  real form of the complexification of $G$.
  For example,   the  counterpart  of  the $SU(2)\times SU(2)/U(1)$ model 
 would be   $SL(2,\mathbb{R})\times SU(2)/U(1)$.\la{an}
 

Another interesting open question is why the integrable $G\times G$ model was automatically stable under the 2-loop RG flow, while the gauged $G\times G/H$ analog requires a non-trivial quantum deformation of the ``integrable surface'' in the space of couplings. This is analogous to WZW models, which are conformal without any $\a'$-corrections, and gauged WZW models, which require a non-trivial tower of $\a'$ corrections (e.g.\ in eq.\ \eqref{6}) to remain conformal beyond 1-loop.
One possible resolution, which we shall consider below in Section \ref{1910TO}, is to reformulate the $G\times G/H$ model as a theory with a gauge field and redefine the gauge field in terms of $H$-valued scalars; as for the ``tripled'' formulation of the  $\l$-model in Chapter \ref{CT}, such a reformulation could  
 restore higher-loop renormalizability without needing any quantum corrections to the geometry.



==> v arxiv v2/refs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{thebibliography}{999}
\renewcommand{\bibname}{References}
\addcontentsline{toc}{chapter}{\bibname}
%
%%%refs
%
%\cite{Hoare:2018jim}
\bibitem{HLTS}{
B.~Hoare, N.~Levine and A.~A.~Tseytlin,
``On the massless tree-level S-matrix in 2d sigma models,''
\doilink{J. Phys. A \textbf{52}, no.14, 144005 (2019)}{
doi:10.1088/1751-8121/ab0b79}
\arxivlink{1812.02549}.
%16 citations counted in INSPIRE as of 11 Jul 2021
%
%
}\bibitem{HLT1}{
B.~Hoare, N.~Levine and A.~A.~Tseytlin,
``Integrable 2d sigma models: quantum corrections to geometry from RG flow,''
\doilink{Nucl. Phys. B \textbf{949}, 114798 (2019)}{10.1016/j.nuclphysb.2019.114798}
\arxivlink{1907.04737}.
%
}\bibitem{HLT2}{
B.~Hoare, N.~Levine and A.~A.~Tseytlin,
``Integrable sigma models and 2-loop RG flow,''
\doilink{JHEP {\bf 1912}, 146 (2019)}{doi:10.1007/JHEP12(2019)146}
\arxivlink{1910.00397}.
%
%\cite{Hoare:2020fye}
}\bibitem{HLT2008}{
B.~Hoare, N.~Levine and A.~A.~Tseytlin,
``Sigma models with local couplings: a new integrability -- RG flow connection,''
\doilink{JHEP \textbf{11}, 020 (2020)}{10.1007/JHEP11(2020)020}
\arxivlink{2008.01112}.
%8 citations counted in INSPIRE as of 01 Jul 2021
%
%
%\cite{Levine:2021fof}
}\bibitem{LT2103}{
N.~Levine and A.~A.~Tseytlin,
``Integrability vs. RG flow in $G \times G$ and $G \times G /H$ sigma models,''
\doilink{JHEP \textbf{05}, 076 (2021)}{
doi:10.1007/JHEP05(2021)076}
\arxivlink{2103.10513}.
%3 citations counted in INSPIRE as of 11 Jul 2021
%
%
%
%
%
%
%
%\cite{Maldacena:1997re}
}
\bibitem{Maldacena:1997re}{
J.~M.~Maldacena,
``The Large N limit of superconformal field theories and supergravity,''
\doilink{Adv. Theor. Math. Phys. \textbf{2}, 231-252 (1998)}{10.1023/A:1026654312961}
\arxivlink{hep-th/9711200}.
%16616 citations counted in INSPIRE as of 13 May 2021
%
%\cite{Witten:1998qj}
}\bibitem{Witten:1998qj}{
E.~Witten,
``Anti-de Sitter space and holography,''
\doilink{Adv. Theor. Math. Phys. \textbf{2}, 253-291 (1998)}{10.4310/ATMP.1998.v2.n2.a2}
\arxivlink{hep-th/9802150}.
%10776 citations counted in INSPIRE as of 05 Jul 2021
%
%\cite{Gubser:1998bc}
}\bibitem{Gubser:1998bc}{
S.~S.~Gubser, I.~R.~Klebanov and A.~M.~Polyakov,
``Gauge theory correlators from noncritical string theory,''
\doilink{Phys. Lett. B \textbf{428}, 105-114 (1998)}{10.1016/S0370-2693(98)00377-3}
\arxivlink{hep-th/9802109}.
%9133 citations counted in INSPIRE as of 05 Jul 2021
%
%
%%\cite{Metsaev:1998it}
}\bibitem{Metsaev:1998it}{
R.~R.~Metsaev and A.~A.~Tseytlin,
``Type IIB superstring action in AdS(5) x S**5 background,''
\doilink{Nucl. Phys. B \textbf{533}, 109-126 (1998)}{
doi:10.1016/S0550-3213(98)00570-7}
\arxivlink{hep-th/9805028}.
%%763 citations counted in INSPIRE as of 13 May 2021
%%
%%\cite{Bena:2003wd}
}
\bibitem{Bena:2003wd}{
I.~Bena, J.~Polchinski and R.~Roiban,
``Hidden symmetries of the AdS(5) x S**5 superstring,''
\doilink{Phys. Rev. D \textbf{69}, 046002 (2004)}{
doi:10.1103/PhysRevD.69.046002}
\arxivlink{hep-th/0305116}.
%925 citations counted in INSPIRE as of 13 May 2021
%
%\cite{Das:2004hy}
}\bibitem{Das:2004hy}{
A.~K.~Das, J.~Maharana, A.~Melikyan and M.~Sato,
``The algebra of transition matrices for the AdS(5) x S**5 superstring,''
\doilink{JHEP \textbf{12}, 055 (2004)}{
doi:10.1088/1126-6708/2004/12/055}
\arxivlink{hep-th/0411200}.
%72 citations counted in INSPIRE as of 13 May 2021
%
%\cite{Young:2005jv}
}\bibitem{Tseytlin:1988rr}{
A.~A.~Tseytlin,
``Sigma model approach to string theory,''
\doilink{Int. J. Mod. Phys. A \textbf{4}, 1257 (1989)}{
doi:10.1142/S0217751X8900056X}.
}\bibitem{Young:2005jv}{
C.~A.~S.~Young,
``Non-local charges, Z(m) gradings and coset space actions,''
\doilink{Phys. Lett. B \textbf{632}, 559-565 (2006)}{doi:10.1016/j.physletb.2005.10.090}
\arxivlink{hep-th/0503008}.
%
%\cite{Magro:2008dv}
}\bibitem{Magro:2008dv}{
M.~Magro,
``The classical exchange algebra of AdS(5) x S**5,''
\doilink{JHEP \textbf{01}, 021 (2009)}{
doi:10.1088/1126-6708/2009/01/021}
\arxivlink{0810.4136}.
%41 citations counted in INSPIRE as of 01 Jun 2021
%
%\cite{Vicedo:2009sn}
}\bibitem{Vicedo:2009sn}{
B.~Vicedo,
``Hamiltonian dynamics and the hidden symmetries of the AdS(5) x S**5 superstring,''
\doilink{JHEP \textbf{01}, 102 (2010)}{
doi:10.1007/JHEP01(2010)102}
\arxivlink{0910.0221}.
%29 citations counted in INSPIRE as of 01 Jun 2021
%
%
%
%\cite{Zamolodchikov:1989cf}
}\bibitem{ZTBA}{
A.~B.~Zamolodchikov,
``Thermodynamic Bethe Ansatz in relativistic models. Scaling three state Potts and Lee-Yang models,''
\doilink{Nucl. Phys. B \textbf{342}, 695-720 (1990)}
{doi:10.1016/0550-3213(90)90333-9}.
%642 citations counted in INSPIRE as of 02 Jul 2021
%
%\cite{Yang:1968rm}
}\bibitem{YTBA}{
C.~N.~Yang and C.~P.~Yang,
``Thermodynamics of one-dimensional system of bosons with repulsive delta function interaction,''
\doilink{J. Math. Phys. \textbf{10}, 1115-1122 (1969)}{
doi:10.1063/1.1664947}.
%585 citations counted in INSPIRE as of 02 Jul 2021
%
%\cite{Gromov:2013pga}
}\bibitem{Gromov:2013pga}{
N.~Gromov, V.~Kazakov, S.~Leurent and D.~Volin,
``Quantum spectral curve for Planar $\mathcal{N} = 4$ super-Yang-Mills theory,''
\doilink{Phys. Rev. Lett. \textbf{112}, no.1, 011602 (2014)}{
doi:10.1103/PhysRevLett.112.011602}
\arxivlink{1305.1939}.
%238 citations counted in INSPIRE as of 05 Jul 2021
%
%\cite{Levkovich-Maslyuk:2019awk}
}\bibitem{Levkovich-Maslyuk:2019awk}{
F.~Levkovich-Maslyuk,
``A review of the AdS/CFT Quantum Spectral Curve,''
\doilink{J. Phys. A \textbf{53}, no.28, 283004 (2020)}{
doi:10.1088/1751-8121/ab7137}
\arxivlink{1911.13065}.
%6 citations counted in INSPIRE as of 05 Jul 2021
%
%\cite{Minahan:2002ve}
}\bibitem{Minahan:2002ve}{
J.~A.~Minahan and K.~Zarembo,
``The Bethe ansatz for N=4 superYang-Mills,''
\doilink{JHEP \textbf{03}, 013 (2003)}{
doi:10.1088/1126-6708/2003/03/013}
\arxivlink{hep-th/0212208}.\\
%1317 citations counted in INSPIRE as of 01 Jun 2021
%\cite{Beisert:2003yb}
%}\bibitem{Beisert:2003yb}
%
N.~Beisert and M.~Staudacher,
``The N=4 SYM integrable super spin chain,''
\doilink{Nucl. Phys. B \textbf{670}, 439-463 (2003)}{
doi:10.1016/j.nuclphysb.2003.08.015}
\arxivlink{hep-th/0307042}.
%684 citations counted in INSPIRE as of 02 Jul 2021
%
%\cite{Beisert:2003tq}
}\bibitem{BeisertHL}{
N.~Beisert, C.~Kristjansen and M.~Staudacher,
``The Dilatation operator of conformal N=4 superYang-Mills theory,''
\doilink{Nucl. Phys. B \textbf{664}, 131-184 (2003)}{
doi:10.1016/S0550-3213(03)00406-1}
\arxivlink{hep-th/0303060}.
%714 citations counted in INSPIRE as of 02 Jul 2021
%\cite{Beisert:2005fw}
}\bibitem{BeisertBA}{
N.~Beisert and M.~Staudacher,
``Long-range psu(2,2|4) Bethe Ansatze for gauge theory and strings,''
\doilink{Nucl. Phys. B \textbf{727}, 1-62 (2005)}{
doi:10.1016/j.nuclphysb.2005.06.038}
\arxivlink{hep-th/0504190}.
%620 citations counted in INSPIRE as of 02 Jul 2021
%
%\cite{Beisert:2005tm}
}\bibitem{BeisertS}{
N.~Beisert,
``The SU(2|2) dynamic S-matrix,''
\doilink{Adv. Theor. Math. Phys. \textbf{12}, 945-979 (2008)}{
doi:10.4310/ATMP.2008.v12.n5.a1}
\arxivlink{hep-th/0511082}.
%641 citations counted in INSPIRE as of 02 Jul 2021
%
%
%\cite{Eden:2012fe}
}\bibitem{Eden:2012fe}{
B.~Eden, P.~Heslop, G.~P.~Korchemsky, V.~A.~Smirnov and E.~Sokatchev,
``Five-loop Konishi in N=4 SYM,''
\doilink{Nucl. Phys. B \textbf{862}, 123-166 (2012)}{
doi:10.1016/j.nuclphysb.2012.04.015}
\arxivlink{1202.5733}.\\
%54 citations counted in INSPIRE as of 05 Jul 2021
%%\cite{Gromov:2015dfa}
%}\bibitem{Gromov:2015dfa}
%
N.~Gromov and F.~Levkovich-Maslyuk,
``Quantum Spectral Curve for a cusped Wilson line in $ \mathcal{N}=4 $ SYM,''
\doilink{JHEP \textbf{04}, 134 (2016)}{
doi:10.1007/JHEP04(2016)134}
\arxivlink{1510.02098}.
%72 citations counted in INSPIRE as of 05 Jul 2021
%\cite{Lovelace:1983yv}
}\bibitem{Lovelace:1983yv}{
C.~Lovelace,
``Strings in curved space,''
\doilink{Phys. Lett. B \textbf{135}, 75-77 (1984)}{
doi:10.1016/0370-2693(84)90456-8}.\\
%400 citations counted in INSPIRE as of 05 Jul 2021
%\cite{Candelas:1985en}
%}\bibitem{Candelas:1985en}
P.~Candelas, G.~T.~Horowitz, A.~Strominger and E.~Witten,
``Vacuum configurations for superstrings,''
\doilink{Nucl. Phys. B \textbf{258}, 46-74 (1985)}{
doi:10.1016/0550-3213(85)90602-9}.\\
%2870 citations counted in INSPIRE as of 05 Jul 2021
%
%\cite{Sen:1985eb}
%}\bibitem{Sen:1985eb}
A.~Sen,
``The heterotic string in arbitrary background field,''
\doilink{Phys. Rev. D \textbf{32}, 2102 (1985)}{
doi:10.1103/PhysRevD.32.2102}.\\
%427 citations counted in INSPIRE as of 05 Jul 2021
%\cite{Callan:1985ia}
%}\bibitem{Callan:1985ia}
C.~G.~Callan, Jr., E.~J.~Martinec, M.~J.~Perry and D.~Friedan,
``Strings in background fields,''
\doilink{Nucl. Phys. B \textbf{262}, 593-609 (1985)}{
doi:10.1016/0550-3213(85)90506-1}.
%1779 citations counted in INSPIRE as of 05 Jul 2021
%
}\bibitem{kdv}{
C.~S.~Gardner, J.~M.~Greene, M.~D.~Kruskal and R.~M.~Miura,
``Method for solving the Korteweg-deVries equation,''
\doilink{Phys.\ Rev.\ Lett.\ 19(19), 1095 (1967)}{10.1103/PhysRevLett.19.1095}.
%
}\bibitem{lax}{
P.~D.~Lax,
``Integrals of nonlinear equations of evolution and solitary waves,''
\doilink{Commun. Pure Appl. Math. \textbf{21}, 467-490 (1968)}{10.1002/cpa.3160210503}.
%365 citations counted in INSPIRE as of 29 Jul 2021
%
%
}\bibitem{zs}{
V.~E.~E.~Zakharov and A.~B.~Shabat,
 ``Exact theory of two-dimensional self-focusing and one-dimensional self-modulation of waves in nonlinear media,''
  Soviet physics JETP, 34(1), 62 (1972);
``A scheme for integrating the nonlinear equations of mathematical physics by the method of the inverse scattering problem. I,''
\doilink{Functional Analysis and Its Applications 8(3), 226-235 (1974)}{10.1007/BF01075696};
``Integration of nonlinear equations of mathematical physics by the method of inverse scattering. II,''
\doilink{Functional Analysis and Its Applications, 13(3), 166-174 (1979)}{10.1007/BF01077483}.
%
%\cite{Zakharov:1973pp}
}\bibitem{zm}{
V.~E.~Zakharov and A.~V.~Mikhailov,
``Relativistically invariant two-dimensional models in field theory integrable by the inverse problem technique. (In Russian),''
Sov. Phys. JETP \textbf{47}, 1017-1027 (1978).
%398 citations counted in INSPIRE as of 05 Jul 2021
%
%\cite{Bernard:1990jw}
}\bibitem{Bernard:1990jw}{
D.~Bernard,
``Hidden Yangians in 2-D massive current algebras,''
\doilink{Commun. Math. Phys. \textbf{137}, 191-208 (1991)}{
doi:10.1007/BF02099123}.
%115 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Eichenherr:1979ci}
}\bibitem{Eichenherr:1979ci}{
H.~Eichenherr and M.~Forger,
``On the dual symmetry of the nonlinear sigma models,''
\doilink{Nucl. Phys. B \textbf{155}, 381-393 (1979)}{
doi:10.1016/0550-3213(79)90276-1}.
%237 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Luscher:1977rq}
}\bibitem{lp}{
M.~Luscher and K.~Pohlmeyer,
``Scattering of massless lumps and nonlocal charges in the two-dimensional classical nonlinear sigma Model,''
\doilink{Nucl. Phys. B \textbf{137}, 46-54 (1978)}{
doi:10.1016/0550-3213(78)90049-4}.\\
%318 citations counted in INSPIRE as of 06 Jul 2021
%\cite{Pohlmeyer:1975nb}
%}\bibitem{Pohlmeyer:1975nb}
%
K.~Pohlmeyer,
``Integrable Hamiltonian systems and interactions through quadratic constraints,''
\doilink{Commun. Math. Phys. \textbf{46}, 207-221 (1976)}{
doi:10.1007/BF01609119}.
%628 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Alvarez:1994dn}
}\bibitem{Alvarez:1994dn}{
E.~Alvarez, L.~Alvarez-Gaume and Y.~Lozano,
``An introduction to T duality in string theory,''
\doilink{Nucl. Phys. B Proc. Suppl. \textbf{41}, 1-20 (1995)}{
doi:10.1016/0920-5632(95)00429-D}
\arxivlink{hep-th/9410237}.
%260 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Buscher:1987sk}
%}\bibitem{Buscher:1987sk}{
%T.~H.~Buscher:
%``A symmetry of the string background field equations,''
%\doilink{Phys. Lett. B \textbf{194}, 59-62 (1987)}{
%doi:10.1016/0370-2693(87)90769-6};
%%898 citations counted in INSPIRE as of 06 Jul 2021
%%\cite{Buscher:1987qj}
%%}\bibitem{Buscher:1987qj}
%%T.~H.~Buscher,
%``Path Integral Derivation of Quantum Duality in Nonlinear Sigma Models,''
%\doilink{Phys. Lett. B \textbf{201}, 466-472 (1988)}{
%doi:10.1016/0370-2693(88)90602-8}.
%%918 citations counted in INSPIRE as of 06 Jul 2021
%%
%%
%%\cite{delaOssa:1992vci}
}\bibitem{delaOssa:1992vci}{
X.~C.~de la Ossa and F.~Quevedo,
``Duality symmetries from nonAbelian isometries in string theory,''
\doilink{Nucl. Phys. B \textbf{403}, 377-394 (1993)}{
doi:10.1016/0550-3213(93)90041-M}
\arxivlink{hep-th/9210021}.
%311 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Wess:1971yu}
}\bibitem{Wess:1971yu}{
J.~Wess and B.~Zumino,
``Consequences of anomalous Ward identities,''
\doilink{Phys. Lett. B \textbf{37}, 95-97 (1971)}{
doi:10.1016/0370-2693(71)90582-X}.
%2832 citations counted in INSPIRE as of 06 Jul 2021
%
}\bibitem{novikov}{
 S. P. Novikov, 
 ``Multivalued Functions and Functionals. An Analogue of the Morse Theory,''
Dokl. Akad. Nauk SSSR Sect. Matem. 260, 31 (1981).
%
%}\bibitem{Witten:1983ar}
%E.~Witten,
%``Nonabelian Bosonization in Two-Dimensions,''
%Commun. Math. Phys. \textbf{92}, 455-472 (1984)
%doi:10.1007/BF01215276
%%2136 citations counted in INSPIRE as of 06 Jul 2021
%
%
%\cite{Piette:1987bt}
}\bibitem{cherednik}{
I.~V.~Cherednik,
``Integrability of the equation of a two-dimesional asymmetric $O(3)$ field and of its quantum analog,''
Yad. Fiz. \textbf{33}, 278 (1981) [Sov. J. Nucl. Phys. \textbf{33}, 144 (1981)].
}\bibitem{Piette:1987bt}{
B.~Piette, R.~A.~Zait and W.~J.~Zakrzewski,
``Solutions of the U(n) sigma models with the Wess-Zumino term,''
Z. Phys. C \textbf{39}, 359 (1988),
DTP-87/33.
%2 citations counted in INSPIRE as of 06 Jul 2021
%
%
%\cite{Knizhnik:1984nr}
}\bibitem{Knizhnik:1984nr}{
V.~G.~Knizhnik and A.~B.~Zamolodchikov,
``Current algebra and Wess-Zumino model in two-dimensions,''
\doilink{Nucl. Phys. B \textbf{247}, 83-103 (1984)}{
doi:10.1016/0550-3213(84)90374-2}.
%1533 citations counted in INSPIRE as of 06 Jul 2021
%
%
}\bibitem{Polyakov:1983tt}{
A.~M.~Polyakov and P.~B.~Wiegmann,
``Theory of nonabelian Goldstone bosons,''
\doilink{Phys.\ Lett.\ B {\bf 131}, 121 (1983)}{10.1016/0370-2693(83)91104-8}.
%%CITATION = doi:10.1016/0370-2693(83)91104-8;%%
%
%\cite{Polyakov:1984et}
}\bibitem{Polyakov:1984et}{
A.~M.~Polyakov and P.~B.~Wiegmann,
``Goldstone fields in two-dimensions with multivalued actions,''
\doilink{Phys. Lett. B \textbf{141}, 223-228 (1984)}{
doi:10.1016/0370-2693(84)90206-5}.
%429 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Goddard:1984vk}
}\bibitem{Goddard:1984vk}{
P.~Goddard, A.~Kent and D.~I.~Olive,
``Virasoro algebras and coset space models,''
\doilink{Phys. Lett. B \textbf{152}, 88-92 (1985)}{
doi:10.1016/0370-2693(85)91145-1}.
%752 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Frishman:1992mr}
}\bibitem{Frishman:1992mr}{
Y.~Frishman and J.~Sonnenschein,
``Bosonization and QCD in two-dimensions,''
\doilink{Phys. Rept. \textbf{223}, 309-348 (1993)}{
doi:10.1016/0370-1573(93)90145-4}
\arxivlink{hep-th/9207017}.\\
%78 citations counted in INSPIRE as of 06 Jul 2021
%
P.~Bowcock,
``Canonical quantization of the gauged {Wess-Zumino} model,''
\doilink{Nucl. Phys. B \textbf{316}, 80-100 (1989)}{
doi:10.1016/0550-3213(89)90387-8}.\\
%84 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Gawedzki:1988nj}
%}\bibitem{Gawedzki:1988nj}
K.~Gawedzki and A.~Kupiainen,
``Coset construction from functional integrals,''
\doilink{Nucl. Phys. B \textbf{320}, 625-668 (1989)}{
doi:10.1016/0550-3213(89)90015-1}.
%\\
%321 citations counted in INSPIRE as of 06 Jul 2021
%
%\cite{Karabali:1988au}
%}\bibitem{Karabali:1988au}
%D.~Karabali, Q.~H.~Park, H.~J.~Schnitzer and Z.~Yang,
%``A GKO construction based on a path integral formulation of gauged Wess-Zumino-Witten actions,''
%\doilink{Phys. Lett. B \textbf{216}, 307-312 (1989)}{
%doi:10.1016/0370-2693(89)91120-9}.
%241 citations counted in INSPIRE as of 06 Jul 2021
%
%
%
}\bibitem{Delduc:2017fib}{
F.~Delduc, B.~Hoare, T.~Kameyama and M.~Magro,
``Combining the bi-Yang-Baxter deformation, the Wess-Zumino term and TsT transformations in one integrable $\sigma$-model,''
\doilink{JHEP \textbf{10}, 212 (2017)}{
doi:10.1007/JHEP10(2017)212}
\arxivlink{1707.08371}.
%34 citations counted in INSPIRE as of 06 Jul 2021
%
%
%
%%\cite{Demulder:2017zhz}
%}\bibitem{Demulder:2017zhz}
%S.~Demulder, S.~Driezen, A.~Sevrin and D.~C.~Thompson,
%``Classical and Quantum Aspects of Yang-Baxter Wess-Zumino Models,''
%JHEP \textbf{03}, 041 (2018)
%doi:10.1007/JHEP03(2018)041
%[arXiv:1711.00084 [hep-th]].
%%31 citations counted in INSPIRE as of 07 Jul 2021
%
%\cite{Delduc:2016ihq}
}\bibitem{Delduc:2016ihq}{
F.~Delduc, S.~Lacroix, M.~Magro and B.~Vicedo,
``On q-deformed symmetries as Poisson\textendash{}Lie symmetries and application to Yang\textendash{}Baxter type models,''
\doilink{J. Phys. A \textbf{49}, no.41, 415402 (2016)}{
doi:10.1088/1751-8113/49/41/415402}
\arxivlink{1606.01712}.
%23 citations counted in INSPIRE as of 07 Jul 2021
%
%\cite{Delduc:2014kha}
}\bibitem{Delduc:2014kha}{
F.~Delduc, M.~Magro and B.~Vicedo,
``Derivation of the action and symmetries of the $q$-deformed $AdS_{5} \times S^{5}$ superstring,''
\doilink{JHEP \textbf{10}, 132 (2014)}{
doi:10.1007/JHEP10(2014)132}
\arxivlink{1406.6286}.
%143 citations counted in INSPIRE as of 08 Jul 2021
%
%
%\cite{
}\bibitem{Arutyunov:2015qva}{
G.~Arutyunov, R.~Borsato and S.~Frolov,
``Puzzles of $\eta$-deformed AdS$_5 \times$ S$^5$,''
\doilink{JHEP \textbf{12}, 049 (2015)}{
doi:10.1007/JHEP12(2015)049}
\arxivlink{1507.04239}.
%97 citations counted in INSPIRE as of 08 Jul 2021
%
%\cite{Arutyunov:2015mqj}
}\bibitem{Arutyunov:2015mqj}{
G.~Arutyunov, S.~Frolov, B.~Hoare, R.~Roiban and A.~A.~Tseytlin,
``Scale invariance of the $\eta$-deformed $AdS_5\times S^5$ superstring, T-duality and modified type II equations,''
\doilink{Nucl. Phys. B \textbf{903}, 262-303 (2016)}{
doi:10.1016/j.nuclphysb.2015.12.012}
\arxivlink{1511.05795}.
%138 citations counted in INSPIRE as of 08 Jul 2021
%
%
}\bibitem{etaspec}{
G.~Arutyunov, M.~de Leeuw and S.~J.~van Tongeren,
``The exact spectrum and mirror duality of the $(\text{AdS}_5{\times}S^5)_\eta$ superstring,''
\doilink{Theor. Math. Phys. \textbf{182}, no.1, 23-51 (2015)}{10.1007/s11232-015-0243-9} \arxivlink{1403.6104}.\\
%89 citations counted in INSPIRE as of 17 Oct 2020
%
R.~Klabbers and S.~J.~van Tongeren,
``Quantum Spectral Curve for the eta-deformed AdS$_5$xS$^5$ superstring,''
\doilink{Nucl. Phys. B \textbf{925}, 252-318 (2017)}{10.1016/j.nuclphysb.2017.10.005}
\arxivlink{1708.02894}.
%
%
%
}\bibitem{Parke:1980ki}{
S.~J.~Parke,
``Absence of particle production and factorization of the $S$ matrix in (1+1)-dimensional models,''
\doilink{Nucl. Phys. B \textbf{174}, 166-182 (1980)}{
doi:10.1016/0550-3213(80)90196-0}.
%62 citations counted in INSPIRE as of 08 Jul 2021
%
%\cite{}
}\bibitem{Zamolodchikov:1978xm}{
A.~B.~Zamolodchikov and A.~B.~Zamolodchikov,
``Factorized S matrices in two-dimensions as the exact solutions of certain relativistic quantum field models,''
\doilink{Annals Phys. \textbf{120}, 253-291 (1979)}{
doi:10.1016/0003-4916(79)90391-9}.
%1464 citations counted in INSPIRE as of 08 Jul 2021
%
%
%\cite{Polyakov:1977vm}
}\bibitem{Polyakov:1977vm}{
A.~M.~Polyakov,
``Hidden symmetry of the two-dimensional chiral fields,''
\doilink{Phys. Lett. B \textbf{72}, 224-226 (1977)}{
doi:10.1016/0370-2693(77)90707-9}.
%124 citations counted in INSPIRE as of 16 Jul 2021
%
%\cite{Luscher:1977uq}
}\bibitem{Luscher:1977uq}{
M.~Luscher,
``Quantum nonlocal charges and absence of particle production in the two-dimensional nonlinear sigma model,''
\doilink{Nucl. Phys. B \textbf{135}, 1-19 (1978)}{
doi:10.1016/0550-3213(78)90211-0}.
%283 citations counted in INSPIRE as of 16 Jul 2021
%
%\cite{Dorey:1996gd}
}\bibitem{Dorey:1996gd}{
P.~Dorey,
``Exact S matrices,''
\arxivlink{hep-th/9810026}.
%126 citations counted in INSPIRE as of 08 Jul 2021
%
%\cite{Wiegmann:1984pw} %all pcm
}\bibitem{Wiegmann:1984pw}{
P.~B.~Wiegmann,
``On the theory of nonabelian Goldstone bosons in two-dimensions: exact solution of the SU(N)xSU(n) nonlinear $\sigma$ model,''
\doilink{Phys. Lett. B \textbf{141}, 217 (1984)}{
doi:10.1016/0370-2693(84)90205-3}.\\
%
%
%112 citations counted in INSPIRE as of 08 Jul 2021
%\cite{Wiegmann:1984ec}
%}\bibitem{Wiegmann:1984ec}
P.~Wiegmann,
``Exact factorizaed S-matrix of the chiral field in two dimensions,''
\doilink{Phys. Lett. B \textbf{142}, 173-176 (1984)}{
doi:10.1016/0370-2693(84)91256-5}.
%88 citations counted in INSPIRE as of 08 Jul 2021
%
%
%\cite{Fateev:1994ai}
}\bibitem{Fateev:1994ai}{
V.~A.~Fateev, V.~A.~Kazakov and P.~B.~Wiegmann,
``Principal chiral field at large N,''
\doilink{Nucl. Phys. B \textbf{424}, 505-520 (1994)}{
doi:10.1016/0550-3213(94)90405-7}
\arxivlink{hep-th/9403099}.
%61 citations counted in INSPIRE as of 08 Jul 2021
%
%
%
%
%%\cite{Beisert:2010kk}
}\bibitem{qds}{
%\cite{Beisert:2008tw}
%}\bibitem{Beisert:2008tw}
N.~Beisert and P.~Koroteev,
``Quantum deformations of the one-dimensional Hubbard model,''
\doilink{J. Phys. A \textbf{41}, 255204 (2008)}{
doi:10.1088/1751-8113/41/25/255204}
\arxivlink{0802.0777}.\\
%118 citations counted in INSPIRE as of 08 Jul 2021
%
N.~Beisert,
``The classical trigonometric r-matrix for the quantum-deformed Hubbard chain,''
\doilink{J. Phys. A \textbf{44}, 265202 (2011)}{
doi:10.1088/1751-8113/44/26/265202}
\arxivlink{1002.1097}.\\
%37 citations counted in INSPIRE as of 08 Jul 2021
%
%\cite{Hoare:2011wr}
%}\bibitem{Hoare:2011wr}
B.~Hoare, T.~J.~Hollowood and J.~L.~Miramontes,
``q-deformation of the $AdS_5 x S^5$ superstring S-matrix and its relativistic limit,''
\doilink{JHEP \textbf{03}, 015 (2012)}{
doi:10.1007/JHEP03(2012)015}
\arxivlink{1112.4485}.
%71 citations counted in INSPIRE as of 08 Jul 2021
%
%
%\cite{Seibold:2020ywq}
}\bibitem{ses}{
F.~K.~Seibold, S.~J.~Van Tongeren and Y.~Zimmermann,
``The twisted story of worldsheet scattering in $\eta$-deformed $AdS_5 \times S^5$,''
\doilink{JHEP \textbf{12}, 043 (2020)}{
doi:10.1007/JHEP12(2020)043}
\arxivlink{2007.09136}.\\
%4 citations counted in INSPIRE as of 08 Jul 2021
%
%\cite{Bocconcello:2020qkt}
%}\bibitem{Bocconcello:2020qkt}
M.~Bocconcello, I.~Masuda, F.~K.~Seibold and A.~Sfondrini,
``S matrix for a three-parameter integrable deformation of AdS$_{3} \times$  S$^{3}$ strings,''
\doilink{JHEP \textbf{11}, 022 (2020)}{
doi:10.1007/JHEP11(2020)022}
\arxivlink{2008.07603}.
%3 citations counted in INSPIRE as of 08 Jul 2021
% 
%
}\bibitem{Vicedo:2017cge}{
B.~Vicedo,
``On integrable field theories as dihedral affine Gaudin models,''
\doilink{Int. Math. Res. Not. \textbf{2020}, no.15, 4513-4601 (2020)}{
doi:10.1093/imrn/rny128}
\arxivlink{1701.04856}.
%34 citations counted in INSPIRE as of 09 Jul 2021}
%14 citations counted in INSPIRE as of 09 Jul 2021
%
%\cite{Lacroix:2018njs}
}\bibitem{Lacroix:2018njs}{
S.~Lacroix,
``Integrable models with twist function and affine Gaudin models,''
\arxivlink{1809.06811}.
%9 citations counted in INSPIRE as of 09 Jul 2021
%
%
%\cite{Lacroix:2020flf}
}\bibitem{Lacroix:2020flf}{
S.~Lacroix and B.~Vicedo,
``Integrable $\mathcal{E}$-models, 4d Chern-Simons theory and affine Gaudin models. I.~Lagrangian aspects,''
\doilink{SIGMA \textbf{17}, 058 (2021)}{
doi:10.3842/SIGMA.2021.058}
\arxivlink{2011.13809}.
%8 citations counted in INSPIRE as of 09 Jul 2021
%
%\cite{Vicedo:2019dej}
}\bibitem{Vicedo:2019dej}{
B.~Vicedo,
``Holomorphic Chern-Simons theory and affine Gaudin models,''
\arxivlink{1908.07511}.
%22 citations counted in INSPIRE as of 09 Jul 2021
%
%
%%\cite{Delduc:2016ihq}
%}\bibitem{Delduc:2016ihq}
%F.~Delduc, S.~Lacroix, M.~Magro and B.~Vicedo,
%``On q-deformed symmetries as Poisson\textendash{}Lie symmetries and application to Yang\textendash{}Baxter type models,''
%J. Phys. A \textbf{49}, no.41, 415402 (2016)
%doi:10.1088/1751-8113/49/41/415402
%[arXiv:1606.01712 [hep-th]].
%%23 citations counted in INSPIRE as of 09 Jul 2021
%
%
%\cite{Sfetsos:1996xj}
}\bibitem{Sfetsos:1996xj}{
K.~Sfetsos,
``Poisson-Lie T duality and supersymmetry,''
\doilink{Nucl. Phys. B Proc. Suppl. \textbf{56}, 302-309 (1997)}{
doi:10.1016/S0920-5632(97)00339-3}
\arxivlink{hep-th/9611199}.
%45 citations counted in INSPIRE as of 12 Jul 2021
%
%
%
%%\cite{Wulff:2016tju}
}\bibitem{Wulff:2016tju}{
L.~Wulff and A.~A.~Tseytlin,
``Kappa-symmetry of superstring sigma model and generalized 10d supergravity equations,''
\doilink{JHEP \textbf{06}, 174 (2016)}{
doi:10.1007/JHEP06(2016)174}
\arxivlink{1605.04884}.
%114 citations counted in INSPIRE as of 13 Jul 2021
%
%\cite{Bassi:2019aaf}
}\bibitem{Bassi:2019aaf}{
C.~Bassi and S.~Lacroix,
``Integrable deformations of coupled $\sigma$-models,''
\doilink{JHEP \textbf{05}, 059 (2020)}{
doi:10.1007/JHEP05(2020)059}
\arxivlink{1912.06157}.
%15 citations counted in INSPIRE as of 14 Jul 2021
%
%
%%\cite{Hoare:2010fb}
%}\bibitem{Hoare:2010fb}
%B.~Hoare and A.~A.~Tseytlin,
%``On the perturbative S-matrix of generalized sine-Gordon models,''
%JHEP \textbf{11}, 111 (2010)
%doi:10.1007/JHEP11(2010)111
%[arXiv:1008.4914 [hep-th]].
%%27 citations counted in INSPIRE as of 15 Jul 2021
%
%
%\cite{Coleman:1973ci}
}\bibitem{Coleman:1973ci}{
S.~R.~Coleman,
``There are no Goldstone bosons in two-dimensions,''
\doilink{Commun. Math. Phys. \textbf{31}, 259-264 (1973)}{
doi:10.1007/BF01646487}.
%1025 citations counted in INSPIRE as of 15 Jul 2021
%
}\bibitem{Zamolodchikov:1992zr}{
A.~B.~Zamolodchikov and A.~B.~Zamolodchikov,
``Massless factorized scattering and \sms with topological terms,''
\doilink{Nucl.\ Phys.\ B {\bf 379}, 602 (1992)}{10.1016/0550-3213(92)90136-Y}.\\
%
%doi:10.1016/0550-3213(92)90136-Y
%%CITATION = doi:10.1016/0550-3213(92)90136-Y;%%
P.~Fendley and H.~Saleur,
``Massless integrable quantum field theories and massless scattering in (1+1)-dimensions,''
\arxivlink{hep-th/9310058}.
%%CITATION = HEP-TH/9310058;%%
%
}\bibitem{Nappi:1979ig}{C.~R.~Nappi,
``Some properties of an analog of the nonlinear $\sigma$ model,''
\doilink{Phys.\ Rev.\ D {\bf 21}, 418 (1980)}{doi:10.1103/PhysRevD.21.418}.\\
%%CITATION = doi:10.1103/PhysRevD.21.418;%%
F.~E.~Figueirido,
``Particle creation in a conformally invariant supersymmetric model,''
\doilink{Phys.\ Lett.\ B {\bf 227}, 392 (1989)}{
doi:10.1016/0370-2693(89)90949-0}.
%%CITATION = doi:10.1016/0370-2693(89)90949-0;%%
}\bibitem{Wulff}{
L.~Wulff,
``Condition on Ramond-Ramond fluxes for factorization of worldsheet scattering in anti\textendash{}de Sitter space,''
\doilink{Phys. Rev. D \textbf{96}, no.10, 101901 (2017)}{
doi:10.1103/PhysRevD.96.101901}
\arxivlink{1708.09673};
%14 citations counted in INSPIRE as of 15 Jul 2021
``Classifying integrable symmetric space strings via factorized scattering,''
\doilink{JHEP \textbf{02}, 106 (2018)}{
doi:10.1007/JHEP02(2018)106}
\arxivlink{1711.00296};
%10 citations counted in INSPIRE as of 15 Jul 2021
%L.~Wulff,
``Constraining integrable AdS/CFT with factorized scattering,''
\doilink{JHEP \textbf{04}, 133 (2019)}{
doi:10.1007/JHEP04(2019)133}
\arxivlink{1903.08660}.
%11 citations counted in INSPIRE as of 15 Jul 2021
%
%\cite{Berenstein:2002jq}
}\bibitem{BMN}{
D.~E.~Berenstein, J.~M.~Maldacena and H.~S.~Nastase,
``Strings in flat space and pp waves from N=4 superYang-Mills,''
\doilink{JHEP \textbf{04}, 013 (2002)}{
doi:10.1088/1126-6708/2002/04/013}
\arxivlink{hep-th/0202021}.
%1849 citations counted in INSPIRE as of 15 Jul 2021
%
%\cite{Gubser:2002tv}
}\bibitem{Gubser:2002tv}{
S.~S.~Gubser, I.~R.~Klebanov and A.~M.~Polyakov,
``A semiclassical limit of the gauge / string correspondence,''
\doilink{Nucl. Phys. B \textbf{636}, 99-114 (2002)}{
doi:10.1016/S0550-3213(02)00373-5}
\arxivlink{hep-th/0204051}.
%1013 citations counted in INSPIRE as of 15 Jul 2021
%
%\cite{Kruczenski:2002fb}
}\bibitem{Kruczenski}{
M.~Kruczenski,
``A Note on twist two operators in N=4 SYM and Wilson loops in Minkowski signature,''
\doilink{JHEP \textbf{12}, 024 (2002)}{
doi:10.1088/1126-6708/2002/12/024}
\arxivlink{hep-th/0210115}.
%200 citations counted in INSPIRE as of 15 Jul 2021
%
M.~Kruczenski, R.~Roiban, A.~Tirziu and A.~A.~Tseytlin,
``Strong-coupling expansion of cusp anomaly and gluon amplitudes from quantum open strings in AdS(5) x S**5,''
\doilink{Nucl. Phys. B \textbf{791}, 93-124 (2008)}{
doi:10.1016/j.nuclphysb.2007.09.005}
\arxivlink{0707.4254}.
%107 citations counted in INSPIRE as of 15 Jul 2021
%
%
}\bibitem{Dubovsky}{
S.~Dubovsky, R.~Flauger and V.~Gorbenko,
``Effective string theory revisited,''
\doilink{JHEP {\bf 1209}, 044 (2012)}{
doi:10.1007/JHEP09(2012)044}
\arxivlink{1203.1054};
%%CITATION = doi:10.1007/JHEP09(2012)044;%%
%S.~Dubovsky, R.~Flauger and V.~Gorbenko,
``Solving the simplest theory of quantum gravity,''
\doilink{JHEP {\bf 1209}, 133 (2012)}{
doi:10.1007/JHEP09(2012)133}
\arxivlink{1205.6805}.\\
%%CITATION = doi:10.1007/JHEP09(2012)133;%%
%
%}\bibitem{Cooper:2014noa}
 P.~Cooper, S.~Dubovsky, V.~Gorbenko, A.~Mohsen and S.~Storace,
``Looking for integrability on the worldsheet of confining strings,''
\doilink{JHEP {\bf 1504}, 127 (2015)}{
doi:10.1007/JHEP04(2015)127}
\arxivlink{1411.0703}.
%%CITATION = doi:10.1007/JHEP04(2015)127;%%
%
}\bibitem{Fradkin:1985ys}{
E.~S.~Fradkin and A.~A.~Tseytlin,
``Quantum string theory effective action,''
\doilink{Nucl. Phys. B \textbf{261}, 1-27 (1985)}{doi:10.1016/0550-3213(85)90559-0} 
Erratum: [Nucl. Phys. B \textbf{269}, 745-745 (1986)].
%doi:10.1016/0550-3213(85)90559-0
%850 citations counted in INSPIRE as of 16 Jul 2021
%
%%\cite{Borsato:2016ose}
%}\bibitem{Borsato:2016ose}
%R.~Borsato and L.~Wulff,
%``Target space supergeometry of $\eta$ and $\lambda$-deformed strings,''
%JHEP \textbf{10}, 045 (2016)
%doi:10.1007/JHEP10(2016)045
%[arXiv:1608.03570 [hep-th]].
%%98 citations counted in INSPIRE as of 16 Jul 2021
%
%\cite{Gross:1986iv}
}\bibitem{Gross:1986iv}{
D.~J.~Gross and E.~Witten,
``Superstring modifications of Einstein's equations,''
\doilink{Nucl. Phys. B \textbf{277}, 1 (1986)}{
doi:10.1016/0550-3213(86)90429-3}.
%862 citations counted in INSPIRE as of 16 Jul 2021
%
%\cite{Roiban:2007jf}
}\bibitem{Roiban:2007jf}{
R.~Roiban, A.~Tirziu and A.~A.~Tseytlin,
``Two-loop world-sheet corrections in AdS(5) x S**5 superstring,''
\doilink{JHEP \textbf{07}, 056 (2007)}{
doi:10.1088/1126-6708/2007/07/056}
\arxivlink{0704.3638}.
%119 citations counted in INSPIRE as of 16 Jul 2021
%
%\cite{Valent:1984rj}
}\bibitem{Valent:1984rj}{
G.~Valent,
``Perturbative renormalization of the CP(N) model,''
\doilink{Nucl. Phys. B \textbf{238}, 142-166 (1984)}{
doi:10.1016/0550-3213(84)90470-X}.\\
%14 citations counted in INSPIRE as of 16 Jul 2021
%
%}\bibitem{Hikami:1979ih}
S.~Hikami,
``Renormalization group functions of {CP}$^{N-1}$ nonlinear sigma model and $N$ component scalar {QED} model,''
\doilink{Prog. Theor. Phys. \textbf{62}, 226 (1979)}{
doi:10.1143/PTP.62.226}.
%50 citations counted in INSPIRE as of 16 Jul 2021
%
%
%\cite{Rosenhaus:2019utc}
}\bibitem{Rosenhaus:2019utc}{
V.~Rosenhaus and M.~Smolkin,
``Integrability and renormalization under $T \bar T$,''
\doilink{Phys. Rev. D \textbf{102}, no.6, 065009 (2020)}{
doi:10.1103/PhysRevD.102.065009}
\arxivlink{1909.02640}.
%23 citations counted in INSPIRE as of 24 Jul 2021
%
%\cite{Zamolodchikov:2004ce}
}\bibitem{TTbar}{
A.~B.~Zamolodchikov,
``Expectation value of composite field T anti-T in two-dimensional quantum field theory,''
\arxivlink{hep-th/0401146}.\\
%187 citations counted in INSPIRE as of 24 Jul 202
%\cite{Cavaglia:2016oda}
%}\bibitem{Cavaglia:2016oda}
%
A.~Cavagli\`a, S.~Negro, I.~M.~Sz\'ecs\'enyi and R.~Tateo,
``$T \bar{T}$-deformed 2D quantum field theories,''
\doilink{JHEP \textbf{10}, 112 (2016)}{
doi:10.1007/JHEP10(2016)112}
\arxivlink{1608.05534}.\\
%220 citations counted in INSPIRE as of 24 Jul 2021
%\cite{Smirnov:2016lqw}
%}\bibitem{Smirnov:2016lqw}
%
F.~A.~Smirnov and A.~B.~Zamolodchikov,
``On space of integrable quantum field theories,''
\doilink{Nucl. Phys. B \textbf{915}, 363-383 (2017)}{
doi:10.1016/j.nuclphysb.2016.12.014}
\arxivlink{1608.05499}.
%243 citations counted in INSPIRE as of 24 Jul 2021
%
%
%%\cite{Chung:1992mj}
%}\bibitem{Chung:1992mj}
%S.~w.~Chung and S.~H.~H.~Tye,
%``Chiral gauged WZW theories and coset models in conformal field theory,''
%Phys. Rev. D \textbf{47}, 4546-4566 (1993)
%doi:10.1103/PhysRevD.47.4546
%[arXiv:hep-th/9202002 [hep-th]].
%%17 citations counted in INSPIRE as of 26 Jul 2021
%
%
%\cite{Sfetsos:1993sr}
%}\bibitem{Sfetsos:1993sr}
%6 citations counted in INSPIRE as of 26 Jul 2021
%
%}\bibitem{Sfetsos:1993bh}
%K.~Sfetsos and A.~A.~Tseytlin,
%``Chiral gauged WZNW models and heterotic string backgrounds,''
%Nucl. Phys. B \textbf{415}, 116-154 (1994)
%doi:10.1016/0550-3213(94)90069-8
%[arXiv:hep-th/9308018 [hep-th]].
%%20 citations counted in INSPIRE as of 26 Jul 2021
%
%\cite{Arutyunov:2009ga}
}\bibitem{Arutyunov:2009ga}{
G.~Arutyunov and S.~Frolov,
``Foundations of the AdS$_{5} \times S^{5}$ superstring. Part I,''
\doilink{J. Phys. A \textbf{42}, 254003 (2009)}{
doi:10.1088/1751-8113/42/25/254003}
\arxivlink{0901.4937}.
%345 citations counted in INSPIRE as of 26 Jul 2021
%
%\cite{vanTongeren:2013gva}
}\bibitem{vanTongeren:2013gva}{
S.~J.~van Tongeren,
``Integrability of the ${\rm Ad}{{{\rm S}}_{5}}\times {{{\rm S}}^{5}}$ superstring and its deformations,''
\doilink{J. Phys. A \textbf{47}, 433001 (2014)}{
doi:10.1088/1751-8113/47/43/433001}
\arxivlink{1310.4854}.
%53 citations counted in INSPIRE as of 26 Jul 2021
%
%\cite{Bombardelli:2016rwb}
}\bibitem{Bombardelli:2016rwb}{
D.~Bombardelli, A.~Cagnazzo, R.~Frassek, F.~Levkovich-Maslyuk, F.~Loebbert, S.~Negro, I.~M.~Sz\'ecs\'enyi, A.~Sfondrini, S.~J.~van Tongeren and A.~Torrielli,
``An integrability primer for the gauge-gravity correspondence: An introduction,''
\doilink{J. Phys. A \textbf{49}, no.32, 320301 (2016)}{
doi:10.1088/1751-8113/49/32/320301}
\arxivlink{1606.02945}.
%46 citations counted in INSPIRE as of 26 Jul 2021
%
%
%\cite{Tseytlin:2004xa}
}\bibitem{Tseytlin:2004xa}{
A.~A.~Tseytlin,
``Semiclassical strings and AdS/CFT,''
\arxivlink{hep-th/0409296}.
%151 citations counted in INSPIRE as of 26 Jul 2021
%
%\cite{Nemeschansky:1986yx}
}\bibitem{Nemeschansky:1986yx}{
D.~Nemeschansky and A.~Sen,
``Conformal invariance of supersymmetric $\sigma$ models on Calabi-yau manifolds,''
\doilink{Phys. Lett. B \textbf{178}, 365-369 (1986)}{
doi:10.1016/0370-2693(86)91394-8}.
%127 citations counted in INSPIRE as of 27 Jul 2021
%
%\cite{Novikov}
}\bibitem{Novikov}{
V.~A.~Novikov, M.~A.~Shifman, A.~I.~Vainshtein and V.~I.~Zakharov,
``Exact Gell-Mann-Low function of supersymmetric Yang-Mills theories from instanton calculus,''
\doilink{Nucl. Phys. B \textbf{229}, 381-393 (1983)}{
doi:10.1016/0550-3213(83)90338-3}.\\
%766 citations counted in INSPIRE as of 27 Jul 2021
%
V.~A.~Novikov, M.~A.~Shifman, A.~I.~Vainshtein and V.~I.~Zakharov,
``Two-dimensional sigma models: modeling nonperturbative effects of quantum chromodynamics,''
\doilink{Phys. Rept. \textbf{116}, 103 (1984)}{
doi:10.1016/0370-1573(84)90021-8}.
%199 citations counted in INSPIRE as of 27 Jul 2021
%
%\cite{Grisaru:1986px}
}\bibitem{Grisaru2}{
M.~T.~Grisaru, A.~E.~M.~van de Ven and D.~Zanon,
%``Four Loop beta Function for the N=1 and N=2 Supersymmetric Nonlinear Sigma Model in Two-Dimensions,''
%Phys. Lett. B \textbf{173}, 423-428 (1986)
%doi:10.1016/0370-2693(86)90408-9;
``Two-dimensional supersymmetric sigma models on Ricci flat Kahler manifolds are not finite,''
\doilink{Nucl. Phys. B \textbf{277}, 388-408 (1986)}{
doi:10.1016/0550-3213(86)90448-7}; 
``Four loop divergences for the N=1 supersymmetric nonlinear sigma model in two-dimensions,''
\doilink{Nucl. Phys. B \textbf{277}, 409-428 (1986)}{
doi:10.1016/0550-3213(86)90449-9}.
%236 citations counted in INSPIRE as of 27 Jul 2021
%233 citations counted in INSPIRE as of 27 Jul 2021
%
%\cite{Zumino:1979et}
%\cite{Borsato:2019oip}
}\bibitem{Borsato:2019oip}{
R.~Borsato and L.~Wulff,
``Two-loop conformal invariance for Yang-Baxter deformed strings,''
\doilink{JHEP \textbf{03}, 126 (2020)}{
doi:10.1007/JHEP03(2020)126}
\arxivlink{1910.02011}.
}\bibitem{Babelon}{
O.~Babelon, D.~Bernard and M.~Talon,
``Introduction to classical integrable systems,''
\doilink{Cambridge University Press (2009)}{10.1017/CBO9780511535024}.
}\bibitem{Zumino:1979et}{
B.~Zumino,
``Supersymmetry and Kahler manifolds,''
\doilink{Phys. Lett. B \textbf{87}, 203 (1979)}{
doi:10.1016/0370-2693(79)90964-X}.
%676 citations counted in INSPIRE as of 27 Jul 2021
%
%\cite{Abdalla:1985nm}
}\bibitem{Abdalla:1985nm}{
E.~Abdalla and M.~Forger,
``Integrable nonlinear $\sigma$ models with fermions,''
\doilink{Commun. Math. Phys. \textbf{104}, 123 (1986)}{
doi:10.1007/BF01210796}.
%21 citations counted in INSPIRE as of 28 Jul 2021
%
%\cite{Borsato:2016zcf}
}\bibitem{Borsato:2016zcf}{
R.~Borsato, A.~A.~Tseytlin and L.~Wulff,
``Supergravity background of $\lambda$-deformed model for AdS$_2 \times$  S$^2$ supercoset,''
\doilink{Nucl. Phys. B \textbf{905}, 264-292 (2016)}{
doi:10.1016/j.nuclphysb.2016.02.018}
\arxivlink{1601.08192}.
%61 citations counted in INSPIRE as of 28 Jul 2021
%
%\cite{Chervonyi:2016ajp}
}\bibitem{Lunin}{
O.~Lunin, R.~Roiban and A.~A.~Tseytlin,
``Supergravity backgrounds for deformations of AdS$_{n} \times S^n$ supercoset string models,''
\doilink{Nucl. Phys. B \textbf{891}, 106-127 (2015)}{
doi:10.1016/j.nuclphysb.2014.12.006}
\arxivlink{1411.1066}.\\
%67 citations counted in INSPIRE as of 28 Jul 2021
%
%
Y.~Chervonyi and O.~Lunin,
``Supergravity background of the $\lambda$-deformed AdS$_3 \times$ S$^3$ supercoset,''
\doilink{Nucl. Phys. B \textbf{910}, 685-711 (2016)}{
doi:10.1016/j.nuclphysb.2016.07.023}
\arxivlink{1606.00394}.
%48 citations counted in INSPIRE as of 28 Jul 2021
%
%\cite{Seibold:2019dvf}
}\bibitem{Seibold:2019dvf}{
F.~K.~Seibold,
``Two-parameter integrable deformations of the $AdS_3 \times S^3 \times T^4$ superstring,''
\doilink{JHEP \textbf{10}, 049 (2019)}{
doi:10.1007/JHEP10(2019)049}
\arxivlink{1907.05430}.
%11 citations counted in INSPIRE as of 28 Jul 2021
%
%
%\cite{Osten:2016dvf}
}\bibitem{Osten:2016dvf}{
D.~Osten and S.~J.~van Tongeren,
``Abelian Yang\textendash{}Baxter deformations and TsT transformations,''
\doilink{Nucl. Phys. B \textbf{915}, 184-205 (2017)}{
doi:10.1016/j.nuclphysb.2016.12.007}
\arxivlink{1608.08504}.
%78 citations counted in INSPIRE as of 28 Jul 2021
%
}\bibitem{homog}{
I.~Kawaguchi, T.~Matsumoto and K.~Yoshida,
``Jordanian deformations of the $AdS_5 x S^5$ superstring,''
\doilink{JHEP \textbf{04}, 153 (2014)}{
doi:10.1007/JHEP04(2014)153}
\arxivlink{1401.4855}.\\
%176 citations counted in INSPIRE as of 28 Jul 2021
%
T.~Matsumoto and K.~Yoshida,
``Yang\textendash{}Baxter sigma models based on the CYBE,''
\doilink{Nucl. Phys. B \textbf{893}, 287-304 (2015)}{
doi:10.1016/j.nuclphysb.2015.02.009}
\arxivlink{1501.03665}.\\
%79 citations counted in INSPIRE as of 28 Jul 2021
%
S.~J.~van Tongeren,
``Yang\textendash{}Baxter deformations, AdS/CFT, and twist-noncommutative gauge theory,''
\doilink{Nucl. Phys. B \textbf{904}, 148-175 (2016)}{
doi:10.1016/j.nuclphysb.2016.01.012}
\arxivlink{1506.01023}.
%93 citations counted in INSPIRE as of 28 Jul 2021
%
}\bibitem{homog2}{
B.~Hoare and A.~A.~Tseytlin,
``Homogeneous Yang-Baxter deformations as non-abelian duals of the $\mathrm{AdS}_5 \sigma$-model,''
J. Phys. A \textbf{49}, no.49, 494001 (2016)
doi:10.1088/1751-8113/49/49/494001
[arXiv:1609.02550 [hep-th]].
%63 citations counted in INSPIRE as of 28 Jul 2021
%
}\bibitem{homog3}{
R.~Borsato and L.~Wulff,
``Integrable feformations of $T$-dual $\sigma$ models,''
\doilink{Phys. Rev. Lett. \textbf{117}, no.25, 251602 (2016)}{
doi:10.1103/PhysRevLett.117.251602}
\arxivlink{1609.09834}; 
%72 citations counted in INSPIRE as of 31 Jul 2021
``On non-abelian T-duality and deformations of supercoset string sigma-models,''
\doilink{JHEP \textbf{10}, 024 (2017)}{
doi:10.1007/JHEP10(2017)024}
\arxivlink{1706.10169}.
%45 citations counted in INSPIRE as of 28 Jul 2021
%
%%%%%%%%%%%%%%%%%%here
%
%
%}\bibitem{HLT1} B.~Hoare, N.~Levine and A.~A.~Tseytlin,
%``Integrable 2d sigma models: quantum corrections to geometry from RG flow,''
%\arxivlink{1907.04737}.
%%%CITATION = ARXIV:1907.04737;%%
%
}\bibitem{Fukushima:2021eni}{
O.~Fukushima, J.~i.~Sakamoto and K.~Yoshida,
``Integrable deformed $T^{1,1}$ sigma models from 4D Chern-Simons theory,''
\arxivlink{2105.14920}.
}\bibitem{ecker}{G.~Ecker and J.~Honerkamp,
``Application of invariant renormalization to the nonlinear chiral invariant pion lagrangian in the one-loop approximation,''
\doilink{Nucl.\ Phys.\ B {\bf 35}, 481 (1971)}{10.1016/0550-3213(71)90468-8}.\\
%%CITATION = %doi:10.1016/0550-3213(71)90468-8;%%
%
%
J.~Honerkamp,
``Chiral multiloops,''
\doilink{Nucl.\ Phys.\ B {\bf 36}, 130 (1972)}{10.1016/0550-3213(72)90299-4}.
%%CITATION = doi:10.1016/0550-3213(72)90299-4;%%
%
}\bibitem{friedan}{D.~H.~Friedan,
``Nonlinear models in two + epsilon dimensions,''
\doilink{Annals Phys.\ {\bf 163}, 318 (1985)}{doi:10.1016/0003-4916(85)90384-7};
%%CITATION = %doi:10.1016/0003-4916(85)90384-7;%%
``Nonlinear models in two + epsilon dimensions,''
\doilink{Phys.\ Rev.\ Lett.\ {\bf 45}, 1057 (1980)}{10.1103/PhysRevLett.45.1057}.
%%CITATION = doi:10.1103/PhysRevLett.45.1057;%%
%
%
%
%
%}\bibitem{ricci}{R.~Ricci, A.~A.~Tseytlin and M.~Wolf,
%``On T-duality and integrability for strings on AdS backgrounds,''
%\doilink{JHEP {\bf 0712}, 082 (2007)}{doi:10.1088/1126-6708/2007/12/082}
%\arxivlink{0711.0707}.
%%CITATION = %doi:10.1088/1126-6708/2007/12/082;%%
%
}\bibitem{Fateev:1992tk}{V.~A.~Fateev, E.~Onofri and A.~B.~Zamolodchikov,
``Integrable deformations of the $O(3)$ sigma model. The sausage model,''
\doilink{Nucl.\ Phys.\ B {\bf 406}, 521 (1993)}{10.1016/0550-3213(93)90001-6}.
%%CITATION = doi:10.1016/0550-3213(93)90001-6;%%
%
}\bibitem{fateev96}{V.~A.~Fateev,
``The sigma model (dual) representation for a two-parameter family of integrable quantum field theories,''
\doilink{Nucl.\ Phys.\ B {\bf 473}, 509 (1996)}{10.1016/0550-3213(96)00256-8}.
%%CITATION = %doi:10.1016/0550-3213(96)00256-8;%%
%
}\bibitem{lukyanov}{S.~L.~Lukyanov,
``The integrable harmonic map problem versus Ricci flow,''
\doilink{Nucl.\ Phys.\ B {\bf 865}, 308 (2012)}{10.1016/j.nuclphysb.2012.08.002}
\arxivlink{1205.3201}.
%%CITATION = doi:10.1016/j.nuclphysb.2012.08.002;%%
%
}\bibitem{Fateev:2019xuq}{V.~Fateev,
``Classical and quantum integrable sigma models. Ricci flow, ``nice duality" and perturbed rational conformal field theories,''
\doilink{J. Exp. Theor. Phys. \textbf{129}, no.4, 566-590 (2019)}{
doi:10.1134/S1063776119100042}
\arxivlink{1902.02811}.
%%CITATION = ARXIV:1902.02811;%%
%
}\bibitem{Fateev:2018yos}{V.~A.~Fateev and A.~V.~Litvinov,
``Integrability, duality and sigma models,''
\doilink{JHEP {\bf 1811}, 204 (2018)}{10.1007/JHEP11(2018)204}
\arxivlink{1804.03399}.
%%CITATION = doi:10.1007/JHEP11(2018)204;%%
%
}\bibitem{Demulder:2017zhz}{S.~Demulder, S.~Driezen, A.~Sevrin and D.~C.~Thompson,
``Classical and quantum aspects of Yang-Baxter Wess-Zumino models,''
\doilink{JHEP {\bf 1803}, 041 (2018)}{10.1007/JHEP03(2018)041}
\arxivlink{1711.00084}.
%%CITATION = doi:10.1007/JHEP03(2018)041;%%
%
}\bibitem{Klimcik:2019kkf}{C.~Klimcik,
``Dressing cosets and multi-parametric integrable deformations,''
\doilink{JHEP \textbf{07}, 176 (2019)}{
doi:10.1007/JHEP07(2019)176}
\arxivlink{1903.00439}.
%%CITATION = ARXIV:1903.00439;%%
%
}\bibitem{Litvinov:2018bou}{A.~V.~Litvinov and L.~A.~Spodyneiko,
``On dual description of the deformed $O(N)$ sigma model,''
\doilink{JHEP {\bf 1811}, 139 (2018)}{10.1007/JHEP11(2018)139}
\arxivlink{1804.07084}.
%%CITATION = doi:10.1007/JHEP11(2018)139;%%
%
}\bibitem{Tseytlin:1991wr}{A.~A.~Tseytlin,
``Duality and dilaton,''
\doilink{Mod.\ Phys.\ Lett.\ A {\bf 6}, 1721 (1991)}{10.1142/S021773239100186X}, \\
{\small \url{https://www.academia.edu/40796716/Tseytlin1991_duality_dilaton_MPLA} }\ .
%%CITATION = %doi:10.1142/S021773239100186X;%%
%
}\bibitem{Panvel:1992he}{J.~Panvel,
``Higher order conformal invariance of string backgrounds obtained by $O(d,d)$ transformations,''
\doilink{Phys.\ Lett.\ B {\bf 284}, 50 (1992)}{10.1016/0370-2693(92)91923-W}
\arxivlink{hep-th/9204024}.
%%CITATION = doi:10.1016/0370-2693(92)91923-W;%%
%
}\bibitem{Haagensen:1997er}{P.~E.~Haagensen and K.~Olsen,
``T duality and two loop renormalization flows,''
\doilink{Nucl.\ Phys.\ B {\bf 504}, 326 (1997)}{10.1016/S0550-3213(97)00496-3}
\arxivlink{hep-th/9704157}.
%%CITATION = doi:10.1016/S0550-3213(97)00496-3;%%
%
}\bibitem{Haagensen:1997bh}{P.~E.~Haagensen,
``Duality and the renormalization group,''
\arxivlink{hep-th/9708110}.
%%CITATION = HEP-TH/9708110;%%
%
}\bibitem{Dijkgraaf:1991ba}{R.~Dijkgraaf, H.~L.~Verlinde and E.~P.~Verlinde,
``String propagation in a black hole geometry,''
\doilink{Nucl.\ Phys.\ B {\bf 371}, 269 (1992)}{10.1016/0550-3213(92)90237-6}.
%%CITATION = %doi:10.1016/0550-3213(92)90237-6;%%
%
}\bibitem{Bars:1992sr}{I.~Bars and K.~Sfetsos,
``Conformally exact metric and dilaton in string theory on curved space-time,''
\doilink{Phys.\ Rev.\ D {\bf 46}, 4510 (1992)}{10.1103/PhysRevD.46.4510}
\arxivlink{hep-th/9206006}.
%%CITATION = doi:10.1103/PhysRevD.46.4510;%%
%
}\bibitem{Tseytlin:1992ri}{A.~A.~Tseytlin,
``Effective action of gauged WZW model and exact string solutions,''
\doilink{Nucl.\ Phys.\ B {\bf 399}, 601 (1993)}{10.1016/0550-3213(93)90511-M}
\arxivlink{hep-th/9301015}.
%%CITATION = %doi:10.1016/0550-3213(93)90511-M;%%
%
%\cite{Karabali:1988au}
}\bibitem{Karabali}{
D.~Karabali, Q.~H.~Park, H.~J.~Schnitzer and Z.~Yang,
``A GKO construction based on a path integral formulation of gauged Wess-Zumino-Witten actions,''
\doilink{Phys. Lett. B \textbf{216}, 307-312 (1989)}{
doi:10.1016/0370-2693(89)91120-9}.\\
%241 citations counted in INSPIRE as of 29 Jun 2021
%\cite{Karabali:1989dk}
%
D.~Karabali and H.~J.~Schnitzer,
``BRST quantization of the gauged WZW action and coset conformal field theories,''
\doilink{Nucl. Phys. B \textbf{329}, 649-666 (1990)}{
doi:10.1016/0550-3213(90)90075-O}.
%259 citations counted in INSPIRE as of 29 Jun 2021
%
}\bibitem{bs}{I.~Bars and K.~Sfetsos,
``Exact effective action and space-time geometry in gauged WZW models,''
\doilink{Phys.\ Rev.\ D {\bf 48}, 844 (1993)}{10.1103/PhysRevD.48.844}
\arxivlink{hep-th/9301047}.
%%CITATION = %doi:10.1103/PhysRevD.48.844;%%
%
}\bibitem{Tseytlin:1993my}{A.~A.~Tseytlin,
``Conformal sigma models corresponding to gauged Wess-Zumino-Witten theories,''
\doilink{Nucl.\ Phys.\ B {\bf 411}, 509 (1994)}{10.1016/0550-3213(94)90461-8}
\arxivlink{hep-th/9302083}.
%%CITATION = %doi:10.1016/0550-3213(94)90461-8;%%
%
}\bibitem{Tseytlin:1993df}{A.~A.~Tseytlin,
``On field redefinitions and exact solutions in string theory,''
\doilink{Phys.\ Lett.\ B {\bf 317}, 559 (1993)}{10.1016/0370-2693(93)91372-T}
\arxivlink{hep-th/9308042}.
%%CITATION = doi:10.1016/0370-2693(93)91372-T;%%
%
}\bibitem{Horowitz:1994ei}{G.~T.~Horowitz and A.~A.~Tseytlin,
``On exact solutions and singularities in string theory,''
\doilink{Phys.\ Rev.\ D {\bf 50}, 5204 (1994)}{10.1103/PhysRevD.50.5204}
\arxivlink{hep-th/9406067}.
%%CITATION = doi:10.1103/PhysRevD.50.5204;%%
%
}\bibitem{Tseytlin:1995fh}{A.~A.~Tseytlin,
``Exact solutions of closed string theory,''
\doilink{Class.\ Quant.\ Grav.\ {\bf 12}, 2365 (1995)}{10.1088/0264-9381/12/10/003},
\arxivlink{hep-th/9505052}.
%%CITATION = doi:10.1088/0264-9381/12/10/003;%%
%
}\bibitem{Bardacki:1990wj}{K.~Bardakci, M.~J.~Crescimanno and E.~Rabinovici,
``Parafermions From coset models,''
\doilink{Nucl.\ Phys.\ B {\bf 344}, 344 (1990)}{10.1016/0550-3213(90)90365-K}.
%%CITATION = doi:10.1016/0550-3213(90)90365-K;%%
%
}\bibitem{Witten:1991yr}{E.~Witten,
``On string theory and black holes,''
\doilink{Phys.\ Rev.\ D {\bf 44}, 314 (1991)}{10.1103/PhysRevD.44.314}.
%%CITATION = doi:10.1103/PhysRevD.44.314;%%
%
}\bibitem{Tseytlin:1991ht}{A.~A.~Tseytlin,
``On the form of the black hole solution in D = 2 theory,''
\doilink{Phys.\ Lett.\ B {\bf 268}, 175 (1991)}{10.1016/0370-2693(91)90800-6}.
%%CITATION = doi:10.1016/0370-2693(91)90800-6;%%
%
}\bibitem{Jack:1992mk}{I.~Jack, D.~R.~T.~Jones and J.~Panvel,
``Exact bosonic and supersymmetric string black hole solutions,''
\doilink{Nucl.\ Phys.\ B {\bf 393}, 95 (1993)}{10.1016/0550-3213(93)90239-L}
\arxivlink{hep-th/9201039}.
%%CITATION = doi:10.1016/0550-3213(93)90239-L;%%
%
%}\bibitem{FernandezPousa:1996hi}{C.~R.~Fernandez-Pousa, M.~V.~Gallas, T.~J.~Hollowood and J.~L.~Miramontes,
%``The symmetric space and homogeneous sine-Gordon theories,''
%\doilink{Nucl.\ Phys.\ B {\bf 484}, 609 (1997)}{10.1016/S0550-3213(96)00603-7}
%\arxivlink{hep-th/9606032}.
%%%CITATION = doi:10.1016/S0550-3213(96)00603-7;%%
%
}\bibitem{Hoare:2010fb}{B.~Hoare and A.~A.~Tseytlin,
``On the perturbative S-matrix of generalized sine-Gordon models,''
\doilink{JHEP {\bf 1011}, 111 (2010)}{10.1007/JHEP11(2010)111}
\arxivlink{1008.4914}.
%%CITATION = doi:10.1007/JHEP11(2010)111;%%
%
%}\bibitem{deVega:1982sh}{H.~J.~de Vega and J.~M.~Maillet,
%``Semiclassical quantization of the complex {sine-Gordon} field theory,''
%\doilink{Phys.\ Rev.\ D {\bf 28}, 1441 (1983)}{10.1103/PhysRevD.28.1441}.
%%%CITATION = doi:10.1103/PhysRevD.28.1441;%%
%
%}\bibitem{Bonneau:1984pj}{G.~Bonneau and F.~Delduc,
%``S matrix properties versus renormalizability in two-dimensional $O(N)$ symmetric models,''
%\doilink{Nucl.\ Phys.\ B {\bf 250}, 561 (1985)}{10.1016/0550-3213(85)90495-X}.
%%%CITATION = doi:10.1016/0550-3213(85)90495-X;%%
%%
}\bibitem{Schwarz:1992te}{A.~S.~Schwarz and A.~A.~Tseytlin,
``Dilaton shift under duality and torsion of elliptic complex,''
\doilink{Nucl.\ Phys.\ B {\bf 399}, 691 (1993)}{10.1016/0550-3213(93)90514-P}
\arxivlink{hep-th/9210015}.
%%CITATION = %doi:10.1016/0550-3213(93)90514-P;%%
%
}\bibitem{Gerasimov:1990fi}{A.~Gerasimov, A.~Morozov, M.~Olshanetsky, A.~Marshakov and S.~L.~Shatashvili,
``Wess-Zumino-Witten model as a theory of free fields,''
\doilink{Int.\ J.\ Mod.\ Phys.\ A {\bf 5}, 2495 (1990)}{10.1142/S0217751X9000115X}.
%%CITATION = doi:10.1142/S0217751X9000115X;%%
%
%}\bibitem{Buscher:1987qj} T.~H.~Buscher,
%``Path integral Derivation of Quantum Duality in Nonlinear Sigma Models,''
%\doilink{Phys.\ Lett.\ B {\bf 201}, 466 (1988)}{10.1016/0370-2693(88)90602-8}.
%%%CITATION = doi:10.1016/0370-2693(88)90602-8;%%
%
%
}\bibitem{Buscher:1987qj}{
T.~H.~Buscher,
``A symmetry of the string background field equations,''
\doilink{Phys. Lett. B \textbf{194}, 59-62 (1987)}{
doi:10.1016/0370-2693(87)90769-6};
%898 citations counted in INSPIRE as of 06 Jul 2021
%\cite{Buscher:1987qj}
%}\bibitem{Buscher:1987qj}
%T.~H.~Buscher,
``Path integral derivation of quantum duality in nonlinear sigma models,''
\doilink{Phys. Lett. B \textbf{201}, 466-472 (1988)}{
doi:10.1016/0370-2693(88)90602-8}.
%918 citations counted in INSPIRE as of 06 Jul 2021
%
}\bibitem{DeJaegher:1998pp}{J.~De Jaegher, J.~Raeymaekers, A.~Sevrin and W.~Troost,
``Dilaton transformation under Abelian and nonAbelian T duality in the path integral approach,''
\doilink{Nucl.\ Phys.\ B {\bf 548}, 563 (1999)}{10.1016/S0550-3213(99)00157-1}
\arxivlink{hep-th/9812207}.
%%CITATION = doi:10.1016/S0550-3213(99)00157-1;%%
%
}\bibitem{Klimcik:2002zj}{C.~Klimcik,
``Yang-Baxter sigma models and dS/AdS T duality,''
\doilink{JHEP {\bf 0212}, 051 (2002)}{10.1088/1126-6708/2002/12/051}
\arxivlink{hep-th/0210095}.
%%CITATION = doi:10.1088/1126-6708/2002/12/051;%%
%
}\bibitem{Penna:2020uky}{
R.~F.~Penna,
``A Twistor Action for Integrable Systems,''
\arxivlink{2011.05831}.
%5 citations counted in INSPIRE as of 04 Aug 2021
}\bibitem{Klimcik:2008eq}{C.~Klimcik,
``On integrability of the Yang-Baxter sigma-model,''
\doilink{J.\ Math.\ Phys.\ {\bf 50}, 043508 (2009)}{10.1063/1.3116242}
\arxivlink{0802.3518}.
%%%CITATION = doi:10.1063/1.3116242;%
%
}\bibitem{Ki}{C.~Klimcik,
``Integrability of the bi-Yang-Baxter sigma-model,''
\doilink{Lett.\ Math.\ Phys.\ {\bf 104}, 1095 (2014)}{10.1007/s11005-014-0709-y}
\arxivlink{1402.2105}.
%%CITATION = doi:10.1007/s11005-014-0709-y;%%
%\cite{Alfimov:2020jpy}
}\bibitem{Alfimov:2020jpy}{
M.~Alfimov, B.~Feigin, B.~Hoare and A.~Litvinov,
``Dual description of $\eta$-deformed OSP sigma models,''
\doilink{JHEP \textbf{12}, 040 (2020)}{
doi:10.1007/JHEP12(2020)040}
\arxivlink{2010.11927}.
%0 citations counted in INSPIRE as of 31 Jul 2021
}\bibitem{Bazhanov:1984gu}{
V.~V.~Bazhanov,
``Trigonometric solution of triangle equations and classical Lie algebras,''
\doilink{Phys. Lett. B \textbf{159}, 321-324 (1985)}{
doi:10.1016/0370-2693(85)90259-X}.\\
M.~Jimbo,
``Quantum r matrix for the generalized Toda system,''
\doilink{Commun. Math. Phys. \textbf{102}, 537-547 (1986)}{
doi:10.1007/BF01221646}.
%529 citations counted in INSPIRE as of 31 Jul 2021
%
%118 citations counted in INSPIRE as of 31 Jul 2021
}\bibitem{Delduc:2013fga}{F.~Delduc, M.~Magro and B.~Vicedo,
``On classical $q$-deformations of integrable sigma-models,''
\doilink{JHEP {\bf 1311}, 192 (2013)}{10.1007/JHEP11(2013)192}
\arxivlink{1308.3581}.
%%CITATION = doi:10.1007/JHEP11(2013)192;%%
%
}\bibitem{Sfetsos:2013wia}{K.~Sfetsos,
``Integrable interpolations: From exact CFTs to non-Abelian T-duals,''
\doilink{Nucl.\ Phys.\ B {\bf 880}, 225 (2014)}{10.1016/j.nuclphysb.2014.01.004}
\arxivlink{1312.4560}.
%%CITATION = doi:10.1016/j.nuclphysb.2014.01.004;%%
%
}\bibitem{Hollowood:2014rla}{T.~J.~Hollowood, J.~L.~Miramontes and D.~M.~Schmidtt,
``Integrable deformations of strings on symmetric spaces,''
\doilink{JHEP {\bf 1411}, 009 (2014)}{10.1007/JHEP11(2014)009}
\arxivlink{1407.2840}.
%%CITATION = doi:10.1007/JHEP11(2014)009;%%
%
}\bibitem{n1}{A.~Subbotin and I.~V.~Tyutin,
``On the equivalence of dual theories,''
\doilink{Int.\ J.\ Mod.\ Phys.\ A {\bf 11}, 1315 (1996)}{10.1142/S0217751X96000596},
Erratum: [Int.\ J.\ Mod.\ Phys.\ A {\bf 11}, 2231 (1996)]
\arxivlink{hep-th/9506132}.
%%CITATION = %doi:10.1142/S0217751X96000596;%%
%
}\bibitem{n2}{J.~Balog, P.~Forgacs, Z.~Horvath and L.~Palla,
``Perturbative quantum (in)equivalence of dual sigma models in two-dimensions,''
\doilink{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf 49}, 16 (1996)}{10.1016/0920-5632(96)00311-8}
\arxivlink{hep-th/9601091}.
%%CITATION = %doi:10.1016/0920-5632(96)00311-8;%%
%
}\bibitem{n3}{L.~K.~Balazs, J.~Balog, P.~Forgacs, N.~Mohammedi, L.~Palla and J.~Schnittger,
``Quantum equivalence of sigma models related by nonAbelian duality transformations,''
\doilink{Phys.\ Rev.\ D {\bf 57}, 3585 (1998)}{10.1103/PhysRevD.57.3585}
\arxivlink{hep-th/9704137}.
%%CITATION = %doi:10.1103/PhysRevD.57.3585;%%
%
}\bibitem{Bonneau:2001za}{G.~Bonneau and P.~Y.~Casteill,
``Dualized sigma models at the two loop order,''
\doilink{Nucl.\ Phys.\ B {\bf 607}, 293 (2001)}{10.1016/S0550-3213(01)00216-4}
\arxivlink{hep-th/0103260}.
%%CITATION = doi:10.1016/S0550-3213(01)00216-4;%%
%
}\bibitem{Zamolodchikov:1980ku}{A.~B.~Zamolodchikov and V.~A.~Fateev,
``Model factorized S matrix and an integrable Heisenberg chain with spin 1. (in Russian),''
Sov.\ J.\ Nucl.\ Phys.\ {\bf 32}, 298 (1980),
[Yad.\ Fiz.\ {\bf 32}, 581 (1980)].
%%CITATION = SJNCA,32,298;%%
%
}\bibitem{Hoare:2014pna}{B.~Hoare, R.~Roiban and A.~A.~Tseytlin,
``On deformations of $AdS_n$ x $S^n$ supercosets,''
\doilink{JHEP {\bf 1406}, 002 (2014)}{10.1007/JHEP06(2014)002}
\arxivlink{1403.5517}.
%%CITATION = doi:10.1007/JHEP06(2014)002;%%
%
}\bibitem{Graham:1987ep}{S.~J.~Graham,
``Three loop beta function for the bosonic nonlinear $\sigma$ model,''
\doilink{Phys.\ Lett.\ B {\bf 197}, 543 (1987)}{10.1016/0370-2693(87)91052-5}.
%%CITATION = doi:10.1016/0370-2693(87)91052-5;%%
%
}\bibitem{Foakes:1987ij}{A.~P.~Foakes and N.~Mohammedi,
``Three loop calculation of the beta function for the purely metric nonlinear $\sigma$ model,''
\doilink{Phys.\ Lett.\ B {\bf 198}, 359 (1987)}{10.1016/0370-2693(87)90679-4}.
%%CITATION = %doi:10.1016/0370-2693(87)90679-4;%%
%
}\bibitem{Foakes:1987gg}{A.~P.~Foakes and N.~Mohammedi,
``An explicit three loop calculation for the purely metric two-dimensional nonlinear $\sigma$ model,''
\doilink{Nucl.\ Phys.\ B {\bf 306}, 343 (1988)}{10.1016/0550-3213(88)90696-7}.
%%CITATION = %doi:10.1016/0550-3213(88)90696-7;%%
%
%}\bibitem{Zamolodchikov:1978xm} A.~B.~Zamolodchikov and A.~B.~Zamolodchikov,
%``Factorized S-Matrices in Two-Dimensions as the Exact Solutions of Certain Relativistic Quantum Field Models,''
%\doilink{Annals Phys.\ {\bf 120}, 253 (1979)}{10.1016/0003-4916(79)90391-9}.
%%%CITATION = doi:10.1016/0003-4916(79)90391-9;%%
%
}\bibitem{Grisaru:1986px}{M.~T.~Grisaru, A.~E.~M.~van de Ven and D.~Zanon,
``Four loop beta function for the N=1 and N=2 supersymmetric nonlinear sigma model in two-dimensions,''
\doilink{Phys.\ Lett.\ B {\bf 173}, 423 (1986)}{10.1016/0370-2693(86)90408-9}.
%%CITATION = doi:10.1016/0370-2693(86)90408-9;%%
%
}\bibitem{BDCGR}{A.~A.~Belavin and V.~G.~Drinfel'd,
``Triangle equations and simple Lie algebras''
\doilink{Sov. Sci. Rev. {\bf C4}, 93 (1984)}{10.1007/BF01041913}.\\
%
M.~Cahen, S.~Gutt and J.~Rawnsley,
``Some remarks on the classification of Poisson Lie groups,''
\doilink{Contemp. Math. {\bf 179} (1994) 1}{10.1090/conm/179/01932}.
%
}\bibitem{Hoare:2015gda}{B.~Hoare and A.~A.~Tseytlin,
``On integrable deformations of superstring sigma models related to $AdS_n \times S^n$ supercosets,''
\doilink{Nucl.\ Phys.\ B {\bf 897}, 448 (2015)}{10.1016/j.nuclphysb.2015.06.001}
\arxivlink{1504.07213}.
%%CITATION = doi:10.1016/j.nuclphysb.2015.06.001;%%
%
}\bibitem{Itsios:2014lca}{G.~Itsios, K.~Sfetsos and K.~Siampos,
``The all-loop non-Abelian Thirring model and its RG flow``,
\doilink{Phys.\ Lett.\ B {\bf 733}, 265 (2014)}{10.1016/j.physletb.2014.04.061}
\arxivlink{1404.3748}.
%%CITATION = ARXIV:1404.3748;%%
%
}\bibitem{Appadu:2015nfa}{C. Appadu and T.J. Hollowood,
``Beta function of k deformed ${\text AdS}_{5} \times S^5$ string theory``,
\doilink{JHEP {\bf 1511}, 095 (2015)}{10.1007/JHEP11(2015)095}
\arxivlink{1507.05420}.
%%CITATION = doi:10.1007/JHEP11(2015)095;%%
%
}\bibitem{Fridling:1983ha}{B.~E.~Fridling and A.~Jevicki,
``Dual representations and ultraviolet divergences in nonlinear $\sigma$ models,''
\doilink{Phys.\ Lett.\ {\bf 134B}, 70 (1984)}{10.1016/0370-2693(84)90987-0}.
%%CITATION = doi:10.1016/0370-2693(84)90987-0;%%
%
}\bibitem{Fradkin:1984ai}{E.~S.~Fradkin and A.~A.~Tseytlin,
``Quantum equivalence of dual field theories,''
\doilink{Annals Phys.\ {\bf 162}, 31 (1985)}{10.1016/0003-4916(85)90225-8}.
%%CITATION = doi:10.1016/0003-4916(85)90225-8;%%
%
}\bibitem{Vicedo:2015pna}{B.~Vicedo,
``Deformed integrable $\sigma$-models, classical $R$-matrices and classical exchange algebra on Drinfel'd doubles,''
\doilink{J.\ Phys.\ A {\bf 48}, no. 35, 355203 (2015)}{10.1088/1751-8113/48/35/355203}
\arxivlink{1504.06303}.
%%CITATION = doi:10.1088/1751-8113/48/35/355203;%%
%
%
%
%
%
%
%
}\bibitem{Sfetsos:2015nya}{K.~Sfetsos, K.~Siampos and D.~C.~Thompson,
``Generalised integrable $\lambda$- and $\eta$-deformations and their relation,''
\doilink{Nucl.\ Phys.\ B {\bf 899}, 489 (2015)}{10.1016/j.nuclphysb.2015.08.015}
\arxivlink{1506.05784}.
%%CITATION = doi:10.1016/j.nuclphysb.2015.08.015;%%
%
}\bibitem{Klimcik:2015gba}{C.~Klimcik,
``$\eta$ and $\lambda$ deformations as $\mathcal{E}$-models,''
\doilink{Nucl.\ Phys.\ B {\bf 900}, 259 (2015)}{10.1016/j.nuclphysb.2015.09.011}
\arxivlink{1508.05832}.
%%%CITATION = doi:10.1016/j.nuclphysb.2015.09.011;%%
%
}\bibitem{Hoare:2017ukq}{B.~Hoare and F.~K.~Seibold,
``Poisson-Lie duals of the $\eta$ deformed symmetric space sigma model,''
\doilink{JHEP {\bf 1711}, 014 (2017)}{10.1007/JHEP11(2017)014}
\arxivlink{1709.01448}.
%%CITATION = doi:10.1007/JHEP11(2017)014;%%
%
}\bibitem{Klimcik:1995dy}{C.~Klimcik and P.~Severa,
``Poisson-Lie T duality and loop groups of Drinfeld doubles,''
\doilink{Phys.\ Lett.\ B {\bf 372}, 65 (1996)}{10.1016/0370-2693(96)00025-1}
\arxivlink{hep-th/9512040}.
%%CITATION = doi:10.1016/0370-2693(96)00025-1;%%
%
}\bibitem{Valent:2009nv}{G.~Valent, C.~Klimcik and R.~Squellari,
``One loop renormalizability of the Poisson-Lie sigma models,''
\doilink{Phys.\ Lett.\ B {\bf 678}, 143 (2009)}{10.1016/j.physletb.2009.06.001}
\arxivlink{0902.1459}.
%%CITATION = doi:10.1016/j.physletb.2009.06.001;%%
%
}\bibitem{Sfetsos:2009dj}{K.~Sfetsos and K.~Siampos,
``Quantum equivalence in Poisson-Lie T-duality,''
\doilink{JHEP {\bf 0906}, 082 (2009)}{10.1088/1126-6708/2009/06/082}
\arxivlink{0904.4248}.
%%CITATION = doi:10.1088/1126-6708/2009/06/082;%%
%
}\bibitem{mt}{R.~R.~Metsaev and A.~A.~Tseytlin,
``Order alpha-prime (two loop) equivalence of the string equations of motion and the sigma model Weyl invariance conditions: dependence on the dilaton and the antisymmetric tensor,''
\doilink{Nucl.\ Phys.\ B {\bf 293}, 385 (1987)}{10.1016/0550-3213(87)90077-0};
%%CITATION = doi:10.1016/0550-3213(87)90077-0;%%
``Two loop beta function for the generalized bosonic sigma model,''
\doilink{Phys.\ Lett.\ B {\bf 191}, 354 (1987)}{doi:10.1016/0370-2693(87)90622-8}.
%%CITATION = doi:10.1016/0370-2693(87)90622-8;%%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%% 1910 refs:
%
%%}\bibitem{Fateev:1992tk} V.~A.~Fateev, E.~Onofri and A.~B.~Zamolodchikov,
%%``The sausage model (integrable deformations of $O(3)$ sigma model),''
%%\doilink{Nucl.\ Phys.\ B {\bf 406}, 521 (1993)}{10.1016/0550-3213(93)90001-6}.
%%%%CITATION = doi:10.1016/0550-3213(93)90001-6;%%
%%\\ V.~A.~Fateev,
%%``The sigma model (dual) representation for a two-parameter family of integrable quantum field theories,''
%%\doilink{Nucl.\ Phys.\ B {\bf 473}, 509 (1996)}{10.1016/0550-3213(96)00256-8}.
%%%%CITATION = %doi:10.1016/0550-3213(96)00256-8;%%
%%\\ S.~L.~Lukyanov,
%%``The integrable harmonic map problem versus Ricci flow,''
%%\doilink{Nucl.\ Phys.\ B {\bf 865}, 308 (2012)}{10.1016/j.nuclphysb.2012.08.002},
%%\arxivlink{1205.3201}.
%%%%CITATION = doi:10.1016/j.nuclphysb.2012.08.002;%%
%
%%}\bibitem{Fateev:2019xuq} V.~Fateev,
%%``Classical and quantum integrable sigma models. Ricci flow, ``nice duality'' and perturbed rational conformal field theories,''
%%\arxivlink{1902.02811}.
%%%%CITATION = ARXIV:1902.02811;%%
%%\\ V.~A.~Fateev and A.~V.~Litvinov,
%%``Integrability, Duality and Sigma Models,''
%%\doilink{JHEP {\bf 1811}, 204 (2018)}{10.1007/JHEP11(2018)204},
%%\arxivlink{1804.03399}.
%%%%CITATION = doi:10.1007/JHEP11(2018)204;%%
%%\\ A.~V.~Litvinov and L.~A.~Spodyneiko, %v3
%%``On dual description of the deformed $O(N)$ sigma model,''
%%\doilink{JHEP {\bf 1811}, 139 (2018)}{10.1007/JHEP11(2018)139},
%%\arxivlink{1804.07084}.
%%%%CITATION = doi:10.1007/JHEP11(2018)139;%%
%
%
%
}\bibitem{Sfetsos:1993bh}{
K.~Sfetsos,
``Effective action and exact geometry in chiral gauged WZW models,''
\arxivlink{hep-th/9305074}.\\
K.~Sfetsos and A.~A.~Tseytlin,
``Chiral gauged WZNW models and heterotic string backgrounds,''
\doilink{Nucl.\ Phys.\ B {\bf 415}, 116 (1994)}{10.1016/0550-3213(94)90069-8}
\arxivlink{hep-th/9308018}.
%%CITATION = doi:10.1016/0550-3213(94)90069-8;%%
%
%
}\bibitem{Sfetsos:19932}{K.~Sfetsos and A.~A.~Tseytlin,
``Antisymmetric tensor coupling and conformal invariance in sigma models corresponding to gauged WZNW theories,''
\doilink{Phys.\ Rev.\ D {\bf 49}, 2933 (1994)}{10.1103/PhysRevD.49.2933}
\arxivlink{hep-th/9310159}.
%%CITATION = doi:10.1103/PhysRevD.49.2933;%%
%
}\bibitem{Tseytlin:1993hm}{A.~A.~Tseytlin,
``On a `universal' class of WZW type conformal models,''
\doilink{Nucl.\ Phys.\ B {\bf 418}, 173 (1994)}{10.1016/0550-3213(94)90243-7}
\arxivlink{hep-th/9311062}.
%%CITATION = doi:10.1016/0550-3213(94)90243-7;%%
%
}\bibitem{Chung:1992mj}{S.~W.~Chung and S.~H.~H.~Tye,
``Chiral gauged WZW theories and coset models in conformal field theory,''
\doilink{Phys.\ Rev.\ D {\bf 47}, 4546 (1993)}{doi:10.1103/PhysRevD.47.4546}
\arxivlink{hep-th/9202002}.
%%CITATION = doi:10.1103/PhysRevD.47.4546;%%
%
%}\bibitem{Itsios:2014lca} G.~Itsios, K.~Sfetsos and K.~Siampos,
%``The all-loop non-abelian Thirring model and its RG flow,''
%\doilink{Phys.\ Lett.\ B {\bf 733}, 265 (2014)}{doi:10.1016/j.physletb.2014.04.061},
%\arxivlink{1404.3748}.
%%%CITATION = doi:10.1016/j.physletb.2014.04.061;%%
%
%
}\bibitem{Kutasov:1989aw}{D.~Kutasov,
``Duality off the critical point in two-dimensional systems with non-abelian symmetries,''
\doilink{Phys.\ Lett.\ B {\bf 233} (1989) 369}{doi:10.1016/0370-2693(89)91325-7}.
%%CITATION = doi:10.1016/0370-2693(89)91325-7;%%
%
%}\bibitem{n1} A.~Subbotin and I.~V.~Tyutin,
%``On the equivalence of dual theories,''
%\doilink{Int.\ J.\ Mod.\ Phys.\ A {\bf 11}, 1315 (1996)}{10.1142/S0217751X96000596},
%Erratum: [Int.\ J.\ Mod.\ Phys.\ A {\bf 11}, 2231 (1996)],
%\arxivlink{hep-th/9506132}.
%%%CITATION = %doi:10.1142/S0217751X96000596;%%
%
%L.~K.~Balazs, J.~Balog, P.~Forgacs, N.~Mohammedi, L.~Palla and J.~Schnittger,
%``Quantum equivalence of sigma models related by non-abelian duality transformations,''
%\doilink{Phys.\ Rev.\ D {\bf 57}, 3585 (1998)}{10.1103/PhysRevD.57.3585},
%\arxivlink{hep-th/9704137}.
%%%CITATION = %doi:10.1103/PhysRevD.57.3585;%%
%
%Bonneau Casteill
%
}\bibitem{Braaten:1985is}{E.~Braaten, T.~L.~Curtright and C.~K.~Zachos,
``Torsion and geometrostasis in nonlinear sigma models,''
\doilink{Nucl.\ Phys.\ B {\bf 260}, 630 (1985)}{10.1016/0550-3213(85)90053-7},
Erratum: [\doilink{Nucl.\ Phys.\ B {\bf 266}, 748 (1986)}{10.1016/0550-3213(86)90196-3}].
%%CITATION = doi:10.1016/0550-3213(86)90196-3, 10.1016/0550-3213(85)90053-7;%%
%
}\bibitem{Hull:1987pc}{C.~M.~Hull and P.~K.~Townsend,
``The two loop beta function for $\sigma$ models with torsion,''
\doilink{Phys.\ Lett.\ B {\bf 191}, 115 (1987)}{10.1016/0370-2693(87)91331-1}.\\
%%CITATION = doi:10.1016/0370-2693(87)91331-1;%%
%
D.~Zanon,
``Two loop beta functions and low-energy string effective action for the two-dimensional bosonic nonlinear $\sigma$ model with a {Wess-Zumino}-Witten  term,''
\doilink{Phys.\ Lett.\ B {\bf 191}, 363 (1987)}{10.1016/0370-2693(87)90623-X}.
%%CITATION = doi:10.1016/0370-2693(87)90623-X;%%
%
}\bibitem{adscftsol}{N.~Beisert {\it et al.}, %v3
``Review of AdS/CFT integrability: an overview,''
\doilink{Lett.\ Math.\ Phys.\ {\bf 99}, 3 (2012)}{10.1007/s11005-011-0529-2}
\arxivlink{1012.3982}.
%%CITATION = doi:10.1007/s11005-011-0529-2;%%
%
%}\bibitem{adscftsol2}
%N.~Gromov, V.~Kazakov, S.~Leurent and D.~Volin,
%``Quantum Spectral Curve for Planar $\mathcal{N} = 4$ Super-Yang-Mills Theory,''
%\doilink{Phys.\ Rev.\ Lett.\ {\bf 112}, no. 1, 011602 (2014)}{10.1103/PhysRevLett.112.011602},
%\arxivlink{1305.1939}.
%%%CITATION = doi:10.1103/PhysRevLett.112.011602;%%
%
}\bibitem{Zarembo:2010sg}{K.~Zarembo,
``Strings on semisymmetric superspaces,''
\doilink{JHEP {\bf 1005}, 002 (2010)}{doi:10.1007/JHEP05(2010)002}
\arxivlink{1003.0465}.
%%CITATION = doi:10.1007/JHEP05(2010)002;%%
%
}\bibitem{Wulff:2014kja}{L.~Wulff,
``Superisometries and integrability of superstrings,''
\doilink{JHEP {\bf 1405}, 115 (2014)}{10.1007/JHEP05(2014)115}
\arxivlink{1402.3122}.
%%CITATION = doi:10.1007/JHEP05(2014)115;%%
%
}\bibitem{betadef}{O.~Lunin and J.~M.~Maldacena,
``Deforming field theories with $U(1) \times U(1)$ global symmetry and their gravity duals,''
\doilink{JHEP {\bf 0505}, 033 (2005)}{10.1088/1126-6708/2005/05/033}
\arxivlink{hep-th/0502086}.\\
%%CITATION = doi:10.1088/1126-6708/2005/05/033;%%
%
S.~A.~Frolov, R.~Roiban and A.~A.~Tseytlin,
``Gauge-string duality for superconformal deformations of $\mathcal{N}=4$ super Yang-Mills theory,''
\doilink{JHEP {\bf 0507}, 045 (2005)}{10.1088/1126-6708/2005/07/045}
\arxivlink{hep-th/0503192}.\\
%%CITATION = doi:10.1088/1126-6708/2005/07/045;%%
%
S.~Frolov,
``Lax pair for strings in Lunin-Maldacena background,''
\doilink{JHEP {\bf 0505}, 069 (2005)}{10.1088/1126-6708/2005/05/069}
\arxivlink{hep-th/0503201}.
%%CITATION = doi:10.1088/1126-6708/2005/05/069;%%
%
}\bibitem{Hollowood:2014qma}{T.~J.~Hollowood, J.~L.~Miramontes and D.~M.~Schmidtt,
``An integrable deformation of the $AdS_5 \times S^5$ superstring,''
\doilink{J.\ Phys.\ A {\bf 47}, no. 49, 495402 (2014)}{doi:10.1088/1751-8113/47/49/495402}
\arxivlink{1409.1538}.
%%CITATION = doi:10.1088/1751-8113/47/49/495402;%%
%
}\bibitem{Delduc:2013qra}{F.~Delduc, M.~Magro and B.~Vicedo,
``An integrable deformation of the $AdS_5 \times S^5$ superstring action,''
\doilink{Phys.\ Rev.\ Lett.\ {\bf 112}, no. 5, 051601 (2014)}{10.1103/PhysRevLett.112.051601}
\arxivlink{1309.5850}.
%%CITATION = doi:10.1103/PhysRevLett.112.051601;%%
%
%}\bibitem{klimcik} \la{testc}
%C.~Klimcik,
%``Yang-Baxter sigma models and dS/AdS T duality,''
%\doilink{JHEP {\bf 0212}, 051 (2002)}{10.1088/1126-6708/2002/12/051},
%\arxivlink{hep-th/0210095}.
%%%CITATION = doi:10.1088/1126-6708/2002/12/051;%%
%
%}\bibitem{dmv} F.~Delduc, M.~Magro and B.~Vicedo,
%``On classical $q$-deformations of integrable sigma-models,''
%\doilink{JHEP {\bf 1311}, 192 (2013)}{doi:10.1007/JHEP11(2013)192},
%\arxivlink{1308.3581}.
%%%CITATION = doi:10.1007/JHEP11(2013)192;%%
%
}\bibitem{poissonlie}{C.~Klimcik and P.~Severa,
``Dual non-Abelian duality and the Drinfeld double,''
\doilink{Phys.\ Lett.\ B {\bf 351}, 455 (1995)}{10.1016/0370-2693(95)00451-P}
\arxivlink{hep-th/9502122}.\\
%%CITATION = doi:10.1016/0370-2693(95)00451-P;%%
%
C.~Klimcik,
``Poisson-Lie T-duality,''
\doilink{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf 46}, 116 (1996)}{10.1016/0920-5632(96)00013-8}
\arxivlink{hep-th/9509095}.
%%CITATION = doi:10.1016/0920-5632(96)00013-8;%%
%
}
%\bibitem{pld}{B.~Vicedo,
%``Deformed integrable $\sigma$-models, classical R-matrices and classical exchange algebra on Drinfel'd doubles,''
%\doilink{J.\ Phys.\ A {\bf 48}, no. 35, 355203 (2015)}{doi:10.1088/1751-8113/48/35/355203}
%\arxivlink{1504.06303}.\\
%%%CITATION = doi:10.1088/1751-8113/48/35/355203;%%
%%
%% K.~Sfetsos, K.~Siampos and D.~C.~Thompson,
%%``Generalised integrable $\lambda$- and $\eta$-deformations and their relation,''
%%\doilink{Nucl.\ Phys.\ B {\bf 899}, 489 (2015)}{doi:10.1016/j.nuclphysb.2015.08.015},
%%\arxivlink{1506.05784}.
%%%%CITATION = doi:10.1016/j.nuclphysb.2015.08.015;%%
%%
%C.~Klimcik,
%``$\eta$ and $\lambda$ deformations as E-models,''
%\doilink{Nucl.\ Phys.\ B {\bf 900}, 259 (2015)}{doi:10.1016/j.nuclphysb.2015.09.011}
%\arxivlink{1508.05832}.
%}%\cite{Bykov:2020tao}
\bibitem{byk3}{
D.~Bykov,
%``Quantum flag manifold $\sigma$-models and Hermitian Ricci flow,''
%\arxivlink{2006.14124};
``The $\mathsf{CP^{n-1}}$-model with fermions: a new look,''
\arxivlink{2009.04608};
``Flag manifold sigma-models and nilpotent orbits,''
\doilink{Proc. Steklov Inst. Math. \textbf{309}, 78-86 (2020)}{
doi:10.1134/S0081543820030062}
\arxivlink{1911.07768}.
}\bibitem{byk4}{
I.~Affleck, D.~Bykov and K.~Wamer,
``Flag manifold sigma models: spin chains and integrable theories,''
\arxivlink{2101.11638}.\\
%5 citations counted in INSPIRE as of 30 Jul 2021
D.~Bykov,
``Sigma models as Gross\textendash{}Neveu models,''
\doilink{Teor. Mat. Fiz. \textbf{208}, no.2, 165-179 (2021)}{
doi:10.1134/S0040577921080018}
\arxivlink{2106.15598}.
}\bibitem{Gross:1974jv}{
D.~J.~Gross and A.~Neveu,
``Dynamical symmetry breaking in asymptotically free field theories,''
\doilink{Phys. Rev. D \textbf{10}, 3235 (1974)}{
doi:10.1103/PhysRevD.10.3235}.
%1818 citations counted in INSPIRE as of 30 Jul 2021
%0 citations counted in INSPIRE as of 30 Jul 2021
%4 citations counted in INSPIRE as of 30 Jul 2021
%%CITATION = doi:10.1016/j.nuclphysb.2015.09.011;%%
%
%}\bibitem{hs} B.~Hoare and F.~K.~Seibold,
%``Poisson-Lie duals of the $\eta$ deformed symmetric space sigma model,''
%\doilink{JHEP {\bf 1711}, 014 (2017)}{doi:10.1007/JHEP11(2017)014},
%\arxivlink{1709.01448}.
%%%CITATION = doi:10.1007/JHEP11(2017)014;%%
%
}\bibitem{Klose:2010ki}{
T.~Klose,
``Review of AdS/CFT integrability, chapter IV.3: N=6 Chern-Simons and strings on AdS4xCP3,''
\doilink{Lett. Math. Phys. \textbf{99}, 401-423 (2012)}{
doi:10.1007/s11005-011-0520-y}
\arxivlink{1012.3999}.
%103 citations counted in INSPIRE as of 30 Jul 2021
}\bibitem{ABJM}{
O.~Aharony, O.~Bergman, D.~L.~Jafferis and J.~Maldacena,
``N=6 superconformal Chern-Simons-matter theories, M2-branes and their gravity duals,''
\doilink{JHEP \textbf{10}, 091 (2008)}{
doi:10.1088/1126-6708/2008/10/091}
\arxivlink{0806.1218}.
}\bibitem{sugra}{R.~Borsato and L.~Wulff,
``Target space supergeometry of $\eta$ and $\lambda$-deformed strings,''
\doilink{JHEP {\bf 1610}, 045 (2016)}{10.1007/JHEP10(2016)045}
\arxivlink{1608.03570}.
%%CITATION = doi:10.1007/JHEP10(2016)045;%%
%
}\bibitem{hsei}{
B.~Hoare and F.~K.~Seibold,
``Supergravity backgrounds of the $\eta$-deformed $AdS_2 \times S^2 \times T^6 $ and $AdS_5 \times S^5$ superstrings,''
\doilink{JHEP {\bf 1901}, 125 (2019)}{10.1007/JHEP01(2019)125}
\arxivlink{1811.07841}.
%%CITATION = doi:10.1007/JHEP01(2019)125;%%
%
%\cite{Seibold:2020ywq}
}\bibitem{seibold}{
F.~K.~Seibold, S.~J.~van Tongeren and Y.~Zimmermann, 
``The twisted story of worldsheet scattering in $\eta$-deformed $AdS_5 \times S^5$,''
\doilink{JHEP \textbf{12}, 043 (2020)}{
doi:10.1007/JHEP12(2020)043}
\arxivlink{2007.09136}.
%1 citations counted in INSPIRE as of 17 Oct 2020
%
%
}\bibitem{Polyakov:1988qz}{A.~M.~Polyakov,
``Two-dimensional quantum gravity: Superconductivity at high $T_c$,''
in: ``Fields, Strings and Critical Phenomena, Proc. of Les Houches 1988,''
eds.: E.~Brezin and J.~Zinn-Justin, North-Holland (1990).
%%CITATION = INSPIRE-273902;%%
%
}\bibitem{Guadagnini:1987ty}{E.~Guadagnini, M.~Martellini and M.~Mintchev,
``Scale invariant sigma models on homogeneous spaces,''
\doilink{Phys.\ Lett.\ B {\bf 194}, 69 (1987)}{10.1016/0370-2693(87)90771-4}.
%%CITATION = doi:10.1016/0370-2693(87)90771-4;%%
%
}\bibitem{Bardakci:1996gs}{K.~Bardakci, L.~M.~Bernardo and N.~Sochen, %v3a
``Integrable generalized Thirring model,''
\doilink{Nucl.\ Phys.\ B {\bf 487}, 513 (1997)}{doi:10.1016/S0550-3213(96)00715-8}
\arxivlink{hep-th/9607018}.
%%CITATION = doi:10.1016/S0550-3213(96)00715-8;%%
%
}\bibitem{Hull:1995gj}{O.~A.~Solovev,
``Towards conversion of the space of Thirring models into the model space for groups,''
\doilink{Phys.\ Lett.\ B {\bf 309}, 275 (1993)}{10.1016/0370-2693(93)90933-9}.\\
%%CITATION = doi:10.1016/0370-2693(93)90933-9;%%
%
C.~M.~Hull and O.~A.~Solovev,
``Conformal points and duality of non-abelian Thirring Models and interacting WZNW models,''
\doilink{Nucl.\ Phys.\ B {\bf 459}, 243 (1996)}{10.1016/0550-3213(95)00603-6}
\arxivlink{hep-th/9503021}.
%%CITATION = doi:10.1016/0550-3213(95)00603-6;%%
%
K.~Bardakci and L.~M.~Bernardo, %v3a
``The conformal points of the generalized Thirring model. 2.,''
\doilink{Nucl.\ Phys.\ B {\bf 450} 695 (1995)}{10.1016/0550-3213(95)00324-L}
\arxivlink{hep-th/9503143}.
%%CITATION = doi:10.1016/0550-3213(95)00324-L;%%
%
%}\bibitem{Georgiou:2016urf} G.~Georgiou and K.~Sfetsos,
%``A new class of integrable deformations of CFTs,''
%\doilink{JHEP {\bf 1703}, 083 (2017)}{10.1007/JHEP03(2017)083},
%\arxivlink{1612.05012}.
%%%CITATION = doi:10.1007/JHEP03(2017)083;%%
%
%
%
%
}\bibitem{Georgiou:2017aei}{G.~Georgiou, E.~Sagkrioti, K.~Sfetsos and K.~Siampos,
``Quantum aspects of doubly deformed CFTs,''
\doilink{Nucl.\ Phys.\ B {\bf 919}, 504 (2017)}{10.1016/j.nuclphysb.2017.04.004}
\arxivlink{1703.00462}.
%%CITATION = doi:10.1016/j.nuclphysb.2017.04.004;%%
%
}\bibitem{Georgiou:2017oly}{G.~Georgiou, K.~Sfetsos and K.~Siampos,
``Double and cyclic $\lambda$-deformations and their canonical equivalents,''
\doilink{Phys.\ Lett.\ B {\bf 771}, 576 (2017)}{10.1016/j.physletb.2017.06.007}
\arxivlink{1704.07834}.
%%CITATION = doi:10.1016/j.physletb.2017.06.007;%%
%
}\bibitem{Georgiou:2017jfi}{G.~Georgiou and K.~Sfetsos,
``Integrable flows between exact CFTs,''
\doilink{JHEP {\bf 1711}, 078 (2017)}{10.1007/JHEP11(2017)078}
\arxivlink{1707.05149}.
%%CITATION = doi:10.1007/JHEP11(2017)078;%%
%
}\bibitem{Gerganov:2000mt}{B.~Gerganov, A.~LeClair and M.~Moriconi,
``On the beta function for anisotropic current interactions in 2-D,''
\doilink{Phys.\ Rev.\ Lett.\ {\bf 86}, 4753 (2001)}{10.1103/PhysRevLett.86.4753}
\arxivlink{hep-th/0011189}.
%%CITATION = doi:10.1103/PhysRevLett.86.4753;%%
%
}\bibitem{LeClair:2001yp}{A.~LeClair,
``Chiral stabilization of the renormalization group for flavor and color anisotropic current interactions,''
\doilink{Phys.\ Lett.\ B {\bf 519}, 183 (2001)}{10.1016/S0370-2693(01)01089-9}
\arxivlink{hep-th/0105092}.
%%CITATION = doi:10.1016/S0370-2693(01)01089-9;%%
%
}\bibitem{Sfetsos:2014jfa}{K.~Sfetsos and K.~Siampos,
``Gauged WZW-type theories and the all-loop anisotropic non-abelian Thirring model,''
\doilink{Nucl.\ Phys.\ B {\bf 885}, 583 (2014)}{10.1016/j.nuclphysb.2014.06.012}
\arxivlink{1405.7803}.
%%CITATION = doi:10.1016/j.nuclphysb.2014.06.012;%%
%
}\bibitem{Witten:1983ar}{E.~Witten,
``Non-abelian bosonization in two dimensions,''
\doilink{Commun.\ Math.\ Phys.\ {\bf 92}, 455 (1984)}{10.1007/BF01215276}.
%%CITATION = doi:10.1007/BF01215276;%%
%
}\bibitem{Bos:1987mw}{M.~Bos,
``Dimensional regularization in the Wess-Zumino-Witten model,''
\doilink{Phys.\ Lett.\ B {\bf 189}, 435 (1987)}{10.1016/0370-2693(87)90656-3}.
%%CITATION = doi:10.1016/0370-2693(87)90656-3;%%
%
}\bibitem{McKane:1979cm}{A.~McKane and M.~Stone,
``Nonlinear sigma models: a perturbative approach to symmetry restoration,''
\doilink{Nucl.\ Phys.\ B {\bf 163} (1980) 169}{10.1016/0550-3213(80)90396-X}.
%%CITATION = doi:10.1016/0550-3213(80)90396-X;%%
%
}\bibitem{Hikami:1980hi}{S.~Hikami,
``Three loop beta-functions of nonlinear sigma models on symmetric spaces,''
\doilink{Phys.\ Lett.\ {\bf 98B}, 208 (1981)}{10.1016/0370-2693(81)90989-8}.
%%CITATION = doi:10.1016/0370-2693(81)90989-8;%%
%
}\bibitem{Brezin:1975sq}{E.~Brezin and J.~Zinn-Justin,
``Renormalization of the nonlinear sigma model in 2 + epsilon dimensions. Application to the Heisenberg ferromagnets,''
\doilink{Phys.\ Rev.\ Lett.\ {\bf 36}, 691 (1976)}{10.1103/PhysRevLett.36.691}.\\
%%CITATION = doi:10.1103/PhysRevLett.36.691;%%
%
S.~Hikami and E.~Brezin,
``Three loop calculations in the two-dimensional nonlinear sigma model,''
\doilink{J.\ Phys.\ A {\bf 11}, 1141 (1978)}{10.1088/0305-4470/11/6/015}.\\
%%CITATION = doi:10.1088/0305-4470/11/6/015;%%
%
E.~Brezin, S.~Hikami and J.~Zinn-Justin,
``Generalized nonlinear $\sigma$ models with gauge invariance,''
\doilink{Nucl.\ Phys.\ B {\bf 165}, 528 (1980)}{10.1016/0550-3213(80)90047-4}.
%%CITATION = doi:10.1016/0550-3213(80)90047-4;%%
%
}\bibitem{Balog:1993es}{%v3a
J.~Balog, P.~Forgacs, Z.~Horvath and L.~Palla,
``A new family of $SU(2)$ symmetric integrable sigma models,''
\doilink{Phys.\ Lett.\ B {\bf 324}, 403 (1994)}{10.1016/0370-2693(94)90213-5}
\arxivlink{hep-th/9307030}.\\
%%CITATION = doi:10.1016/0370-2693(94)90213-5;%%
%
J.~M.~Evans and T.~J.~Hollowood,
``Integrable theories that are asymptotically CFT,''
\doilink{ Nucl.\ Phys.\ B {\bf 438}, 469 (1995)}{10.1016/0550-3213(94)00473-R}
\arxivlink{hep-th/9407113}.
%%CITATION = doi:10.1016/0550-3213(94)00473-R;%%
%
}\bibitem{Kawaguchi:2010jg}{I.~Kawaguchi and K.~Yoshida,
``Hidden Yangian symmetry in sigma model on squashed sphere,''
\doilink{JHEP {\bf 1011}, 032 (2010)}{10.1007/JHEP11(2010)032}
\arxivlink{1008.0776}.
%%CITATION = doi:10.1007/JHEP11(2010)032;%%
%
}\bibitem{Kaloper:1997ux}{N.~Kaloper and K.~A.~Meissner,
``Duality beyond the first loop,''
\doilink{Phys.\ Rev.\ D {\bf 56}, 7940 (1997)}{10.1103/PhysRevD.56.7940}
\arxivlink{hep-th/9705193}.
%%CITATION = doi:10.1103/PhysRevD.56.7940;%%
%
}\bibitem{Parsons:1999ze}{S.~Parsons,
``T duality and conformal invariance at two loops,''
\doilink{Phys.\ Rev.\ D {\bf 61}, 086002 (2000)}{10.1103/PhysRevD.61.086002}
\arxivlink{hep-th/9912105}.\\
%%CITATION = doi:10.1103/PhysRevD.61.086002;%%
%
I.~Jack and S.~Parsons,
``$O(d,d)$ invariance at two loops and three loops,''
\doilink{Phys.\ Rev.\ D {\bf 62}, 026003 (2000)}{10.1103/PhysRevD.62.026003}
\arxivlink{hep-th/9911064}.
%%CITATION = doi:10.1103/PhysRevD.62.026003;%%
%
}\bibitem{Tseytlin:1990va}{
A.~A.~Tseytlin,
%\cite{Tseytlin:1990nb}
%}\bibitem{Tseytlin:1990nb}
%A.~A.~Tseytlin,
``Duality symmetric formulation of string world sheet dynamics,''
Phys. Lett. B \textbf{242}, 163-174 (1990)
doi:10.1016/0370-2693(90)91454-J; 
%307 citations counted in INSPIRE as of 13 Jul 2021
``Duality symmetric closed string theory and interacting chiral scalars,''
\doilink{Nucl.\ Phys.\ B {\bf 350}, 395 (1991)}{10.1016/0550-3213(91)90266-Z}.
%%CITATION = doi:10.1016/0550-3213(91)90266-Z;%%
%
%
}\bibitem{Rocek:1997hi}{M.~Rocek and A.~A.~Tseytlin,
``Partial breaking of global $D = 4$ supersymmetry, constrained superfields, and three-brane actions,''
\doilink{Phys.\ Rev.\ D {\bf 59}, 106001 (1999)}{10.1103/PhysRevD.59.106001}
\arxivlink{hep-th/9811232}.
%%CITATION = doi:10.1103/PhysRevD.59.106001;%%
%
}\bibitem{Abdalla:1980jt}{E.~Abdalla, M.~C.~B.~Abdalla and M.~Gomes,
``Anomaly in the nonlocal quantum charge of the $\mathbb{C}\mathbf{P}^{n-1}$ model,''
\doilink{Phys.\ Rev.\ D {\bf 23}, 1080 (1981)}{10.1103/PhysRevD.23.1800}.\\
%%CITATION = doi:10.1103/PhysRevD.23.1800;%%
%
E.~Abdalla, M.~Forger and M.~Gomes,
``On the origin of anomalies in the quantum nonlocal charge for the generalized nonlinear $\sigma$ models,''
\doilink{Nucl.\ Phys.\ B {\bf 210}, 181 (1982)}{doi:10.1016/0550-3213(82)90238-3}.
%%CITATION = doi:10.1016/0550-3213(82)90238-3;%%
%
}\bibitem{ey1}{J.~M.~Evans, D.~Kagan and C.~A.~S.~Young,
``Nonlocal charges and quantum integrability of sigma models on the symmetric spaces $SO(2n)/SO(n)\times SO(n)$ and $Sp(2n) / Sp(n) \times Sp(n)$,''
\doilink{Phys.\ Lett.\ B {\bf 597}, 112 (2004)}{doi:10.1016/j.physletb.2004.04.042}
\arxivlink{hep-th/0404003}.\\
%%CITATION = doi:10.1016/j.physletb.2004.04.042;%%
J.~M.~Evans, D.~Kagan, N.~J.~MacKay and C.~A.~S.~Young,
``Quantum, higher-spin, local charges in symmetric space sigma models,''
\doilink{JHEP {\bf 0501}, 020 (2005)}{doi:10.1088/1126-6708/2005/01/020}
\arxivlink{hep-th/0408244}.
%%CITATION = doi:10.1088/1126-6708/2005/01/020;%%
%
}\bibitem{cpn1}{A.~V.~Litvinov,
``Integrable $\mathfrak{gl}(n|n)$ Toda field theory and its sigma-model dual,''
\doilink{Pisma Zh. Eksp. Teor. Fiz. \textbf{110}, no.11, 723-726 (2019)}{
doi:10.1134/S0021364019230048}
\arxivlink{1901.04799}.
%%CITATION = ARXIV:1901.04799;%%
%
}\bibitem{bbr}{D.~Bykov,
``The worldsheet low-energy limit of the $AdS_4 \times \mathbb{C}\mathbf{P}^3$ superstring,''
\doilink{Nucl.\ Phys.\ B {\bf 838} (2010) 47}{doi:10.1016/j.nuclphysb.2010.05.013}
\arxivlink{1003.2199}.\\
%%CITATION = doi:10.1016/j.nuclphysb.2010.05.013;%%
%
B.~Basso and A.~Rej,
``On the integrability of two-dimensional models with $U(1) \times SU(N)$ symmetry,''
\doilink{Nucl.\ Phys.\ B {\bf 866} (2013) 337}{doi:10.1016/j.nuclphysb.2012.09.003}
\arxivlink{1207.0413}.
%
}\bibitem{Gomes:1982qh}{M.~Gomes, E.~Abdalla and M.~C.~B.~Abdalla,
``On the nonlocal charge of the {CP}$^{(N-1)}$ model and its supersymmetric extension to all orders,''
\doilink{Phys.\ Rev.\ D {\bf 27}, 825 (1983)}{10.1103/PhysRevD.27.825}.
%%CITATION = doi:10.1103/PhysRevD.27.825;%%
%
}\bibitem{Squellari:2014jfa}{R.~Squellari, %v3a
``Yang-Baxter $\sigma$ model: Quantum aspects,''
\doilink{Nucl.\ Phys.\ B {\bf 881}, 502 (2014)}{10.1016/j.nuclphysb.2014.02.009}
\arxivlink{1401.3197}.
%%CITATION = doi:10.1016/j.nuclphysb.2014.02.009;%%
%
}\bibitem{oneloopeta}{%v3a
C.~Klimcik and G.~Valent,
``One loop renormalizability of all 2-D dimensional Poisson-Lie sigma models,''
\doilink{Phys.\ Lett.\ B {\bf 565}, 237 (2003)}{10.1016/S0370-2693(03)00764-0}
\arxivlink{hep-th/0304053}.
%%CITATION = doi:10.1016/S0370-2693(03)00764-0;%%
%
%G.~Valent, C.~Klimcik and R.~Squellari,
%``One loop renormalizability of the Poisson-Lie sigma models,''
%\doilink{Phys.\ Lett.\ B {\bf 678}, 143 (2009)}{10.1016/j.physletb.2009.06.001},
%\arxivlink{0902.1459}.
%%%CITATION = doi:10.1016/j.physletb.2009.06.001;%%
%
}\bibitem{Kagan:2005wt}{D.~Kagan and C.~A.~S.~Young,
``Conformal sigma-models on supercoset targets,''
\doilink{Nucl.\ Phys.\ B {\bf 745}, 109 (2006)}{10.1016/j.nuclphysb.2006.02.027}
\arxivlink{hep-th/0512250}.
%%CITATION = doi:10.1016/j.nuclphysb.2006.02.027;%%
%
}\bibitem{Babichenko:2006uc}{A.~Babichenko,
``Conformal invariance and quantum integrability of sigma models on symmetric superspaces,''
\doilink{Phys.\ Lett.\ B {\bf 648}, 254 (2007)}{doi:10.1016/j.physletb.2007.03.003}
\arxivlink{hep-th/0611214}.
%%CITATION = doi:10.1016/j.physletb.2007.03.003;%%
%
%}\bibitem{Castellani:1999fz}{R. Gilmore,
%``Lie algebras and some of their applications,'' (Dover, 2005).\\
%%
%A.~Salam and J.~A.~Strathdee,
%``On Kaluza-Klein Theory,''
%\doilink{Annals Phys.\ {\bf 141}, 316 (1982)}{10.1016/0003-4916(82)90291-3}.\\
%%%CITATION = doi:10.1016/0003-4916(82)90291-3;%%
%%
%L.~Castellani,
%``On $G/H$ geometry and its use in M theory compactifications,''
%\doilink{Annals Phys.\ {\bf 287}, 1 (2001)}{10.1006/aphy.2000.6097}
%\arxivlink{hep-th/9912277}.
%%%CITATION = doi:10.1006/aphy.2000.6097;%%
%%
}\bibitem{bonneau}{G.~Bonneau, G.~Valent and F.~Delduc,
``Renormalization properties of bosonic nonlinear sigma models built on compact homogeneous Kahler manifolds,''
\doilink{Phys.\ Lett.\ B {\bf 196}, 456 (1987)}{10.1016/0370-2693(87)90801-X}.\\
%%CITATION = doi:10.1016/0370-2693(87)90801-X;%%
%
C.~Becchi, A.~Blasi, G.~Bonneau, R.~Collina and F.~Delduc,
``Renormalizability and infrared finiteness of nonlinear $\sigma$ models: a regularization independent analysis for compact coset spaces,''
\doilink{Commun.\ Math.\ Phys.\ {\bf 120}, 121 (1988)}{10.1007/BF01223209}.\\
%%CITATION = doi:10.1007/BF01223209;%%
%
A.~V.~Bratchikov,
``Renormalization properties of two-dimensional homogeneous symplectic sigma models,''
\doilink{Mod.\ Phys.\ Lett.\ A {\bf 7}, 2229 (1992)}{10.1142/S0217732392001993}.
%%%CITATION = doi:10.1142/S0217732392001993;%%
%
%%%%%%%%%%%%%%%%%
%% 2103 refs:
%
%%}\bibitem{intRG} 
%%V.~A.~Fateev, E.~Onofri and A.~B.~Zamolodchikov,
%%``Integrable deformations of the $O(3)$ sigma model. The sausage model,''
%%\doilink{Nucl.\ Phys.\ B {\bf 406}, 521 (1993)}{10.1016/0550-3213(93)90001-6}.
%%
%%V.~A.~Fateev,
%%``Classical and Quantum Integrable Sigma Models. Ricci Flow, ``Nice Duality'' and Perturbed Rational Conformal Field Theories,''
%%\doilink{J. Exp. Theor. Phys. \textbf{129}, no.4, 566-590 (2019)}{10.1134/S1063776119100042}
%%\arxivlink{1902.02811}.
%%
%%S.~L.~Lukyanov,
%%``The integrable harmonic map problem versus Ricci flow,''
%%\doilink{Nucl.\ Phys.\ B {\bf 865}, 308 (2012)}{10.1016/j.nuclphysb.2012.08.002}
%%\arxivlink{1205.3201}.
% 
%
}\bibitem{DLMV}{
F.~Delduc, S.~Lacroix, M.~Magro and B.~Vicedo,
``Integrable coupled $\sigma$ models,''
\doilink{Phys. Rev. Lett. \textbf{122}, no.4, 041601 (2019)}{doi:10.1103/PhysRevLett.122.041601}
\arxivlink{1811.12316};
``Assembling integrable $\sigma$-models as affine Gaudin models,''
\doilink{JHEP \textbf{06}, 017 (2019)}{doi:10.1007/JHEP06(2019)017}
\arxivlink{1903.00368}.
%
}\bibitem{ABL}{
G.~Arutyunov, C.~Bassi and S.~Lacroix,
``New integrable coset sigma models,''
\doilink{JHEP {\bf 2103}, 062 (2021)}{doi:10.1007/JHEP03(2021)062}
\arxivlink{2010.05573}.
%  
%}\bibitem{klim} 
%C.~Klimcik,
%``Yang-Baxter sigma models and dS/AdS T-duality,''
%\doilink{JHEP \textbf{12}, 051 (2002)}{doi:10.1088/1126-6708/2002/12/051}
%\arxivlink{hep-th/0210095};
%``On integrability of the Yang-Baxter sigma-model,''
%\doilink{J. Math. Phys. \textbf{50}, 043508 (2009)}{doi:10.1063/1.3116242}
%\arxivlink{0802.3518}.
%
%}\bibitem{balog}
%J.~Balog, P.~Forgacs, Z.~Horvath and L.~Palla,
%``A New family of SU(2) symmetric integrable sigma models,''
%\doilink{Phys.\ Lett.\ B {\bf 324}, 403 (1994)}{doi:10.1016/0370-2693(94)90213-5}
%\arxivlink{hep-th/9307030}.
%
}\bibitem{DMV}{
F.~Delduc, M.~Magro and B.~Vicedo,
%``On classical $q$-deformations of integrable sigma-models,''
%\doilink{JHEP \textbf{11}, 192 (2013)}{doi:10.1007/JHEP11(2013)192}
%\arxivlink{1308.3581};
``Integrable double deformation of the principal chiral model,''
\doilink{Nucl. Phys. B \textbf{891}, 312-321 (2015)}{doi:10.1016/j.nuclphysb.2014.12.018}
\arxivlink{1410.8066}.
%
}\bibitem{today}{
F.~Delduc, S.~Lacroix, K.~Sfetsos and K.~Siampos,
``RG flows of integrable $\sigma$-models and the twist function,''
\doilink{JHEP {\bf 2102}, 065 (2021)}{doi:10.1007/JHEP02(2021)065}
\arxivlink{2010.07879}.
%  
%%  
%%}\bibitem{mt} R.~R.~Metsaev and A.~A.~Tseytlin, 
%%``Order alpha-prime (two loop) equivalence of the string equations of motion and the sigma model Weyl invariance conditions: dependence on the dilaton and the antisymmetric tensor,''
%%\doilink{Nucl.\ Phys.\ B {\bf 293}, 385 (1987)}{10.1016/0550-3213(87)90077-0};
%%``Two loop $\beta$-function for the generalized bosonic sigma model,''
%%\doilink{Phys.\ Lett.\ B {\bf 191}, 354 (1987)}{doi:10.1016/0370-2693(87)90622-8}.
%
%%}\bibitem{Bos}
%%M.~Bos,
%%``Dimensional Regularization in the Wess-Zumino-Witten Model,''
%%\doilink{Phys. Lett. B \textbf{189}, 435-441 (1987)}{doi:10.1016/0370-2693(87)90656-3}.
%
}\bibitem{Ketov}{
%C.~M.~Hull and P.~K.~Townsend,
%``The Two Loop Beta Function for $\sigma$ Models With Torsion,''
%\doilink{Phys.\ Lett.\ B {\bf 191}, 115 (1987)}{doi:10.1016/0370-2693(87)91331-1}.
%
S.~V.~Ketov,
``Two loop calculations in $\sigma$ model with torsion,''
\doilink{Nucl.\ Phys.\ B {\bf 294}, 813 (1987)}{doi:10.1016/0550-3213(87)90609-2}.
%
%D.~Zanon,
%``Two Loop Beta Functions and Low-energy String Effective Action for the Two-dimensional Bosonic Nonlinear $\sigma$ Model With a {Wess-Zumino}-witten Term,''
%\doilink{Phys.\ Lett.\ B {\bf 191}, 363 (1987)}{doi:10.1016/0370-2693(87)90623-X}.
%
}\bibitem{Bap}{
M.~Bos,
``An example of dimensional regularization with antisymmetric tensors,''
\doilink{Annals Phys. \textbf{181}, 177 (1988)}{doi:10.1016/0003-4916(88)90164-9}.
%
}\bibitem{KZ}{
V.~G.~Knizhnik and A.~B.~Zamolodchikov,
``Current algebra and Wess-Zumino model in two-dimensions,''
\doilink{Nucl. Phys. B \textbf{247}, 83 (1984)}{doi:10.1016/0550-3213(84)90374-2}.
%
}\bibitem{shifman}{
D.~Schubring and M.~Shifman,
``Sigma model on a squashed sphere with a Wess-Zumino term,''
\doilink{Phys.\ Rev.\ D {\bf 103}, no. 2, 025016 (2021)}{doi:10.1103/PhysRevD.103.025016}
\arxivlink{2002.04696}.
%
}\bibitem{romans}{
D.~N.~Page and C.~N.~Pope,
``Which compactifications of $D=11$ supergravity are stable?,''
\doilink{Phys.\ Lett.\  {\bf 144B}, 346 (1984)}{doi:10.1016/0370-2693(84)91275-9}.\\
%
L.~J.~Romans,
``New compactifications of chiral N=2,  d=10 supergravity,''
\doilink{Phys. Lett. B \textbf{153}, 392 (1985)}{doi:10.1016/0370-2693(85)90479-4}.\\
%
P.~Candelas and X.~C.~de la Ossa,
``Comments on conifolds,''
\doilink{Nucl. Phys. B \textbf{342}, 246 (1990)}{doi:10.1016/0550-3213(90)90577-Z}.\\
%
I.~R.~Klebanov and E.~Witten,
``Superconformal field theory on three-branes at a Calabi-Yau singularity,''
\doilink{Nucl. Phys. B \textbf{536}, 199 (1998)}{doi:10.1016/S0550-3213(98)00654-3}
\arxivlink{hep-th/9807080}.
%
}\bibitem{GMM}{
E.~Guadagnini, M.~Martellini and M.~Mintchev,
``Scale invariance of sigma models  on homogeneous spaces,''
\doilink{Phys. Lett. B \textbf{194}, 69 (1987)}{doi:10.1016/0370-2693(87)90771-4}.\\
%
E.~Guadagnini,
``Current algebra in $\sigma$ models on homogeneous spaces,''
\doilink{Nucl. Phys. B \textbf{290}, 417 (1987)}{doi:10.1016/0550-3213(87)90195-7}.
%
%
}\bibitem{PZT}{
L.~A.~Pando Zayas and A.~A.~Tseytlin,
``Conformal sigma models for a class of T(p,q) spaces,''
\doilink{Class. Quant. Grav. \textbf{17}, 5125-5131 (2000)}{doi:10.1088/0264-9381/17/24/312}
\arxivlink{hep-th/0007086}.
%
}\bibitem{maillet}{
J.~M.~Maillet,
``Kac-Moody algebra and extended Yang-Baxter relations in the O($N$) nonlinear $\sigma$ model,''
\doilink{Phys. Lett. B \textbf{162}, 137 (1985)}{doi:10.1016/0370-2693(85)91075-5};
``New integrable canonical structures in two-dimensional models,''
\doilink{Nucl. Phys. B \textbf{269}, 54 (1986)}{doi:10.1016/0550-3213(86)90365-2}.
%
}\bibitem{LMV}{
S.~Lacroix, M.~Magro and B.~Vicedo,
``Local charges in involution and hierarchies in integrable sigma-models,''
\doilink{JHEP \textbf{09}, 117 (2017)}{doi:10.1007/JHEP09(2017)117}
\arxivlink{1703.01951}.
%
%}\bibitem{Sfetsos:2013wia} 
%K.~Sfetsos,
%``Integrable interpolations: From exact CFTs to non-Abelian T-duals,''
%\doilink{Nucl.\ Phys.\ B {\bf 880}, 225 (2014)}{doi:10.1016/j.nuclphysb.2014.01.004}
%\arxivlink{1312.4560}.
%
%T.~J.~Hollowood, J.~L.~Miramontes and D.~M.~Schmidtt,
%``Integrable Deformations of Strings on Symmetric Spaces,''
%\doilink{JHEP \textbf{11}, 009 (2014)}{doi:10.1007/JHEP11(2014)009}
%\arxivlink{1407.2840}.
%
}\bibitem{sfetsos}{G.~Georgiou and K.~Sfetsos,
``A new class of integrable deformations of CFTs,''
\doilink{JHEP {\bf 1703}, 083 (2017)}{10.1007/JHEP03(2017)083}
\arxivlink{1612.05012}.
%``Integrable flows between exact CFTs,''
%\doilink{JHEP {\bf 1711}, 078 (2017)}{10.1007/JHEP11(2017)078}
%\arxivlink{1707.05149}.
%
%G.~Georgiou, E.~Sagkrioti, K.~Sfetsos and K.~Siampos,
%``Quantum aspects of doubly deformed CFTs,''
%\doilink{Nucl.\ Phys.\ B {\bf 919}, 504 (2017)}{10.1016/j.nuclphysb.2017.04.004}
%\arxivlink{1703.00462}.
%
%G.~Georgiou, K.~Sfetsos and K.~Siampos,
%``Double and cyclic $\lambda$-deformations and their canonical equivalents,''
%\doilink{Phys.\ Lett.\ B {\bf 771}, 576 (2017)}{10.1016/j.physletb.2017.06.007}
%\arxivlink{1704.07834}.
%
}\bibitem{s19}{
G.~Georgiou, E.~Sagkrioti, K.~Sfetsos and K.~Siampos,
``An exact symmetry in $\lambda$-deformed CFTs,''
\doilink{JHEP \textbf{01}, 083 (2020)}{doi:10.1007/JHEP01(2020)083}
\arxivlink{1911.02027}.
%
%}\bibitem{ss}
%K.~Sfetsos and K.~Siampos,
%``Gauged WZW-type theories and the all-loop anisotropic non-abelian Thirring model,''
%\doilink{Nucl.\ Phys.\ B {\bf 885}, 583 (2014)}{10.1016/j.nuclphysb.2014.06.012},
%\arxivlink{1405.7803}.
%
%}\bibitem{ah}
%C.~Appadu and T.~J.~Hollowood,
%``Beta function of $k$ deformed $AdS_5 \times S^5$ string theory,''
%\doilink{JHEP {\bf 1511}, 095 (2015)}{10.1007/JHEP11(2015)095},
%\arxivlink{1507.05420}.
%
}\bibitem{HS}{
C.~M.~Hull and B.~J.~Spence,
``The gauged nonlinear $\sigma$ model with {Wess-Zumino} term,''
\doilink{Phys. Lett. B \textbf{232}, 204-210 (1989)}{doi:10.1016/0370-2693(89)91688-2}.
%
}\bibitem{witten}{
E.~Witten,
``On holomorphic factorization of WZW and coset models,''
\doilink{Commun. Math. Phys. \textbf{144}, 189-212 (1992)}{doi:10.1007/BF02099196}.
%
}\bibitem{belo}{
V.~V.~Belokurov and P.~M.~de Barrush Pasheku Seara de Sa,
``Ultraviolet finiteness of the Wess-Zumino-Witten gauge model on homogeneous manifolds,''
Moscow Univ.\ Phys.\ Bull.\  {\bf 45N3}, 13 (1990)
[Vestn.\ Mosk.\ Univ.\ Fiz.\ Astron.\  {\bf 31N3}, 13 (1990)].
%
%}\bibitem{BBS}
%K.~Bardakci, L.~M.~Bernardo and N.~Sochen,
%``Integrable generalized Thirring model,''
%\doilink{Nucl. Phys. B \textbf{487}, 513-525 (1997)}{doi:10.1016/S0550-3213(96)00715-8}
%\arxivlink{hep-th/9607018}.
%
}\bibitem{bpz}{
P.~Basu and L.~A.~Pando Zayas,
``Chaos rules out integrability of strings on AdS$_5 \times T^{1,1}$,''
\doilink{Phys. Lett. B \textbf{700}, 243-248 (2011)}{doi:10.1016/j.physletb.2011.04.063}
\arxivlink{1103.4107}.
%
}\bibitem{Basu:2011fw}{
P.~Basu and L.~A.~Pando Zayas,
``Analytic non-integrability in string theory,''
\doilink{Phys. Rev. D \textbf{84}, 046006 (2011)}{10.1103/PhysRevD.84.046006}
\arxivlink{1105.2540}.
%
}\bibitem{yosh}{
I.~Kawaguchi, D.~Orlando and K.~Yoshida,
``Yangian symmetry in deformed WZNW models on squashed spheres,''
\doilink{Phys.\ Lett.\ B {\bf 701}, 475 (2011)}{doi:10.1016/j.physletb.2011.06.007}
\arxivlink{1104.0738}.\\
%  
I.~Kawaguchi and K.~Yoshida,
``A deformation of quantum affine algebra in squashed Wess-Zumino-Novikov-Witten models,''
\doilink{J.\ Math.\ Phys.\  {\bf 55}, 062302 (2014)}{doi:10.1063/1.4880341}
\arxivlink{1311.4696}.
%
%S.~Demulder, S.~Driezen, A.~Sevrin and D.~C.~Thompson,
%``Classical and Quantum Aspects of Yang-Baxter Wess-Zumino Models,''
%\doilink{JHEP {\bf 1803}, 041 (2018)}{doi:10.1007/JHEP03(2018)041}
%\arxivlink{1711.00084}.
%
%}\bibitem{Tseytlin:1991wr} 
%A.~A.~Tseytlin,
%``Duality and dilaton,''
%\doilink{Mod.\ Phys.\ Lett.\ A {\bf 6}, 1721 (1991)}{10.1142/S021773239100186X}, \\
%{\small \url{https://www.academia.edu/40796716/Tseytlin1991_duality_dilaton_MPLA} }
%
%P.~E.~Haagensen and K.~Olsen,
%``T duality and two loop renormalization flows,''
%\doilink{Nucl.\ Phys.\ B {\bf 504}, 326 (1997)}{doi:10.1016/S0550-3213(97)00496-3}
%\arxivlink{hep-th/9704157}.
%
%N.~Kaloper and K.~A.~Meissner,
%``Duality beyond the first loop,''
%\doilink{Phys. Rev. D \textbf{56}, 7940-7953 (1997)}{doi:10.1103/PhysRevD.56.7940}
%\arxivlink{hep-th/9705193}.
%
%}\bibitem{bu}
%T.~H.~Buscher,
%``Path Integral Derivation of Quantum Duality in Nonlinear Sigma Models,''
%\doilink{Phys.\ Lett.\ B {\bf 201}, 466 (1988)}{doi:10.1016/0370-2693(88)90602-8}.
%
%A.~S.~Schwarz and A.~A.~Tseytlin,
%``Dilaton shift under duality and torsion of elliptic complex,''
%\doilink{Nucl.\ Phys.\ B {\bf 399}, 691 (1993)}{doi:10.1016/0550-3213(93)90514-P}
%\arxivlink{hep-th/9210015}.
%  
}\bibitem{hassler}{
F.~Hassler and T.~B.~Rochais,
``O($D$,$D$)-covariant two-loop $\beta$-functions and Poisson-Lie T-duality,''
\arxivlink{2011.15130}.\\
%
F.~Hassler,
``RG flow of integrable $\mathcal{E}$-models,''
\doilink{Phys. Lett. B \textbf{818}, 136367 (2021)}{
doi:10.1016/j.physletb.2021.136367}
\arxivlink{2012.10451}.
%
}\bibitem{Tseytlin:1992pq}{A.~A.~Tseytlin,
``String vacuum backgrounds with covariantly constant null Killing vector and 2-d quantum gravity,''
\doilink{Nucl. Phys. B \textbf{390}, 153-172 (1993)}{10.1016/0550-3213(93)90389-7}
\arxivlink{hep-th/9209023};
``Finite $\s$-models and exact string solutions with Minkowski signature metric,''
\doilink{Phys.\ Rev.\ D {\bf 47}, 3421 (1993)}{10.1103/PhysRevD.47.3421}
\arxivlink{hep-th/9211061}.
%
%%}\bibitem{HLT3}
%%B.~Hoare, N.~Levine and A.~A.~Tseytlin,
%%``Sigma models with local couplings: a new integrability -- RG flow connection,''
%%\doilink{JHEP \textbf{11}, 020 (2020)}{10.1007/JHEP11(2020)020}
%%\arxivlink{2008.01112}.
%
%
%%%%%%%%%%%%%%%%%%%%
%%%%%% 2008 refs
%
%%%Fateev:1992tk,Fateev:2019xuq,lukyanov
%%}\bibitem{Fateev:2019xuq} V.~A.~Fateev, E.~Onofri and A.~B.~Zamolodchikov,
%%``Integrable deformations of the $O(3)$ sigma model. The sausage model,''
%%\doilink{Nucl.\ Phys.\ B {\bf 406}, 521 (1993)}{10.1016/0550-3213(93)90001-6}.
%%%%CITATION = doi:10.1016/0550-3213(93)90001-6;%%
%%
%%V.~A.~Fateev,
%%``Classical and Quantum Integrable Sigma Models. Ricci Flow, ``Nice Duality'' and Perturbed Rational Conformal Field Theories,''
%%\doilink{J. Exp. Theor. Phys. \textbf{129}, no.4, 566-590 (2019)}{10.1134/S1063776119100042}
%%\arxivlink{1902.02811}.
%%
%%S.~L.~Lukyanov,
%%``The integrable harmonic map problem versus Ricci flow,''
%%\doilink{Nucl.\ Phys.\ B {\bf 865}, 308 (2012)}{10.1016/j.nuclphysb.2012.08.002}
%%\arxivlink{1205.3201}.
%%%%CITATION = doi:10.1016/j.nuclphysb.2012.08.002;%%
%
%%% HLT1,HLT2
%%}\bibitem{HLT} B.~Hoare, N.~Levine and A.~A.~Tseytlin,
%%``Integrable 2d sigma models: quantum corrections to geometry from RG flow,''
%%\doilink{Nucl. Phys. B \textbf{949}, 114798 (2019)}{10.1016/j.nuclphysb.2019.114798}
%%\arxivlink{1907.04737}.
%%
%%B.~Hoare, N.~Levine and A.~A.~Tseytlin,
%%``Integrable sigma models and 2-loop RG flow,''
%%\doilink{JHEP {\bf 1912}, 146 (2019)}{doi:10.1007/JHEP12(2019)146}
%%\arxivlink{1910.00397}.
%%%%CITATION = doi:10.1007/JHEP12(2019)146;%%
%
%%}\bibitem{Klimcik:2002zj} C.~Klim\v{c}\'{i}k,
%%``Yang-Baxter sigma models and dS/AdS T duality,''
%%\doilink{JHEP \textbf{12}, 051 (2002)}{10.1088/1126-6708/2002/12/051}
%%\arxivlink{hep-th/0210095}.
%
%%}\bibitem{Delduc:2013fga} F.~Delduc, M.~Magro and B.~Vicedo,
%%``On classical $q$-deformations of integrable sigma-models,''
%%\doilink{JHEP {\bf 1311}, 192 (2013)}{10.1007/JHEP11(2013)192}
%%\arxivlink{1308.3581}.
%%%%CITATION = doi:10.1007/JHEP11(2013)192;%%
%
%%}\bibitem{Sfetsos:2013wia} K.~Sfetsos,
%%``Integrable interpolations: From exact CFTs to non-Abelian T-duals,''
%%\doilink{Nucl.\ Phys.\ B {\bf 880}, 225 (2014)}{10.1016/j.nuclphysb.2014.01.004}
%%\arxivlink{1312.4560}.
%%%%CITATION = doi:10.1016/j.nuclphysb.2014.01.004;%%
%
%%}\bibitem{Hollowood:2014rla} T.~J.~Hollowood, J.~L.~Miramontes and D.~M.~Schmidtt,
%%``Integrable Deformations of Strings on Symmetric Spaces,''
%%\doilink{JHEP {\bf 1411}, 009 (2014)}{10.1007/JHEP11(2014)009}
%%\arxivlink{1407.2840}.
%%%%CITATION = doi:10.1007/JHEP11(2014)009;%%
%
%%}\bibitem{Valent:2009nv} G.~Valent, C.~Klim\v{c}\'{i}k and R.~Squellari,
%%``One loop renormalizability of the Poisson-Lie sigma models,''
%%\doilink{Phys. Lett. B \textbf{678}, 143-148 (2009)}{10.1016/j.physletb.2009.06.001}
%%\arxivlink{0902.1459}.
%
%%%Itsios:2014lca,Sfetsos:2014jfa
%%}\bibitem{Sfetsos:2014jfa}
%%%v2
%%G.~Itsios, K.~Sfetsos and K.~Siampos,
%%``The all-loop non-Abelian Thirring model and its RG flow,''
%%\doilink{Phys. Lett. B \textbf{733}, 265-269 (2014)}{10.1016/j.physletb.2014.04.061}
%%\arxivlink{1404.3748}.
%%
%%K.~Sfetsos and K.~Siampos,
%%``Gauged WZW-type theories and the all-loop anisotropic non-abelian Thirring model,''
%%\doilink{Nucl.\ Phys.\ B {\bf 885}, 583 (2014)}{10.1016/j.nuclphysb.2014.06.012}
%%\arxivlink{1405.7803}.
%%%%CITATION = doi:10.1016/j.nuclphysb.2014.06.012;%%
%
%%%ah
%%}\bibitem{Appadu:2015nfa} C.~Appadu and T.~J.~Hollowood,
%%``Beta function of $k$ deformed $AdS_5 \times S^5$ string theory,''
%%\doilink{JHEP {\bf 1511}, 095 (2015)}{10.1007/JHEP11(2015)095}
%%\arxivlink{1507.05420}.
%%%%CITATION = doi:10.1007/JHEP11(2015)095;%%
%
}\bibitem{t-dep-1d}{S. Bouquet and A. Bourdier,
``Notion of integrability for time-dependent Hamiltonian systems:
Illustrations from the relativistic motion of a charged particle,''
\doilink{Phys.\ Rev.\ E \textbf{57}, 1273 (1998)}{10.1103/PhysRevE.57.1273}.\\
%
M. V. Bartuccelli and G. Gentile,
``On a class of integrable time-dependent dynamical systems,''
\doilink{Phys.\ Lett.\ A \textbf{307}, 274-280 (2003)}{10.1016/S0375-9601(02)01731-0}.\\
%
R. M. Angelo, E. I. Duzzioni and A. D. Ribeiro,
``Integrability in time-dependent systems with one degree of freedom,''
\doilink{J. Phys. A \textbf{45}, 5 (2012)}{10.1088/1751-8113/45/5/055101}
\arxivlink{1106.6034}.
%
}\bibitem{Papadopoulos:2002bg}{G.~Papadopoulos, J.~Russo and A.~A.~Tseytlin,
``Solvable model of strings in a time dependent plane wave background,''
\doilink{Class. Quant. Grav. \textbf{20}, 969-1016 (2003)}{10.1088/0264-9381/20/5/313}
\arxivlink{hep-th/0211289}.\\
%
M.~Blau, M.~O'Loughlin, G.~Papadopoulos and A.~A.~Tseytlin,
``Solvable models of strings in homogeneous plane wave backgrounds,''
\doilink{Nucl.\ Phys.\ B {\bf 673}, 57 (2003)}{10.1016/j.nuclphysb.2003.09.018}
\arxivlink{hep-th/0304198}.
%%CITATION = doi:10.1016/j.nuclphysb.2003.09.018;%%
%
}\bibitem{yoshida}{A.~Borowiec, H.~Kyono, J.~Lukierski, J.~I.~Sakamoto and K.~Yoshida,
``Yang-Baxter sigma models and Lax pairs arising from $\kappa$-Poincar\'e $r$-matrices,''
\doilink{JHEP {\bf 1604}, 079 (2016)}{10.1007/JHEP04(2016)079}
\arxivlink{1510.03083}.\\
%%CITATION = doi:10.1007/JHEP04(2016)079;%%
%
H.~Kyono, J.~I.~Sakamoto and K.~Yoshida,
``Lax pairs for deformed Minkowski space-times,''
\doilink{JHEP {\bf 1601}, 143 (2016)}{10.1007/JHEP01(2016)143}
\arxivlink{1512.00208}.
%%CITATION = doi:10.1007/JHEP01(2016)143;%%
%
}\bibitem{Maldacena:2002fy}{J.~M.~Maldacena and L.~Maoz,
``Strings on pp waves and massive two-dimensional field theories,''
\doilink{JHEP \textbf{12}, 046 (2002)}{10.1088/1126-6708/2002/12/046}
\arxivlink{hep-th/0207284}.
%
}\bibitem{Russo:2002qj}{J.~G.~Russo and A.~A.~Tseytlin,
``A class of exact pp wave string models with interacting light cone gauge actions,''
\doilink{JHEP \textbf{09}, 035 (2002)}{10.1088/1126-6708/2002/09/035}
\arxivlink{hep-th/0208114}.
%
}\bibitem{Bakas:2002kt}{I.~Bakas and J.~Sonnenschein,
``On Integrable models from pp wave string backgrounds,''
\doilink{JHEP \textbf{12}, 049 (2002)}{10.1088/1126-6708/2002/12/049}
\arxivlink{hep-th/0211257}.
%
%}\bibitem{Tseytlin:1992pq} A.~A.~Tseytlin,
%``String vacuum backgrounds with covariantly constant null Killing vector and 2-d quantum gravity,''
%\doilink{Nucl. Phys. B \textbf{390}, 153-172 (1993)}{10.1016/0550-3213(93)90389-7}
%\arxivlink{hep-th/9209023};
%%v2
%``A class of finite two-dimensional sigma models and string vacua,''
%\doilink{Phys. Lett. B \textbf{288}, 279 (1992)}{doi:10.1016/0370-2693(92)91104-H}
%\arxivlink{hep-th/9205058}.
%%%CITATION = doi:10.1016/0370-2693(92)91104-H;%%
%
}\bibitem{Tseytlin:1992ee}{A.~A.~Tseytlin,
``Finite $\s$-models and exact string solutions with Minkowski signature metric,''
\doilink{Phys.\ Rev.\ D {\bf 47}, 3421 (1993)}{10.1103/PhysRevD.47.3421}
\arxivlink{hep-th/9211061}.
%%CITATION = doi:10.1103/PhysRevD.47.3421;%%
%
}\bibitem{Schmidhuber:1994bv}{C.~Schmidhuber and A.~A.~Tseytlin,
``On string cosmology and the RG flow in 2-d field theory,''
\doilink{Nucl.\ Phys.\ B {\bf 426}, 187 (1994)}{10.1016/0550-3213(94)90131-7}
\arxivlink{hep-th/9404180}.
%%CITATION = doi:10.1016/0550-3213(94)90131-7;%%
%
%v2
}\bibitem{Belinsky:1971nt}{
V.~A.~Belinsky and V.~E.~Zakharov,
``Integration of the Einstein Equations by the Inverse Scattering Problem Technique and the Calculation of the Exact Soliton Solutions,''
Sov.\ Phys.\ JETP {\bf 48}, 985 (1978)
[Zh.\ Eksp.\ Teor.\ Fiz.\ {\bf 75}, 1953 (1978)];
``Stationary Gravitational Solitons with Axial Symmetry,''
Sov.\ Phys.\ JETP {\bf 50}, 1 (1979)
[Zh.\ Eksp.\ Teor.\ Fiz.\ {\bf 77}, 3 (1979)].\\
%%CITATION = SPHJA,50,1;%%
%
%%CITATION = SPHJA,48,985;%%
D.~Maison,
``Are the stationary, axially symmetric Einstein equations completely integrable?,''
\doilink{Phys.\ Rev.\ Lett.\ {\bf 41}, 521 (1978)}{doi:10.1103/PhysRevLett.41.521};
%%CITATION = doi:10.1103/PhysRevLett.41.521;%%
``Stationary, Axially Symmetric Einstein Spaces: A Completely Integrable Hamiltonian System?,''
\doilink{J.\ Math.\ Phys.\ {\bf 20}, 871 (1979)}{doi:10.1063/1.524134}.
%%CITATION = doi:10.1063/1.524134;%%
%
}\bibitem{Breitenlohner:1986um}{
P.~Breitenlohner and D.~Maison,
``On the Geroch group,''
Ann.\ Inst.\ H.\ Poincare Phys.\ Theor.\ {\bf 46}, 215 (1987).
%
}\bibitem{Nicolai:1991tt}{
H.~Nicolai,
``Two-dimensional gravities and supergravities as integrable system,''
\doilink{Lect.\ Notes Phys.\ {\bf 396}, 231 (1991)}{doi:10.1007/3-540-54978-1_12}.\\
%%CITATION = doi:10.1007/3-540-54978-1_12;%%
%
H.~Nicolai, D.~Korotkin and H.~Samtleben,
``Integrable classical and quantum gravity,''
NATO Advanced Study Institute on Quantum Fields and Quantum Space Time,
22 July--3 August 1996. Cargese, France, pp. 203--243.
\arxivlink{hep-th/9612065}.
%%CITATION = HEP-TH/9612065;%%
%
%%%
%
}\bibitem{Arutyunov:2003za}{G.~Arutyunov, J.~Russo and A.~A.~Tseytlin,
``Spinning strings in $AdS_5 \times S^5$: New integrable system relations,''
\doilink{Phys.\ Rev.\ D {\bf 69} (2004) 086009}{10.1103/PhysRevD.69.086009}
\arxivlink{hep-th/0311004}.
%%CITATION = doi:10.1103/PhysRevD.69.086009;%%
%
}\bibitem{Goldschmidt:1980wq}{Y.~Y.~Goldschmidt and E.~Witten,
``Conservation laws in some two-dimensional models,''
\doilink{Phys. Lett. B \textbf{91}, 392-396 (1980)}{10.1016/0370-2693(80)91004-7}.
%
}\bibitem{Evans:1999mj}{
J.~M.~Evans, N.~J.~MacKay and M.~Hassan,
``Conserved charges and supersymmetry in principal chiral models,''
\arxivlink{hep-th/9711140}.\\
%13 citations counted in INSPIRE as of 06 Jul 2021
%
J.~M.~Evans, M.~Hassan, N.~J.~MacKay and A.~J.~Mountain,
``Local conserved charges in principal chiral models,''
\doilink{Nucl. Phys. B \textbf{561}, 385-412 (1999)}{10.1016/S0550-3213(99)00489-7}
\arxivlink{hep-th/9902008}.
%\cite{Evans:1997xu}
%}\bibitem{Evans:1997xu}
%
%
}\bibitem{Evans:2000qx}{J.~M.~Evans and A.~J.~Mountain,
``Commuting charges and symmetric spaces,''
\doilink{Phys. Lett. B \textbf{483}, 290-298 (2000)}{10.1016/S0370-2693(00)00566-9}
\arxivlink{hep-th/0003264}.
%
%LMV
}\bibitem{Lacroix:2017isl}{S.~Lacroix, M.~Magro and B.~Vicedo,
``Local charges in involution and hierarchies in integrable sigma-models,''
\doilink{JHEP \textbf{09}, 117 (2017)}{10.1007/JHEP09(2017)117}
\arxivlink{1703.01951}.
%
%}\bibitem{Faddeev:1985qu}{L.~D.~Faddeev and N.~Y.~Reshetikhin, %removed
%``Integrability of the principal chiral field model in (1+1)-dimension,''
%\doilink{Annals Phys. \textbf{167}, 227 (1986)}{10.1016/0003-4916(86)90201-0}.
%
% -> DLMV
%}\bibitem{Delduc:2019bcl} F.~Delduc, S.~Lacroix, M.~Magro and B.~Vicedo,
%``Assembling integrable $\sigma$-models as affine Gaudin models,''
%\doilink{JHEP \textbf{06}, 017 (2019)}{10.1007/JHEP06(2019)017}
%\arxivlink{1903.00368}.
%
%% -> maillet
%}\bibitem{Maillet:1985ek} J.~M.~Maillet,
%``New Integrable Canonical Structures in Two-dimensional Models,''
%\doilink{Nucl. Phys. B \textbf{269}, 54-76 (1986)}{10.1016/0550-3213(86)90365-2}
%
%}\bibitem{Sevostyanov:1995hd}{A.~Sevostyanov, %removed
%``The classical R matrix method for nonlinear sigma model,''
%\doilink{Int. J. Mod. Phys. A \textbf{11}, 4241-4254 (1996)}{10.1142/S0217751X96001978}
%\arxivlink{hep-th/9509030}.
%
%}\bibitem{Basu:2011fw} P.~Basu and L.~A.~Pando Zayas,
%``Analytic Non-integrability in String Theory,''
%\doilink{Phys. Rev. D \textbf{84}, 046006 (2011)}{10.1103/PhysRevD.84.046006}
%\arxivlink{1105.2540}.
%
}\bibitem{Stepanchuk:2012xi}{A.~Stepanchuk and A.~A.~Tseytlin,
``On (non)integrability of classical strings in p-brane backgrounds,''
\doilink{J. Phys. A \textbf{46}, 125401 (2013)}{10.1088/1751-8113/46/12/125401}
\arxivlink{1211.3727}.
%
}\bibitem{Osborn:1987au}{H.~Osborn,
``Renormalization and composite operators in nonlinear $\sigma$ models,''
\doilink{Nucl.\ Phys.\ B {\bf 294}, 595 (1987)}{10.1016/0550-3213(87)90599-2};
%%CITATION = doi:10.1016/0550-3213(87)90599-2;%%
``Weyl consistency conditions and a local renormalization group equation for general renormalizable field theories,''
\doilink{Nucl.\ Phys.\ B {\bf 363}, 486 (1991)}{10.1016/0550-3213(91)80030-P}.
%%CITATION = doi:10.1016/0550-3213(91)80030-P;%%
%
%v3
}\bi{byk}{
D.~Bykov and D.~Lust,
``Deformed $\sigma$-models, Ricci flow and Toda field theories,''
\arxivlink{2005.01812}.
%%CITATION = ARXIV:2005.01812;%%
%
%v3
}\bi{byk2}{
D.~Bykov,
``Quantum flag manifold $\sigma$-models and Hermitian Ricci flow,''
\arxivlink{2006.14124}.
%%CITATION = ARXIV:2006.14124;%%
%
%
%
%%--> Young:2005jv
%C.~A.~S.~Young,
%``Non-local charges, Z(m) gradings and coset space actions,''
%\doilink{Phys. Lett. B \textbf{632}, 559-565 (2006)}{doi:10.1016/j.physletb.2005.10.090},
%\arxivlink{hep-th/0503008}.
%
}\bibitem{yo}{
D.~Kagan and C.~A.~S.~Young,
``Conformal sigma-models on supercoset targets,''
\doilink{Nucl. Phys. B \textbf{745}, 109-122 (2006)}{doi:10.1016/j.nuclphysb.2006.02.027}
\arxivlink{hep-th/0512250}.
%
%\cite{Levkov:2020lfa}
}\bibitem{Levkov:2020lfa}{D.~G.~Levkov, V.~E.~Maslov and E.~Y.~Nugaev,
``Chaotic solitons in driven sine-Gordon model,''
\doilink{Fractals {\bf 139}, 110079 (2020)}{doi:10.1016/j.chaos.2020.110079}
\arxivlink{2004.13052}.
%%CITATION = doi:10.1016/j.chaos.2020.110079;%%
}\bibitem{Tseytlin:1986ws}{
A.~A.~Tseytlin,
``Conformal anomaly in two-dimensional sigma model on curved background and strings,''
\doilink{Phys. Lett. B \textbf{178}, 34 (1986)}{
doi:10.1016/0370-2693(86)90465-X};
``$\sigma$ model Weyl invariance conditions and string equations of motion,''
\doilink{Nucl. Phys. B \textbf{294}, 383-411 (1987)}{
doi:10.1016/0550-3213(87)90588-8}.
}\bibitem{Ishii:2021asw}{
T.~Ishii, S.~Kushiro and K.~Yoshida,
``Chaotic string dynamics in deformed $T^{1,1}$,''
\doilink{JHEP \textbf{05}, 158 (2021)}{doi:10.1007/JHEP05(2021)158}
\arxivlink{2103.12416}.
%2 citations counted in INSPIRE as of 31 Jul 2021
}\bibitem{Costello:2019tri}{K.~Costello, E.~Witten and M.~Yamazaki,
``Gauge theory and integrability, I,''
\doilink{ICCM Not. 6, 46-191 (2018)}{10.4310/ICCM.2018.v6.n1.a6}
\arxivlink{1709.09993}.\\
%%CITATION = doi:10.4310/ICCM.2018.v6.n1.a6;%%
%
K.~Costello and M.~Yamazaki,
``Gauge theory and integrability, III''
\arxivlink{1908.02289}.
%
}\bibitem{Delduc:2019whp}{F.~Delduc, S.~Lacroix, M.~Magro and B.~Vicedo,
``A unifying 2d action for integrable $\sigma$-models from 4d Chern-Simons theory,''
\doilink{Lett. Math. Phys. {\bf 110}, 1645 (2020)}{10.1007/s11005-020-01268-y}
\arxivlink{1909.13824}.
%%CITATION = doi:10.1007/s11005-020-01268-y;%%
%
}\bibitem{Lax:1968fm}{L.~D.~Faddeev and L.~A.~Takhtajan,
``Hamiltonian methods in the theory of solitons,''
Berlin, Springer (1987).
%
%\cite{Borsato:2020wwk}
}\bibitem{BW}{
R.~Borsato and L.~Wulff,
``Quantum correction to generalized $T$ dualities,''
\doilink{Phys. Rev. Lett. \textbf{125}, no.20, 201603 (2020)}{
doi:10.1103/PhysRevLett.125.201603}
\arxivlink{2007.07902}.\\
%19 citations counted in INSPIRE as of 28 Jun 2021
%\cite{Codina:2020yma}
%
%\cite{Hassler:2020tvz}
F.~Hassler and T.~Rochais,
``$\alpha'$-corrected Poisson-Lie T-duality,''
\doilink{Fortsch. Phys. \textbf{68}, no.9, 2000063 (2020)}{
doi:10.1002/prop.202000063}
\arxivlink{2007.07897}.\\
%15 citations counted in INSPIRE as of 28 Jun 2021
%
T.~Codina and D.~Marques,
``Generalized dualities and higher derivatives,''
\doilink{JHEP \textbf{10}, 002 (2020)}{
doi:10.1007/JHEP10(2020)002}
\arxivlink{2007.09494}.
}
%19 citations counted in INSPIRE as of 28 Jun 2021
%
\end{thebibliography}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
